Logical Relations for Monadic Types

Logical relations and their generalizations are a fundamental tool in proving properties of lambda-calculi, e.g., yielding sound principles for observational equivalence. We propose a natural notion of logical relations able to deal with the monadic types of Moggi's computational lambda-calculus. The treatment is categorical, and is based on notions of subsconing, mono factorization systems, and monad morphisms. Our approach has a number of interesting applications, including cases for lambda-calculi with non-determinism (where being in logical relation means being bisimilar), dynamic name creation, and probabilistic systems.

==> adjstrong.tex <==
\section{Proof of Proposition~\ref{prop:adj:distr:3}}
\label{app:adjstrong}

\paragraph{Diagram~(\ref{eq:strong:l})} is obtained by considering the following
diagram.  We drop subscripts on natural transformations so as to save space;
they can be inferred from context.  {\small
  \[
  \xymatrix{
    {\Id \tensord \funbara {\tc \discr F}}
    \ar[r]^{\unita_\Id \tensord \identity {}}
    \ar[rd]|{\tstri \tensord \identity {}}^{(\ref{eq:moneta:I})}
    \ar@/_45pt/[ddrrrr]^{\ld {\funbara {\tc \discr F}}}
    \ar@{}[ddrr]|(0.8){(\ref{eq:theta:coh:l})}
    &
    {\funbara {\discr \Id} \tensord \funbara {\tc \discr F}}
    \ar[r]^{\tstrna}
    &
    {\funbara {\discr \Id \tensorc \tc \discr F}}
    \ar[r]^{\funbara {\strcna}}
    &
    {\funbara {\tc (\discr \Id \tensorc \discr F)}}
    \ar[r]^{\funbara {\tc \tstrcna}}
    &
    {\funbara {\tc \discr (\Id \tensord F)}}
    \ar[dd]|(0.4){\funbara {\tc \discr \ld F}}
    \\
    &
    {\funbara \Ic \tensord \funbara {\tc \discr F}}
    \ar[u]|{\funbara \tstrci \tensord \identity {}}
    \ar[r]_{\tstrna}
    \ar@{}[ru]|{\txt{(natural-\\ity of $\tstrna$)}}
    &
    {\funbara {\Ic \tensorc \tc \discr F}}
    \ar[u]|{\funbara {\tstrci \tensorc \identity {}}}
    \ar[r]_{\funbara \strcna}
    \ar@{}[ru]|{\txt{(natural-\\ity of $\funbara \tc$)}}
    \ar@/_20pt/[rrd]|{\funbara {\lc {\tc \discr F}}}
    &
    {\funbara {\tc (\Ic \tensorc \discr F)}}
    \ar[u]|{\funbara {\tc (\tstrci \tensorc \identity {})}}
    \ar[rd]|{\funbara {\tc \lc {\discr F}}}
    \ar@{}[r]|(0.6){\funbara {\tc (\ref{eq:theta:coh:l})}}
    \ar@{}[d]|{(\ref{eq:strong:l})}
    &
    \\
    &&&&
    {\funbara {\tc \discr F}}
    }
  \]
  } We have also decorated the interior of each face with the justification
why its edges commute.  For example, the top left triangle is a copy of
(\ref{eq:moneta:I}), one of the diagrams stating that the adjunction is
monoidal.  The bottom face, whose bottom edge is a curved arrow, commutes by
the coherence square (\ref{eq:theta:coh:l}) for $\tstrna$.  The rightmost
parallelogram commutes by $\funbara \tc$ applied to another coherence square
(\ref{eq:theta:coh:l}), this time for $\tstrcna$.  Now the topmost composition
of arrows is $\strd \Id F$, the bottommost arrow from $\Id \tensord \funbara
{\tc \discr F}$ to $\funbara {\tc \discr F}$ is $\ld {\td F}$, and the
rightmost vertical arrow is $\td \ld F$.
  
\paragraph{Diagram~(\ref{eq:strong:eta}).}
This is the diagram below.  We recognize $\strd E F$ as the rightmost
composition of vertical arrows, $\identity E \tensord \unitd F$ as the topmost
composition of horizontal arrows, and $\unitd {E \tensord F}$ is the diagonal
from $E \tensord F$ to $\funbara {\tc \discr (E \tensord F)}$. {\small
  \[
  \xymatrix@C+50pt{
    E \tensord F
    \ar[r]^{\identity{} \tensord \unita_F}
    \ar[rd]|{\unita_E \tensord \unita_F}
    \ar@{}[rrd]|{\txt{(functoriality of $\tensord$)}}
    \ar[rddd]_{\unita_{E \tensord F}}
    \ar@{}[rdd]|(0.7){\txt{(monoidal\\adjunction\\(\ref{eq:moneta:tensor}))}}
    &
    E \tensord \funbara {\discr F}
    \ar[r]^{\identity{} \tensord \funbara {\unitc {\discr F}}}
    &
    E \tensord \funbara {\tc \discr F}
    \ar[d]^{\unita_E \tensord \identity{}}
    \\
    &
    {\funbara {\discr E} \tensord \funbara {\discr F}}
    \ar[r]^{\identity{} \tensord \funbara {\unitc {\discr F}}}
    \ar[d]^{\tstr {\discr E} {\discr F}}
    \ar@{}[rd]|{\txt{(naturality of $\tstrna$)}}
    &
    {\funbara {\discr E} \tensord \funbara {\tc \discr F}}
    \ar[d]|{\tstr {\discr E} {\tc \discr F}}
    \\
    &
    {\funbara {\discr E \tensorc \discr F}}
    \ar[r]^{\funbara {\identity{} \tensorc \unitc {\discr F}}}
    \ar[rd]_{\funbara {\unitc {\discr E \tensorc \discr F}}}^{\txt{(strength
        law (\ref{eq:strong:eta}))}}
    \ar[d]|{\funbara {\tstrc E F}}
    &
    {\funbara {\discr E \tensorc \tc \discr F}}
    \ar[d]^{\funbara {\strc {\discr E} {\discr F}}}
    \\
    &
    {\funbara {\discr (E \tensord F)}}
    \ar[rd]_{\funbara {\unitc {\discr (E \tensord F)}}}
    \ar@{}[r]|{\txt{(naturality of $\funbara {\unitc {}}$)}}
    &
    {\funbara {\tc (\discr E \tensorc \discr F)}}
    \ar[d]^{\funbara {\tc \tstrc E F}}
    \\
    &&
    {\funbara {\tc \discr (E \tensord F)}}
    }
  \]
  }

\paragraph{Diagram~(\ref{eq:strong:double}).}
For reasons of space, we flip the diagram so that arrows involving strengths
are vertical, and arrows involving associativities are horizontal.  Again, we
drop most subscripts from natural transformations, which are inferrable from
context.  {\small
  \[
  \xymatrix@R-5pt@C-10pt{
    \ar@{}[ddrrrr]|{\txt{(naturality of $\alphadna$)}}
    \ar@{}[ddddr]|{\txt{(monoidal\\adjunction\\(\ref{eq:moneta:tensor}))}}
    {\hbox{$
        \begin{array}{c}
          (E \tensord F)\\
          \tensord \funbara {\tc \discr G}
        \end{array}
        $}
      }
    \ar[rrrr]^{\alphadna}
    \ar[rdd]^{(\unita_E \tensord \unita_F) \tensord \identity {}}
    \ar[ddd]|{\unita_{E \tensord F} \tensord \identity {}}
    &&&&
    {\hbox{$
        \begin{array}{c}
          E \tensord (F \tensord\\
          \funbara {\tc \discr G})
        \end{array}
        $}
      }
    \ar[d]|{\identity {} \tensord (\unita_F \tensord \identity {})}
    \\
    &&&&
    {\hbox{$
        \begin{array}{c}
          E \tensord (\funbara {\discr F} \tensord\\
          \funbara {\tc \discr G})
        \end{array}
        $}
      }
    \ar[ld]_{\unita_E \tensord \identity {}}
    \ar[d]|{\identity {} \tensord \tstrna}
    \\
    &
    {\hbox{$
        \begin{array}{c}
          (\funbara {\discr E} \tensord\\
          \funbara {\discr F})\\
          \tensord \funbara {\tc \discr G}
        \end{array}
        $}
      }
    \ar[rr]^{\alphadna}
    \ar[d]_{\tstrna \tensord \identity {}}
    \ar@{}[rrdd]|{\txt{(coherence\\(\ref{eq:theta:coh:alpha})\\of $\tstrna$)}}
    &&
    {\hbox{$
        \begin{array}{c}
          \funbara {\discr E} \tensord\\
          (\funbara {\discr F} \tensord\\
          \funbara {\tc \discr G})
        \end{array}
        $}
      }
    \ar[d]|{\identity {} \tensord \tstrna}
    \ar@{}[rdd]|{\txt{(functor-\\iality of\\$\tensord$)}}
    &
    {\hbox{$
        \begin{array}{c}
          E \tensord\\
          \funbara {\discr F \tensorc \tc \discr G}
        \end{array}
        $}
      }
    \ar[d]|{\identity {} \tensord \funbara {\strdna}}
    \\
    {\hbox{$
        \begin{array}{c}
          \funbara {\discr (E \tensord F)}\\
          \tensord \funbara {\tc \discr G}
        \end{array}
        $}
      }
    \ar[d]_{\tstrna}
    \ar@{}[rd]|{\txt{(naturality\\of $\tstrna$)}}
    &
    {\hbox{$
        \begin{array}{c}
          \funbara {
            \begin{array}{c}
              \discr E\\\tensorc \discr F
            \end{array}
            }\\
          \tensord \funbara {\tc \discr G}
        \end{array}
        $}
      }
    \ar[l]_{\funbara {\tstrcna} \tensord \identity {}}^{=\funbara {\tstrcna}
      \tensord \funbara {\identity {}}}
    \ar[d]_{\tstrna}
    &&
    {\hbox{$
        \begin{array}{c}
          \funbara {\discr E} \tensord\\
          \funbara {
            \begin{array}{c}
              \discr F \tensorc\\\tc \discr G
            \end{array}
            }
        \end{array}
        $}
      }
    \ar[ld]^{\tstrna}
    \ar[d]|{\identity {} \tensord \funbara {\strcna}}
    &
    {\hbox{$
        \begin{array}{c}
          E \tensord\\
          \funbara {\tc (\discr F \tensorc \discr G)}
        \end{array}
        $}
      }
    \ar[d]|{\identity {} \tensord \funbara {\tc \tstrcna}}
                                %\ar[d]|{\eta_A \otimes^{\cal C} UF \identity \relax}
    \\
    {\hbox{$
        \funbara {
          \begin{array}{c}
            \discr (E \tensord F)\\
            \tensorc \tc \discr G
          \end{array}
          }
        $}
      }
    \ar[d]_{\funbara {\strcna}}
    \ar@{}[rd]|{\txt{(naturality\\of $\funbara \strcna$)}}
    &
    {\hbox{$
        \funbara {
          \begin{array}{c}
            (\discr E\\\tensorc \discr F)\\
            \tensorc \tc \discr G
          \end{array}
          }
        $}
      }
    \ar[l]_{\funbara {\tstrcna \tensorc \identity {}}}^{= \funbara {\tstrcna
        \tensorc \tc \identity {}}}
    \ar[d]_{\funbara {\strcna}}
    \ar[r]^{\funbara {\alphacna}}
    &
    {\hbox{$
        \funbara {
          \begin{array}{c}
            {\discr E} \tensorc\\
            (\discr F \tensorc\\\tc \discr G)
          \end{array}
          }
        $}
      }
    \ar[d]^{\funbara {\identity {} \tensorc \strcna}}
    &
    {\hbox{$
        \begin{array}{c}
          \funbara {\discr E} \tensord\\
          \funbara {
            \begin{array}{c}
              \tc (\discr F\\\tensorc \discr G)
            \end{array}
            }
        \end{array}
        $}
      }
    \ar[rd]|{\identity {} \tensord \funbara {\tc \tstrcna}}
    &
    {\hbox{$
        \begin{array}{c}
          E \tensord\\
          \funbara {\tc \discr (F \tensord G)}
        \end{array}
        $}
      }
    \ar[d]|{\unita_E \tensord \identity {}}
    \\
    {\hbox{$
        \funbara {\tc \left(
            \begin{array}{c}
              \discr (E \\\tensord F)\\
              \tensorc \discr G
            \end{array}
          \right)}
        $}
      }
    \ar[ddd]|{\funbara {\tc \tstrcna}}
    \ar@{}[dddrr]|{\txt{(coherence $\funbara {\tc
          (\ref{eq:theta:coh:alpha})}$ of $\tstrcna$)}}
    &
    {\hbox{$
        \funbara {\tc \left(
            \begin{array}{c}
              (\discr E \tensorc\\\discr F)\\
              \tensorc \discr G
            \end{array}
          \right)}
        $}
      }
    \ar[l]_{\funbara {\tc (\tstrcna \tensorc \identity {})}}
    \ar[rd]_{\funbara {\tc \alphacna}}
    \ar@{}[ru]|{\txt{(strength\\law (\ref{eq:strong:double}))}}
    &
    {\hbox{$
        \funbara {
          \begin{array}{c}
            \discr E \tensorc\\
            \tc (\discr F\\\tensorc \discr G)
          \end{array}
          }
        $}
      }
    \ar[rrd]|{\funbara {\identity {} \tensorc \tc \tstrcna}}
    \ar[d]^{\funbara {\strcna}}
    \ar@{}[rr]|{\txt{(naturality\\of $\tstrna$)}}
    &&
    {\hbox{$
        \begin{array}{c}
          \funbara {\discr E} \tensord\\
          \funbara {\tc \discr (F \tensord G)}
        \end{array}
        $}
      }
    \ar[d]|{\tstrna}
    \\
    &&
    {\hbox{$
        \funbara {\tc \left(
            \begin{array}{c}
              \discr E \tensorc\\
              (\discr F \tensorc\\
              \discr G)
            \end{array}
          \right)}
        $}
      }
    \ar[rrd]|{\funbara {\tc (\identity {} \tensorc \tstrcna)}}
    \ar@{}[rr]|{\txt{(naturality\\of $\funbara {\strcna}$)}}
    &&
    {\hbox{$
        \funbara {
          \begin{array}{c}
            \discr E \tensorc\\
            \tc \discr (F \tensord G)
          \end{array}
          }
        $}
      }
    \ar[d]|{\funbara {\strcna}}
    \\
    &&&&
    {\hbox{$
        \funbara {\tc \left(
            \begin{array}{c}
              \discr E \tensorc\\
              \discr (F \tensord G)
            \end{array}
          \right)}
        $}
      }
    \ar[d]|{\funbara {\tc \tstrcna}}
    \\
    {\hbox{$
        \funbara {\tc \discr \left(
            \begin{array}{c}
              (E\\\tensord F)\\
              \tensord G
            \end{array}
          \right)
          }
        $}
      }
    \ar[rrrr]_{\funbara {\tc \discr \alphadna}}
    &&&&
    {\hbox{$
        \funbara {\tc \discr \left(
            \begin{array}{c}
              E \tensord\\
              (F \tensord G)
            \end{array}
          \right)}
        $}
      }
    }
  \]
  } The vertical arrows on the left compose to form $t_{A \otimes^{\cal C} B,
  C}$, while the vertical arrows on the right compose to form $\identity
\relax \otimes^{\cal C} t_{B, C}$ followed by $t_{A, B \otimes^{\cal C} C}$,
whence the result.

\paragraph{Diagram~(\ref{eq:strong:mu}).}  This is the diagram below.  Again,
the diagram is flipped sideways, and certain subscripts have been dropped. The
topmost arrow from $E \tensord \funbara {\tc \discr \funbara {\tc \discr F}}$
to $E \tensord \funbara {\tc \discr F}$ is $\identity E \tensord \multd F$ by
definition, while the bottommost arrow from $\funbara {\tc \discr \funbara
  {\tc \discr (E \tensord F)}}$ to $\funbara {\tc \discr (E \tensord F)}$ is
$\multc {E \tensord F}$.  The rightmost composition of vertical arrows, from
$E \tensord \funbara {\tc \discr F}$ to $\funbara {\tc \discr (E \tensord F)}$
is $\multc {E \tensord F}$, is $\strd E F$, and the lefmost one is $\strd E
{\td F}$ followed by $\td \strd E F$.  (Recall that $\td = \funbara {\tc
  \discr}$.) {\small
  \[
  \xymatrix@C-10pt{
    {E \tensord \funbara {\tc \discr \funbara {\tc \discr F}}}
    \ar[rr]^{\identity E \tensord \funbara {\tc \counita_{\tc \discr F}}}
    \ar[d]|{\unita_E \tensord \identity {}}
    \ar@{}[rrrrd]|{\txt{(functoriality of $\tensord$)}}
    &&
    {E \tensord \funbara {\tc^2 \discr F}}
    \ar[rr]^{\identity E \tensord \funbara {\multc {\discr F}}}
    &&
    {E \tensord \funbara {\tc \discr F}}
    \ar[dd]|{\unita_E \tensord \identity {\funbara {\tc \discr F}}}
    \\
    {\funbara {\discr E} \tensord \funbara {\tc \discr \funbara {\tc \discr
          F}}}
    \ar[rr]^{\identity{} \tensord \funbara {\tc \counita_{\tc \discr
          F}}}_{=\funbara {\identity {}} \tensord \funbara {\tc \counita_{\tc \discr
          F}}}
    \ar[d]|{\tstr {\discr E} {\tc \discr \funbara {\tc \discr F}}}
    \ar@{}[rrd]|{\txt{(naturality\\of $\tstrna$)}}
    &&
    {\funbara {\discr E} \tensord \funbara {\tc^2 \discr F}}
    \ar[d]|{\tstr {\discr E} {\tc^2 \discr F}}
    \ar[rrd]^{\funbara {\identity {}} \tensord \funbara {\multc {\discr F}}}
    \ar@{}[rrdd]|{\txt{(naturality\\of $\tstrna$)}}
    &&
    \\
    {\funbara {\discr E \tensorc \tc \discr \funbara {\tc \discr
          F}}}
    \ar[rr]|{\funbara {\identity {} \tensorc \tc \counita_{\tc \discr F}}}
    \ar[d]|{\funbara {\strc {\discr E} {\discr \funbara {\tc \discr F}}}}
    \ar@{}[rrd]|{\txt{(naturality\\of $\funbara {\strcna}$)}}
    &&
    {\funbara {\discr E \tensorc \tc^2 \discr F}}
    \ar[d]|{\funbara {\strc {\discr E} {\tc \discr F}}}
    \ar[rrdd]^{\funbara {\identity {} \tensorc \multc {\discr F}}}
    &&
    {\funbara {\discr E} \tensord \funbara {\tc \discr F}}
    \ar[dd]|{\tstr {\discr E} {\tc \discr F}}
    \\
    {\funbara {\tc (\discr E \tensorc \discr \funbara {\tc \discr F})}}
    \ar[rr]|{\funbara {\tc (\identity {} \tensorc \counita_{\tc \discr
          F})}}
    \ar@{}[rrd]^{\txt{(adjunction law)}}
    \ar[rd]|{\funbara {\tc (\discr \unita_E \tensorc \identity {\discr
          \funbara {\tc \discr F}})}}
    \ar[d]|{\funbara {\tc \tstrc E {\funbara {\tc \discr F}}}}
    &&
    {\funbara {\tc (\discr E \tensorc \tc \discr F)}}
    \ar[dd]^{\funbara {\tc \strc {\discr E} {\discr F}}}
    &&
    \\
    {\funbara {\tc \discr (E \tensord \funbara {\tc \discr F})}}
    \ar[d]|{\funbara {\tc \discr (\unita_E \tensord \identity {\funbara {\tc
            \discr F}})}}
    \ar@{}[r]|{\txt{(natur-\\ality\\of $\funbara {\tc \tstrcna}$)}}
    &
    {\hbox{$
        \funbara {\tc \left(
            \begin{array}{c}
              \discr \funbara {\discr E} \tensorc\\
              \discr \funbara {\tc \discr F}
            \end{array}
        \right)}
        $}}
    \ar[ru]|{\funbara {\tc (\counita_{\discr E} \tensorc \counita_{\tc \discr
          F})}}
    \ar[ld]^{\funbara {\tc \tstrc {\funbara {\discr E}} {\funbara {\tc \discr F}}}}
    &
    &&
    {\funbara {\discr E \tensorc \tc \discr F}}
    \ar[dd]|{\funbara {\strc {\discr E} {\discr F}}}
    \\
    {\funbara {\tc \discr (\funbara {\discr E} \tensord \funbara {\tc \discr
          F})}}
    \ar[d]|{\funbara{\tc \discr \tstr {\discr E} {\tc \discr F}}}
    &&
    {\funbara {\tc^2 (\discr E \tensorc \discr F)}}
    \ar[rrd]^{\funbara {\multc {\discr E \tensorc \discr F}}}
    \ar@{}[rru]|{\txt{(strength law $\funbara {(\ref{eq:strong:mu})}$)}}
    \ar[ddd]|{\funbara {\tc^2 \tstrc E F}}
    &&
    \\
    {\funbara {\tc \discr \funbara {\discr E \tensorc \tc \discr F}}}
    \ar@/_30pt/[rruuu]_{\funbara {\tc \counita_{\discr E \tensorc \tc \discr
          F}}}
    \ar@{}[rruu]|(0.4){\txt{monoidal\\adjunction\\law $\funbara {\tc (\ref{eq:moneps:tensor})}$}}
    \ar[d]|{\funbara {\tc \discr \funbara {\strc {\discr E} {\discr F}}}}
    &&
    &&
    {\funbara {\tc (\discr E \tensorc \discr F)}}
    \ar[dd]|{\funbara {\tc \tstrc E F}}
    \\
    {\funbara {\tc \discr \funbara {\tc (\discr E \tensorc \discr F)}}}
    \ar@/_20pt/[rruu]_{\funbara {\tc \counita_{\tc (\discr E \tensorc \discr
          F)}}}
    \ar@{}[rruu]|{\txt{(naturality of $\funbara {\tc \counita}$)}}
    \ar[d]|{\funbara {\tc \discr \funbara {\tc \tstrc E F}}}
    &&
    &&
    \\
    {\funbara {\tc \discr \funbara {\tc \discr (E \tensord F)}}}
    \ar[rr]_{\funbara {\tc \counita_{\tc \discr (E \tensord F)}}}
    \ar@{}[rru]|{\txt{(naturality of $\funbara {\tc \counita}$)}}
    &&
    {\funbara {\tc^2 \discr (E \tensord F)}}
    \ar[rr]_{\funbara {\multc {\discr (E \tensord F)}}}
    &&
    {\funbara {\tc \discr (E \tensord F)}}
    \ar@{}[lluu]|{\txt{(naturality\\of $\funbara {\multc {}}$)}}
    }
  \]
  }

\paragraph{Diagram~(\ref{d_diststr}).}  Again, we flip the diagram sideways.
We recognize $\funbara {\strc {A_1} {A_2}}$ as the rightmost vertical arrow,
$\strd {\funbara {A_1}} {\funbara {A_2}}$ as the leftmost composition of
vertical arrows, $\identity {\funbara {A_1}} \tensord \dist {A_2}$ followed by
$\tstr {A_1} {\tc {A_2}}$ on the top row, and $\td (\tstr {A_1} {A_2})$
followed by $\dist {{A_1} \tensorc {A_2}}$ on the bottom row. {\small
  \[
  \xymatrix@C+10pt{
    {\funbara {A_1} \tensord \funbara {\tc \discr \funbara {A_2}}}
    \ar[r]^{\identity {\funbara {A_1}} \tensord \funbara {\tc \counita_{A_2}}}
    \ar[d]|{\unita_{\funbara {A_1}} \tensord \identity {}}
    \ar@{}[rd]|{\txt{(functoriality\\of $\tensord$)}}
    &
    {\funbara {A_1} \tensord \funbara {\tc {A_2}}}
    \ar[r]^{\identity {}}_{\txt{(adjunction law)}}
    \ar[d]|{\unita_{\funbara {A_1}} \tensord \identity{}}
    &
    {\funbara {A_1} \tensord \funbara {\tc {A_2}}}
    \ar[r]^{\tstr {A_1} {\tc {A_2}}}
    &
    {\funbara {{A_1} \tensorc \tc {A_2}}}
    \ar[dddd]|{\funbara {\strc {A_1} {A_2}}}
    \ar@{}[ddddll]|{\txt{(naturality\\of $\funbara {\strcna}$)}}
    \\
    {\funbara {\discr \funbara {A_1}} \tensord \funbara {\tc \discr \funbara {A_2}}}
    \ar[r]^{\funbara {\identity {}} \tensord \funbara {\tc \counita_{A_2}}}
    \ar[d]|{\tstr {\discr \funbara {A_1}} {\tc \discr \funbara {A_2}}}
    \ar@{}[rd]|{\txt{(naturality\\of $\tstrna$)}}
    &
    {\funbara {\discr \funbara {A_1}} \tensord \funbara {\tc {A_2}}}
    \ar[ru]|{\funbara {\counita_{A_1}} \tensord \identity {\funbara {\tc {A_2}}}}
    \ar[d]|{\tstr {\discr \funbara {A_1}} {\tc {A_2}}}
    &&
    \\
    {\funbara {\discr \funbara {A_1} \tensorc \tc \discr \funbara {A_2}}}
    \ar[r]^{\funbara {\identity {} \tensorc \tc \counita_{A_2}}}
    \ar@{}[rd]|{\txt{(naturality\\of $\funbara \strcna$)}}
    \ar[d]|{\funbara {\strc {\discr \funbara {A_1}} {\discr \funbara {A_2}}}}
    &
    {\funbara {\discr \funbara {A_1} \tensorc \tc {A_2}}}
    \ar[rruu]_{\funbara {\counita_{A_1} \tensorc \identity {\tc {A_2}}}}
    \ar@{}[ruu]|{\txt{(naturality\\of $\tstrna$)}}
    \ar[d]|{\funbara {\strc {\discr \funbara {A_1}} {A_2}}}
    &&
    \\
    {\funbara {\tc (\discr \funbara {A_1} \tensorc \discr \funbara {A_2})}}
    \ar[r]^{\funbara {\tc (\identity {} \tensorc \counita_{A_2})}}
    \ar[d]|{\funbara {\tc \tstrc {\funbara {A_1}} {\funbara {A_2}}}}
    \ar@{}[rrd]|{\txt{(monoidal natural\\transformation law $\funbara {\tc (\ref{eq:moneps:tensor})}$)}}
    &
    {\funbara {\tc (\discr \funbara {A_1} \tensorc {A_2})}}
    \ar[rrd]_{\funbara {\tc (\counita_{A_1} \tensorc \identity {A_2})}}
    &&
    \\
    {\funbara {\tc \discr (\funbara {A_1} \tensord \funbara {A_2})}}
    \ar[r]_{\funbara {\tc \discr \tstr {A_1} {A_2}}}
    &
    {\funbara {\tc \discr \funbara {{A_1} \tensorc {A_2}}}}
    \ar[rr]_{\funbara {\tc \counita_{{A_1} \tensorc {A_2}}}}
    &&
    {\funbara {\tc ({A_1} \tensorc {A_2})}}
    }
  \]
  }
\qed


==> bistrong.tex <==


\section{Monoidal Monads, Commutative Monads}
\label{app:monoidal}


\subsection{From Mediators to Strengths and Dual Strengths}
\label{app:monoidal:->}

Let $(\td, \unitd{}, \multd{}, \bistrdna)$ be a monoidal monad.  Let $\strd A
B = \bistrd A B \circ (\unitd A \tensord \identity {\td B})$, $\strd A B' =
\bistrd A B \circ (\identity {\td A} \tensord \unitd B)$. We show that
$\strdna$ is a strength, $\strdna'$ a dual strength, and that
Diagrams~(\ref{eq:tt'_alpha}) and~(\ref{eq:tt'}) commute.

\paragraph{Diagram~(\ref{eq:strong:l}).}
This is exactly Diagram~(\ref{eq:monoidal:l}).

\paragraph{Diagram~(\ref{eq:strong:eta}).}
This is exactly Diagram~(\ref{eq:monoidal:eta}).

\paragraph{Diagram~(\ref{eq:strong:double}).}
This is shown by the diagram below.  The topmost row is $\strd {A \tensord B}
C$, while the bottommost composition of morphisms from $\td ((A \tensord B)
\tensord C)$ to $\td (A \tensord (B \tensord C))$ is $\identity A \tensord
\strd B C$ followed by $\strd A {B \tensord C}$.
\[
\xymatrix@R-5pt@C-10pt{
  {(A \tensord B) \tensord \td C}
  \ar[r]^{\unitd {A \tensord B} \tensord \identity {}}
  \ar[ddd]_{\alphad A B {\td C}}
  \ar[rd]_{(\unitd A \tensord \unitd B) \tensord \identity
    {}}^{(\ref{eq:monoidal:eta})}
  \ar@{}[rdd]_{\txt{(naturality\\of $\alphadna$)}}
  &
  {\td (A \tensord B) \tensord \td C}
  \ar[rr]^{\bistrd {A \tensord B} C}
  \ar@{}[rrdd]|{\txt{(mediator law (\ref{eq:monoidal:double}))}}
  &
  &
  {\td ((A \tensord B) \tensord C)}
  \ar[dd]^{\td \alphad A B C}
  \\
  &
  {(\td A \tensord \td B) \tensord \td C}
  \ar[u]_{\bistrd A B \tensord \identity {}}
  \ar[d]^{\alphad {\td A} {\td B} {\td C}}
  &
  &
  \\
  &
  {\td A \tensord (\td B \tensord \td C)}
  \ar[r]_{\identity {} \tensord \bistrd B C}
  \ar@{}[rd]|{\txt{(functoriality\\of $\tensord$)}}
  &
  {\td A \tensord \td (B \tensord C)}
  \ar[r]_{\bistrd A {B \tensord C}}
  &
  {\td (A \tensord (B \tensord C))}
  \\
  {A \tensord (B \tensord \td C)}
  \ar[ru]^{\unitd A \tensord (\unitd B \tensord \identity {})}
  \ar[r]_{\identity {} \tensord (\unitd B \tensord \identity {})}
  &
  {A \tensord (\td B \tensord \td C)}
  %\ar[u]_{\unitd A \tensord \identity {}}
  \ar[r]_{\identity {} \tensord \bistrd B C}
  &
  {A \tensord \td (B \tensord C)}
  \ar[u]_{\unitd A \tensord \identity {}}
  &
  }
\]

\paragraph{Diagram~(\ref{eq:strong:mu}).}
\[
\xymatrix@R-5pt@C-10pt{
  {A \tensord \td^2 B}
  \ar[r]^{\unitd A \tensord \identity {}}
  \ar[dd]_{\identity {} \tensord \multd B}
  \ar@{}[rdd]|{\txt{(functoriality\\of $\tensord$)}}
  &
  {\td A \tensord \td^2 B}
  \ar[r]^{\bistrd A {\td B}}
  \ar[rd]_{\td \unitd A \tensord \td \identity {}}
  \ar@{}[rrd]|{\txt{(naturality\\of $\bistrdna$)}}
  \ar@/_25pt/[rdd]_{\identity {} \tensord \multd B}^(0.7){\txt{(monad\\law)}}
  &
  {\td (A \tensord \td B)}
  \ar[r]^{\td (\unitd A \tensord \identity {})}
  &
  {\td (\td A \tensord \td B)}
  \ar[r]^{\td \bistrd A B}
  &
  {\td^2 (A \tensord B)}
  \ar[dd]^{\multd {A \tensord B}}
  \\
  &
  &
  {\td^2 A \tensord \td^2 B}
  \ar[ru]_{\bistrd {\td A} {\td B}}
  \ar[d]^{\multd A \tensord \multd B}
  &
  &
  \\
  {A \tensord \td B}
  \ar[rr]_{\unitd A \tensord \identity {}}
  &
  &
  {\td A \tensord \td B}
  \ar[rr]_{\bistrd A B}
  \ar@{}[rruu]_{\txt{(mediator\\law (\ref{eq:monoidal:mu}))}}
  &
  &
  {\td (A \tensord B)}
  }
\]

So $\tstrna$ is a strength.  That $\tstrna'$ is a dual strength is proved
similarly.  We use Diagram~(\ref{eq:monoidal:r}) instead of
Diagram~(\ref{eq:monoidal:l}) to prove the dual form of
Diagram~(\ref{eq:strong:l}).

\paragraph{Diagram~(\ref{eq:tt'_alpha}).}
In the diagram below, the top row is $\strd A B \tensord \identity {}$
followed by $\strd {A \tensord B} C'$, while the bottom row is $\identity {}
\tensord \strd B C'$ followed by $\strd A {B \tensord C}$.
\[
\xymatrix@C-10pt@R-5pt{
  {\hbox{$
      \begin{array}{c}
        (A \tensord \td B)\\\tensord C
      \end{array}
      $}}
  \ar[r]^{(\unitd A \tensord \identity {})}_{\tensord \identity {}}
  \ar[ddd]|{\alphad A {\td B} C}
  \ar[rrd]_{(\unitd A \tensord \identity {}) \tensord \unitd C}
  \ar@{}[rrrrd]|{\txt{(functoriality\\of $\tensord$)}}
  &
  {\hbox{$
      \begin{array}{c}
        (\td A \tensord \td B)\\\tensord C
      \end{array}
      $}}
  \ar[r]^{\bistrd A B \tensord \identity {}}
  &
  {\hbox{$
      \begin{array}{c}
        \td (A \tensord B)\\ \tensord C
      \end{array}
      $}}
  \ar[r]^{\identity {} \tensord \unitd C}
  &
  {\hbox{$
      \begin{array}{c}
        \td (A \tensord B)\\ \tensord \td C
      \end{array}
      $}}
  \ar[r]^{\bistrd {A \tensord B} C}
  &
  {\hbox{$
      \begin{array}{c}
        \td ((A \tensord B)\\ \tensord C)
      \end{array}
      $}}
  \ar[ddd]|{\td \alphad A B C}
  \\
  &
  &
  {(\td A \tensord \td B) \tensord \td C}
  \ar[ru]_{\bistrd A B \tensord \identity {}}
  \ar[d]^{\alphad {\td A} {\td B} {\td C}}
  &
  &
  \\
  &
  &
  {\td A \tensord (\td B \tensord \td C)}
  \ar[rd]^{\identity {} \tensord \bistrd B C}
  &
  &
  \\
  {\hbox{$
      \begin{array}{c}
        A \tensord \\(\td B \tensord C)
      \end{array}
      $}}
  \ar[r]^{\identity {} \tensord}_{(\identity {} \tensord \unitd C)}
  \ar[rru]^{\unitd A \tensord (\identity {} \tensord \unitd C)}
  \ar@{}[rrrru]|{\txt{(functoriality\\of $\tensord$)}}
  \ar@{}[rruuu]|{\txt{(naturality\\of $\alphadna$)}}
  &
  {\hbox{$
      \begin{array}{c}
        A \tensord \\(\td B \tensord \tc C)
      \end{array}
      $}}
  \ar[r]_{\identity {} \tensord \bistrd B C}
  &
  {\hbox{$
      \begin{array}{c}
        A \tensord \\\td (\td \tensord C)
      \end{array}
      $}}
  \ar[r]_{\unitd A \tensord \identity {}}
  &
  {\hbox{$
      \begin{array}{c}
        \td A \tensord\\\td (B \tensord C)
      \end{array}
      $}}
  \ar[r]_{\bistrd A {B \tensord C}}
  \ar@{}[uuu]|{\txt{(mediator\\law (\ref{eq:monoidal:double}))}}
  &
  {\hbox{$
      \begin{array}{c}
        \td (A \tensord \\(B \tensord C))
      \end{array}
      $}}
  }
\]

\paragraph{Diagram (\ref{eq:tt'}).}  This is the diagram below, where the top
row is $\strd {\td A} B$, the leftmost vertical arrows form $\strd A {\td
  B}'$, the rightmost ones form $\td \strd A B'$ followed by $\multd {A
  \tensord B}$, and the bottom row is $\td \strd A B$ followed by $\multd {A
  \tensord B}$. Note that, as announced, the common diagonal from the top left
corner to the bottom right corner is $\bistrd A B$.
\[
\xymatrix@R-5pt@C-10pt{
  {\td A \tensord \td B}
  \ar[rr]^{\unitd {\td A} \tensord \identity {}}
  \ar[dd]|{\identity {} \tensord \unitd {\td B}}
  \ar[rrdd]|{\identity {} \tensord \identity {}}^{\txt{(monad laws}}_{\txt{and functor-\\iality of $\tensord$)}}
  &
  &
  {\td^2 A \tensord \td B}
  \ar[rr]^{\bistrd {\td A} B}
  \ar[d]_{\identity{} \tensord \td \unitd B}
  \ar@{}[rrd]|{\txt{(natur-\\ality of\\$\bistrdna$)}}
  &
  &
  {\td (\td A \tensord B)}
  \ar[dd]^{\td (\identity {} \tensord \unitd B)}
  \\
  &
  &
  {\td^2 A \tensord \td^2 B}
  \ar[d]_{\multd A \tensord \multd B}
  \ar[rrd]|{\bistrd {\td A} {\td B}}
  \ar@{}[rrdd]|{\txt{(mediator\\law (\ref{eq:monoidal:mu}))}}
  &
  &
  \\
  {\td A \tensord \td^2 B}
  \ar[dd]|{\bistrd A {\td B}}
  \ar[r]^{\td \unitd A \tensord \identity {}}
  \ar@{}[rdd]|{\txt{(natur-\\ality of\\$\bistrdna$)}}
  &
  {\td^2 A \tensord \td^2 B}
  \ar[r]^{\multd A \tensord \multd B}
  \ar[rdd]|{\bistrd {\td A} {\td B}}
  \ar@{}[rrdd]|{\txt{(mediator\\law (\ref{eq:monoidal:mu}))}}
  &
  {\td A \tensord \td B}
  \ar[rrdd]|{\bistrd A B}
  &
  &
  {\td (\td A \tensord \td B)}
  \ar[d]^{\td \bistrd A B}
  \\
  &
  &
  &
  &
  {\td^2 (A \tensord B)}
  \ar[d]^{\multd {A \tensord B}}
  \\
  {\td (A \tensord \td B)}
  \ar[rr]_{\td (\unitd A \tensord \identity {})}
  &
  &
  {\td (\td A \tensord \td B)}
  \ar[r]_{\td \bistrd A B}
  &
  {\td^2 (A \tensord B)}
  \ar[r]_{\multd {A \tensord B}}
  &
  {\td (A \tensord B)}
  }
\]


\subsection{From Strengths and Dual Strengths to Mediators}
\label{app:monoidal:<-}

Let $(\td, \unitd{}, \multd{})$ be a monad such that $\strdna$ is a strength
and $\strdna'$ is a dual strength making Diagrams~(\ref{eq:tt'_alpha})
and~(\ref{eq:tt'}) commute.  Let $\bistrdna$ be the common diagonal of
Diagram~(\ref{eq:tt'}), i.e., $\bistrd A B = \multd {A \tensord B} \circ \td
\strd A B' \circ \strd {\td A} B = \multd {A \tensord B} \circ \td \strd A B
\circ \strd A {\td B}'$.  We show that $\bistrdna$ is a mediator, which
means that we check Diagrams~(\ref{eq:monoidal:l}), (\ref{eq:monoidal:r}),
(\ref{eq:monoidal:eta}), (\ref{eq:monoidal:double}), and
(\ref{eq:monoidal:mu}).  By convention, call (\ref{eq:strong:l}'),
(\ref{eq:strong:eta}'), (\ref{eq:strong:double}'), (\ref{eq:strong:mu}') the
dual diagrams satisfied by the dual strength $\strdna'$.

First, notice that $\strd A B = \bistrd A B \circ (\unitd A \tensord \identity
{\td B})$.  Indeed, using the definition $\bistrd A B = \multd {A \tensord B}
\circ \td \strd A B' \circ \strd {\td A} B$, $\bistrd A B \circ (\unitd A
\tensord \identity {\td B})$ is the top row of the following diagram, while
$\strd A B$ is the bottom composition of arrows from $A \tensord \td B$ to
$\td (A \tensord B)$.
\[
\xymatrix@R+15pt{
  {A \tensord \td B}
  \ar[r]^{\unitd A \tensord \identity {\td B}}
  \ar[rrd]_{\strd A B}
  &
  {\td A \tensord \td B}
  \ar[r]^{\strd {\td A} B}
  &
  {\td {\td A \tensord B}}
  \ar[r]^{\td \strd A B'}
  &
  {\td^2 (A \tensord B)}
  \ar[r]^{\multd {A \tensord B}}
  &
  {\td (A \tensord B)}
  \\
  &
  &
  {\td (A \tensord B)}
  \ar[u]|{\td (\unitd A \tensord \identity B)}
  \ar@{}[lu]|(0.6){\txt{(naturality\\of $\strdna$)}}
  \ar[ru]|{\td \unitd {A \tensord B}}^{(\ref{eq:strong:eta}')}
  \ar@/_20pt/[rru]_{\identity {\td (A \tensord B)}}^{\txt{(monad law)}}
  &
  &
  }
\]

\paragraph{Diagram~(\ref{eq:monoidal:l})}
is then just Diagram~(\ref{eq:strong:l}).

\paragraph{Diagram~(\ref{eq:monoidal:r}).}
Similarly, $\strd A B' = \bistrd A B \circ (\identity {\td A} \tensord \unitd
B)$ (here we use the other characterization of $\bistrd A B$ as $\multd {A
  \tensord B} \circ \td \strd A B \circ \strd A {\td B}'$ and
(\ref{eq:strong:eta})), so Diagram~(\ref{eq:monoidal:r}) is just
Diagram~(\ref{eq:strong:l}').

\paragraph{Diagram~(\ref{eq:monoidal:eta}).}
Immediate using (\ref{eq:strong:eta}) and $\strd A B = \bistrd A B \circ
(\unitd A \tensord \identity {\td B})$: $\bistrd A B \circ (\unitd A \tensord
\unitd B) = \strd A B \circ (\unitd A \circ \identity B) = \unitd {A \tensord
  B}$.

\paragraph{Diagram~(\ref{eq:monoidal:double}).}
This one is harder, and is proved by considering the diagram below. The top
row is $\bistrd A B \tensord \identity {\td C}$, the rightmost vertical arrows
form $\bistrd {A \tensord B} C$ followed by $\td \alphad A B C$, while the
leftmost ones form $\alphad {\td A} {\td B} {\td C}$ followed by $\identity
{\td A} \tensord \bistrd B C$, and the bottommost row is $\bistrd A {B
  \tensord C}$. {\small
\[
\xymatrix@C-15pt@R-5pt{
  {\hbox{$
      \begin{array}{c}
        (\td A \tensord \td B)\\\tensord \td C
      \end{array}
      $}}
  \ar[r]^{\strd A {\td B}'}_{\tensord \identity{}}
  \ar[dd]|(0.6){\alphad {\td A} {\td B} {\td C}}
  \ar@{}[rdd]|(0.4){\txt{(dual\\strength\\law\\(\ref{eq:strong:double}'))}}
  &
  {\hbox{$
      \begin{array}{c}
        \td (A \tensord \td B)\\\tensord \td C
      \end{array}
      $}}
  \ar[r]^{\td \strd A B}_{\tensord \identity {}}
  \ar[d]|{\strd {A \tensord \td B} {\td C}'}
  \ar@{}[rd]|{\txt{(natur-\\ality\\of $\strdna'$)}}
  &
  {\hbox{$
      \begin{array}{c}
        \td^2 (A \tensord B)\\\tensord \td C
      \end{array}
      $}}
  \ar[d]|{\strd {\td (A \tensord B)} {\td C}'}
  \ar[rrr]^{\multd {A \tensord B} \tensord \identity {}}
  \ar@{}[rrrdd]|{\txt{(dual strength\\law (\ref{eq:strong:mu}'))}}
  &
  &
  &
  {\hbox{$
      \begin{array}{c}
        \td (A \tensord B)\\\tensord \td C
      \end{array}
      $}}
  \ar[d]|{\strd {A \tensord B} {\td C}'}
  \\ %\\
  &
  {\hbox{$
      \begin{array}{c}
        \td ((A \tensord \td B)\\\tensord \td C)
      \end{array}
      $}}
  \ar[r]^{\td (\strd A B}_{\tensord \identity {})}
  \ar[d]|{\td \alphad A {\td B} {\td C}}
  \ar@{}[rdd]|{\txt{((\ref{eq:tt'_alpha}))}}
  &
  {\hbox{$
      \begin{array}{c}
        \td (\td (A \tensord B)\\\tensord \td C)
      \end{array}
      $}}
  \ar[d]|{\td \strd {A \tensord B} {\td C}'}
  &
  &
  &
  {\hbox{$
      \begin{array}{c}
        \td ((A \tensord B)\\\tensord \td C)
      \end{array}
      $}}
  \ar[d]|{\td \strd {A \tensord B} C}
  \\ %\\
  {\hbox{$
      \begin{array}{c}
        \td A \tensord \\ (\td B \tensord \td C)
      \end{array}
      $}}
  \ar[r]^{\strd A {\td B \tensord \td C}'}
  \ar[d]|{\identity {} \tensord \strd B {\td C}'}
  \ar@{}[rddd]|{\txt{(natur-\\ality\\of $\strdna'$)}}
  &
  {\hbox{$
      \begin{array}{c}
        \td (A \tensord \\ (\td B \tensord \td C))
      \end{array}
      $}}
  \ar[d]|{\td (\identity {} \tensord \strd B {\td C}')}
  &
  {\hbox{$
      \begin{array}{c}
        \td^2 ((A\\ \tensord B) \\ \tensord \td C)
      \end{array}
      $}}
  \ar[d]|{\td^2 \alphad A B {\td C}}
  \ar[r]_{\td^2 \strd {A \tensord B} C}
  \ar@{}[rdd]|{\txt{($\td^2$ of\\strength\\law\\(\ref{eq:strong:double}))}}
  \ar[rrru]|{\multd {(A \tensord B) \tensord \td C}}
  &
  {\hbox{$
      \begin{array}{c}
        \td^3 ((A\\ \tensord B) \\ \tensord C)
      \end{array}
      $}}
  \ar[dd]|{\td^3 \alphad A B C}
  \ar[rd]^{\td \multd {
                                %(A \tensord B) \tensord C
      }}
  \ar@{}[rddd]|{\txt{(natur-\\ality of\\$\td \multd{}$)}}
  \ar[rr]^{\multd {\td ((A \tensord B) \tensord C)}}
  \ar@{}[rrd]^{\txt{(monad law)}}
  \ar@{}[rru]_{\txt{(naturality of $\multd{}$)}}
  &
  &
  {\hbox{$
      \begin{array}{c}
        \td^2 ((A \tensord B) \\ \tensord C)
      \end{array}
      $}}
  \ar[d]|{\multd {}}
  \\ %\\
  {\hbox{$
      \begin{array}{c}
        \td A \tensord \\ \td (B \tensord \td C)
      \end{array}
      $}}
  %\ar[r]^{\strd A {\td (B \tensord \td C)}'}
  \ar[d]|{\identity {} \tensord \td \strd B C}
  &
  {\hbox{$
      \begin{array}{c}
        \td (A \tensord \\ \td (B \tensord \td C))
      \end{array}
      $}}
  \ar[d]|{\td (\identity {} \tensord \td \strd B C)}
  \ar[r]^{\td \strd A {B \tensord \td C}}
  \ar@{}[rd]|{\txt{(natur-\\ality\\of $\td \strdna$)}}
  &
  {\hbox{$
      \begin{array}{c}
        \td^2 (A \tensord \\ (B \tensord \td C))
      \end{array}
      $}}
  \ar[d]|{\td^2 (\identity {} \tensord \strd B C)}
  &
  &
  {\hbox{$
      \begin{array}{c}
        \td^2 ((A \tensord B)\\ \tensord C)
      \end{array}
      $}}
  \ar[dd]|{\td^2 \alphad A B C}
  \ar@{}[rdd]|{\txt{(natur-\\ality\\of $\multd{}$)}}
  \ar[r]^{\multd {}}
  &
  {\hbox{$
      \begin{array}{c}
        \td ((A \tensord B)\\ \tensord C)
      \end{array}
      $}}
  \ar[dd]|{\td \alphad A B C}
  \\ %\\
  {\hbox{$
      \begin{array}{c}
        \td A \tensord \\ \td^2 (B \tensord C)
      \end{array}
      $}}
  %\ar[r]^{\strd A {\td^2 (B \tensord C)}'}
  \ar[d]|{\identity {} \tensord \multd {B \tensord C}}
  &
  {\hbox{$
      \begin{array}{c}
        \td (A \tensord \\ \td^2 (B \tensord C))
      \end{array}
      $}}
  \ar[d]|{\td (\identity {} \tensord \multd {B \tensord C})}
  \ar[r]^{\td \strd A {\td (B \tensord C)}}
  \ar@{}[rrrd]|{\txt{($\td$ of strength\\law (\ref{eq:strong:mu}))}}
  &
  {\hbox{$
      \begin{array}{c}
        \td^2 (A \tensord \\ \td (B \tensord C))
      \end{array}
      $}}
  \ar[r]^{\td^2 \strd A {B \tensord C}}
  &
  {\hbox{$
      \begin{array}{c}
        \td^3 (A \tensord \\ (B \tensord C))
      \end{array}
      $}}
  \ar[rd]|{\td \multd {A \tensord (B \tensord C)}}
  &
  &
  \\ %\\
  {\hbox{$
      \begin{array}{c}
        \td A \tensord \\ \td (B \tensord C)
      \end{array}
      $}}
  \ar[r]^{\strd A {\td (B \tensord C)}'}
  &
  {\hbox{$
      \begin{array}{c}
        \td (A \tensord \\ \td (B \tensord C))
      \end{array}
      $}}
  \ar[rrr]_{\td \strd A {B \tensord C}}
  &
  &
  &
  {\hbox{$
      \begin{array}{c}
        \td^2 (A \tensord \\ (B \tensord C))
      \end{array}
      $}}
  \ar[r]_{\multd {}}
  &
  {\hbox{$
      \begin{array}{c}
        \td (A \tensord \\ (B \tensord C))
      \end{array}
      $}}
  }
\]
}

\paragraph{Diagram~(\ref{eq:monoidal:mu}).}

First, we notice that
\begin{eqnarray}
  \label{eq:mu_td_t'}
  \multd {A \tensord B} \circ \td \bistrd A B \circ \strd {\td A} {\td B}'
  & = &
  \bistrd A B \circ (\multd A \tensord \identity {\td B})
\end{eqnarray}

\noindent
\begin{minipage}{3.7cm}
  This is shown using the diagram on the right.  The left-hand side is the
  path from the top left corner to the bottom right corner on the right that
  goes down then right, and the right-hand side is the path going right then
  down.
\end{minipage}
\begin{minipage}{8.3cm}
  \[
  \xymatrix@C+30pt@R-10pt{
    {\td^2 A \tensord \td B}
    \ar[r]^{\multd A \tensord \identity {}}
    \ar[d]_{\strd {\td A} {\td B}'}
    \ar@{}[rdd]|{\txt{(dual strength\\law (\ref{eq:strong:mu}'))}}
    &
    {\td A \tensord \td B}
    \ar[d]^{\strd A {\td B}'}
    \\
    {\td (\td A \tensord \td B)}
    \ar[d]_{\td \strd A {\td B}}
    &
    {\td (A \tensord \td B)}
    \ar[d]^{\td \strd A B}
    \\
    {\td^2 (A \tensord \td B)}
    \ar[ru]|{\multd {A \tensord \td B}}
    \ar[d]_{\td^2 \strd A B}
    \ar@{}[r]|{\txt{(naturality\\of $\multd{}$)}}
    &
    {\td^2 (A \tensord B)}
    \ar[dd]^{\multd {A \tensord B}}
    \\
    {\td^3 (A \tensord B)}
    \ar[ru]|{\multd {\td (A \tensord B)}}
    \ar[d]_{\td \multd {A \tensord B}}
    \ar@{}[r]|{\txt{(monad law)}}
    &
    \\
    {\td^2 (A \tensord B)}
    \ar[r]_{\multd {A \tensord B}}
    &
    {\td (A \tensord B)}
    }
  \]
\end{minipage}

\noindent
By symmetry, the following also holds:
\begin{eqnarray}
  \label{eq:mu_td_t}
  \multd {A \tensord B} \circ \td \bistrd A B \circ \strd {\td A} {\td B}
  & = &
  \bistrd A B \circ (\identity {\td A} \tensord \multd B)
\end{eqnarray}

Diagram~(\ref{eq:monoidal:mu}) then follows.  The top row below is $\bistrd
{\td A} {\td B}$, while the leftmost vertical arrows form $\multd A \tensord
\multd B$.
\[
\xymatrix@C-5pt{
  {\td^2 A \tensord \td^2 B}
  \ar[r]^{\strd {\td^2 A} {\td B}}
  \ar[dd]_{\multd A \tensord \identity {\td^2 B}}
  \ar@{}[rdd]|{\txt{(natur-\\ality\\of $\strdna$)}}
  &
  {\td (\td^2 A \tensord \td B)}
  \ar[r]^{\td \strd {\td A} {\td B}'}
  \ar[dd]|{\td (\multd A \tensord \identity {\td B})}
  \ar@{}[rdd]|{\txt{(\ref{eq:mu_td_t'})}}
  &
  {\td^2 (\td A \tensord \td B)}
  \ar[r]^{\multd {\td A \tensord \td B}}
  \ar[d]|{\td^2 \bistrd A B}
  \ar@{}[rd]|{\txt{(naturality\\of $\multd{}$)}}
  &
  {\td (\td A \tensord \td B)}
  \ar[d]^{\td \bistrd A B}
  \\
  &
  &
  {\td^3 (A \tensord B)}
  \ar[r]^{\multd {\td (A \tensord B)}}
  \ar[d]|{\td \multd {A \tensord B}}
  \ar@{}[rd]|{\txt{(monad\\law)}}
  &
  {\td^2 (A \tensord B)}
  \ar[dd]^{\multd {A \tensord B}}
  \\
  {\td A \tensord \td^2 B}
  \ar[r]_{\strd {\td A} {\td B}}
  \ar[d]_{\identity {\td A} \tensord \multd B}
  \ar@{}[rrrd]|{\txt{(\ref{eq:mu_td_t})}}
  &
  {\td (\td A \tensord \td B)}
  \ar[r]_{\td \bistrd A B}
  &
  {\td^2 (A \tensord B)}
  \ar[rd]_{\multd {A \tensord B}}
  &
  \\
  {\td A \tensord \td B}
  \ar[rrr]_{\bistrd A B}
  &
  &
  &
  {\td (A \tensord B)}
  }
\]


\subsection{Monoidal Monad Morphisms}
\label{app:monoidal:monmor}

We first show that every monoidal monad morphism from $(\tc, \unitc{},
\multc{}, \bistrcna)$ to $(\td, \unitd{}, \multd{}, \bistrdna)$ is both a
strong monad morphism from $(\tc, \unitc{}, \multc{}, \strcna)$ to $(\td,
\unitd{}, \multd{}, \strdna)$ and (by symmetry) a dual strong monad morphism
from $(\tc, \unitc{}, \multc{}, \strcna')$ to $(\td, \unitd{}, \multd{},
\strdna')$, where $\strd A B = \bistrd A B \circ (\unitd A \tensord \identity
{\td B})$, $\strd A B' = \bistrd A B \circ (\identity {\td A} \tensord \unitd
B)$.  This is by the following diagram.

\[
\xymatrix@C+10pt{
  {\funbara{A_1} \tensord \td \funbara{A_2}}
  \ar[r]^{\unitd {\funbara {A_1}} \tensord \identity {}}
  \ar[rd]_{\funbara {\unitc {A_1}} \tensord \dist
    {A_2}}^{\txt{(\ref{d_distlaw})}}
  \ar[d]_{\identity {} \tensord \dist {A_2}}
  &
  {\td \funbara{A_1} \tensord \td \funbara{A_2}}
  \ar[r]^{\bistrd{\funbara{A_1}}{\funbara{A_2}}}
  \ar[d]|{\dist {A_1} \tensord \dist {A_2}}
  \ar@{}[rdd]|{\txt{(monoidal\\monad\\morphism\\(\ref{d_distbistr}))}}
  &
  {\td (\funbara {A_1} \tensord \funbara {A_2})}
  \ar[d]^{\td (\tstr {A_1} {A_2})}
  \\
  {\funbara {A_1} \tensord \funbara {\tc {A_2}}}
  \ar[r]_{\funbara {A_1} \tensord \identity {}}
  \ar[d]_{\tstr {A_1} {\tc {A_2}}}
  \ar@{}[rd]|{\txt{(naturality\\of $\tstrna$)}}
  &
  {\funbara {\tc {A_1}} \tensord \funbara {\tc {A_2}}}
  \ar[d]|{\tstr {\tc {A_1}} {\tc {A_2}}}
  &
  {\td \funbara {A_1 \tensorc A_2}}
  \ar[d]^{\dist {A_1 \tensorc A_2}}
  \\
  {\funbara {A_1} \tensorc \tc {A_2}}
  \ar[r]_{\funbara {\unitc {A_1} \tensorc \identity {}}}
  &
  {\funbara {\tc {A_1} \tensorc \tc {A_2}}}
  \ar[r]_{\funbara {\bistrc {A_1} {A_2}}}
  &
  {\funbara {\tc (A_1 \tensorc A_2)}}
  }
\]

Conversely, let $\dist{}$ be both a strong monad morphism from $(\tc,
\unitc{}, \multc{}, \strcna)$ to $(\td, \unitd{}, \multd{}, \strdna)$ and a
dual strong monad morphism from $(\tc, \unitc{}, \multc{}, \strcna')$ to
$(\td, \unitd{}, \multd{}, \strdna')$.  Let $\bistrdna$ be the common diagonal
of Diagram~(\ref{eq:tt'}), i.e., $\bistrd A B = \multd {A \tensord B} \circ
\td \strd A B' \circ \strd {\td A} B = \multd {A \tensord B} \circ \td \strd A
B \circ \strd A {\td B}'$.  Define $\bistrcna$ similarly.

In the diagram below, the top row is $\bistrd {\funbara {A_1}} {\td {\funbara
    {A_1}}}$, while the leftmost vertical arrows from $\dist {A_1} \tensord
\dist {A_2}$ followed by $\tstr {\tc {A_1}} {\tc {A_2}}$.  The bottom row is
$\funbara {\bistrc {A_1} {A_2}}$ followed by $\funbara {\multc {A_1 \tensorc
    A_2}}$.
\[
\xymatrix{
  {\td \funbara {A_1} \tensord \td \funbara {A_2}}
  \ar[r]^{\strd {\funbara {A_1}} {\td {\funbara {A_2}}}'}
  \ar[d]|{\identity {} \tensord \dist {A_2}}
  \ar@{}[rd]|{\txt{(naturality\\of $\strdna'$)}}
  &
  {\td (\funbara {A_1} \tensord \td \funbara {A_2})}
  \ar[r]^{\td \strd {\funbara {A_1}} {\funbara {A_2}}}
  \ar[d]|{\td (\identity {} \tensord \dist {A_2})}
  \ar@{}[rdd]|{\txt{(strong\\monad\\morphism\\(\ref{d_distbistr}))}}
  &
  {\td^2 (\funbara {A_1} \tensord \funbara {A_2})}
  \ar[r]^{\multd {\funbara {A_1} \tensord \funbara {A_2}}}
  \ar[d]|{\td^2 \tstr {A_1} {A_2}}
  \ar@{}[rd]|{\txt{(natur-\\ality\\of $\multd{}$)}}
  &
  {\td (\funbara {A_1} \tensord \funbara {A_2})}
  \ar[d]|{\td \tstr {A_1} {A_2}}
  \\
  {\td \funbara {A_1} \tensord \funbara {\tc {A_2}}}
  \ar[r]_{\strd {\funbara {A_1}} {\funbara {\tc {A_2}}}'}
  \ar[d]|{\dist {A_1} \tensord \identity {}}
  \ar@{}[rdd]|{\txt{(dual\\strong\\monad\\morphism\\(\ref{d_distbistr}'))}}
  &
  {\td (\funbara {A_1} \tensord \funbara {\tc {A_2}})}
  \ar[d]|{\td \tstr {A_1} {\tc {A_2}}}
  &
  {\td^2 \funbara {A_1 \tensorc A_2}}
  \ar[d]|{\td \dist {A_1 \tensorc A_2}}
  \ar[r]_{\multd {\funbara {A_1 \tensorc A_2}}}
  \ar@{}[rdd]|{\txt{(monad\\morph-\\ism (\ref{d_distlaw}))}}
  &
  {\td \funbara {A_1 \tensorc A_2}}
  \ar[dd]|{\dist {A_1 \tensorc A_2}}
  \\
  {\funbara {\tc {A_1}} \tensord \funbara {\tc {A_2}}}
  \ar[d]|{\tstr {\tc {A_1}} {\tc {A_2}}}
  &
  {\td \funbara {A_1 \tensorc \tc {A_2}}}
  \ar[d]|{\dist {A_1 \tensorc \tc {A_2}}}
  \ar[r]^{\td \funbara {\strc {A_1} {A_2}}}
  \ar@{}[rd]|{\txt{(naturality\\of $\dist{}$)}}
  &
  {\td \funbara {\tc (A_1 \tensorc A_2)}}
  \ar[d]|{\dist {\tc (A_1 \tensorc A_2)}}
  &
  \\
  {\funbara {\tc {A_1} \tensorc \tc {A_2}}}
  \ar[r]_{\funbara {\strc {A_1} {\tc {A_2}}'}}
  &
  {\funbara {\tc (A_1 \tensorc \tc {A_2})}}
  \ar[r]_{\funbara {\tc \strc {A_1} {A_2}}}
  &
  {\funbara {\tc^2 (A_1 \tensorc A_2)}}
  \ar[r]_{\funbara {\multc {A_1 \tensorc A_2}}}
  &
  {\funbara {\tc (A_1 \tensorc A_2)}}
  }
\]


\subsection{Commutative Monads are Monoidal}
\label{app:commmonoidal}

Let $(\td, \unitd{}, \multd{}, \tstrna)$ be a strong monad on a symmetrical
monoidal category.  Let $\strd A B'$ be the dual strength $\td {\cd B A} \circ
\strd B A \circ \cd {\td A} B$.  That $\td$ is a commutative monad means that
Diagram~(\ref{eq:tt'}) commutes.  To show that $\bistrd A B = \multd {A
  \tensord B} \circ \td {\strd A B'} \circ \strd {\td A} B = \multd {A
  \tensord B} \circ \td {\strd A B} \circ \strd A {\td B}'$ is a mediator,
it then suffices to show that Diagram~(\ref{eq:tt'_alpha}) commutes.  In the
diagram below, the top row is $\strd A B \tensord \identity C$ followed by
$\strd {A \tensord B} C'$, the bottom row is $\identity A \tensord \strd B C'$
followed by $\strd A {B \tensord C}$. The two triangles involving $\cdna$ on
the left side are instances of the identity $\cdna \circ \cdna = \identity
{}$.

\[
\xymatrix{
  {\hbox{$
      \begin{array}{c}
        (A \tensord \td B)\\ \tensord C
      \end{array}
      $}}
  \ar[r]^{\strd A B \tensord \identity {}}
  \ar[rd]_{\cdna}
  \ar[d]|{\identity {}}
  &
  {\hbox{$
      \begin{array}{c}
        \td (A \tensord B)\\ \tensord C
      \end{array}
      $}}
  \ar[r]^{\cdna}
  &
  {\hbox{$
      \begin{array}{c}
        C \tensord\\ \td (A \tensord B)
      \end{array}
      $}}
  \ar[r]^{\strd C {A \tensord B}}
  &
  {\hbox{$
      \begin{array}{c}
        \td (C \tensord\\ (A \tensord B))
      \end{array}
      $}}
  \ar[r]^{\td \cdna}
  \ar@{}[rdddd]|{\txt{($\td$ of\\coher-\\ence\\(\ref{eq:alpha:coh:c}))}}
  &
  {\hbox{$
      \begin{array}{c}
        \td ((A \tensord B)\\ \tensord C)
      \end{array}
      $}}
  \ar[dddd]|{\td \alphad A B C}
  \\ %\\
  {\hbox{$
      \begin{array}{c}
        (A \tensord \td B)\\ \tensord C
      \end{array}
      $}}
  \ar[dd]|{\alphad A {\td B} C}
  \ar@{}[rdd]|{\txt{(coher-\\ence\\(\ref{eq:alpha:coh:c}))}}
  &
  {\hbox{$
      \begin{array}{c}
        C \tensord\\ (A \tensord \td B)
      \end{array}
      $}}
  \ar[ru]_{\identity {} \tensord \strd A B}
  \ar@{}[u]|{\txt{(naturality\\of $\cdna$)}}
  \ar[l]^{\cdna}
  &
  &
  {\hbox{$
      \begin{array}{c}
        \td ((C \tensord A)\\ \tensord B)
      \end{array}
      $}}
  \ar[u]|{\td \alphad C A B}
  \ar[d]|{\td (\cdna \tensord \identity {})}
  &
  \\ %\\
  &
  {\hbox{$
      \begin{array}{c}
        (C \tensord A) \\ \tensord \td B
      \end{array}
      $}}
  \ar[u]|{\alphad C A {\td B}}
  \ar[d]|{\cdna \tensord \identity {}}
  \ar[rru]_{\strd {C \tensord A} B}^{\txt{(strength\\law\\(\ref{eq:strong:double}))}}
  &
  &
  {\hbox{$
      \begin{array}{c}
        \td ((A \tensord C)\\ \tensord B)
      \end{array}
      $}}
  \ar[d]|{\td \alphad A C B}
  &
  \\ %\\
  {\hbox{$
      \begin{array}{c}
        A \tensord \\(\td B \tensord C)
      \end{array}
      $}}
  \ar[d]|{\identity {}}
  &
  {\hbox{$
      \begin{array}{c}
        (A \tensord C) \\ \tensord \td B
      \end{array}
      $}}
  \ar[d]|{\alphad A C {\td B}}
  \ar[rru]_{\strd {A \tensord C} B}^{\txt{(naturality\\of $\strdna$)}}
  &
  &
  {\hbox{$
      \begin{array}{c}
        \td (A \tensord \\ (C \tensord B))
      \end{array}
      $}}
  \ar[rd]^{\td (\identity {} \tensord \cdna)}
  &
  \\ %\\
  {\hbox{$
      \begin{array}{c}
        A \tensord \\(\td B \tensord C)
      \end{array}
      $}}
  \ar[r]_{\identity {} \tensord \cdna}
  &
  {\hbox{$
      \begin{array}{c}
        A \tensord \\(C \tensord \td B)
      \end{array}
      $}}
  \ar[lu]^{\identity {} \tensord \cdna}
  \ar[r]_{\identity {} \tensord \strd C B}
  \ar@{}[rruu]|{\txt{(strength\\law (\ref{eq:strong:double}))}}
  &
  {\hbox{$
      \begin{array}{c}
        A \tensord \\\td (C \tensord B)
      \end{array}
      $}}
  \ar[ru]^{\strd A {C \tensord B}}
  \ar[r]_{\identity {} \tensord \td \cdna}
  &
  {\hbox{$
      \begin{array}{c}
        A \tensord \\\td (B \tensord C)
      \end{array}
      $}}
  \ar[r]_{\strd A {B \tensord C}}
  \ar@{}[u]|{\txt{(naturality\\of $\strdna$)}}
  &
  {\hbox{$
      \begin{array}{c}
        \td (A \tensord \\ (B \tensord C))
      \end{array}
      $}}
  }
\]

We now observe that Diagram~(\ref{eq:monoidal:comm}) commutes:
{\small
\[
\xymatrix@C-10pt{
  {\td A \tensord \td B}
  \ar[r]^{\cdna}
  \ar[d]_{\cdna}
  &
  {\td B \tensord \td A}
  \ar[r]^{\strd {\td B} A}
  &
  {\td (\td B \tensord A)}
  \ar[r]^{\td \cdna}
  &
  {\td (A \tensord \td B)}
  \ar[r]^{\td \strd A B}
  &
  {\td^2 (A \tensord B)}
  \ar[r]^{\multd {A \tensord B}}
  \ar@{}[rd]|{\txt{(naturality\\of $\multd {}$)}}
  &
  {\td (A \tensord B)}
  \ar[d]|{\td \cdna}
  \\
  {\td B \tensord \td A}
  \ar[ru]^{\identity {}}
  \ar[r]_{\strd {\td B} A}
  &
  {\td (\td B \tensord A)}
  \ar[r]_{\td \cdna}
  &
  {\td (A \tensord \td B)}
  \ar[r]_{\td \strd A B}
  &
  {\td^2 (A \tensord B)}
  \ar[r]_{\td^2 \cdna}
  \ar[ru]^{\identity {}}
  &
  {\td^2 (B \tensord A)}
  \ar[r]_{\multd {B \tensord A}}
  &
  {\td (B \tensord A)}
  }
\]
} Indeed, the leftmost triangle is by $\cdna \circ \cdna = \identity {}$, the
inner parallelogram obviously commutes, and the top and bottom rows are the
two ways of writing $\bistrd A B$.

\noindent
\begin{minipage}{6cm}
  Conversely, given any monoidal monad making Diagram~(\ref{eq:monoidal:comm})
  commute, we claim that the derived strength $\strdna$ and dual strength
  $\strdna'$ are related by $\strd A B' = \td {\cd B A} \circ \strd B A \circ
  \cd {\td A} B$.  Equivalently, since $\cdna \circ \cdna = \identity {}$, we
  check that $\strd A B' \circ \cd B {\td A} = \td {\cd B A} \circ \strd B A$.
  This is obvious:
\end{minipage}
\begin{minipage}{6cm}
  \[
  \xymatrix{
    {B \tensord \td A}
    \ar[r]^{\cd B {\td A}}
    \ar[d]_{\unitd B \tensord \identity {\td A}}
    \ar@{}[rd]|{\txt{(naturality\\of $\cdna$)}}
    &
    {\td A \tensord B}
    \ar[d]^{\identity {\td A} B}
    \\
    {\td B \tensord \td A}
    \ar[d]_{\cd {\td B} {\td A}}
    \ar[r]^{\bistrd B A}
    \ar@{}[rd]|{\txt{(\ref{eq:monoidal:comm})}}
    &
    {\td (B \tensord A)}
    \ar[d]^{\td \cd B A}
    \\
    {\td A \tensord \td B}
    \ar[r]_{\bistrd A B}
    &
    {\td (A \tensord B)}
    }
  \]
\end{minipage}



==> bistrong2unitmon.tex <==
\section{Proof of Lemma~\ref{lemma:monoidal->unitmon}}
\label{app:monoidal->unitmon}


%  Before we embark on the proof, let us notice that the following diagrams
%  commute:
%  \begin{equation}
%    \label{eq:d}
%    \xymatrix{
%      &&&
%      T^2 A \otimes^{\cal C} T^2 A'
%      \ar[d]^{d_{T A, T A'}}
%      \ar[ld]_{\mu_A \otimes^{\cal C} \mu_{A'}}
%      \\
%      &
%      T A \otimes^{\cal C} T A'
%      \ar[d]^{d_{A, A'}}
%      &
%      T A \otimes^{\cal C} T A'
%      \ar[d]_{d_{A, A'}}
%      &
%      T (T A \otimes^{\cal C} T A')
%      \ar[d]^{T d_{A, A'}}
%      \\
%      A \otimes^{\cal C} A'
%      \ar[ru]^{\eta_A \otimes^{\cal C} \eta_{A'}}
%      \ar[r]_{\eta_{A \otimes^{\cal C} A'}}
%      &
%      T (A \otimes^{\cal C} A')
%      &
%      T (A \otimes^{\cal C} A')
%      &
%      T^2 (A \otimes^{\cal C} A')
%      \ar[l]^{\mu_{A \otimes^{\cal C} A'}}
%      }
%  \end{equation}
%  The diagram on the left is indeed a consequence of (\ref{eq:strong:eta}) and
%  the identity $t_{A, A'} = d_{A, A'} \circ (\eta_A \otimes^{\cal C} \identity
%  {T A'})$.  The diagram on the right is more complex; here is a quick
%  argument, using rather deeply the fact that $\Kleisli T$ is a category.
%  Write temporarily $\overline\circ$ the notion of composition in ${\cal D} =
%  \Kleisli T$, and notice that $\mu_{A \otimes^{\cal C} A'} \circ T d_{A, A'}
%  \circ d_{T A, T A'}$ is just $d_{A, A'} \overline\circ d_{T A, T A'}$.  The
%  diagram on the right means that $d_{A, A'} \overline\circ d_{T A, T A'} =
%  d_{A, A'} \circ (\mu_A \otimes^{\cal C} \mu_{A'})$.  Then notice that by
%  definition $d_{X, Y} = t_{X, Y} \overline\circ t'_{X, TY} = t'_{X, Y}
%  \overline\circ t_{T X, Y}$ for all objects $X$, $Y$, so:
%  \begin{eqnarray*}
%    d_{A, A'} \overline\circ d_{T A, T A'}
%    & = & (t_{A, A'} \overline\circ t'_{A, T A'})
%    \overline\circ
%    (t_{T A, T A'} \overline\circ t'_{T A, T^2 A'})
%    \\
%    & = & t_{A, A'} \overline\circ
%    (t'_{A, T A'} \overline\circ t_{T A, T A'})
%    \overline\circ t'_{T A, T^2 A'}
%    \\
%    & = & t_{A, A'} \overline\circ
%    d_{A, T A'}
%    \overline\circ t'_{T A, T^2 A'}
%    \\
%    & = & t_{A, A'} \overline\circ
%    (t_{A, T A'} \overline\circ t'_{A, T^2 A'})
%    \overline\circ t'_{T A, T^2 A'}
%    \\
%    & = & (t_{A, A'} \overline\circ t_{A, T A'})
%    \overline\circ
%    (t'_{A, T^2 A'} \overline\circ t'_{T A, T^2 A'})
%  \end{eqnarray*}
%  Now by the strength law (\ref{eq:strong:mu}), $t_{A, A'} \overline\circ
%  t_{A, T A'} = \mu_{A \otimes^{\cal C} A'} \circ T t_{A, A'} \circ t_{A, T
%    A'} = t_{A, A'} \circ (\identity A \otimes^{\cal C} \mu_{A'})$, and
%  similarly $t'_{A, T^2 A'} \overline\circ t'_{T A, T^2 A'} = t'_{A, T^2 A'}
%  \circ (\mu_A \otimes^{\cal C} \identity {T^2 A'})$.  So
%  \begin{eqnarray*}
%    d_{A, A'} \overline\circ d_{T A, T A'}
%    & = & (t_{A, A'} \circ (\identity A \otimes^{\cal C} \mu_{A'}))
%    \overline\circ
%    (t'_{A, T^2 A'} \circ (\mu_A \otimes^{\cal C} \identity {T^2 A'}))
%    \\
%    & = & \mu_{A \otimes^{\cal C} A'}
%    \circ T t_{A, A'} \circ T (\identity A \otimes^{\cal C} \mu_{A'})
%    \circ t'_{A, T^2 A'} \circ (\mu_A \otimes^{\cal C} \identity {T^2 A'})
%    \\
%    & = & \mu_{A \otimes^{\cal C} A'}
%    \circ T t_{A, A'} \circ t'_{A, T A'}
%    \circ (T (\identity A) \otimes^{\cal C} \mu_{A'})
%    \circ (\mu_A \otimes^{\cal C} \identity {T^2 A'})
%    \\
%    && \qquad \mbox{(by naturality of $t'$)}
%    \\
%    & = & d_{A, A'} \circ (\mu_A \otimes^{\cal C} \mu_{A'})
%  \end{eqnarray*}
%  and we are done.  Notice that (\ref{eq:d}) equivalently means that
%  $(\otimes^{\cal C}, d)$ is a morphism from the monad $T$ on $\cal C$ to the
%  monad $T \otimes^{\cal C} T$ on ${\cal C} \times {\cal C}$.
%!!! are these two diagrams a characterization of monoidal monads?
  
  
  We first check that $({\cal D}, I^{\cal D}, \otimes^{\cal D}, \alpha^{\cal
    D}, \ell^{\cal D}, r^{\cal D})$ is a monoidal category.  Write
  $\overline\circ$ the notion of composition in ${\cal D} = \Kleisli T$, i.e.,
  $g \overline\circ f = \mu \circ T g \circ f$.
%  We notice the following
%  formulae:
%  \begin{itemize}
%  \item $(\eta \circ f) \overline\circ g = \mu \circ T (\eta \circ f) \circ g
%    = \mu \circ T \eta \circ T f \circ g = T f \circ g$
%  \item $f \overline\circ (g \otimes^{\cal D} h) =$.
%Indeed, $f \overline\circ (g \otimes^{\cal D} h) =
%\mu \circ T f \circ d \circ (g \otimes^{\cal C} h)$
%  \end{itemize}
  \begin{itemize}
  \item Functoriality of $\otimes^{\cal D}$.  First, $\otimes^{\cal D}$
    applied to the identity on $(A, B)$ is $\identity A \otimes^{\cal D}
    \identity B = \identity {\KlF T (A)} \otimes^{\cal D} \identity {\KlF T
      (B)} = \KlF T (\identity A) \otimes^{\cal D} \KlF T (\identity B) = \KlF
    T (\identity A \otimes^{\cal C} \identity B) = \KlF T (\identity {A
      \otimes^{\cal C} B}) = \identity {\KlF T (A \otimes^{\cal C} B)} =
    \identity {A \otimes^{\cal D} B}$.
    
    Second, $\otimes^{\cal D}$ preserves composition.  Indeed, let $f, f', g,
    g'$ be morphisms from $A$ to $B$, from $A'$ to $B'$, from $B$ to $C$ and
    from $B'$ to $C'$ respectively in $\cal D$.  Then the composition of $g
    \otimes^{\cal D} g'$ with $f \otimes^{\cal D} f'$ in $\cal D$ is the
    morphism $\mu_{C \otimes^{\cal C} C'} \circ T (d_{C, C'} \circ (g
    \otimes^{\cal C} g')) \circ d_{B, B'} \circ (f \otimes^{\cal C} f')$ in
    $\cal C$.  The following diagram then commutes:
    {\small
      \[
      \xymatrix@R-10pt{
        A \otimes^{\cal C} A'
        \ar[r]^{f \otimes^{\cal C} f'}
        \ar@/_25pt/[rrddd]_{(g \overline\circ f) \otimes^{\cal C} (g' \overline\circ f')}
        &
        T B \otimes^{\cal C} T B'
        \ar[r]^{d_{B, B'}}
        \ar[d]_{T g \otimes^{\cal C} T g'}
        \ar@{}[rd]|{\txt{(naturality\\of $d$)}}
        &
        T (B \otimes^{\cal C} B')
        \ar[d]^{T (g \otimes^{\cal C} g')}
        \\
        &
        T^2 C \otimes^{\cal C} T^2 C'
        \ar[r]_{d_{T C, T C'}}
        \ar[rdd]|{\mu_C \otimes^{\cal C} \mu_{C'}}
        \ar@{}[rd]|{\txt{(\ref{eq:monoidal:mu})}}
        &
        T (T C \otimes^{\cal C} T C')
        \ar[d]^{T d_{C, C'}}
        \\
        &
        &
        T^2 (C \otimes^{\cal C} C')
        \ar[d]^{\mu_{C \otimes^{\cal C} C'}}
        \\
        &
        &
        T (C \otimes^{\cal C} C')
        }
      \]
      }
    The top right route from $A \otimes^{\cal C} A'$ to $T (C \otimes^{\cal C}
    C')$ is $(g \otimes^{\cal D} g') \overline\circ (f \otimes^{\cal D} f')$,
    while the straight line diagonal is $(g \overline\circ f) \otimes^{\cal D}
    (g' \overline\circ f')$.
  \item Naturality of $\alpha^{\cal D}$.  Let $f$, $g$, $h$ be morphisms from
    $A$ to $A'$, $B$ to $B'$ and $C$ to $C'$ respectively in $\cal D$.  Then
    $\alpha^{\cal D}$ composed in $\cal D$ with $(f \otimes^{\cal D} g)
    \otimes^{\cal D} h$ is $\mu \circ T (\eta \circ \alpha^{\cal C}) \circ d
    \circ ((d \circ (f \otimes^{\cal C} g)) \otimes^{\cal C} h) = T
    \alpha^{\cal C} \circ d \circ (d \otimes^{\cal C} \identity{}) \circ ((f
    \otimes^{\cal C} g) \otimes^{\cal C} h)$ (the route going all the way down
    then right from the top left corner to the bottom right corner below),
    while $f \otimes^{\cal D} (g \otimes^{\cal D} h)$ composed with
    $\alpha^{\cal D}$ in $\cal D$ is $\mu \circ T (d \circ (f \otimes^{\cal C}
    (d \circ (g \otimes^{\cal C} h)))) \circ \eta \circ \alpha^{\cal C} = \mu
    \circ T d \circ T (\identity{} \otimes^{\cal C} d) \circ T (f
    \otimes^{\cal C} (g \otimes^{\cal C} h)) \circ \eta \circ \alpha^{\cal C}$
    (the other route, going right then down).  {\small
      \[
      \xymatrix{
        (A \otimes^{\cal C} B) \otimes^{\cal C} C
        \ar[r]^{\alpha^{\cal C}}
        \ar[d]_{(f \otimes^{\cal C} g) \otimes^{\cal C} h}
        \ar@{}[rd]|{\txt{(naturality\\of $\alpha^{\cal C}$)}}
        &
        A \otimes^{\cal C} (B \otimes^{\cal C} C)
        \ar[r]^{\eta
          %_{A \otimes^{\cal C} (B \otimes^{\cal C} C)}
          }
        \ar[d]|{f \otimes^{\cal C} (g \otimes^{\cal C} h)}
        \ar@{}[rddd]|{\txt{(natur-\\ality\\of $\eta$)}}
        &
        T (A \otimes^{\cal C} (B \otimes^{\cal C} C))
        \ar[d]|{T (f \otimes^{\cal C} (g \otimes^{\cal C} h))}
        \\
        {\hbox{$
            \begin{array}{c}
              (T A' \otimes^{\cal C} T B')\\\otimes^{\cal C} T C'
          \end{array}
          $}}
        \ar[d]_{d_{A', B'} \otimes^{\cal C} \identity {T C'}}
        \ar[r]_{\alpha^{\cal C}}
        \ar@{}[rdd]|{\txt{(mediator\\law (\ref{eq:monoidal:double}))}}
        &
        T A' \otimes^{\cal C} (T B' \otimes^{\cal C} T C')
        \ar[d]|{\identity {T A'} \otimes^{\cal C} d_{B', C'}}
        &
        {\hbox{$
            \begin{array}{c}
              T (T A' \otimes^{\cal C}\\ (T B' \otimes^{\cal C} T C'))
          \end{array}
          $}}
        \ar[d]|{T (\identity {T A'} \otimes^{\cal C} d_{B', C'})}
        \\
        {\hbox{$
            \begin{array}{c}
              T (A' \otimes^{\cal C} B')\\ \otimes^{\cal C} T C'
          \end{array}
          $}}
        \ar[d]_{d_{A' \otimes^{\cal C} B', C'}}
        &
        {\hbox{$
            \begin{array}{c}
              T A' \otimes^{\cal C}\\ T (B' \otimes^{\cal C} C')
            \end{array}
            $}}
        \ar[d]|{d_{A', B' \otimes^{\cal C} C'}}
        &
        {\hbox{$
            \begin{array}{c}
              T (T A' \otimes^{\cal C}\\ T (B' \otimes^{\cal C} C'))
            \end{array}
            $}}
        \ar[d]|{T d_{A', B' \otimes^{\cal C} C'}}
        \\
        {\hbox{$
            \begin{array}{c}
              T ((A' \otimes^{\cal C} B')\\ \otimes^{\cal C} C')
          \end{array}
          $}}
        \ar[r]_{T \alpha^{\cal C}}
        &
        T (A' \otimes^{\cal C} (B' \otimes^{\cal C} C'))
        \ar[r]_{\eta}
        \ar[rd]_{\identity {T (A' \otimes^{\cal C} (B' \otimes^{\cal C}
            C'))}}^{\txt{(monad law)}}
        &
        {\hbox{$
            \begin{array}{c}
              T^2 (A' \otimes^{\cal C}\\ (B' \otimes^{\cal C} C'))
            \end{array}
            $}}
        \ar[d]|{\mu_{A' \otimes^{\cal C} (B' \otimes^{\cal C} C')}}
        \\
        &
        &
        {\hbox{$
            \begin{array}{c}
              T (A' \otimes^{\cal C}\\ (B' \otimes^{\cal C} C'))
            \end{array}
            $}}
        }
      \]
      }
  \item Naturality of $\ell^{\cal D}$.  Let $f$ be any morphism from $B$ to
    $B'$ in $\cal D$.  Then the composition of $f$ with $\ell^{\cal D}$ in
    $\cal D$ is $\mu \circ T f \circ \eta \circ \ell^{\cal C}$ (route going
    right then down), while the composition of $\ell^{\cal D}$ with
    $(\identity {}^{\cal D} \otimes^{\cal D} f)$ is $\mu \circ T (\eta \circ
    \ell^{\cal C}) \circ d \circ (\eta \otimes^{\cal C} f)$ (dented route
    going down then right).  {\small
      \[
      \xymatrix@R-10pt@C+30pt{
        I^{\cal C} \otimes^{\cal C} B
        \ar[r]^{\ell^{\cal C}}
        \ar[d]_{\identity {I^{\cal C}} \otimes^{\cal C} f}
        \ar@{}[rd]|{\txt{(naturality\\of $\ell^{\cal C}$)}}
        &
        B
        \ar[r]^{\eta_B}
        \ar[d]_{f}
        \ar@{}[rd]|{\txt{(naturality\\of $\eta$)}}
        &
        T B
        \ar[d]^{T f}
        \\
        I^{\cal C} \otimes^{\cal C} T B'
        \ar[r]|{\ell^{\cal C}_{T B'}}
        \ar[d]_{\eta_{I^{\cal C}} \otimes \identity {T B'}}
        &
        T B'
        \ar[r]|{\eta_{T B'}}
        \ar[rdd]|{\identity {T B'}}^{\txt{(monad\\law)}}
        \ar[dd]|{T \eta_{B'}}
        &
        T^2 B'
        \ar[dd]^{\mu_B}
        \\
        T I^{\cal C} \otimes^{\cal C} T B'
        \ar[d]_{d_{I^{\cal C}, B'}}
        \ar@{}[ru]|{\txt{(\ref{eq:monoidal:l})}}
        &&
        \\
        T (I^{\cal C} \otimes^{\cal C} B')
        \ar[ruu]_{T \ell^{\cal C}_{B'}}
        &
        T^2 B'
        \ar[r]^{\mu_{B'}}
        &
        T B'
        }
      \]
      }
  \item Naturality of $r^{\cal D}$ is obtained similarly, using
    (\ref{eq:monoidal:r}) instead of (\ref{eq:monoidal:l}).
  \item $\alpha^{\cal D}$, $\ell^{\cal D}$, $r^{\cal D}$ are isomorphisms:
    indeed $\alpha^{\cal D} = \KlF T (\alpha^{\cal C})$, $\alpha^{\cal C}$ is
    an isomorphism, and every functor preserves isomorphisms.  Similarly for
    $\ell^{\cal D}$ and $r^{\cal D}$.  Since they are natural, they are
    natural isomorphisms.
  \item Pentagon identity (\ref{eq:alpha:coh1}).  We have to check that
    (dropping subscripts) $\alpha^{\cal D} \overline\circ \alpha^{\cal D} =
    (\identity{}^{\cal D} \otimes^{\cal D} \alpha^{\cal D}) \overline\circ
    \alpha^{\cal D} \overline\circ (\alpha^{\cal D} \otimes^{\cal D}
    \identity{}^{\cal D})$.  Note that the left-hand side is $\mu \circ T
    (\eta \circ \alpha^{\cal C}) \circ \eta \circ \alpha^{\cal C} = T
    \alpha^{\cal C} \circ \eta \circ \alpha^{\cal C} = \eta \circ \alpha^{\cal
      C} \circ \alpha^{\cal C}$ (by naturality of $\eta$, $T f \circ \eta =
    \eta \circ f$ for any $f$).  Now notice that by (\ref{eq:monoidal:eta}),
    $d \circ (\eta \otimes^{\cal C} \eta) = \eta$.  Also, $\mu \circ T \eta =
    \identity{}$.  So the right-hand side is:
    \begin{eqnarray*}
      &&
      \mu \circ T (d \circ (\eta \otimes^{\cal C} (\eta \circ \alpha^{\cal
        C})))
      \circ [\alpha^{\cal D} \overline\circ (\alpha^{\cal D} \otimes^{\cal D}
      \identity{}^{\cal D})]
      \\
      & = & \mu \circ T (d \circ (\eta \otimes^{\cal C} \eta)) \circ T
      (\identity {} \otimes^{\cal C} \alpha^{\cal C})
      \circ [\alpha^{\cal D} \overline\circ (\alpha^{\cal D} \otimes^{\cal D}
      \identity{}^{\cal D})]
      \\
      & = & \mu \circ T \eta \circ T
      (\identity {} \otimes^{\cal C} \alpha^{\cal C})
      \circ [\alpha^{\cal D} \overline\circ (\alpha^{\cal D} \otimes^{\cal D}
      \identity{}^{\cal D})]
      \qquad \mbox{(by (\ref{eq:monoidal:eta}))}
      \\
      & = & T
      (\identity {} \otimes^{\cal C} \alpha^{\cal C})
      \circ [\alpha^{\cal D} \overline\circ (\alpha^{\cal D} \otimes^{\cal D}
      \identity{}^{\cal D})]
      \\
      & = & T
      (\identity {} \otimes^{\cal C} \alpha^{\cal C})
      \circ \mu \circ T (\eta \circ \alpha^{\cal C})
      \circ (\alpha^{\cal D} \otimes^{\cal D} \identity{}^{\cal D})
      \\
      & = & T
      (\identity {} \otimes^{\cal C} \alpha^{\cal C})
      \circ T \alpha^{\cal C}
      \circ (\alpha^{\cal D} \otimes^{\cal D} \identity{}^{\cal D})
      \\
      & = & T
      (\identity {} \otimes^{\cal C} \alpha^{\cal C})
      \circ T \alpha^{\cal C}
      \circ d \circ ((\eta \circ \alpha^{\cal C}) \otimes^{\cal C} \eta)
      \\
      & = & T
      (\identity {} \otimes^{\cal C} \alpha^{\cal C})
      \circ T \alpha^{\cal C}
      \circ d \circ (\eta \otimes^{\cal C} \eta) \circ (\alpha^{\cal C}
      \otimes^{\cal C} \identity {})
      \\
      & = & T
      (\identity {} \otimes^{\cal C} \alpha^{\cal C})
      \circ T \alpha^{\cal C}
      \circ \eta \circ (\alpha^{\cal C}
      \otimes^{\cal C} \identity {})
      \qquad \mbox{(by (\ref{eq:monoidal:eta}))}
      \\
      & = & \eta \circ
      (\identity {} \otimes^{\cal C} \alpha^{\cal C})
      \circ \alpha^{\cal C} \circ (\alpha^{\cal C}
      \otimes^{\cal C} \identity {})
      \qquad \mbox{(by naturality of $\eta$)}
    \end{eqnarray*}
    and we are done, since by the pentagon identity (\ref{eq:alpha:coh1}) for
    $\alpha^{\cal C}$, $\alpha^{\cal C} \circ \alpha^{\cal C} = (\identity {}
    \otimes^{\cal C} \alpha^{\cal C}) \circ \alpha^{\cal C} \circ
    (\alpha^{\cal C} \otimes^{\cal C} \identity {})$.
  \item Triangle identity (\ref{eq:alpha:cohlr}).  We must check that
    $(\identity{}^{\cal D} \otimes^{\cal D} \ell^{\cal D}) \overline\circ
    \alpha^{\cal D} = r^{\cal D}$.  The left-hand side is $\mu \circ T (d
    \circ (\eta \otimes^{\cal C} (\eta \circ \ell^{\cal C})) \circ \eta \circ
    \alpha^{\cal C} = \mu \circ T (d \circ (\eta \otimes^{\cal C} \eta) \circ
    (\identity{} \otimes^{\cal C} \ell^{\cal C})) \circ \eta \circ
    \alpha^{\cal C} = \mu \circ T (\eta \circ (\identity{} \otimes^{\cal C}
    \ell^{\cal C})) \circ \eta \circ \alpha^{\cal C}$ (by
    (\ref{eq:monoidal:eta})) $= T (\identity{} \otimes^{\cal C} \ell^{\cal C})
    \circ \eta \circ \alpha^{\cal C}$ (by the monad laws) $= \eta \circ
    (\identity{} \otimes^{\cal C} \ell^{\cal C}) \circ \alpha^{\cal C}$ (by
    naturality of $\eta$) $= \eta \circ r^{\cal C}$ (by the triangle identity
    (\ref{eq:alpha:cohlr}) in $\cal C$) $= r^{\cal D}$, which is the
    right-hand side.
  \end{itemize}
  
  We must now check that $\KlF T \dashv \KlU T$ is a monoidal adjunction.  We
  already know that it is an adjunction.
  \begin{itemize}
  \item $(\theta^{\KlF T}, \iota^{\KlF T})$ is mediating for $F$.  Indeed,
    both $\theta^{\KlF T}_{A, B}$ and $\iota^{\KlF T}$ are just identity
    morphisms in $\cal D$, from which the coherence conditions
    (\ref{eq:theta:coh:alpha}), (\ref{eq:theta:coh:l}) and
    (\ref{eq:theta:coh:r}) are clear.  The first reduces to showing that $\KlF
    T (\alpha^{\cal C}) = \alpha^{\cal D}$, the second to $\KlF T (\ell^{\cal
      C}) = \ell^{\cal D}$, the third to $\KlF T (r^{\cal C}) = r^{\cal D}$,
    which hold by construction.
  \item $(\theta^{\KlU T}, \iota^{\KlU T})$ is mediating for $\KlU T$.
    Indeed, the first coherence condition~(\ref{eq:theta:coh:alpha}) is just
    Diagram~(\ref{eq:monoidal:double}), since $\KlU T \alpha^{\cal D} = \KlU T
    \KlF T \alpha^{\cal C} = T \alpha^{\cal C}$.  The second coherence
    condition~(\ref{eq:theta:coh:l}) is exactly Diagram~(\ref{eq:monoidal:l}),
    and the third, (\ref{eq:theta:coh:r}), is exactly
    Diagram~(\ref{eq:monoidal:r}).
  \item The unit $\eta$ and the counit $\epsilon$ are monoidal natural
    transformations.  (Recall that $\epsilon_A$ is the identity morphism from
    $T A$ to $T A$ in $\cal C$, seen as a morphism from $T A$ to $A$ in $\cal
    D$.)  Indeed, Diagram~(\ref{eq:moneta:I}) (in $\cal C$) means that
    $\eta_{I^{\cal C}} = \KlU T (\iota^{\KlF T}) \circ \iota^{\KlU T} = \KlU T
    (\identity{}) \circ \eta_{I^{\cal C}}$, which is obvious.
    Diagram~(\ref{eq:moneta:tensor}) states that $\KlU T (\theta^{\KlF T}_{A,
      B}) \circ \theta^{\KlU T} \circ (\eta_A \otimes^{\cal C} \eta_B) =
    \eta_{A \otimes^{\cal C} B}$, i.e., $d_{A, B} \circ (\eta_A \otimes^{\cal
      C} \eta_B) = \eta_{A \otimes^{\cal C} B}$, which is just
    Diagram~(\ref{eq:monoidal:eta}).  Turning to diagrams in $\cal D$,
    Diagram~(\ref{eq:moneps:I}) means that $\epsilon_{I^{\cal D}} \overline
    \circ \KlF T (\iota^{\KlU T}) \overline \circ \iota^{\KlF T}$ is the
    identity in $\cal D$; seen as a morphism in $\cal C$, this is
    \begin{eqnarray*}
      \mu \circ T (\identity {}) \circ [\KlF T (\iota^{\KlU T})
      \overline \circ \iota^{\KlF T}]
      & = &
      \mu \circ [\KlF T (\iota^{\KlU T}) \overline \circ \iota^{\KlF T}]
      \\
      & = & \mu \circ \mu \circ T (\KlF T (\iota^{\KlU T})) \circ \iota^{\KlF
        T} \\
      & = & \mu \circ \mu \circ T (\eta_{T I^{\cal C}} \circ \eta_{I^{\cal
          C}}) \circ \eta_{I^{\cal C}}
      = \eta_{I^{\cal C}}    
    \end{eqnarray*}
    (by the monad laws), and the latter is just the identity on $I^{\cal D}$
    in $\cal D$, as required.  Finally, Diagram~(\ref{eq:moneps:tensor}) means
    that $\epsilon_{A \otimes^{\cal D} B} \overline\circ \KlF T \theta^{\KlU
      T} \overline\circ \theta^{\KlF T} = \epsilon_A \otimes^{\cal D}
    \epsilon_B$.  Seen as a morphism in $\cal C$, the left-hand side is
    \begin{eqnarray*}
      && \mu_{A \otimes^{\cal C} B} \circ T \epsilon_{A \otimes^{\cal D} B} \circ [\KlF T \theta^{\KlU
        T} \overline\circ \theta^{\KlF T}] \\
      & = & \mu_{A \otimes^{\cal C} B} \circ T \identity{} \circ [\KlF T \theta^{\KlU
        T} \overline\circ \theta^{\KlF T}]
      \\
      & = & \mu_{A \otimes^{\cal C} B} \circ [\KlF T \theta^{\KlU T} \overline\circ \theta^{\KlF T}]
      \\
      & = & \mu_{A \otimes^{\cal C} B} \circ \mu_{T (A \otimes^{\cal C} B)} \circ T (\KlF T \theta^{\KlU T}) \circ \theta^{\KlF
        T}
      \\
      & = & \mu_{A \otimes^{\cal C} B} \circ \mu_{T (A \otimes^{\cal C} B)} \circ T (\eta_{T (A \otimes^{\cal C} B)} \circ d_{A, B}) \circ \eta_{A \otimes^{\cal
          C} B}
%      \\
%      & = & \mu \circ \mu \circ T (\eta \circ d) \circ \eta \\
%      & = & \mu \circ \mu \circ \eta \circ (\eta \circ d)
%      \qquad \mbox{(by naturality of $\eta$)}
    \end{eqnarray*}
    which we recognize as the long trip in the diagram below from the top left
    corner that goes down, right, and up to the top right corner.
    {\small
      \[
      \xymatrix{
        T A \otimes^{\cal C} T B
        \ar[d]_{\eta_{A \otimes^{\cal C} B}}
        \ar[r]^{d_{A, B}}
        \ar@{}[rd]|{\txt{(natur-\\ality\\of $\eta$)}}
        &
        T (A \otimes^{\cal C} B)
        \ar[rr]^{\identity {T (A \otimes^{\cal C} B)}}
        \ar[d]^{\eta_{T (A \otimes^{\cal C} B)}}
        \ar@{}[rrd]|{\txt{(monad law)}}
        &
        &
        T (A \otimes^{\cal C} B)
        \\
        T (T A \otimes^{\cal C} T B)
        \ar[r]_{T d_{A, B}}
        &
        T^2 (A \otimes^{\cal C} B)
        \ar[rd]_{T \eta_{T (A \otimes^{\cal C} B)}}
        \ar[rr]^{\identity {T^2 (A \otimes^{\cal C} B)}}_{\txt{(monad law)}}
        &
        &
        T^2 (A \otimes^{\cal C} B)
        \ar[u]_{\mu_{A \otimes^{\cal C} B}}
        \\
        &
        &
        T^3 (A \otimes^{\cal C} B)
        \ar[ru]_{\mu_{T (A \otimes^{\cal C} B)}}
        &
        }
      \]
      }
    Then the composition of arrows from the top left corner to the top right
    corner is $d_{A, B}$.  This is exactly the desired morphism $\epsilon_A
    \otimes^{\cal D} \epsilon_D$ of $\cal D$, which, seen as a morphism of
    $\cal C$, is $d_{A, B} \circ (\identity {T A} \otimes^{\cal C} \identity
    {T B})$ by definition.
  \end{itemize}
  
  We check finally that $\KlF T \dashv \KlU T$ generates the monoidal monad.
  The only thing to check is $d_{A, B} = \KlU T \theta^{\KlF T}_{A, B} \circ
  \theta^{\KlU T}_{\KlF T (A), \KlF T (B)}$.  This is clear, since the
  right-hand side is $\KlU T (\identity {A \otimes^{\cal D} B}) \circ d_{A, B}
  = d_{A, B}$.  \qed


==> ccc.tex <==


\section{Lifting Closed Structures to the Subscone}
\label{ccc.s}


If we are to lift the whole structure of a cartesian-closed category together
with a strong monad on it, to the subscone, the only thing that remains is to
lift exponential objects. As this is essentially the subject of \cite{MS93}
(together with the fact that subscones generalize logical relations), it would
be legitimate to skip over this construction, knowing that it has been dealt
with elsewhere.

However, we notice that the standard lifting construction of exponentials to
the subscone requires $\funbar$ to preserve products, at least up to natural
isos.  That is, it requires $\funbara {\termobjc} \cong \termobjd$, $\funbara
{A \times B} \cong \funbara A \times \funbara B$. This is certainly the case
for the functor $\funbar = \homset \catc \termobjc \_$, which is the standard
choice in sconing constructions \cite{MS93}.

Until now, we have only assumed that $\funbar$ was a monoidal
(Section~\ref{sec:monoidal:1}), resp.\ a symmetric monoidal
(Section~\ref{sec:monoidal:sym}), resp.\ a cartesian monoidal
(Section~\ref{sec:monoidal:cart}) functor.  It would therefore be nice if we
could dispense with the stringent requirement that $\funbar$ preserved
monoidal or cartesian structure exactly.  This would also afford us some added
generality.

It turns out that having a monoidal mono factorization system is all
we need: exponentials lift to the subscone without any additional
requirements compared to Section~\ref{sec:monoidal}.  This only
requires a slight adjustment of the standard exponential lifting
diagrams.
\ifmscs
\else
%This is the topic of Section~\ref{ccc.s:expo}.
%We deal with fragments of the linear $\lambda$-calculus in
%Section~\ref{ccc.s:linear}.

\comment{DN 07/01/04
We use the added generality to show in Section~\ref{ccc.s:simplicial}
that, as soon as we can lift a strong monad to a subscone, then we can
lift it without any extra effort to a much richer subscone (one of
Kripke logical relations indexed by the simplicial category $\Delta$),
under mild assumptions.
}

%\subsection{Lifting Exponentials}
%\label{ccc.s:expo}

Recall that an {\em exponential}, or {\em internal hom object\/} (on
the right), in a monoidal category $(\catd, \tensord, \Id, \alphadna,
\ld{}, \rd{})$, is an object $\ihom A B$ together with a morphism
$\App$ from $\ihom A B \tensord A$ to $B$ and, for every morphism $u$
from $C \tensord A$ to $B$, a morphism $\Lambda (u)$ from $C$ to
$\ihom A B$ satisfying the two equations

\begin{equation}
  \label{eq:beta}
  \xymatrix@C+20pt{
    C \tensord A
    \ar[r]^{\Lambda (u) \tensord \identity A}
    \ar[rd]_{u}
    &
    \ihom A B \tensord A
    \ar[d]^{\App}
    \\
    &
    B
    }
\end{equation}
for every morphism $u$ from $C \tensord A$ to $B$ ({\em $\beta$-equivalence\/}),
and
\begin{equation}
  \label{eq:eta}
  \Lambda \left(
    \xymatrix@C+10pt{
      C \tensord A
      \ar[r]^{v \tensord \identity A}
      &
      \ihom A B \tensord A
      \ar[r]^{\App}
      &
      B
      }
  \right)
  = v
\end{equation}
for every morphism $v$ from $C$ to $\ihom A B$ ({\em $\eta$-equivalence\/}).
$\Lambda (u)$ is called the {\em currification\/} or the {\em abstraction\/}
of $u$.

A more traditional definition is to require the existence of a {\em
unique\/} morphism $\Lambda (u)$ as in Diagram~(\ref{eq:beta}).
Uniqueness is indeed implied by (\ref{eq:eta}): if there were two
morphisms $v$ and $v'$ such that $u = \App \circ (v \tensord \identity
A) = \App \circ (v' \tensord \identity A)$, then $v = \Lambda (\App
\circ (v \tensord \identity A)) = \Lambda (u) = \Lambda (\App \circ
(v' \tensord \identity A)) = v'$.  Conversely, uniqueness of $\Lambda
(u)$ implies Diagram~(\ref{eq:eta}): take $u = \App \circ (v \tensord
\identity A)$ in Diagram~(\ref{eq:beta}).

Exponentials on the right are unique up to iso when they exist. A monoidal
category is said to be {\em monoidal closed\/} (on the right) if and only if
the exponential $\ihom A B$ exists for all objects $A$ and $B$. Similarly, we
call exponential on the left any object $\ihoml A B$ with a morphism $\Appl$
from $A \tensord \ihoml A B$ to $B$ such that, for every morphism $u$ from $A
\tensord C$ to $B$, there is a unique morphism $(u) \Lambda$ from $C$ to
$\ihoml A B$ such that $u = \Appl \circ (\identity A \tensord (u) \Lambda)$.
In a {\em symmetric\/} monoidal category, it is equivalent to require the
existence of exponentials on the right or on the left, and they coincide up to
iso.  A category with finite products that is also monoidal closed (for the
monoidal structure induced by the product) is called {\em cartesian closed}.

Note that, in a monoidal closed category, there is a functor $\ihom A \_ $ for
each object $A$, which maps every object $B$ to $\ihom A B$, and every
morphism $B {\buildrel f \over\longrightarrow} B'$ to $\ihom A f = \Lambda (f
\circ \App)$, from $\ihom A B$ to $\ihom A {B'}$.  In fact, there is a
bifunctor from $\catd^{op} \times \catd$ to $\catd$ mapping $A, B$ to $\ihom A
B$.
%  This is indeed a functor,
%since $\Lambda (\identity B \circ \App) = \Lambda (\App) = \Lambda (\App \circ
%(\identity {\ihom A B} \tensord \identity A)) = \identity {\ihom A B}$ by
%(\ref{eq:eta}), and $\Lambda (f \circ \App) \circ \Lambda (g \circ \App) =
%\Lambda ((f \circ g) \circ \App)$.  Indeed, $\Lambda (f \circ \App) \circ
%\Lambda (g \circ \App) = \Lambda (\App \circ ((\Lambda (f \circ \App) \circ
%\Lambda (g \circ \App)) \tensord \identity {}))$ (by (\ref{eq:eta})) $=
%\Lambda (\App \circ (\Lambda (f \circ \App) \tensord \identity {}) \circ
%(\Lambda (g \circ \App) \tensord \identity {})) = \Lambda (f \circ \App \circ
%(\Lambda (g \circ \App) \tensord \identity {}))$ (by (\ref{eq:beta}) $=
%\Lambda (f \circ g \circ \App)$ (by (\ref{eq:beta}) again).

Moreover, the functor $\ihom A \_$ preserves monos: if $m$ is mono, then so is
$\ihom A m = \Lambda (m \circ \App)$.  It suffices to show that there is at
most one morphism $f$ such that $\Lambda (m \circ \App) \circ f = h$ where $h$
is given.  Indeed, $\App \circ (h \tensord \identity {}) = \App \circ (\Lambda
(m \circ \App) \tensord \identity {}) \circ (f \tensord \identity {}) = m
\circ \App \circ (f \tensord \identity {})$ by (\ref{eq:beta}); if there were
two such morphisms $f$ and $f'$, then $m \circ \App \circ (f \tensord
\identity {}) = m \circ \App \circ (f' \tensord \identity {})$, so $\App \circ
(f \tensord \identity {}) = \App \circ (f' \tensord \identity {})$ since $m$
is mono.  Applying $\Lambda$ on both sides implies $f = f'$ by (\ref{eq:eta}).

Once this is known, the standard way of lifting exponentials to the subscone
is to require that $\catc$ and $\catd$ are cartesian closed, $\catd$ has
pullbacks, and that $\funbar$ preserves finite products (exactly, or up to
natural iso).  This standard construction actually does not require cartesian
closedness, and works equally well with monoidal closed categories, assuming
$\catd$ has pullbacks and $\funbar$ preserves unit and tensor.

We recall this construction now.  As $\funbar$ preserves unit, the unit
(terminal object in the cartesian closed case) $\IS$ is $\langle \Id,
\identity \Id, \Ic\rangle$ witness by the arrow $\Id {\buildrel {\identity
    \Id} \over \longrightarrow} \funbara {\Ic} = \Id$, tensor product (binary
product in the cartesian closed case) is given by $\langle S_1, m_1, A_1
\rangle \tensorS \langle S_2, m_2, A_2 \rangle = \langle S_1 \tensord S_2, m_1
\tensord m_2, A_1 \tensorc A_2 \rangle$, and the exponential $\langle \lift
S^1_2, \lift m^1_2, \ihom {A_1} {A_2}\rangle = \ihom {\langle S_1, m_1, A_1
  \rangle} {\langle S_2, m_2, A_2\rangle}$ is given by the square on the left
below.
\[
\xymatrix@R-15pt@C+5pt{
  {\lift S^1_2\SEpbk}
  \ar@{^{(}.>}[rr]^{\lift m^1_2}
  \ar@{.>}[ddd]_{\ell^1_2}
  &&
  {\funbara {\ihom {A_1} {A_2}}}
  \ar[ddd]|-{\Lambda \left(\funbara {\App} \circ \left(\identity {\funbara {\ihom {A_1} {A_2}}} \tensord m_1\right)\right)}
  & 
  {\funbara {\ihom {A_1} {A_2}} \tensord S_1}
  \ar[d]^{\identity {\funbara {\ihom {A_1} {A_2}}} \tensord m_1}
  \\
  &&&
  {\funbara {\ihom {A_1} {A_2}} \tensord \funbara {A_1}}
  \ar@{=}[d] \\
  &&&
  {\funbara {\ihom {A_1} {A_2} \tensorc A_1}}
  \ar[d]^{\funbara {\App}} \\
  {\ihom {S_1} {S_2}}
  \arrmonoxy[rr]^{\ihom {S_1} {m_2}}
  &&
  {\ihom {S_1} {\funbara {A_2}}}
  &
  {\funbara {A_2}}
%  \\
%  {\ihom {S_1} {S_2} \tensord S_1}
%  \ar[r]^(0.7){\App}
%  &
%  S_2
%  \ar[r]^{m_2}
%  &
%  {\funbara {A_2}}
%  &
  }
\]
where the vertical morphism $\Lambda \left(\funbara \App \circ \left(\identity
    {\funbara {\ihom {A_1} {A_2}}} \tensord m_1\right)\right)$ is $\Lambda$
applied to the composition of vertical morphisms on the right, the morphism
$\ihom {S_1} {m_2}$ is mono because $\ihom {S_1} \_$ preserves monos, and
$\lift m^1_2$ is mono because pullbacks preserve monos.  (We temporarily
revert to the notation $\xymatrix{\arrmonoxy[r]&}$ to denote all monos.)

Application from $\langle \lift S^1_2, \lift m^1_2, \ihom {A_1} {A_2}\rangle
\tensorS \langle S_1, m_1, A_1\rangle$ in the subscone is given by
\[
\xymatrix@C+15pt@R-5pt{
  {\lift S^1_2 \tensord S_1}
  \ar[r]^{\lift m^1_2 \tensord \identity {S_1}}
  \ar[d]_{\ell^1_2 \tensord \identity {S_1}}
  &
  {\funbara {\ihom {A_1} {A_2}} \tensord S_1}
  \ar[r]^{\identity {} \tensord m_1}
  \ar[d]|{\Lambda (\funbara \App \circ (\identity {} \tensord m_1)) \tensord
    \identity {S_1}}
  &
  {\funbara {\ihom {A_1} {A_2}} \tensord \funbara {A_1}}
  \ar@{=}[dd]
  \\
  {\ihom {S_1} {S_2} \tensord S_1}
  \ar[r]_{\ihom {S_1} {m_2} \tensord \identity {S_1}}
  \ar[d]_{\App} &
  {\ihom {S_1} {\funbara {A_2}} \tensord S_1}
  \ar[d]^{\App}
  &
  \\
  {S_2}
  \arrmonoxy[r]_{m_2}
  &
  {\funbara {A_2}}
  &
  {\funbara {\ihom {A_1} {A_2} \tensorc A_1}}
  \ar[l]_{\funbara {\App}}
  }
\]
where the top left square is the definition of the exponential $\langle \lift
S^1_2, \lift m^1_2, \ihom {A_1} {A_2}\rangle$ tensor $S_1$ on the right.  The
bottom left square and the right square commute by (\ref{eq:beta}). Then,
application in the subscone is $\langle \App \circ (\ell^1_2 \tensord
\identity {}), \funbara \App\rangle$.

Abstraction of the morphism $\langle u, v\rangle$ in the subscone from
$\langle S, m, A\rangle \tensorS \langle S_1, m_1, A_1\rangle$ to $\langle
S_2, m_2, A_2\rangle$ is then the pair $\langle \tilde u, \Lambda (v)\rangle$
given by the diagram
\[
\xymatrix@C+5pt@R-10pt{
  S
  \arrmonoxy[rrr]^{m}
  \ar@{.>}[rd]^{\lift u}
  \ar[rdd]_{\Lambda (u)}
  &&&
  {\funbara A}
  \ar[d]^{\funbara {\Lambda (v)}}
  \\
  &
  {\lift S^1_2\SEpbk}
  \arrepixy[rr]^{\lift m^1_2}
  \arrmonoxy[d]_{\ell^1_2}
  &&
  {\funbara {\ihom {A_1} {A_2}}}
  \ar[d]^{\Lambda \left(\funbara {\App} \circ \left(\identity {} \tensord m_1\right)\right)}
  \\
  &
  {\ihom {S_1} {S_2}}
  \arrmonoxy[rr]^{\ihom {S_1} {m_2}}
  &&
  {\ihom {S_1} {\funbara {A_2}}}
  }
\]
where $\lift u$ is given by the universal property of pullbacks.  To this
end, we must first check that the outer contour of the diagram commutes.  We
leave this to the reader.
%Now
%two morphims $f, g$ from $S$ to $\ihom {S_1} {\funbara {A_2}}$ are equal if
%and only if $\App \circ (f \tensord \identity {S_1}) = \App \circ (g \tensord
%\identity {S_1})$.  But
%\begin{eqnarray*}
%  &&
%  \App \circ ((\Lambda (\funbara \App \circ (\identity {} \tensord m_1))
%  \circ \funbara {\Lambda (v)} \circ m) \tensord \identity {})
%  \\
%  & = & \App \circ (\Lambda (\funbara \App \circ (\identity {} \tensord m_1))
%  \tensord \identity {})
%  \circ (\funbara {\Lambda (v)} \tensord \identity {})
%  \circ (m \tensord \identity {})
%  \\
%  & = & \funbara \App \circ (\identity {} \tensord m_1)
%  \circ (\funbara {\Lambda (v)} \tensord \identity {})
%  \circ (m \tensord \identity {})
%  \qquad \mbox{(by (\ref{eq:beta}))}
%  \\
%  & = & \funbara \App
%  \circ (\funbara {\Lambda (v)} \tensord \identity {})
%  \circ (m \tensord m_1)
%  \\
%  & = & \funbara {\App \circ (\Lambda (v) \tensorc \identity {})}
%  \circ (m \tensord m_1)
%  \\
%  & = & \funbara v \circ (m \tensord m_1)
%  \qquad \mbox{(by (\ref{eq:beta}))}
%\end{eqnarray*}
%while
%\begin{eqnarray*}
%  \App \circ ((\ihom {S_1} {m_2} \circ \Lambda (u)) \tensord \identity {})
%  & = &
%  \App \circ ((\Lambda (m_2 \circ \App) \circ \Lambda (u)) \tensord \identity
%  {})
%  \\
%  & = &
%  \App \circ (\Lambda (m_2 \circ \App) \tensord \identity {})
%  \circ (\Lambda (u) \tensord \identity {})
%  \\
%  & = &
%  m_2 \circ \App
%  \circ (\Lambda (u) \tensord \identity {})
%  \qquad \mbox{(by (\ref{eq:beta}))}
%  \\
%  & = &
%  m_2 \circ u
%  \qquad \mbox{(by (\ref{eq:beta}))}
%\end{eqnarray*}
%and $\funbara v \circ (m \tensord m_1) = m_2 \circ u$, since $\langle u,
%v\rangle$ is a morphism from $\langle S, m, A\rangle \tensorS \langle S_1,
%m_1, A_1\rangle$ to $\langle S_2, m_2, A_2\rangle$ in the subscone.

The equations (\ref{eq:beta}) and (\ref{eq:eta}) then hold in the subscone,
because they hold in $\catc$, and using Fact~\ref{f_eq}.
\fi

In the case we are interested in here, $\funbar$ does not preserve unit and
tensor.  Rather, we have required $\funbar$ to be a monoidal functor, a
strictly weaker notion.  We have already seen in Section~\ref{sec:monoidal}
that this was enough to lift monoidal structure to the subscone, using a
monoidal mono factorization.  We now realize that this is also enough to lift
monoidal {\em closed\/} structure to the subscone.  This requires only minor
adjustments to the constructions above.

First, we require that the functor $\ihom A \_$ preserves {\em
relevant\/} monos, for all $A$.  While it always preserves monos, it
is not clear that it should preserve relevant monos, hence the added
assumption.  (We return to our convention that
$\xymatrix{\arrmonoxy[r]&}$ denotes relevant monos only.)  We might
also require that pullbacks preserve relevant monos, but this is not
necessary, as we can use the mono factorization instead.  Summing up,
the exponential $\langle \lift S^1_2, \lift m^1_2, \ihom {A_1}
{A_2}\rangle = \ihom {\langle S_1, m_1, A_1 \rangle} {\langle S_2,
m_2, A_2\rangle}$ is given by the diagram on the left below.
\begin{equation}
  \label{d_expo}
  \xymatrix@R-15pt@C+5pt{
    {\widehat S^1_2 \SEpbk}
    \ar@{.>>}[r]^{\lift e^1_2}
    \ar@{.>}[ddd]
    &
    {\lift S^1_2}
    \ar@{^{(}.>}[r]^{\lift m^1_2}
    \ar@{.>}[lddd]_{\ell^1_2}
    &
    {\funbara {\ihom {A_1} {A_2}}}
    \ar[ddd]|-{\Lambda \left(\funbara {\App} \circ \tstrna \circ \left(\identity {} \tensord m_1\right)\right)}
    & 
    {\funbara {\ihom {A_1} {A_2}} \tensord S_1}
    \ar[d]^{\identity {\funbara {\ihom {A_1} {A_2}}} \tensord m_1}
    \\
    &&&
    {\funbara {\ihom {A_1} {A_2}} \tensord \funbara {A_1}}
    \ar[d]^{\tstr {\ihom {A_1} {A_2}} {A_1}} \\
    &&&
    {\funbara {\ihom {A_1} {A_2} \tensorc A_1}}
    \ar[d]^{\funbara {\App}} \\
    {\ihom {S_1} {S_2}}
    \arrmonoxy[rr]^{\ihom {S_1} {m_2}}
    &&
    {\ihom {S_1} {\funbara {A_2}}}
    &
    {\funbara {A_2}}
                                %  \\
                                %  {\ihom {S_1} {S_2} \tensord S_1}
                                %  \ar[r]^(0.7){\App}
                                %  &
                                %  S_2
                                %  \ar[r]^{m_2}
                                %  &
                                %  {\funbara {A_2}}
                                %  &
    }
\end{equation}
where the vertical morphism $\Lambda \left(\funbara \App \circ \tstrna \circ
  \left(\identity {} \tensord m_1\right)\right)$ is $\Lambda$ applied to the
composition of vertical morphisms on the right, the morphism $\ihom {S_1}
{m_2}$ is a relevant mono by our assumption that $\ihom {S_1} \_$ preserves
relevant monos, the topmost horizontal composition of arrows (from $\widehat S^1_2$ to
$\funbara {\ihom {A_1} {A_2}}$) is given by pullback, and is factored as
$\lift e^1_2$ followed by $\lift m^1_2$; and finally the morphism $\ell^1_2$
is given by a diagonal fill-in, from two paths from $\widehat S^1_2$ to $\ihom
{S_1} {\funbara {A_2}}$.

Application from $\langle \lift S^1_2, \lift m^1_2, \ihom {A_1} {A_2}\rangle
\tensorS \langle S_1, m_1, A_1\rangle$ is then given by $\langle \widehat\App,
\funbara \App\rangle$ as given in the diagram below.
\begin{equation}
  \label{d_app}
  \xymatrix@C+15pt@R-5pt{
    &
    {\lift S^1_2 \tensord S_1}
    \ar[r]^{\lift m^1_2 \tensord \identity {S_1}}
    \ar[d]_{\ell^1_2 \tensord \identity {S_1}}
    \ar@{.>>}[lddd]_{e_\App}
    &
    {\funbara {\ihom {A_1} {A_2}} \tensord S_1}
    \ar[r]^{\identity {} \tensord m_1}
    \ar[d]|{\Lambda (\funbara \App \circ \tstrna \circ (\identity {} \tensord m_1)) \tensord
      \identity {S_1}}
    &
    {\funbara {\ihom {A_1} {A_2}} \tensord \funbara {A_1}}
    \ar[dd]|{\tstr {\ihom {A_1} {A_2}} {A_1}}
    \\
    &
    {\ihom {S_1} {S_2} \tensord S_1}
    \ar[r]_{\ihom {S_1} {m_2} \tensord \identity {S_1}}
    \ar[d]_{\App} &
    {\ihom {S_1} {\funbara {A_2}} \tensord S_1}
    \ar[d]^{\App}
    &
    \\
    &
    {S_2}
    \arrmonoxy[r]_{m_2}
    &
    {\funbara {A_2}}
    &
    {\funbara {\ihom {A_1} {A_2} \tensorc A_1}}
    \ar[l]_{\funbara {\App}}
    \\
    {S_\App}
    \ar@{^{(}.>}[rrru]_{m_\App}
    \ar@{.>}[ru]|{\widehat\App}
    &&&
    }
\end{equation}
The top left square comes from the definition of the exponential $\langle
\lift S^1_2, \lift m^1_2, \ihom {A_1} {A_2}\rangle$, tensored by $S_1$ on the
right.  The bottom left square commutes because $\App \circ (\ihom {S_1} {m_2}
\tensord \identity {S_1}) = \App \circ (\Lambda (m_2 \circ \App) \tensord
\identity {S_1}) = m_2 \circ \App$%
\ifmscs
.
\else
by (\ref{eq:beta}).  The right square commutes by (\ref{eq:beta}) again.
\fi
The outer contour, defined by $\lift m^1_2
\tensord m_1$ on the top, $\tstr {\ihom {A_1} {A_2}} {A_1}$ on the right,
$e_\App$ on the left, $m_\App$ at the bottom, is the definition of the tensor
product $\langle \lift S^1_2, \lift m^1_2, \ihom {A_1} {A_2}\rangle \tensorS
\langle S_1, m_1, A_1\rangle$ in the subscone.  $\widehat \App$ is given by a
diagonal fill-in, considering the two paths $e_\App$ followed by $\funbara
\App \circ m_\App$ and $\App \circ (\ell^1_2 \tensord \identity {S_1})$
followed by $m_2$ from $\lift S^1_2 \tensord S_1$ to $\funbara {A_2}$.

\noindent
\begin{minipage}{6cm}
  Given any morphism $\langle u, v\rangle$ in the subscone from $\langle S, m,
  A\rangle \tensorS \langle S_1, m_1, A_1\rangle$ to $\langle S_2, m_2,
  A_2\rangle$, by definition the following diagram commutes.  The top square
  is the definition of $\langle S, m, A\rangle \tensorS \langle S_1, m_1,
  A_1\rangle$.
\end{minipage}
\begin{minipage}{6cm}
  \begin{equation}
    \label{eq:expo:uv}
    \xymatrix@R-10pt{
      S \tensord S_1
      \ar[r]^{m \tensord m_1}
      \arrepixy[d]_{e_{.1}}
      &
      {\funbara {A} \tensord \funbara {A_1}}
      \ar[d]_{\tstr {A} {A_1}}
      \\
      S_{.1}
      \arrmonoxy[r]_{m_{.1}}
      \ar[d]_{u}
      &
      {\funbara {A \tensorc A_1}}
      \ar[d]^{\funbara v}
      \\
      S_2
      \ar[r]_{m_2}
      &
      {\funbara {A_2}}
      }    
  \end{equation}
\end{minipage}

\noindent
\begin{minipage}{3.5cm}
  Abstraction of the morphism $\langle u, v\rangle$ in the subscone from
  $\langle S, m, A\rangle \tensorS \langle S_1, m_1, A_1\rangle$ to $\langle
  S_2, m_2, A_2\rangle$ is then the pair $\langle \lift e^1_2 \circ \tilde u,
  \Lambda (v)\rangle$ given by the diagram:
\end{minipage}
\begin{minipage}{8.5cm}
  \begin{equation}
    \label{d_abs}
    \xymatrix@C+5pt@R-5pt{
      S
      \arrmonoxy[rrr]^{m}
      \ar@{.>}[rd]^{\lift u}
      \ar[rdd]_{\Lambda (u \circ e_{.1})}
      &&&
      {\funbara A}
      \ar[d]^{\funbara {\Lambda (v)}}
      \\
      &
      {\widehat S^1_2\SEpbk}
      \arrepixy[r]^{\lift e^1_2}
      \arrmonoxy[d]
      &
      {\lift S^1_2}
      \arrmonoxy[r]^{\lift m^1_2}
      \ar[ld]|{\ell^1_2}
      &
      {\funbara {\ihom {A_1} {A_2}}}
      \ar[d]|-{\Lambda \left(\funbara {\App} \circ \tstrna \circ \left(\identity {} \tensord m_1\right)\right)}
      \\
      &
      {\ihom {S_1} {S_2}}
      \arrmonoxy[rr]^{\ihom {S_1} {m_2}}
      &&
      {\ihom {S_1} {\funbara {A_2}}}
      }
  \end{equation}
\end{minipage}

\noindent
In this diagram, $\lift u$ is given by the universal property of pullbacks,
and this will be justified by the fact that the two outer paths from $S$ to
$\ihom {S_1} {\funbara {A_2}}$ are equal, which we have to check. First, we
note the identity
\begin{equation}
  \label{eq:Lambda:o}
  \Lambda (s) \circ t = \Lambda (s \circ (t \tensord \identity C))
\end{equation}
whenever $t$ is a morphism from $A$ to $B$, and $s$ from $B \tensord C$ to
$D$. Indeed, $\Lambda (s) \circ t = \Lambda (\App \circ ((\Lambda (s) \circ t)
\tensord \identity C))$
\ifmscs
\else
(by (\ref{eq:eta}))
\fi
$= \Lambda (\App \circ (\Lambda
(s) \tensord \identity C) \circ (t \tensord \identity C)) = \Lambda (s \circ
(t \tensord \identity C))$%
\ifmscs
.
\else
(by (\ref{eq:beta})).
\fi
  It follows that the lower
path from $S$ to $\ihom {S_1} {\funbara {A_2}}$ in Diagram~\ref{d_abs} is
\begin{eqnarray*}
  \ihom {S_1} {m_2} \circ \Lambda (u \circ e_{.1})
  & = & \Lambda (m_2 \circ \App) \circ \Lambda (u \circ e_{.1}) \\
  & = & \Lambda (m_2 \circ \App \circ (\Lambda (u \circ e_{.1}) \tensord \identity {S_1}))
  \qquad \mbox{(by (\ref{eq:Lambda:o}))} \\
  & = & \Lambda (m_2 \circ u \circ e_{.1})
  \qquad \ifmscs\else\mbox{(by (\ref{eq:beta}))}\fi
\end{eqnarray*}
while the upper one is
\begin{eqnarray*}
  && \Lambda (\funbara \App \circ \tstrna \circ (\identity {} \tensord m_1))
  \circ \funbara {\Lambda (v)} \circ m \\
  & = & \Lambda (\funbara \App \circ \tstrna \circ (\identity {} \tensord m_1)
  \circ ((\funbara {\Lambda (v)} \circ m) \tensord \identity {S_1}))
  \qquad \mbox{(by (\ref{eq:Lambda:o}))} \\
  & = & \Lambda (\funbara \App \circ \tstrna \circ (\funbara {\Lambda (v)}
  \tensord \identity {\funbara {A_1}}) \circ (m \tensord m_1))
  \\
  & = & \Lambda (\funbara \App \circ \funbara {\Lambda (v) \tensorc \identity
    {A_1}}
  \circ \tstrna \circ (m \tensord m_1))
  \qquad \mbox{(by naturality of $\tstrna$)} \\
  & = & \Lambda (\funbara v \circ \tstrna \circ (m \tensord m_1))
  \qquad \ifmscs\else\mbox{(by (\ref{eq:beta}))}\fi
\end{eqnarray*}
and these two quantities are equal by Diagram~(\ref{eq:expo:uv}).

\ifmscs
\else
Finally, the equations (\ref{eq:beta}) and (\ref{eq:eta}) then hold in the
subscone, because they hold in $\catc$, and using Fact~\ref{f_eq}.
\fi

We sum up what we need to lift exponentials to the subscone, as usual.
To lift exponentials on the right:

\begin{tabular}{|l|}
  \hline
  {\bf (i.a.r)} monoidal closed (on the right) categories $(\catc, \tensorc, \Ic, \alphacna, \lc{},
  \rc{})$ \\
  \qquad and $(\catd, \tensord, \Id, \alphadna, \ld{}, \rd{})$,
  and a monoidal functor $\funbar : \catc \to \catd$,\\
  {\bf (iii.a)} a monoidal mono factorization system on $\catd$.\\
  {\bf (v)} $\catd$ has pullbacks.\\
  {\bf (vi.r)} $\ihom A \_$ preserves relevant monos.\\
  \hline
\end{tabular}

Exponentials are given by (\ref{d_expo}), application by (\ref{d_app}),
abstraction by (\ref{d_abs}).

The construction works equally well to lift exponentials on the left,
reversing arguments to tensor products, so we require in this case:

\begin{tabular}{|l|}
  \hline
  {\bf (i.a.l)} monoidal closed (on the left) categories $(\catc, \tensorc, \Ic, \alphacna, \lc{},
  \rc{})$ \\
  \qquad and $(\catd, \tensord, \Id, \alphadna, \ld{}, \rd{})$
  and a monoidal functor $\funbar : \catc \to \catd$,\\
  {\bf (iii.a)} a monoidal mono factorization system on $\catd$.\\
  {\bf (v)} $\catd$ has pullbacks.\\
  {\bf (vi.l)} $\ihoml A \_$ preserves relevant monos.\\
%corrected JGL 05 may 2004
  \hline
\end{tabular}

Clearly, in the symmetric monoidal closed case we require the following to
get a symmetric monoidal closed subscone:

\begin{tabular}{|l|}
  \hline
  {\bf (i.b)} symmetric monoidal closed categories $(\catc, \tensorc, \Ic, \alphacna, \lc{},
  \rc{}, \ccna)$ \\
  \qquad and $(\catd, \tensord, \Id, \alphadna, \ld{}, \rd{}, \cdna)$,
  and a symmetric monoidal functor $\funbar : \catc \to \catd$,\\
  {\bf (iii.a)} a monoidal mono factorization system on $\catd$.\\
  {\bf (v)} $\catd$ has pullbacks.\\
  {\bf (vi)} $\ihom A \_$ preserves relevant monos.\\
  \hline
\end{tabular}

And in the cartesian closed case, we require:

\begin{tabular}{|l|}
  \hline
  {\bf (i.c)} cartesian closed categories $\catc$ and $\catd$, \\
  \qquad and a cartesian monoidal functor $\funbar : \catc \to \catd$,\\
  {\bf (iii.a)} a monoidal mono factorization system on $\catd$.\\
  {\bf (v)} $\catd$ has pullbacks.\\
  {\bf (vi)} $\ihom A \_$ preserves relevant monos.\\
  \hline
\end{tabular}

Putting all conditions together, we get a notion of subscone for categorical
models of Moggi's meta-language, i.e., for cartesian closed categories with a
strong monad, we require:

\begin{tabular}{|l|}
  \hline
  {\bf (i.c)} cartesian closed categories $\catc$ and $\catd$, \\
  \qquad and a cartesian monoidal functor $\funbar : \catc \to \catd$,\\
  {\bf (ii.a)} a strong monad $( \td, \unitd{}, \multd{}, \strdna)$ on $\catd$,
  related to $(\tc, \unitc{}, \multc{}, \strcna)$ 
  by \\
  \qquad a strong monad morphism $(\funbar, \dist{})$ defined 
  in~(\ref{d_distlaw}) and~(\ref{d_diststr}),\\
  {\bf (iii.a)} a monoidal mono factorization system on $\catd$.\\
  {\bf (iv)} $\td$ maps relevant pseudoepis to pseudoepis.\\
  {\bf (v)} $\catd$ has pullbacks.\\
  {\bf (vi)} $\ihom A \_$ preserves relevant monos.\\
  \hline
\end{tabular}

\ifmscs
\else
\comment{
\subsection{Linear $\lambda$-Calculus}
\label{ccc.s:linear}

Similarly, we may deal with fragments of the linear $\lambda$-calculus. In
particular, the intuitionistic multiplicative fragment has symmetric monoidal
closed categories as models.  (We base ourselves loosely on
\cite{Bierman:whatcatmodel:lin}.)  We sketch how this can be enriched with a
strong monad `$?$'.  (Said otherwise, we take models of
multiplicative-exponential intuitionistic linear logic where the comonad `$!$'
is the identity.)  This will be the framework that we shall use in
Section~\ref{sec:proba:met}, for example.

Syntactically, consider the intuitionistic multiplicative fragment with a
strong monad. Types $\tau$ are given by:
\[
\tau ::= b | 1 | \tau \otimes \tau | \tau \llimp \tau | ? \tau
\]
where $b$ ranges over a given collection of base types. Linear $\lambda$-terms
are given by:
\begin{eqnarray*}
  s, t, u, v, ... & ::= & x | * | \letin {* = s} t | s \otimes t | \letin {x \otimes y =
    s} t | st | \lambda x \cdot s \\
  && | \valu s | \letin {\valu x = s} t
\end{eqnarray*}
Typing rules are given as follows, where contexts $\Gamma$ are multisets of
bindings $x:\tau$, with pairwise distinct variable parts $x$.
\begin{eqnarray*}
  \begin{prooftree}
    \justifies
    x:A \vdash x:A
    \using (Var)
  \end{prooftree}
  &&
  \\
  \begin{prooftree}
    \Gamma \vdash s : 1 \quad
    \Delta, x:1 \vdash t : \tau
    \justifies
    \Gamma, \Delta \vdash \letin {* = s} t : \tau
    \using (1\mathcal E)
  \end{prooftree}
  &&
  \begin{prooftree}
    \justifies
    \vdash * : 1
    \using (1)
  \end{prooftree}
  \\
%  \begin{prooftree}
%    \Gamma \vdash s : \tau \otimes \tau' \quad
%    \Delta, x:\tau, y:\tau' \vdash t : \tau''
%    \justifies
%    \Gamma, \Delta \vdash t [x:=\pi_1 s, y:=\pi_2 s]
%    \using (Proj)
%  \end{prooftree}
  \begin{prooftree}
    \Gamma \vdash s : \tau \otimes \tau' \quad
    \Delta, x : \tau, y : \tau' \vdash t : \tau''
    \justifies
    \Gamma, \Delta \vdash \letin {x \otimes y = s} t : \tau''
    \using (\otimes\mathcal E)
  \end{prooftree}
  &&
  \begin{prooftree}
    \Gamma \vdash s : \tau \quad
    \Delta \vdash t : \tau'
    \justifies
    \Gamma, \Delta \vdash s \otimes t : \tau \otimes \tau'
    \using (Pair)
  \end{prooftree}
  \\
  \begin{prooftree}
    \Gamma \vdash s : \tau \llimp \tau' \quad
    \Delta \vdash t : \tau
    \justifies
    \Gamma, \Delta \vdash st : \tau'
    \using (App)
  \end{prooftree}
  &&
  \begin{prooftree}
    \Gamma, x : \tau \vdash s : \tau'
    \justifies
    \Gamma \vdash \lambda x \cdot s : \tau \llimp \tau'
    \using (Abs)
  \end{prooftree}
  \\
  \begin{prooftree}
    \Gamma \vdash s : ? \tau \quad
    \Delta, x:\tau \vdash t : ? \tau'
    \justifies
    \Gamma, \Delta \vdash \letin {\valu x=s} t : ? \tau'
    \using (Let)
  \end{prooftree}
  &&
  \begin{prooftree}
    \Gamma \vdash s : \tau
    \justifies
    \Gamma \vdash \valu s : ? \tau
    \using (Val)
  \end{prooftree}
\end{eqnarray*}
Conversion rules are given by judgments $\Gamma \vdash s \to t : \tau$ (which we write $s \to
t$ when $\Gamma$ and $\tau$ are clear or irrelevant), of which the most important are:
\begin{eqnarray*}
  \letin {* = *} s \to s
  %\Gamma \vdash s \to * : 1
  &&
  \vdash s \to * : 1
  \\
  \letin {x \otimes y = s \otimes t} u \to u [x:=s, y:=t] &&
  \letin {x \otimes y = s} {x \otimes y} \to s
%  \pi_1 \langle s, t \rangle \to s \quad
%  & \pi_2 \langle s, t \rangle \to t &
%  \quad
%  \langle \pi_1 s, \pi_2 s\rangle \to s
  \\
  (\lambda x \cdot s) t \to s[x:=t] && \lambda x \cdot sx \to s \quad
  \mbox{($x$ not free in $s$)} \\
  \letin {\valu x = \valu s} t \to t[x:=s] &&
  \letin {\valu x = s} {\valu x} \to s \\
  \letin {\valu x = \letin {\valu y = s} t} u
  & \to & \letin {\valu y=s} {\letin {\valu x = t} u}
\end{eqnarray*}
There are other rules, notably the infamous commutative conversion
rules---which originate in \cite{Prawitz:natdeduc}---and which we won't state.
The interpretation in symmetric monoidal closed categories follows the same
lines as those of the ordinary $\lambda$-calculus with a monadic type, replacing
cartesian products by tensor products. Our constructions then yield a notion
of subscone for this kind of calculus and models, requiring:

\begin{tabular}{|l|}
  \hline
  {\bf (i.b)} symmetric monoidal closed categories $(\catc, \tensorc, \Ic, \alphacna, \lc{},
  \rc{}, \ccna)$ \\
  \qquad and $(\catd, \tensord, \Id, \alphadna, \ld{}, \rd{}, \cdna)$,
  and a symmetric monoidal functor $\funbar : \catc \to \catd$,\\
  {\bf (ii.a)} a strong monad $( \td, \unitd{}, \multd{}, \strdna)$ on $\catd$,
  related to $(\tc, \unitc{}, \multc{}, \strcna)$ 
  by \\
  \qquad a strong monad morphism $(\funbar, \dist{})$ defined 
  in~(\ref{d_distlaw}) and~(\ref{d_diststr}),\\
  {\bf (iii.a)} a monoidal mono factorization system on $\catd$.\\
  {\bf (iv)} $\td$ maps relevant pseudoepis to pseudoepis.\\
  {\bf (v)} $\catd$ has pullbacks.\\
  {\bf (vi)} $\ihom A \_$ preserves relevant monos.\\
  \hline
\end{tabular}

We let the reader do similar mixing-and-matching to handle his/her own
favorite model or logic.

%!!! use the constructions of lifting monads from adjunctions, maybe (expo is
 %adjoint to product).
}
\fi

\comment{DN 07/01/04

\subsection{Cosimplicial Subscones From a Lifted Monad}
\label{ccc.s:simplicial}

Logical relations arise from subscones when $\catd = \catset$.  It is often
the case that we require more complex logical relations, e.g., {\em Kripke
  logical relations} \cite{Mit96}; see \cite{Ali95} for a precise account and
relationship between Kripke logical relations and subscones.  Let us just say
that Kripke logical relations indexed by a category $\cal I$ are just the case
of subscones when $\catd$ is the presheaf category $\catset^{\cal I}$, i.e.,
the category of functors from $\cal I$ to $\catset$ with natural
transformations as morphisms.  Recall that any presheaf category is a topos,
hence in particular is cartesian closed and has pullbacks
\cite{McLane:cat:math}.

It is usually difficult to design a Kripke logical relation, and to start
with, it is usually difficult to find the right index category $\cal I$. It
turns out that, using insights due to Barr and Beck \cite{BarrBeck}, there is
a canonical way of building Kripke logical relations indexed by the simplicial
category $\Delta$, which we describe next.

Let $\Delta$ be the category whose objects are sets $[n] = \{0, 1, \ldots,
n\}$, for all integers $n\geq -1$, equipped with the natural ordering, and
whose morphisms are all monotonic functions.  This is usually called the
simplicial category.  (Some authors call it the augmented simplicial category,
and reserve the term simplicial category for the full subcategory of $\Delta$
that does not contain $[-1]$.)  The category $\Delta$ is generated by
morphisms $\delta^i_q : [q-1] \to [q]$ and $\sigma^i_q : [q+1] \to [q]$, for
all $0 \leq i\leq q$, subject to the so-called simplicial identities:
\[
\begin{array}{rlrlrl}
  (i) & \delta^j_q \delta^i_{q-1} = \delta^i_q \delta^{j-1}_{q-1} &
  (ii) & \sigma^{j-1}_q \sigma^i_{q+1} = \sigma^i_q \sigma^j_{q+1} &
  (iii) & \sigma^j_q \delta^i_{q+1} = \delta^i_q \sigma^{j-1}_{q-1} \\
  & (0\leq i<j \leq q) &
  & (0\leq i<j \leq q) &
  & (0\leq i<j \leq q) \\
  (iv) & \sigma^i_q \delta^i_{q+1} = \identity {[q]} &
  (v) & \sigma^i_q \delta^{i+1}_{q+1} = \identity {[q]} &
  (vi) & \delta^j_q \sigma^i_{q-1} = \sigma^i_q \delta^{j+1}_{q+1} \\
  & (0\leq i\leq q) &
  & (0\leq i\leq q) &
  & (0\leq i<j \leq q)
\end{array}
\]

The category $\catd^\Delta$ of all functors from $\Delta$ to $\catd$, with
natural transformations as morphisms, is called the category of {\em
  cosimplicial objects in $\catd$}, and morphisms are called {\em cosimplicial
  maps in $\catd$}.  Alternatively, a cosimplicial object in $\catd$ is a
family ${(A_q)}_{q\geq -1}$ of objects of $\catd$ together with morphisms
$\partial^i_q$ from $A_{q-1}$ to $A_q$ (the {\em cofaces\/}) and $s^i_q$ from
$A_{q+1}$ to $A_q$ (the {\em codegeneracies\/}), $0\leq i\leq q$, satisfying
the {\em cosimplicial equations}, that is the equations $(i)$--$(vi)$ above
with $\partial$ replacing $\delta$, $s$ replacing $\sigma$.  A cosimplicial
map from ${(A_q)}_{q\geq -1}$ to ${(B_q)}_{q\geq -1}$ is a family of morphisms
$f_q$ from $A_q$ to $B_q$ that commute with cofaces and codegeneracies.

Given any monad $(\td, \unitd{}, \multd{})$ on $\catd$, Barr and Beck's
construction yields a functor $\BBna \td : \catd \to \catd^\Delta$ defined as
follows (see \cite{McLane:cat:math}).  For each object $A$ of $\catd$, $\BB
\td A$ is the object ${(\td^{q+1} A)}_{q\geq -1}$.  The coface $\partial^i_q :
\td^q A \to \td^{q+1} A$ is $\td^i \unitd {\td^{q-i} A}$, the codegeneracy
$s^i_q : \td^{q+2} A \to \td^{q+1} A$ is $\td^i \multd {\td^{q-i} A}$.  They
obey the cosimplicial equations precisely because $(\td, \unitd{}, \multd{})$
is a monad.  Finally, for every morphism $A {\buildrel f \over\longrightarrow}
B$ in $\catd$, $\BB \td f$ is the morphism ${(\td^{q+1} f)}_{q\geq -1}$ from
$\BB \td A$ to $\BB \td B$. It is obvious that $\BBna \td$ is an embedding of
$\catd$ into $\catd^\Delta$: in fact there is a projection functor $\BBUna$
from $\catd^\Delta$ to $\catd$ such that $\BBUna \circ \BBna \td$ is the
identity endofunctor on $\catd$, namely $\BBU {{(A_q)}_{q\geq -1}} = A_{-1}$,
$\BBU {{(f_q)}_{q\geq -1}} = f_{-1}$.

Furthermore, the monad $(\td, \unitd{}, \multd{})$ extends to a monad on
$\catd^\Delta$ as follows.  For every simplicial object $\K A = {(A_q)}_{q\geq
  -1}$ with cofaces $\partial^i_q$ and codegeneracies $s^i_q$, let $\decalaged
(\K A)$ ($\decalaged$ is called {\em d\'ecalage\/}) be the cosimplicial object
${(A_{q+1})}_{q\geq -1}$, with cofaces ${\partial^i_q}'$ and codegeneracies
${s^i_q}'$ defined by ${\partial^i_q}' = \partial^{i}_{q+1}$ and ${s^i_q}' =
s^{i}_{q+1}$. $\decalaged$ defines an endofunctor on $\catd^\Delta$, by
defining $\decalaged (\K f)$, where $\K f = {(f_q)}_{q\geq -1}$, to be the
cosimplicial map ${(f_{q+1})}_{q \geq -1}$. Let $\unitBBd {\K A}$ be the
morphism from $\K A$ to $\decalaged (\K A)$ defined by $\unitBBd {\K A, q} =
\partial^{q+1}_{q+1}$, and let $\multBBd {\K A}$ be the morphism from
$\decalaged^2 (\K A)$ to $\decalaged (\K A)$ defined by $\multBBd {\K A, q} =
s^{q+1}_{q+1}$.  It is easy to check that $(\decalaged, \unitBBd {}, \multBBd
{})$ is a monad on $\catd^\Delta$.

\begin{lemma}
  \label{lemma:[-1]:ext}
  Relatively to the embedding $\BBna \td$ of $\catd$ in $\catd^\Delta$, the
  monad $(\decalaged, \unitBBd {}, \multBBd {})$ extends $(\td, \unitd{},
  \multd{})$.  That is, $\BB \td {\td A} = \decalaged {\BB \td A}$, $\BB \td
  {\td f} = \decalaged {\BB \td f}$, $\BB \td {\unitd A} = \unitBBd {\BB \td
    A}$, $\BB \td {\multd A} = \multBBd {\BB \td A}$.
\end{lemma}
\begin{proof}
  $\BB \td {\td A}$ is the cosimplicial object ${(\td^{q+1} \td A)}_{q\geq -1}
  = {(\td^{q+2} A)}_{q\geq -1}$, with coface $\partial^i_q = \td^i \unitd
  {\td^{q-i+1} A}$, codegeneracy $s^i_q = \td^i \multd {\td^{q-i+1} A}$.  This
  is clearly the d\'ecalage of $\BB \td A = {(\td^{q+1} A)}_{q\geq -1}$ with
  coface $i,q$ equal to $\td^i \unitd {\td^{q-i} A}$ and codegeneracy $i,q$
  equal to $\td^i \multd {\td^{q-i} A}$.  The identity $\BB \td {\td f} =
  \decalaged {\BB \td f}$ is similar but simpler.  For the third identity,
  $\BB \td {\unitd A}$ is the cosimplicial map ${(\td^{q+1} \unitd A)}_{q\geq
    -1}$, and $\unitBBd {\BB \td A, q}$ is by definition $\partial^{q+1}_{q+1} =
  \td^{q+1} \unitd {\td^{q+1-(q+1)} A} = \td^{q+1} \unitd A$.  The fourth
  equation is proved similarly.  \qed
\end{proof}

Given a functor $\funbar : \catc \to \catd$, let $\funbarBB : \catc^\Delta \to
\catd^\Delta$ be the functor mapping ${(A_q)}_{q \geq -1}$ (with cofaces
$\partial^i_q$, codegeneracies $s^i_q$) to ${(\funbara {A_q})}_{q \geq -1}$
(with cofaces $\funbara {\partial^i_j}$, codegeneracies $\funbara {s^i_j}$),
and mapping the morphim ${(f_q)}_{q \geq -1}$ to ${(\funbara {f_q})}_{q\geq
  -1}$.

Recall that the idea of using a functor $\funbar : \catc \to \catd$ to build
the subscone is to observe the semantics in $\catc$ through its trace on
$\catd$.  If $\catd$ is $\catset$, we get logical relations, and to move to
Kripke logical relations, we wish to replace $\catd$ by $\catd^\Delta$.  Now
there are {\em two\/} canonical functors from $\catc$ to $\catd^\Delta$,
namely $\BB \td \funbar$ and $\funbarBBa {\BBna \tc}$.  Both lead to monad
morphisms:

\begin{lemma}
  \label{lemma:[-1]:dist}
  Let $(\funbar, \dist{})$ be a monad morphism from the monad $(\tc, \unitc{},
  \multc{})$ on $\catc$ to the monad $(\td, \unitd{}, \multd{})$ on $\catd$.
  
  The pair $(\funbarBBa {\BBna \tc}, \identity {})$ is a monad morphism from
  $\tc$ to $\decalaged$, called the {\em brutal\/} extension of $(\funbar,
  \dist{})$.
  
  The pair $(\BB \td \funbar, \distBB{})$, where $\distBB A : \decalaged {\BB
    \td {\funbara A}} \to \BB \td {\funbara {\tc A}}$ is $(\td^{q+1} \dist A :
  \td^{q+2} (\funbara A) \to \td^{q+1} (\funbara {\tc A}))_{q\geq -1}$, is a
  monad morphism from $\tc$ to $\decalaged$ , called the {\em considerate\/}
  extension of $(\funbar, \dist{})$.
  
%  Then $(\funbarBB, \distBB {}$) is a monad morphism from $(\decalagec,
%  \unitBBc{}, \multBBc{})$ to $(\decalaged, \unitBBd {}, \multBBd {})$ which
%  extends $(\funbar, \dist {})$ in the sense that $\BB \td {\funbara A} =
%  \funbarBBa {\BB \td A}$, $\BB \td {\funbara f} = \funbarBBa {\BB \td f}$,
%  $\BB \td {\dist A} = \distBB {\BB \td A}$.
\end{lemma}
\begin{proof}
  Brutal case.  We must first check that the identity natural transformation
  indeed defines morphisms from $\decalaged {\funbarBBa {\BB \tc A}}$ to
  $\funbarBBa {\BB \tc {\tc A}}$.  Observe that $\decalaged {\funbarBBa {\BB
      \tc A}}$ is ${(\funbara {\tc^{q+2} A})}_{q\geq -1}$ with cofaces
  $\funbara {\tc^i \unitc {\tc^{q+1-i} A}}$ and codegeneracies $\funbara
  {\tc^i \multc {\tc^{q+1-i} A}}$.  Now observe that $\funbarBBa {\BB \tc {\tc
      A}}$ is exactly the same object.  That the identity is natural is
  obvious.  The monad morphism equations (\ref{d_distlaw}) then amount to
  $\unitBBd {\funbarBBa {\BB \tc A}} = \funbarBBa {\BB \tc {\unitc A}}$ and
  $\multBBd {\funbarBBa {\BB \tc A}} = \funbarBBa {\BB \tc {\multc A}}$.  Now
  $\unitBBd {\funbarBBa {\BB \tc A}}$ is ${(\partial^{q+1}_{q+1})}_{q \geq
    -1}$, where $\partial^i_q$ is $\funbara {\tc^i \unitc {\tc^{q-i} A}}$, so
  this is ${(\funbara {\tc^{q+1} \unitc A})}_{q \geq -1} = \funbarBBa {\BB \tc
    {\unitc A}}$.  $\multBBd {\funbarBBa {\BB \tc A}} = \funbarBBa {\BB \tc
    {\multc A}}$ is proved similarly.
  
  Considerate case.  By Lemma~\ref{lemma:[-1]:ext}, $\decalaged {\BB \td
    {\funbara A}} = \BB \td {\td {\funbara A}}$; then $\distBB A$ is just $\BB
  \td {\dist A}$ from $\decalaged {\BB \td {\funbara A}} = \BB \td {\td
    \funbara A}$ to $\BB \td {\funbara {\tc A}}$, and is therefore a natural
  transformation.  The monad morphism equations (\ref{d_distlaw}) are obtained
  from those of $(\funbar, \dist {})$ by applying $\BBna \td$, and using
  Lemma~\ref{lemma:[-1]:ext}.  \qed
\end{proof}

Therefore, as soon as $\catc$, $\tc$, $\catd$, $\td$ satisfy {\bf (i)} and
{\bf (ii)} with monad morphism $(\funbar, \dist{})$, then so do $\catc$,
$\tc$, $\catd^\Delta$, $\decalaged$ and either the brutal monad morphism
$(\funbarBBa {\BBna \tc}, \identity{})$ or the considerate one $(\BB \td
\funbar, \distBB{})$.

In the cartesian case, i.e., when $\catd$ has finite products, we would like
the embedding $\BBna \td$ to preserve products.  This is in general doomed to
failure, as $\BBna \td$ preserves products if and only if $\td$ does.  Indeed,
products in $\catd^\Delta$ are pointwise: ${(A_q)}_{q \geq -1} \times
{(B_q)}_{q\geq -1} = {(A_q \times B_q)}_{q \geq -1}$; if $\BBna \td$ preserved
products then ${\BB \td {(A \times B)}}_0 = \td (A \times B)$ would be equal
to $(\BB \td A \times \BB \td B)_0 = \td A \times \td B$.  Notice that most
monads do not preserve products; e.g., for the powerset monad $(\pow, \{\_\},
\bigcup)$ on $\catset$, preserving products would mean that $\pow (A \times B)
= \pow A \times \pow B$.

We can require instead $\BBna \td$ to be monoidal, as soon as $\td$ is
monoidal (next proposition). Note first that for every monoidal category
$(\catd, \tensord, \Id, \alphadna, \ld{}, \rd{})$, $\catd^\Delta$ is also
monoidal with pointwise tensor products, i.e., ${(A_q)}_{q\geq -1} \tensord
{(B_q)}_{q\geq -1} = {(A_q \tensord B_q)}_{q\geq -1}$ with cofaces and
codegeneracies given by tensor products of cofaces and codegeneracies of $A_q$
and $B_q$ respectively, pointwise unit $\IBBd = {(\Id)}_{q\geq -1}$ (with
identity cofaces and codegeneracies), and the obvious pointwise associativity,
left unit and right unit laws.  Similarly, if $\catd$ is symmetric monoidal or
has finite products, then so does $\catd^\Delta$.

\begin{proposition}
  \label{prop:[-1]:monoidal}
  Let $(\catd, \tensord, \Id, \alphadna, \ld{}, \rd{})$ be a monoidal
  category, and $(\td, \unitd{}, \multd{}, \bistrdna)$ be a monoidal monad on
  it.
  
  Then $\BBna \td$ is a monoidal functor from $\catd$ to $\catd^\Delta$, with
  mediating pair $(\tstrBBna, \tstrBBi)$ defined by $\tstrBB A B = ( \td^q
  \bistrd A B \allowbreak \circ \ldots \allowbreak \circ \td {\bistrd
    {\td^{q-1} A} {\td^{q-1} B}} \allowbreak \circ \bistrd {\td^q A} {\td^q B}
  : \td^{q+1} A \tensord \td^{q+1} B \allowbreak \to \allowbreak \td^{q+1} (A
  \tensord B))_{q\geq -1}$, and $\tstrBBi = {( \td^q \unitd \Id \allowbreak
    \circ \ldots \allowbreak \circ \td \unitd \Id \allowbreak \circ \unitd \Id
    : \Id \allowbreak \to \allowbreak \td^{q+1} \Id)}_{q\geq -1}$.  (Empty
  compositions, i.e., when $q=-1$, denote identities.)
  
%!!! say that it is also sym mon, cart. mon.
  
  Moreover, $(\decalaged, \unitBBd {}, \multBBd {}, \bistrBBdna)$ is a
  monoidal monad on $\catd^\Delta$, where the mediator $\bistrBBd {\K A} {\K
    B}$ is the identity morphism on $\decalaged (\K A \tensord \K B) =
  \decalaged {\K A} \tensord \decalaged {\K B}$.
  
  Finally, $(\BBna \td, \identity{})$ is a monoidal monad morphism from $\td$
  to $\decalaged$.
%  It extends $(\td, \unitd{},
%  \multd{}, \bistrdna)$ in the sense that $\BB \td {\bistrd A B} = \bistrBBd
%  {\BB \td A} {\BB \td B}$ in addition to the equalities of
%  Lemma~\ref{lemma:[-1]:ext}.
\end{proposition}
\begin{proof}
  Let us check that $(\tstrBBna, \tstrBBi)$ is mediating for $\BBna \td$.  We
  first show that $\tstrBB A B$ is a cosimplicial map.  For every $0\leq i\leq
  q$,
  \begin{eqnarray*}
    &&
    \partial^i_q \circ
    (\td^{q-1} \bistrd A B \circ \ldots \circ \td {\bistrd {\td^{q-2} A}
      {\td^{q-2} B}} \circ \bistrd {\td^{q-1} A} {\td^{q-1} B})
    \\
    & = &
    \td^i \unitd {\td^{q-i} (A \tensord B)} \circ
    \td^{q-1} \bistrd A B \circ \ldots \circ \td {\bistrd {\td^{q-2} A}
      {\td^{q-2} B}} \circ \bistrd {\td^{q-1} A} {\td^{q-1} B}
    \\
    & = &
    \td^q \bistrd A B
    \circ \td^i \unitd {\td^{q-1-i} (\td A \tensord \td B)}
    \circ \td^{q-2} \bistrd {\td A} {\td B} \circ
    \ldots \circ \td {\bistrd {\td^{q-2} A}
      {\td^{q-2} B}} \circ \bistrd {\td^{q-1} A} {\td^{q-1} B}
    \\
    && \qquad \mbox{(since $\unitd{}$ is natural)} \\
    & = & \ldots \\
    & = &
    \td^q \bistrd A B \circ \td^{q-1} \bistrd {\td A} {\td B} \circ
    \ldots \circ \td^{i+1} \bistrd {\td^{q-1-i} A} {\td^{q-1-i} B}
    \\
    && \quad
    \circ \td^i \unitd {\td^{q-i} A \tensord \td^{q-i} B}
    \circ \td^{i-1} \bistrd {\td^{q-i} A} {\td^{q-i} B} \circ
    \ldots \circ \td {\bistrd {\td^{q-2} A}
      {\td^{q-2} B}} \circ \bistrd {\td^{q-1} A} {\td^{q-1} B}
    \\
    & = &
    \td^q \bistrd A B \circ \td^{q-1} \bistrd {\td A} {\td B} \circ
    \ldots \circ \td^{i+1} \bistrd {\td^{q-1-i} A} {\td^{q-1-i} B}
    \\
    && \quad
    \circ \td^i \bistrd {\td^{q-i} A} {\td^{q-i} B} \circ \td^i (\unitd
    {\td^{q-i} A} \tensord \unitd {\td^{q-i} B}) \\
    && \quad
    \circ \td^{i-1} \bistrd {\td^{q-i} A} {\td^{q-i} B} \circ
    \ldots \circ \td {\bistrd {\td^{q-2} A}
      {\td^{q-2} B}} \circ \bistrd {\td^{q-1} A} {\td^{q-1} B}
    \qquad \mbox{(by (\ref{eq:monoidal:eta}))}
    \\
    & = &
    \td^q \bistrd A B \circ \td^{q-1} \bistrd {\td A} {\td B} \circ
    \ldots \circ \td^{i+1} \bistrd {\td^{q-1-i} A} {\td^{q-1-i} B}
    \\
    && \quad
    \circ \td^i \bistrd {\td^{q-i} A} {\td^{q-i} B}
    \circ \td^{i-1} \bistrd {\td^{q+1-i} A} {\td^{q+1-i} B}
    \circ \td^{i-1} (\td \unitd {\td^{q-i} A} \tensord \td \unitd {\td^{q-i} B}) \\
    && \quad
    \circ \td^{i-2} \bistrd {\td^{q+1-i} A} {\td^{q+1-i} B} \circ
    \ldots \circ \td {\bistrd {\td^{q-2} A}
      {\td^{q-2} B}} \circ \bistrd {\td^{q-1} A} {\td^{q-1} B}
    \\
    && \qquad \mbox{(since $\bistrdna$ is natural)}
    \\
    & = & \ldots \\
    & = &
    \td^q \bistrd A B \circ \td^{q-1} \bistrd {\td A} {\td B} \circ
    \ldots \circ \td^{i+1} \bistrd {\td^{q-1-i} A} {\td^{q-1-i} B}
    \\
    && \quad
    \circ \td^i \bistrd {\td^{q-i} A} {\td^{q-i} B}
    \circ \td^{i-1} \bistrd {\td^{q+1-i} A} {\td^{q+1-i} B}
    \circ \ldots \\
    && \quad \circ \td \bistrd {\td^{q-1} A} {\td^{q-1} B}
    \circ \bistrd {\td^q A} {\td^q B}
    \circ (\td^i \unitd {\td^{q-i} A} \tensord \td^i \unitd {\td^{q-i} B})
    \\
    & = &
    (\td^q \bistrd A B \circ \td^{q-1} \bistrd {\td A} {\td B} \circ
    \ldots \circ \td \bistrd {\td^{q-1} A} {\td^{q-1} B}
    \circ \bistrd {\td^q A} {\td^q B})
    \circ (\partial^i_q \tensord \partial^i_q)
  \end{eqnarray*}
  The case of codegeneracies is similar and uses (\ref{eq:monoidal:mu})
  instead of (\ref{eq:monoidal:eta}).  Naturality of $\tstrBBna$ in $A, B$ is
  clear, as a composition of natural constructions.  We have noticed in
  Section~\ref{strong.s:monoidal} that any monoidal monad $\td$ induces a
  monoidal functor $\td$ with mediating pair $(\bistrdna, \unitd{})$.  Then,
  for each fixed $q\geq -1$, composing this monoidal functor $q+1$ times with
  itself produces a monoidal functor $\td^{q+1}$, whose mediating pair is just
  the $q$-component of $(\tstrBBna, \tstrBBi)$ (see
  Appendix~\ref{app:monadj:comp} to see what composition of monoidal functors
  look like).  So the coherence laws for $(\tstrBBna, \tstrBBi)$ are
  satisfied.
  
  That $\bistrBBdna$ defined as the identity is natural is obvious.  Note that
  $\decalaged \IBBd = \IBBd$, and that $\unitBBd {\IBBd} =
  {(\partial^{q+1}_{q+1})}_{q\geq -1}$ where $\partial^i_q$ is the coface $i,
  q$ of $\IBBd$, i.e., the identity.  Diagram~(\ref{eq:monoidal:l}) then
  reduces to checking that the d\'ecalage of the left unit law ${(\ld
    {\td^{q+1} B})}_{q \geq -1}$ is the left unit law again, which is obvious.
  Diagram~(\ref{eq:monoidal:r}) is similar.  Since $\bistrBBdna$ is the
  identity, Diagram~(\ref{eq:monoidal:double}) amounts to the fact that the
  d\'ecalage of the associativity law is the associativity law again.
  Diagram~(\ref{eq:monoidal:eta}) means that $\unitBBd A \tensord \unitBBd B =
  \unitBBd {A \tensord B}$, which stems from the fact that cofaces, in
  particular $\partial^{q+1}_{q+1}$, on $A \tensord B$ are just the tensor
  products of corresponding cofaces on $A$ and $B$.  Similar considerations on
  codegeneracies sows that $\multBBd A \tensord \multBBd B = \multBBd {A
    \tensord B}$, that is, Diagram~(\ref{eq:monoidal:mu}).
%  We now check that $\BB \td {\bistrd A B} = \bistrBBd
%  {\BB \td A} {\BB \td B}$.
% \bistrd A B : \td A \tensord \td B \to \td (A \tensord B)
% \BB \td {\bistrd A B} : {( \td^{q+1} (\td A \tensord \td B \to \td (A
 % \tensord B)) )}_{q\geq -1}
  
  That $(\BBna \td, \identity{})$ is a monoidal monad morphism from $\td$ to
  $\decalaged$ means that $\identity{}$ is a natural transformation from
  $\decalaged {\BB \td A}$ to $\BB \td {\td A}$ (trivial) satisfying
  Diagrams~(\ref{d_distlaw}) and~(\ref{d_distbistr}).
  Diagram~(\ref{d_distlaw}) means that $\unitBBd {\BB \td A} = \BB \td {\unitd
    A}$ and $\multBBd {\BB \td A} = \BB \td {\multd A}$, which is clear.
  Diagram~(\ref{d_distbistr}) means that $\decalaged {\tstrBB {A_1} {A_2}}
  \circ \bistrBBd {\BB \td {A_1}} {\BB \td {A_2}} = \BB \td {\bistrd {A_1}
    {A_2}} \circ \tstrBB {\td {A_1}} {\td {A_2}}$, i.e., for each $q\geq -1$:
  \begin{eqnarray*}
    &&
    (\td^{q+1} \bistrd {A_1} {A_2} \circ \td^q \bistrd {\td {A_1}} {\td {A_2}}
    \circ \ldots \circ \td {\bistrd {\td^{q} {A_1}} {\td^{q} {A_2}}}
    \circ \bistrd {\td^{q+1} {A_1}} {\td^{q+1} {A_2}}) \circ \identity {}
    \\
    & = &
    \td^{q+1} \bistrd {A_1} {A_2} \circ 
    (\td^q \bistrd {\td {A_1}} {\td {A_2}} \circ \ldots
    \circ \td {\bistrd {\td^{q-1} {\td {A_1}}} {\td^{q-1} {\td {A_2}}}}
    \circ \bistrd {\td^q {\td {A_1}}} {\td^q {\td {A_2}}})
  \end{eqnarray*}
  which is obvious.  \qed
\end{proof}

\begin{proposition}
  \label{prop:[-1]:monoidal}
  Let $(\tc, \unitc{}, \multc{}, \bistrcna)$ be a monoidal monad on the
  monoidal category $(\catc, \tensorc, \Ic, \alphacna, \lc{}, \rc{})$, $(\td,
  \unitd{}, \multd{}, \bistrdna)$ be a monoidal monad on the monoidal category
  $(\catd, \allowbreak \tensord, \allowbreak \Id, \allowbreak \alphadna,
  \allowbreak \ld{}, \allowbreak \rd{})$, and assume that there is a monoidal
  monad morphism $(\funbar, \dist{})$ from the former to the latter.
  
  Then $(\funbarBBa {\BBna \tc}, \identity{})$ (brutal) and $(\BB \td \funbar,
  \distBB{})$ (considerate) are monoidal monad morphisms from $(\tc, \unitc{},
  \multc{}, \bistrcna)$ to $(\decalaged, \unitBBd {}, \multBBd {},
  \bistrBBdna)$.
\end{proposition}
\begin{proof}
  We first show that $(\funbarBBa {\BBna \tc}, \identity{})$ is a monoidal
  monad morphism from $\tc$ to $\decalaged$.  First, $\funbarBB$ is a monoidal
  functor, with mediating pair $(\tstrna^*, \tstri^*)$ given pointwise, namely
  by $\tstr {\K A} {\K B}^* = {(\tstr {A_q} {B_q})}_{q\geq -1}$ and $\tstri^*
  = {(\tstri)}_{q\geq -1}$.  So $\funbarBBa {\BBna \tc}$ is also monoidal,
  with mediating pair given by $(\funbarBBa {\tstrBBcna} \circ\tstrna^*,
  \funbarBBa {\tstrBBci} \circ \tstri^*)$.  Since the mediator is identity,
  and $\bistrBBdna$ and $\bistrBBcna$ are, too, the monoidal monad
  Diagram~(\ref{d_distbistr}) amounts to $\decalaged {\funbarBBa {\BB \tc
      {\tstrBBc {A_1} {A_2}}} \circ \tstr {\BB \tc {A_1}} {\BB \tc {A_2}}^*} =
  \funbarBBa {\tstrBBc {\tc A_1} {\tc A_2}} \circ \tstr {\BB \tc {\tc {A_1}}}
  {\BB \tc {\tc {A_2}}}^*$, which is obvious since d\'ecalage, $\tstrna^*$ and
  tensor products are pointwise.
  
  Then, we show that $(\BB \td \funbar, \distBB{})$ is a monoidal monad
  morphism from $\tc$ to $\decalaged$.  Since the composition of monoidal
  functors is monoidal, as soon as $\funbar$ is monoidal, so is the
  considerate extension $\BB \td {\funbar}$.  Its mediating pair is $(\BB \td
  {\tstrna} \circ \tstrBBna, \BB \td {\tstri} \circ \tstrBBi)$.  We only have
  to check the mediator Diagram~(\ref{d_distbistr}), which is $\distBB {A_1
    \tensorc A_2} \circ \decalaged (\BB \td {\tstr {A_1} {A_2}} \circ \tstrBB
  {\funbara {A_1}} {\funbara {A_2}}) \circ \bistrBBd {\BB \td {\funbara
      {A_1}}} {\BB \td {\funbara {A_2}}} = \BB \td {\funbara {\bistrc {A_1}
      {A_2}}} \circ (\BB \td {\tstr {\tc A_1} {\tc A_2}} \circ \tstrBB
  {\funbara {\tc {A_1}}} {\funbara {\tc {A_2}}}) \circ (\distBB {A_1} \tensord
  \distBB {A_2})$, that is, for each $q\geq -1$:
  \begin{eqnarray*}
    && \td^{q+1} \dist {A_1 \tensorc A_2}
    \circ \td^{q+2} \tstr {A_1} {A_2} \\
    && \quad
    \circ (\td^{q+1} \bistrd {\funbara {A_1}} {\funbara {A_2}} \circ \td^q \bistrd {\td {\funbara {A_1}}} {\td {\funbara {A_2}}}
    \circ \ldots \circ \td {\bistrd {\td^{q} {\funbara {A_1}}} {\td^{q} {\funbara {A_2}}}}
    \circ \bistrd {\td^{q+1} {\funbara {A_1}}} {\td^{q+1} {\funbara {A_2}}})
    \\
    & = &
    \td^{q+1} {\funbara {\bistrc {A_1} {A_2}}}
    \circ \td^{q+1} \tstr {\tc {A_1}} {\tc {A_2}} \\
    && \quad
    \circ (\td^q \bistrd {\funbara {\tc {A_1}}} {\funbara {\tc {A_2}}}
                                %\circ \td^{q-1} {\bistrd {\td \funbara {\tc {A_1}}} {\td \funbara {\tc {A_2}}}}
    \circ \ldots \circ \td {\bistrd {\td^{q-1} \funbara {\tc {A_1}}} {\td^{q-1}
        \funbara {\tc {A_2}}}}
    \circ \bistrd {\td^q \funbara {\tc {A_1}}} {\td^q \funbara {\tc {A_2}}}) \\
    && \qquad
    \circ (\td^{q+1} \dist {A_1} \tensord \td^{q+1} \dist {A_2})
  \end{eqnarray*}
  Indeed, by naturality of $\bistrdna$ the right-hand side equals
  \begin{eqnarray*}
    &&
    \td^{q+1} {\funbara {\bistrc {A_1} {A_2}}}
    \circ \td^{q+1} \tstr {\tc {A_1}} {\tc {A_2}} \\
    && \quad
    \circ \td^{q+1} (\dist {A_1} \tensord \dist {A_2})
    \circ (\td^q \bistrd {\td {\funbara {A_1}}} {\td {\funbara {A_2}}}
    \circ \ldots \circ \td {\bistrd {\td^{q} {\funbara {A_1}}} {\td^{q} {\funbara {A_2}}}}
    \circ \bistrd {\td^{q+1} {\funbara {A_1}}} {\td^{q+1} {\funbara {A_2}}})
  \end{eqnarray*}
  We conclude since by Diagram~(\ref{d_distbistr}),$\dist {A_1 \tensorc A_2}
  \circ \td \tstr {A_1} {A_2} \circ \bistrd {\funbara {A_1}} {\funbara {A_2}}
  = {\funbara {\bistrc {A_1} {A_2}}} \circ \tstr {\tc {A_1}} {\tc {A_2}}\circ
  (\dist {A_1} \tensord \dist {A_2})$, hence $\td^{q+1} \dist {A_1 \tensorc
    A_2} \circ \td^{q+2} \tstr {A_1} {A_2} \circ \td^{q+1} \bistrd {\funbara
    {A_1}} {\funbara {A_2}} = \td^{q+1} {\funbara {\bistrc {A_1} {A_2}}} \circ
  \td^{q+1} \tstr {\tc {A_1}} {\tc {A_2}}\circ \td^{q+1} (\dist {A_1} \tensord
  \dist {A_2})$. \qed
\end{proof}

Therefore, as soon as $\catc$, $\tc$, $\catd$, $\td$ satisfy {\bf (i.a)} and
{\bf (ii.b)} with monoidal monad morphism $(\funbar, \dist{})$, then so do
$\catc$, $\tc$, $\catd^\Delta$, $\decalaged$ and either the brutal monad
morphism $(\funbarBBa {\BBna \tc}, \identity{})$ or the considerate one $(\BB
\td \funbar, \distBB{})$.

It does not seem that we can lift strong monads to subscones on the presheaf
category $\catd^\Delta$, whence the need for monoidal monads.

We now deal with the symmetric monoidal and cartesian cases.

\begin{lemma}
  \label{lemma:[-1]:symmon}
  Under the assumptions of Proposition~\ref{prop:[-1]:monoidal}, if $\catc$
  and $\catd$ are symmetric monoidal, then $\catd^\Delta$ is a symmetric
  monoidal category.  Moreover, if $\funbar : \catc \to \catd$ is symmetric
  monoidal then:
  \begin{enumerate}
  \item If $(\tc, \unitc{}, \multc{}, \bistrcna)$ is a commutative monad, then
    the brutal functor $\funbarBBa {\BBna \tc}$ is symmetric monoidal.
  \item If $(\td, \unitd{}, \multd{}, \bistrdna)$ is a commutative monad, then
    the considerate functor $\BB \td \funbar$ is symmetric monoidal.
  \end{enumerate}
\end{lemma}
\begin{proof}
  The commutativity $\cdBBna$ is defined pointwise, so the coherence
  conditions extend to $\catd^\Delta$.
  
  1. That the brutal functor $\funbarBBa {\BBna \tc}$ is symmetric monoidal
  (Diagram~(\ref{eq:theta:coh:c})) means that $\tstr {A_2} {A_1}^* \circ \cdBB
  {\funbarBBa {\BBna \tc {A_1}}} {\funbarBBa {\BBna \tc {A_2}}} \allowbreak =
  \funbarBBa {\BBna \tc {\cc {A_1} {A_2}}} \circ \tstr {A_1} {A_2}^*$, i.e.,
  $\funbarBBa {\tstrBBc {A_2} {A_1}} \circ \tstr {\BB \tc {A_2}} {\BB \tc
    {A_1}}^* \circ \cdBB {\funbarBBa {\BBna \tc {A_1}}} {\funbarBBa {\BBna \tc
      {A_2}}} = \funbarBBa {\BBna \tc {\cc {A_1} {A_2}}} \circ \funbarBBa
  {\tstrBBc {A_1} {A_2}} \circ \tstr {\BB \tc {A_1}} {\BB \tc {A_2}}^*$.  For
  each $q\geq -1$, this means
  \begin{eqnarray*}
    &&
    \funbara {\tc^q \bistrc {A_2} {A_1} \circ \ldots \circ \tc \bistrc
      {\tc^{q-1} {A_2}} {\tc^{q-1} {A_1}} \circ \bistrc {\tc^q {A_2}} {\tc^q
        {A_1}}}
    \\
    && \qquad
    \circ \tstr {\tc^{q+1} {A_2}} {\tc^{q+1} {A_1}}
    \circ \cd {\funbara {\tc^{q+1} {A_1}}} {\funbara {\tc^{q+1} {A_2}}}
    \\
    & = &
    \funbara {\tc^{q+1} {\cc {A_1} {A_2}}}
    \circ \funbara {\tc^q \bistrc {A_1} {A_2} \circ \ldots \circ \tc \bistrc
      {\tc^{q-1} {A_1}} {\tc^{q-1} {A_2}} \circ \bistrc {\tc^q {A_1}} {\tc^q
        {A_2}}}
    \\
    && \qquad
    \circ \tstr {\tc^{q+1} {A_1}} {\tc^{q+1} {A_2}}
  \end{eqnarray*}
  which is an easy consequence of $\tstr {\tc^{q+1} {A_2}} {\tc^{q+1} {A_1}}
  \circ \cd {\funbara {\tc^{q+1} {A_1}}} {\funbara {\tc^{q+1} {A_2}}} =
  \funbara {\cc {\tc^{q+1} {A_1}} {\tc^{q+1} {A_2}}} \circ \tstr {\tc^{q+1}
    {A_1}} {\tc^{q+1} {A_2}}$ (Diagram~(\ref{eq:theta:coh:c})) and repeated
  application of Diagram~(\ref{eq:monoidal:comm}), stating that $\tc$ is a
  commutative monad.

  2. That the considerate functor $\BB \td \funbar$ is symmetric monoidal
  means that $\BB \td {\tstr {A_2} {A_1}} \circ \tstrBB {\funbara {A_2}}
  {\funbara {A_1}} \circ \cdBB {\BB \td {\funbara {A_1}}} {\BB \td {\funbara
      {A_2}}} = \BB \td {\funbara {\cc {A_1} {A_2}}} \circ \BB \td {\tstr
    {A_1} {A_2}} \circ \tstrBB {\funbara {A_1}} {\funbara {A_2}}$, that is,
  for each $q\geq -1$:
  \begin{eqnarray*}
    &&
    \td^{q+1} \tstr {A_2} {A_1}
    \circ (\td^q \bistrd {\funbara {A_2}} {\funbara {A_1}} \circ
    \ldots \circ \td \bistrd {\td^{q-1} \funbara {A_2}} {\td^{q-1} \funbara
      {A_1}}
    \circ \bistrd {\td^q \funbara {A_2}} {\td^q \funbara {A_1}})
    \\
    && \qquad
    \circ \cd {\td^{q+1} \funbara {A_1}} {\td^{q+1} \funbara {A_2}}
    \\
    & = &
    \td^{q+1} \funbara {\cc {A_1} {A_2}}
    \circ \td^{q+1} \tstr {A_1} {A_2}
    \\
    && \qquad
    \circ (\td^q \bistrd {\funbara {A_1}} {\funbara {A_2}} \circ
    \ldots \circ \td \bistrd {\td^{q-1} \funbara {A_1}} {\td^{q-1} \funbara
      {A_2}}
    \circ \bistrd {\td^q \funbara {A_1}} {\td^q \funbara {A_2}})
  \end{eqnarray*}
  which is a consequence of repeated application of
  Diagram~(\ref{eq:monoidal:comm}), stating that $\td$ is a commutative monad,
  and of Diagram~(\ref{eq:theta:coh:c}).  \qed
\end{proof}

In the cartesian case, say that a monoidal monad $(\td, \unitd{}, \multd{},
\bistrdna)$ is a {\em cartesian monad\/} if and only if $\td$ is a cartesian
monoidal functor with mediating pair $(\bistrdna, \unitd{})$.  (Recall that
$\td$ is always a monoidal functor with this very mediating pair.)  This means
that $\td \pi_i \circ \bistrd A B = \pi_i$, $i \in \{1, 2\}$.

\begin{lemma}
  \label{lemma:[-1]:cart}
  Under the assumptions of Proposition~\ref{prop:[-1]:monoidal}, if $\catc$
  and $\catd$ have finite products, then $\catd^\Delta$ has finite products.
  Moreover, if $\funbar : \catc \to \catd$ is cartesian monoidal then:
  \begin{enumerate}
  \item If $(\tc, \unitc{}, \multc{}, \bistrcna)$ is a cartesian monad, then
    the brutal functor $\funbarBBa {\BBna \tc}$ is cartesian monoidal.
  \item If $(\td, \unitd{}, \multd{}, \bistrdna)$ is a cartesian monad, then
    the considerate functor $\BB \td \funbar$ is cartesian monoidal.
  \end{enumerate}
\end{lemma}
\begin{proof}
  $\catd^\Delta$ has cartesian products as soon as $\catd$ has, and they are
  defined pointwise.
  
  1. That $\funbarBBa {\BBna \tc}$ is cartesian monoidal means that
  $\funbarBBa {\BB \tc {\pi_i}} \circ \funbarBBa {\tstrBBc {A_1} {A_2}} \circ
  \tstr {\BB \tc {A_1}} {\BB \tc {A_2}}^* = \pi_i$, i.e.:
  \begin{eqnarray*}
    \funbara {\tc^{q+1} \pi_i}
    \circ \funbara {\tc^q \bistrc {A_1} {A_2} \circ \ldots \circ \tc \bistrc
      {\tc^{q-1} A_1} {\tc^{q-1} A_2} \circ \bistrc {\tc^q A_1} {\tc^q A_2}}
    \circ \tstr {\tc^{q+1} A_1} {\tc^{q+1} A_2}
    & = & \pi_i
  \end{eqnarray*}
  This follows by iterated application of $\tc \pi_i \circ \bistrcna = \pi_i$
  ($\tc$ is a cartesian monad), and Diagram~(\ref{eq:theta:coh:proj}) stating
  that $\funbar$ is cartesian monoidal.
  
  2. That $\BB \td \funbar$ is cartesian monoidal means that $\BB \td
  {\funbara {\pi_i}} \circ \BB \td {\tstr {A_1} {A_2}} \circ \tstrBB {\funbara
    {A_1}} {\funbara {A_2}} = \pi_i$, i.e.:
  \begin{eqnarray*}
    \td^{q+1} \funbara {\pi_i}
    \circ \td^{q+1} \tstr {A_1} {A_2}
    \circ (\td^q \bistrd {A_1} {A_2} \circ \ldots \circ
    \td \bistrd {\td^{q-1} A_1} {\td^{q-1} A_2} \circ \bistrd {\td^q A_1}
    {\td^q A_2})
    & = & \pi_i
  \end{eqnarray*}
  This follows by Diagram~(\ref{eq:theta:coh:proj}) stating that $\funbar$ is
  cartesian monoidal, then iterated application of $\td \pi_i \circ \bistrdna
  = \pi_i$ ($\td$ is a cartesian monad).  \qed
\end{proof}


The properties {\bf (iii)} (existence of a mono factorization system on
$\catd$) and {\bf (iii.a)} (same, but monoidal) also lift to $\catd^\Delta$.
This is almost trivial:
\begin{lemma}
  \label{lemma:presh:epimono}
  Assume that $\catd$ has a mono factorization system.  Let $I$ be any
  category.  Let the {\em pointwise pseudoepis\/} from $\K A$ to $\K B$ in
  $\catd^I$ be those natural transformations ${(\xymatrix{A_q
      \arrepixy[r]^{e_q} & B_q})}_{q \in I}$ where $e_q$ is pseudoepi for
  every object $q$ of $I$, and define pointwise relevant monos similarly.
  Then pointwise pseudoepis and pointwise relevant monos define a mono
  factorization system on $\catd^I$.  It is monoidal as soon as the given mono
  factorization system on $\catd$ is monoidal.
\end{lemma}
\begin{proof}
  First, every morphism $\K f$ from $\K A$ to $\K B$ in $\catd^I$ (a natural
  transformation) is such that $f_q$ can be factored as $\xymatrix{A_q
    \arrepixy[r]^{e_q} & C_q \arrmonoxy[r]^{m_q} & B_q}$.

  \noindent
  \begin{minipage}{7cm}
    For every morphism $i {\buildrel g \over\longrightarrow} q$ in $I$, there
    is by definition a morphism $A_i$ from $A_p$ to $A_q$ and a morphism $B_i$
    from $B_p$ to $B_q$, from which we deduce the existence of a morphism
    $C_i$ from $C_p$ to $C_q$ by diagonal fill-in:
  \end{minipage}
  \begin{minipage}{5cm}
    \[
    \xymatrix{
      A_p
      \ar[d]_{A_i}
      \arrepixy[r]^{e_p}
      &
      C_p
      \ar@{.>}[d]|{C_i}
      \arrmonoxy[r]^{m_p}
      &
      B_p
      \ar[d]^{B_i}
      \\
      A_q
      \arrepixy[r]^{e_q}
      &
      C_q
      \arrmonoxy[r]^{m_q}
      &
      B_q
      }
    \]
  \end{minipage}

  \noindent
  Since such diagonal fill-ins are unique, it is easy to see that the mappings
  $q \mapsto C_q$ and $i \mapsto C_i$ define a functor from $I$ to $\catd$.
  Moreover, by the diagram above the families ${(e_q)}_{q\in I}$ and
  ${(m_q)}_{q\in I}$ are natural in $q$.  By construction they define a
  pointwise pseudoepi and a pointwise relevant mono respectively.
  
  \noindent
  \begin{minipage}{6cm}
    The diagonal fill-in property in $\catd^I$ is shown in the obvious way.
    Let $\K f \circ \K e = \K m \circ \K g$, where $\K e$ is pointwise
    pseudoepi and $\K m$ is pointwise relevant mono.  For each object $q$ of
    $I$, there is a unique diagonal fill-in $h_q$ in $\catd$ such that $h_q
    \circ e_q = g_q$ and $m_q \circ h_q = f_q$.
    
    The collection $\K h = {(h_q)}_{q\in I}$ is then natural in $q$, as the
    slanted face with vertices $B_p$, $B_q$, $C_p$, $C_q$ shows in the diagram
    on the right.
  \end{minipage}
  \begin{minipage}{6cm}
    \[
    \xymatrix{
      A_p
      \arrepixy[rr]^{e_p}
      \ar[dd]_{g_p}
      \ar[rd]|{A_i}
      &&
      B_p
      \ar[dd]|\hole^(0.7){f_p}
      \ar[rd]|{B_i}
      \ar[lldd]|\hole^(0.7){h_p}
      &
      \\
      &
      A_q
      \arrepixy[rr]^(0.3){e_q}
      \ar[dd]^(0.3){g_q}
      &&
      B_q
      \ar[dd]^{f_q}
      \ar[lldd]^(0.7){h_q}
      \\
      C_p
      \arrmonoxy[rr]|\hole_(0.7){m_p}
      \ar[rd]|{C_i}
      &&
      D_p
      \ar[rd]|{D_i}
      &
      \\
      &
      C_q
      \arrmonoxy[rr]_{m_q}
      &&
      D_q
      }
    \]
  \end{minipage}

  \noindent
  The fact that every pointwise relevant mono $\K m$ is mono in $\catd^I$ is
  immediate from the fact that every relevant mono $m_q$ is mono.
  
  Finally, assume that the mono factorization system on $\catd$ is monoidal,
  i.e., tensor products of pseudoepis is pseudoepi.  Since tensor products are
  computed pointwise in $\catd^I$, the tensor product of two pointwise
  pseudoepis is clearly pointwise pseudoepi again.  \qed
\end{proof}

Property {\bf (iv)}, that $\td$ maps relevant pseudoepis to pseudoepis, also
lifts to $\catd^\Delta$. This is trivial:
\begin{lemma}
  \label{lemma:presh:iv}
  D\'ecalage $\decalaged$ preserves pointwise pseudoepis.
\end{lemma}

Property {\bf (v)} ($\catd$ has pullbacks) also lifts in the expected way to
$\catd^\Delta$:
\begin{lemma}
  \label{lemma:presh:v}
  If $\catd$ has pullbacks, then so does $\catd^\Delta$.
\end{lemma}
Moreover, they are computed pointwise.  In fact, limits are always computed
pointwise in any functor category (\cite{McLane:cat:math}, V.3).

On the other hand, there is no reason why $\catd^\Delta$ should be monoidal
closed (resp.\ on the right, resp.\ on the left, resp.\ symmetric monoidal
closed, resp.\ cartesian closed), even when $\catd$ is.  Similarly, $\ihom {\K
  A} \_$ does not need to preserve pointwise relevant monos in general.
However, this holds in the case of presheaf categories at least:
\begin{lemma}
  \label{lemma:presh:vi}
  For any presheaf category $\catd = \catset^I$, with its cartesian closed
  structure, $\catd^\Delta$ is cartesian closed.  In $\catd^\Delta$, monos are
  pointwise monos, and $\ihom {\K A} \_$ preserves monos.
\end{lemma}
\begin{proof}
  That any presheaf category is cartesian closed (even an elementary topos) is
  well-known \cite{LS:CCC}.  Then $\catd^\Delta \cong \catd^{I \times \Delta}$
  is also a presheaf category, hence cartesian closed, too.  That monos
  coincide with pointwise monos in presheaves is an easy consequence of
  Yoneda's Lemma.  We have already noticed in Section~\ref{ccc.s:expo} that
  $\ihom {\K A} \_$ always preserves monos.  \qed
\end{proof}

We sum up this section by the slogan:

\begin{quote}
  If we can lift structure to the subscone $\subscone \catc \catd$, then we
  can lift it to the cosimplicial subscone $\subscone \catc {\catd^\Delta}$,
  too.
\end{quote}

Here, by structure, we mean any combination of: monads, monoidal (resp.\ 
closed) structure/monoidal monads, symmetric monoidal (resp.\ closed)
structure/commutative monads, finite products (resp.\ cartesian closed
structure)/car\-tesian monads. In the (monoidal, symmetric monoidal,
cartesian) closed case, we must require $\catd^\Delta$ to be (monoidal,
symmetric monoidal, cartesian) closed and $\ihom {\K A} \_$ to preserve
relevant monos; this comes for free in presheaf categories, by
Lemma~\ref{lemma:presh:vi}.

Moreover, the lifting to $\subscone \catc {\catd^\Delta}$ comes in two
flavors, the brutal and the considerate one.

}


==> cpo.tex <==
\newcommand\uuarrow{\rlap{$\uparrow$}\raise.5ex\hbox{$\uparrow$}}%%
\newcommand\ddarrow{\rlap{$\downarrow$}\raise.5ex\hbox{$\downarrow$}}%%

\subsection{The monad of demonic non-determinism}

Our construction also applies to other categories.  We deal here with
the monad of demonic non-determinism on a suitable subcategory of
$\Dcpo$, the category of cpos and continuous maps.  We refer to
\cite{AJ:domains,GHKLMS:compendium,GHKLMS:contlatt} for all missing
information on cpos and related topics.

Our developments will be much simpler if we can restrict to {\em
  continuous\/} cpos, so we shall consider for $\catc$ the category of
{\em FS-domains\/}, one of the two maximal cartesian-closed categories
of continuous pointed cpos \cite{Jung:CCC}.  By {\em cpo\/} we mean
any ordered set such that any directed family of elements has a least
upper bound.  A pointed cpo is one with a bottom element $\leq$.  A
continuous function $f : A \to A$ is {\em finitely separated from the
  identity\/} if any only if there is a finite subset $M$ of $A$ such
that, for every $x\in A$, there is $\mu \in M$ such that $f (x) \leq \mu \leq x$.
An {\em FS-domain\/} is any continuous pointed cpo such that there is
a directed family ${(f_i)}_{i\in I}$ of continuous functions from $A$ to
$A$, such that each is finitely separated from the identity, and whose
least upper bound is the identity on $A$.

Recall that any cpo $A$ is equipped with its Scott topology,
consisting of all upper sets $O$ such that, for every directed family
${(x_i)}_{i\in I}$ of elements of $A$ whose least upper bound is in $O$,
$x_i$ is in $O$ already for some $i \in I$.  If $A$ is pointed, then $A$
is compact, considered as a topological space.  If $A$ is a continuous
cpo, then as a topological space, $A$ is sober and locally compact.
By the Hofmann-Mislove theorem, given any filtered family ${(Q_i)}_{i\in
  I}$ of compact upper subsets of $A$, for any open $O$, $\bigcap_{i\in I} Q_i
\subseteq O$ if and only if $Q_i \subseteq O$ for some $i\in I$.  Any space that has the
latter property is called {\em well-filtered\/} by Jung
\cite{Jung:scs:prob}.  It follows that any filtered intersection of
non-empty compact upper subsets of $A$ is again non-empty and compact.

The {\em Smyth powerdomain\/} $\mathcal Q (A)$ consists of all
non-empty compact upper subsets of $A$, ordered by {\em reverse\/}
inclusion $\supseteq$.  This is traditionally used to model demonic
non-determinism.  We shall usually write $Q$ for saturated compacts.

If $A$ is a continuous cpo, then $\mathcal Q (A)$ is also a continuous
cpo, and the way-below relation $\ll$ is defined by $Q \ll Q'$ if and only
if the interior of $Q$ contains $Q'$.  The least upper bound of any
directed (for $\supseteq$) family ${(Q_i)}_{i\in I}$ of non-empty compact upper
subsets is $\bigcap_{i\in I} Q_i$.  Moreover, the Scott topology of $\mathcal
Q (A)$ is generated by the basic open sets $\Box U = \{Q \in \mathcal Q (A)
| Q \subseteq U\}$ when $U$ varies over the opens of $A$.  (That $\mathcal Q
(A)$ is a cpo fails if $A$ is not well-filtered; this is why we need
$A$ to be a continuous cpo; and there are only two maximal
subcategories of the category of continuous cpos that are
cartesian-closed, by Jung's results.  This is exactly why we are
interested in FS-domains in the present example.)

For any continuous function $f : A \to B$, let $\mathcal Q (f) :
\mathcal Q (A) \to \mathcal Q (B)$ be defined by: $\mathcal Q (f) (Q)$
is the smallest upper subset $\uparrow f (Q)$ containing the image $f (Q)$ of
$Q$ by $f$.  This makes $\mathcal Q$ a functor.

We observe the following:
\begin{lemma}
  \label{lemma:Q:FS}
  If $A$ is an FS-domain, then so is $\mathcal Q (A)$.
\end{lemma}
\begin{proof}
  We first claim that: (a) if $f$ is finitely separated from the
  identity (in $A$), then $\mathcal Q (f)$ is finitely separated from
  the identity (in $\mathcal Q (A)$).  Since $f$ is finitely separated
  from the identity, there is a finite subset $M$ of $A$ such that for
  every $x \in A$, $f (x) \leq \mu \leq x$ for some $\mu \in M$.  Take $\mathcal M$
  the set of subsets $\uparrow E$, where $E$ ranges over the subsets of $M$.
  Clearly $\mathcal M$ is finite.  We claim that, for every $Q \in
  \mathcal Q (A)$, there is some $\uparrow E$ in $\mathcal M$ such that
  $\mathcal Q (f) (Q) \supseteq \uparrow E \supseteq Q$.  This will establish that $\mathcal
  Q (f)$ is finitely separated from the identity in $\mathcal Q (A)$.
  Take $E$ to be the set of elements $\mu \in M$ such that $f (x) \leq \mu$ for
  some $x \in Q$.
  \begin{itemize}
  \item $\mathcal Q (f) (Q) \supseteq \uparrow E$: this means that $\uparrow f (Q) \supseteq \uparrow E$,
    i.e., every element of $E$ is above some element in $f (Q)$.  This
    is by definition.
  \item $\uparrow E \supseteq Q$: since $f$ is finitely separated from the identity,
    for every $x\in Q$, there is an $\mu \in M$ such that $f (x) \leq \mu \leq x$.
    In particular, $\mu$ is in $E$.  But the fact that every $x \in Q$ is
    above some $\mu \in E$ just means that $\uparrow E \supseteq Q$.
  \end{itemize}
  
  Since $f \leq g$ implies that $\mathcal Q (f) (Q) \supseteq \mathcal Q (g) (Q)$
  for every $Q \in \mathcal Q (A)$, every directed family ${(f_i)}_{i\in
    I}$ gives rise to a family of functions $\mathcal Q (f_i)$ that is
  directed w.r.t.\ $\supseteq$, i.e., which is filtered.

  We claim that: (b) given any directed family ${(f_i)}_{i\in I}$ of
  continuous functions from $A$ to $A$ whose least upper bound is the
  identity on $A$, the least upper bound of $\mathcal Q (f_i)$, $i\in
  I$, is the identity on $\mathcal Q (A)$.  Take any $Q \in \mathcal Q
  (A)$.  We want to show that the least upper bound of $\uparrow f_i (Q)$,
  $i\in I$, is $Q$, i.e., that $\bigcap_{i\in I} \uparrow f_i (Q) = Q$.
  \begin{itemize}
  \item $Q \subseteq \bigcap_{i\in I} \uparrow f_i (Q)$: for every $x\in Q$, since $f_i (x) \leq
    x$, $x \in \uparrow f_i (Q)$, for every $i \in I$.
  \item The converse is harder.  Let $x \in \bigcap_{i\in I} \uparrow f_i (Q)$.  This
    means that $f_i^{-1} (\downarrow x)$ intersects $Q$ for every $i \in I$,
    where $\downarrow x = \{y \in A | y \leq x\}$.  It is well-known that $\downarrow x$ is
    closed, so that $f_i^{-1} (\downarrow x)$ is closed.  Let $O_i$ be the open
    $A \setminus f_i^{-1} (\downarrow x)$.  Let $K_i$ be $f_i^{-1} (\downarrow x) \cap Q$,
    alternatively $K_i = Q \setminus O_i$.  Note that $K_i$ is not empty.
    Clearly $\bigcap_{i\in I} K_i = Q \setminus \bigcup_{i\in I} O_i$ is empty if and only if
    $Q \subseteq \bigcup_{i\in I} O_i$.  Since ${(f_i)}_{i\in I}$ is directed,
    ${(K_i)}_{i\in I}$ is directed, and since $Q$ is compact, $Q \subseteq \bigcup_{i\in
      I} O_i$ would entail $Q \subseteq O_i$ for some $i\in I$ by the
    Heine-Borel property; but $Q \subseteq O_i$ means that $K_i$ would be
    empty, a contradiction.  So $\bigcap_{i\in I} K_i$ is not empty.  Let $y$
    be any element of $\bigcap_{i\in I} K_i$.  By definition $y \in Q$, and $f_i
    (y) \leq x$ for every $i\in I$.  Since the least upper bound of
    ${(f_i)}_{i\in I}$ is the identity, $y \leq x$.  Since $Q$ is upper,
    $x$ is in $Q$.
  \end{itemize}
  We conclude: by (a) $\mathcal Q (f_i)$ is a finitely separated from
  the identity.  Since ${(f_i)}_{i\in I}$ is directed, so is ${(\mathcal
    Q (f_i))}_{i\in I}$.  And by (b) its least upper bound is the
  identity on $\mathcal Q (A)$.  \qed
\end{proof}

Consider $\unitc A : A \to \mathcal Q (A)$ defined by $\unitc A (x) = \uparrow
\{x\}$, $\multc A : \mathcal Q (\mathcal Q (A)) \to \mathcal Q (A)$
defined by $\multc A (\mathcal Q) = \bigcup_{Q\in \mathcal Q} Q$, and $\strc A
B : A \times \mathcal Q (B) \to \mathcal Q (A \times B)$ defined by $\strc A B (x,
Q) = \uparrow \{x\} \times Q$.  This makes $(\mathcal Q, \unitc \relax, \multc
\relax, \strcna)$ a strong monad on the category $\catc$ of
FS-domains.  (To show that $\multc \relax$ is well-defined, use the
fact that $\Box U$, $U$ open of $A$, forms a basis of the topology of
$\mathcal Q (A)$.  To show that $\strcna$ is well-defined, use
Tychonoff's theorem to show that $\uparrow \{x\} \times Q$ is compact, as a product
of two compacts.  Observe also that the topological product coincides
with the product of cpos, in the case that the two cpos are
continuous.)

To apply our construction of logical relations, we need a mono
factorization system.  In $\Dcpo$, as in every category with finite
limits, there are at least two choices for epi-mono factorizations:
taking as relevant monos all monos, or just the regular monos, i.e.,
the equalizers of parallel pairs
\cite[Remark~3.1]{Mog94}.

In FS-domains, the choice seems to be more restricted.  Take any
morphism $f : A \to B$ between FS-domains.  Using each of the above
factorizations yields a diagram $\xymatrix@-5pt{A \arrepixy[r]^e & C
  \arrmonoxy[r]^m & B}$ in $\Dcpo$, but we have not guarantee that the
middle object $C$ is an FS-domain.

However, this is the case when we choose the epi-regular mono
factorization in $\Dcpo$.  In this case, $C$ is the topological
closure $cl (f (B))$ of the range $f (B)$ of $f$ in $B$, $e$ coincides
with $f$ on $A$, and $m$ is the obvious embedding.  Note that $m$ is
still a regular mono in the category of FS-domains.  Indeed, $m$ is
the equalizer of the constant map sending each $y \in B$ to $0$, and the
characteristic map $\bar \chi_C : B \to \mathbb{S}$ that sends each $y \in C
\subseteq B$ to $0$, and each $y \in B \setminus C$ to $1$, where $\mathbb{S}$ is the
Sierpinski space $\{0, 1\}$ ordered by $0 \leq 1$.  It is easy to see that
$\mathbb{S}$ is an FS-domain, so that $m$ is again a regular mono in
the category of FS-domains\ldots{} provided $C$ is itself an FS-domain,
which we show next.  The existence of a diagonal fill-in in Diagram
(\ref{d_factordiag}) will then be automatic, by general properties of
epis and regular monos.

\begin{lemma}
  \label{lemma:closed:FS}
  Any closed subset $F$ of an FS-domain $B$ is an FS-domain.
\end{lemma}
\begin{proof}
  Let $\ll_B$ the way-below relation on $B$, and $\ll_F$ the way-below
  relation on $F$.  If $x, y \in F$ and $x \ll_B y$ then $x \ll_F y$.  Since
  $B$ is a continuous cpo, for any $x\in F$, the set of elements $y \in B$
  such that $y \ll_B x$ is directed, and has $x$ as least upper bound.
  Since $y \ll_B x$ implies $y \leq x$, and since any closed subset of
  lower, every $y \ll_B x$ is in $F$.  So the set $D_x$ of elements $y \in
  F$ such that $y \ll_B x$ is directed, and has $x$ as least upper
  bound.  Since $y \ll_B x$ implies $y \ll_F x$, $x$ is the least upper
  bound of a directed family of elements $y$ of $F$ such that $y \ll_F
  x$.  So $F$ is a continuous cpo.
  
  Since $B$ is an FS-domain, let ${(f_i)}_{i\in I}$ be a directed family
  of continuous functions separated from the identity on $B$.  Let
  $f'_i$ be the restriction of $f_i$ to $F$.  Note that for every $x \in
  F$, $f'_i (x) = f_i (x) \leq x \in F$, so $f'_i$ is a function from $F$
  to $F$.  Since $F$ is closed, $f'_i$ is clearly continuous.  Also,
  since $f_i$ is finitely separated from the identity in $B$, there is
  a finite subset $M$ of $B$ such that, for every $x \in B$, $f_i (x) \leq
  \mu \leq x$ for some $\mu \in M$.  Consider $M' = M \cap F$.  Then, for every $x
  \in F$, $f'_i (x) \leq \mu \leq x$ for some $\mu \in M$; and $\mu \in M'$ since $\mu \leq x
  \in F$.  So $f'_i$ is finitely separated from the identity in $F$.
  \qed
\end{proof}

Here is a more concrete description of epis and regular monos in
$\Dcpo$, and in the category of FS-domains.  A {\em sub-cpo\/} of a
cpo $B$ is a subset of $B$ that is a cpo with the induced ordering;
this is usually called an {\em inductive subset\/} of $B$, and is
characterized as one that is stable under the formation of least upper
bounds of directed subsets; similarly, a {\em sub-FS-domain\/} of a
cpo $B$ is any subset of $B$ that is an FS-domain.
\begin{lemma}
  \label{lemma:FS:epi}
  In $\Dcpo$ or in the category of FS-domains, an epi is any
  continuous function $e : \xymatrix@-5pt{A \arrepixy[r] & C}$ such
  that $e (A)$ is {\em dense\/} in $C$, i.e., such that $cl (e
  (A))=C$.
  
  A regular mono $m : \xymatrix@-5pt{C \arrmonoxy[r] & B}$ in $\Dcpo$,
  resp.\ in the category of FS-domains, is a sub-cpo, resp.\ a
  sub-FS-domain of $B$, up to isomorphism.  More precisely, $m$ is the
  composite of an iso from $C$ to some sup-cpo, resp.\ some
  sub-FS-domain, $m (C)$ of $B$, with the canonical inclusion of $m
  (C)$ in $B$.
\end{lemma}
\begin{proof}
  Let $e$ be epi.  Let $\bar \chi_{cl (e (A))} : C \to \mathbb{S}$ be the
  function mapping each $y \in cl (e (A))$ to $0$, and each $y \not\in cl
  (e (A))$ to $1$.  Clearly $\bar \chi_{cl (e (A))} (e (x)) = 0$ for
  every $x \in A$.  Since $e$ is epi, $\bar \chi_{cl (e (A))} = 0$, so $C =
  cl (e (A))$.  Conversely, let $e$ be such that $cl (e (A)) = C$.
  Then $e$ has an epi-regular mono factorization $\xymatrix@-5pt{A
    \arrepixy[r]^{e'} & cl (e (A)) \arrmonoxy[r]^{m'} & C}$.  By
  definition, $cl (e (A)) = C$, so $e'=e$.  Since $e'$ is epi, $e$ is,
  too.
  
  As far as regular monos are concerned, let us first observe that for
  every regular mono $m : \xymatrix@-5pt{C \arrmonoxy[r] & B}$, there
  is a continuous function $\hat m : cl (m (C)) \to C$ such that $\hat m
  \circ m = \identity {cl (m (C))}$.  Indeed, consider some epi-regular
  mono factorization $\xymatrix@-5pt{C \arrepixy[r]^{e'} & cl (m (C))
    \arrmonoxy[r]^{m'} & B}$ of $m$.  A diagonal fill-in of this with
  the obvious factorization $\xymatrix@-5pt{C \arrepixy[r]^{\identity
      C} & C \arrmonoxy[r]^m & B}$ yields a map $\hat m : cl (m (C)) \to
  C$ such that $\hat m \circ e' = \identity C$.  Since $e'$ coincides with
  $m$ on $C$ by definition, $\hat m \circ m = \identity C$.
  
  In other words, every regular mono is a cpo embedding.  Let $m :
  \xymatrix@-5pt{C \arrmonoxy[r] & B}$ be a regular mono.  So there
  are two morphisms $g_1, g_2 : B \to D$ that $m$ equalizes.  It follows
  that $m (C) = \{y \in B | g_1 (y) = g_2 (y)\}$.  Since $g_1$ and $g_2$
  are continuous, $m (C)$ is clearly inductive, i.e., $m (C)$ is a
  sub-cpo of $B$.
  
  In the FS-domain case, we must show that $m (C)$ is an FS-domain.
  Since $C$ is an FS-domain, pick a directed family of continuous
  functions ${(f_i)}_{i\in I}$ from $C$ to $C$, finitely separated from
  the identity, and whose least upper bound is the identity on $C$.
  Let $f'_i$ be the restriction of $m \circ f_i \circ \hat m$ to $m (C)$.
  This is a continuous function from $m (C)$ to $m (C)$.  Since $f_i$
  is finitely separated from the identity, there is a finite subset
  $M$ of $C$ such that, for every $x \in C$, $f_i (x) \leq \mu \leq x$ for some
  $\mu \in M$.  For every $y \in m (C)$, taking $x = \hat m (y)$, there is
  $\mu \in M$ such that $f_i (\hat m (y)) \leq \mu \leq \hat m (y)$, so $f'_i (y)
  \leq m (\mu) \leq m (\hat m (y))$.  Since $y \in m (C)$, $y$ must be of the
  form $m (z)$ for some $z\in C$, so $m (\hat m (y)) = m (\hat m (m
  (z))) = m (z) = y$, whence $f'_i (y) \leq m (\mu) \leq y$.  Clearly $m (M)$
  is finite, so $f'_i$ is finitely separted from the identity in $m
  (C)$.  Finally, since $m$ is continuous, the least upper bound of
  the family ${(f'_i)}_{i\in I}$ is the restriction of $m \circ \hat m$ to
  $m (C)$, which is the identity on $m (C)$.  So $m (C)$ is an
  FS-domain.  \qed
\end{proof}

The critical condition to apply our construction is that the $\mathcal
Q$ functor preserves pseudoepis (here, epis).  This property obtains
in the present case by the following lemma.
\begin{lemma}
  \label{lemma:Q:epi}
  Let $e : \xymatrix@-5pt{A \arrepixy[r] & C}$ be epi.  Then $\mathcal
  Q (e)$ is epi.
\end{lemma}
\begin{proof}
  For any non-empty open subset $U$ of $C$, we claim that $\Box U$
  intersects the image of $\mathcal Q (e)$.  Since $e$ is epi, $U$
  intersects the image of $e$, so there is an element $x \in A$ with $e
  (x) \in U$.  Consider the compact saturated set $\uparrow x$ in $A$.  Then $\uparrow
  e (\uparrow x) \subseteq U$, since $U$ is upper.  But this means that $\mathcal Q
  (e) (\uparrow x) \in \Box U$.
  
  Since any open subset of $\mathcal Q$ is a union of basic opens of
  the form $\Box U$, the claim follows.  \qed
\end{proof}

\marginpar{I've stopped here for now. -- JGL}
%!!!

The subscone construction then applies to define binary logical
relations by taking $\catc$ the category of pairs of FS-domains,
$\catd$ the category of FS-domains, and $\funbar$ the product functor.
The monad morphism $\dist {(A_1, A_2)} : \mathcal Q (A_1 \times A_2) \to
\mathcal Q (A_1) \times \mathcal Q (A_2)$ is defined by $\dist {(A_1, A_2)}
(Q) = (\pi_1 (Q), \pi_2 (Q))$.  This is well-defined: since $\pi_1$ and
$\pi_2$ are continuous, $\pi_1 (Q)$ and $\pi_2 (Q)$ are compact, and they
are trivially upper.

Take any relation $S$ at type $\tau$, i.e., any regular mono $m :
\xymatrix@-5pt{S \arrmonoxy[r] & {\Eval \tau}_1 \times {\Eval \tau}_2}$; equivalently
take $S$ to be any inductive subset of ${\Eval \tau}_1 \times {\Eval \tau}_2$, and
$m$ the canonical inclusion, up to iso.  Then $\mathcal Q (m)$ maps
any compact upper subset $Q$ of $S$ to $\uparrow m (Q)$, i.e., to the least
upper subset $\uparrow Q$ containing $Q$ in ${\Eval \tau}_1 \times {\Eval \tau}_2$.
Applying $\dist {{\Eval \tau}_2, {\Eval \tau}_2}$ to $\uparrow Q$ produces $(\pi_1 (\uparrow Q),
\pi_2 (\uparrow Q)) = (\uparrow \pi_1 (Q), \uparrow \pi_2 (Q)) \in \mathcal Q ({\Eval \tau}_1) \times
\mathcal Q ({\Eval \tau}_2)$.  The lifted relation $\tS$ is the
subset of $\mathcal Q ({\Eval \tau}_1) \times \mathcal Q ({\Eval \tau}_2)$ defined as
the topological closure of the set $\{(Q_1, Q_2) | \exists Q \mbox{ compact
  upper subset of }S, Q_1 = \uparrow \pi_1 (Q), Q_2 = \uparrow \pi_2 (Q)\}$.

\begin{lemma}
  \label{lemma:tS:Smyth}
  $\tS$ is the set of pairs $(Q_1, Q_2)$ such that
  \begin{itemize}
  \item for every $x_1 \in Q_1$, there is $y_1 \in Q_1$ with $y_1 \leq x_1$
    and $y_2 \in Q_2$ such thath $(y_1, y_2) \in S$;
  \item for every $x_2 \in Q_2$, there is $y_2 \in Q_2$ with $y_2 \leq x_2$
    and $y_1 \in Q_1$ such thath $(y_1, y_2) \in S$.
  \end{itemize}
\end{lemma}


There is another epi-mono factorization system on $\Dcpo$.  The
relevant monos are just the monos, and the pseudoepis are the regular
epis (maps $e : A \to C$ such that $C$ equals the inductive closure of
$e (A)$, i.e., the smallest cpo containing $e (A)$).  It is tempting
to replay a similar construction as above to get another notion of
logical relation on FS-domains for the Smyth powerdomain monad, but
this fails.  The difficulty is that this factorization system on
$\Dcpo$ does not induce one on FS-domains; this is because the
inductive closure of $f (A)$ (which is only closed under repeated
formation of least upper bounds of directed subsets, but not under
taking smaller elements) may fail to be an FS-domain.


==> distr.tex <==

\section{Building Monad Morphisms from Adjunctions}
\label{distr.s}


It is often the case that we have a (strong) monad on $\catc$, and wish to
build another one on $\catd$ related to the latter by a monad morphism. The
following results are then of some help.

%The first deals with monads, the second with strengths.

Recall that, given two categories $\cal C$ and $\cal D$, a pair of functors $F
: {\cal C} \to {\cal D}$ and $U : {\cal D} \to {\cal C}$ is an {\em adjunction\/}
$F \dashv U$ if and only if there are natural transformations $\eta_. : . \to UF .$ (the
{\em unit\/} of the adjunction) and $\epsilon_. : FU . \to .$ (the {\em counit\/}) such
that $\epsilon_{F (A)} \circ F \eta_A = \identity {F (A)}$ and $U \epsilon_A \circ \eta_{U (A)} =
\identity {U (A)}$. $F$ is said to be {\em left adjoint\/} to $U$, $U$ is {\em
  right adjoint\/} to $F$.

Then any adjunction $F \dashv U$ gives rise to a monad $(UF, \eta_., U
\epsilon_{F .})$ on ${\cal C}$. Conversely, there are two standard ways of
retrieving an adjunction from a monad $(T, \eta, \mu)$ on ${\cal C}$, from
Eilenberg-Moore algebras, or from the Kleisli category of the monad.

\subsection{Eilenberg-Moore algebras.}  A {\em $T$-algebra\/} is a morphism
$\xymatrix@-5pt{T (A) \ar[r]^{s} & A}$, for some object $A$ of ${\cal C}$,
satisfying the commutativity conditions:
\begin{equation}
  \label{eq:Talg}
  \xymatrix@-5pt@R-10pt{
    & & &
    T^2 (A) \ar[ld]_{\mu_A} 
    \ar[d]^{T (s)} \\
    & T (A) \ar[d]^{s} & 
    T (A) \ar[d]^{s} & 
    T (A) \ar[d]^{s} \\
    A \ar[ru]^{\eta_A} 
    \ar[r]_{\identity{A}} & 
    A & 
    A & 
    A \ar@{=}[l]      %  ^{\identity{A}}
    }
\end{equation}
$A$ is called the {\em support\/} of the algebra, $s$ its {\em structure map}.
A morphism from $\xymatrix@-5pt{T (A) \ar[r]^{s} & A}$ to $\xymatrix@-5pt{T
  (B) \ar[r]^{u} & B}$ is a morphism $f : A \to B$ in $\catd$ that commutes
with structure maps, i.e., such that $f \circ s = u \circ T (f)$.
$T$-algebras together with these morphisms forms a category $\Talg T$.
  
Then $\AlgF T \dashv \AlgU T$ is an adjunction, where $\AlgU T : \Talg T \to
{\cal C}$ maps objects $\xymatrix@-5pt{T (A) \ar[r]^{s} & A}$ to $A$ and
morphisms $f$ from $\xymatrix@-5pt{T (A) \ar[r]^{s} & A}$ to $\xymatrix@-5pt{T
  (B) \ar[r]^{u} & B}$ to the underlying morphism $f$ from $A$ to $B$ in
${\cal C}$; and where $\AlgF T : {\cal C} \to \Talg T$ maps the object $A$ to
the $T$-algebra $\xymatrix@-5pt{T^2 (A) \ar[r]^{\mu_A} & T (A)}$, and the
morphisms $\xymatrix@-5pt{A \ar[r]^f & B}$ to $f$ seen as morphism from $\AlgF
T (A)$ to $\AlgF T (B)$.  The unit of the adjunction is $\eta$, while the
counit $\epsilon$ is given on each $T$-algebra $\xymatrix@-5pt{T (A)
  \ar[r]^{s} & A}$ as the morphism $s$ itself, from $\AlgF T \AlgU T
(\xymatrix@-5pt{T (A) \ar[r]^{s} & A}) = \xymatrix@-5pt{T^2 (A) \ar[r]^{\mu_A}
  & T (A)}$ to $\xymatrix@-5pt{T (A) \ar[r]^{s} & A}$.
  
Moreover, the monad of this adjunction is the original monad $(T, \eta, \mu)$.

\subsection{Kleisli category.}  The objects of $\Kleisli T$ are the objects of ${\cal
  C}$, while the morphisms $\xymatrix@-5pt{A \ar[r]^f & B}$ of $\Kleisli T$
are the morphisms $\xymatrix@-5pt{A \ar[r]^f & T (B)}$ of ${\cal C}$.  To
avoid confusion, we write $\overline f$ the morphisms $f$ seen as a morphism
in $\Kleisli T$.  The identity $\overline {\identity A}$ on the object $A$ in
$\Kleisli T$ is $\eta_A$, while composition $\overline g \circ \overline f$ is
$\overline {\mu_C \circ T (g) \circ f}$, where $\xymatrix@-5pt{A \ar[r]^f & T
  (B)}$ and $\xymatrix@-5pt{B \ar[r]^g & T (C)}$ in ${\cal C}$.
  
Define $\KlF T : {\cal C} \to \Kleisli T$ as mapping the object $A$ to $A$,
and the morphism $\xymatrix@-5pt{A \ar[r]^f & B}$ to the morphism from $A$ to
$B$ in $\Kleisli T$ defined as $\eta_B \circ f$.  Define $\KlU T : \Kleisli T
\to {\cal C}$ as mapping the object $A$ to $T (A)$, and the morphism
$\overline f$ from $A$ to $B$ in $\Kleisli T$ to $\mu_B \circ T (f)$.  Then
$\KlF T \dashv \KlU T$ is an adjunction, whose unit is $\eta$, and whose
counit $\epsilon$ is the identity morphism from $\KlF T \KlU T (A)$ to $T (A)$
in $\cal C$, seen as a morphism from $\KlF T \KlU T (A)$ to $A$ in $\Kleisli
T$.  The monad of $\KlF T \dashv \KlU T$ is again $(T, \eta, \mu)$.


\subsection{Monad Morphisms from Adjunctions}
\label{distr.s.notstrong}



\begin{proposition}
  \label{prop:adj:distr:1}
  Let $(\tc{}, \unitc{}, \multc{})$ be a monad on a category $\catc$, $\funbar
  : \catc \to \catd$ be a functor with a left adjoint $\discr : \catd \to
  \catc$.  Let $\counita_A : \discr {\funbara A} \to A$ be the counit of the
  adjunction, $\unita_E : E \to \funbara {\discr (E)}$ be the unit of the
  adjunction.
  
  Define $\td {} = \funbar \circ \tc{} \circ \discr = \funbara {\tc \discr}$,
  $\unitd E = \funbara {\unitc {\discr (E)}} \circ \unita_E$, $\multd E =
  \funbara {\multc {\discr (E)} \circ \tc {\counita_{\tc {\discr (E)}}}}$.
  Finally, let $\dist A = \funbara {\tc {\counita_A}} : \td {\funbara A} \to
  \funbara {\tc A}$.  Then $(\td {}, \unitd{}, \multd{})$ is a monad on
  $\catd$ and $(\funbar, \dist {})$ is a monad morphism from $\tc$ to $\td$.
\end{proposition}
\begin{proof*}
  Let $F \dashv U$ be any adjunction generating the monad, i.e., such that $UF
  = \tc{}$, whose unit is $\unitc{}$, and whose counit $\epsilon$ is such that
  $\multc{} = U \epsilon_F$.  We may choose, e.g., $\AlgF T \dashv \AlgU T$ or
  $\KlF T \dashv \KlU T$.  Compose the adjunction $\discr \dashv \funbar$ with
  $F \dashv U$, yielding an adjunction $F \discr \dashv \funbara {U}$.  The
  unit of this adjunction (on object $E$) is $\funbara {\unitc {\discr (E)}}
  \circ \unita_E$, its counit (on object $A$) is $\epsilon_A \circ F
  (\counita_{U A})$.
  
  The monad of this adjunction is $(\funbara {U F \discr}, \funbara {\unitc
    {\discr (.)}}  \circ \unita_., \funbara {U ( \epsilon_{F \discr (.)} \circ
    F (\counita_{UF \discr (.)}))})$.  But the monad of $F \dashv U$ is $(\tc,
  \unitc{}, \multc{})$, so $U F = \tc$ and $\multc{} = U \epsilon_{F}$.  It
  follows that the monad of $F \discr \dashv \funbara {U}$ is $(\funbara {\tc
    \discr}, \funbara {\unitc {\discr (.)}}  \circ \unita_., \funbara {\multc
    {\discr (.)}  \circ \tc (\counita_{\tc \discr (.)})})$.  This is $(\td,
  \unitd{}, \multd{})$, which is therefore a monad.
  

%  As a composition of functors, $\td{}$ is a functor.  As compositions of
%  natural constructions, $\unitd E$ and $\multd E$ are natural in $E$.
%  Similarly, $\dist A$ is natural in $A$.
  
%  \noindent
%  \begin{minipage}{4cm}
%    Recall (\cite{McLane:cat:math}, IV.1) that the adjunction $\discr \vdash
%    \funbar$ is witnessed by the fact that the following diagrams commute:
%  \end{minipage}
%  \begin{minipage}{8cm}
%    \begin{equation}
%      \label{eq:unita}
%      \xymatrix{
%        \discr (E)
%        \ar[r]^{\discr (\unita_E)}
%        \ar[rd]_{\identity {\discr (E)}}
%        & \discr \funbara {\discr (E)}
%        \ar[d]^{\counita_{\discr (E)}}
%        \\
%        & \discr (E)
%        }
%      \quad
%      \xymatrix{
%        \funbara A
%        \ar[d]_{\unita_{\funbara A}}
%        \ar[rd]^{\identity {\funbara A}}
%        \\
%        \funbara {\discr \funbara A}
%        \ar[r]_{\funbara {\counita_A}}
%        & \funbara A
%        }
%    \end{equation}
%  \end{minipage}

%  Checking left and right unit for the monad is done by considering the
%  following diagram.  The top right square commutes by naturality of $\funbara
%  {\tc {\counita}}$, the top left triangles commute by (\ref{eq:unita}), the
%  bottom right triangles commute because $\unitc{}$ is the unit of $(\tc{},
%  \unitc{}, \multc{})$, the bottom left square commutes by naturality of
%  $\funbara {\unitc{}}$.

%  \noindent
%  \begin{minipage}{3.8cm}
%    So $\multd E$ (rightmost vertical path) composed with $\td {\unitd E}$
%    (topmost horizontal path) and $\multd E$ (bottommost horizontal path)
%    composed with $\unitd {\td E}$ (leftmost vertical path) are both equal to
%    the identity (the diagonal path).
%  \end{minipage}
%  \begin{minipage}{8.2cm}
%    \small
%    \[
%    \xymatrix{
%      \funbara {\tc {\discr (E)}} %\td E
%                                %    \ar@/^2pc/[rr]^{\td {\unitd E}}
%                                %    \ar@/_4pc/[dd]_{\unitd {\td E}}
%      \ar[r]^{\td {\unita_E}}
%      \ar[rd]^{\identity {\funbara {\td {\discr (E)}}}}
%      \ar[d]_{\unita_{\td E}}
%      & \funbara{\tc {\discr \funbara {\discr (E)}}}
%      \ar[r]^{\td {\funbara {\unitc {\discr (E)}}}=}_{\funbara{\tc {\discr \funbara {\unitc {\discr (E)}}}}}
%      \ar[d]^{\funbara{\tc {\counita_{\discr (E)}}}}
%      & \funbara{\tc {\discr \funbara {\tc {\discr (E)}}}}
%      \ar[d]|{\funbara{\tc {\counita_{\tc {\discr (E)}}}}}
%                                %    \ar@/^4pc/[dd]^{\multd E}
%      \\
%      \funbara {\discr \funbara{\tc {\discr (E)}}}
%      \ar[r]^{\funbara {\counita_{\tc {\discr (E)}}}}
%      \ar[d]_{\funbara {\unitc {\discr (\td E)}}=}^{\funbara {\unitc {\discr
%            \funbara {\tc {\discr (E)}}}}}
%      & \funbara{\tc {\discr (E)}}
%      \ar[r]^{\funbara{\tc{\unitc{\discr (E)}}}}
%      \ar[rd]^{\identity {\funbara {\td {\discr (E)}}}}
%      \ar[d]^{\funbara {\unitc {\tc {\discr (E)}}}}
%      & \funbara {\tc {\tc {\discr (E)}}}
%      \ar[d]|{\funbara {\multc{\discr (E)}}}
%      \\
%      \funbara {\tc {\discr \funbara {\tc \discr (E)}}}
%      \ar[r]_{\funbara {\tc {\counita_{\tc {\discr (E)}}}}}
%                                %    \ar@/_2pc/[rr]_{\multd E}
%      & \funbara {\tc {\tc {\discr (E)}}}
%      \ar[r]_{\funbara {\multc {\discr (E)}}}
%      & \funbara {\tc {\discr (E)}}
%      \\
%      }
%    \]
%  \end{minipage}
  
%  Associativity of $\multd{}$ follows from the following diagram.  The
%  left-hand rectangle is by naturality of $\funbara {\tc \counita}$, the top
%  right square is by naturality of $\funbara {\multc {}}$, the bottom right
%  square is by associativity of $\multd{}$.  Taking the two outer walks from
%  the top left to the bottom right corner yields associativity $\multd E \circ
%  \multd {\td E} = \multd E \circ \td {\multd E}$.

%  \noindent
%  \begin{minipage}{3cm}
%    Indeed, the topmost horizontal path is $\multd {\td E}$, the leftmost
%    vertical path is $\td {\multd E}$, while the bottommost and rightmost
%    paths are $\multd E$.
%  \end{minipage}
%  \begin{minipage}{9cm}
%    \small
%    \[
%    \xymatrix{
%      \funbara {\tc {\discr \funbara {\tc \discr {\funbara {\tc \discr (E)}}}}}
%      \ar[r]^{\funbara {\tc {\counita_{\tc {\discr {\funbara {\tc {\discr
%                      (E)}}}}}}}}
%      \ar[d]^{\funbara {\tc {\discr {\funbara {\tc \counita_{\tc {\discr
%                    (E)}}}}}}}
%      & \funbara{\tc {\tc {\discr {\funbara {\tc {\discr (E)}}}}}}
%      \ar[r]^{\funbara {\multc {\discr {\funbara {\tc {\discr (E)}}}}}}
%      \ar[d]^{\funbara {\tc {\tc {\counita_{\tc {\discr (E)}}}}}}
%      & \funbara{\tc {\discr {\funbara {\tc {\discr (E)}}}}}
%      \ar[d]|{\funbara {\tc {\counita_{\tc {\discr (E)}}}}}
%      \\
%      \funbara{\tc {\discr {\funbara {\tc {\tc {\discr (E)}}}}}}
%      \ar[d]^{\funbara {\tc {\discr {\funbara {\multc {\discr (E)}}}}}}
%      & \funbara {\tc {\tc {\tc {\discr (E)}}}}
%      \ar[r]^{\funbara {\multc {\tc {\discr (E)}}}}
%      \ar[d]^{\funbara {\tc {\multc {\discr (E)}}}}
%      & \funbara {\tc {\tc {\discr (E)}}}
%      \ar[d]|{\funbara {\multc {\discr (E)}}}
%      \\
%      \funbara {\tc {\discr {\funbara {\tc {\discr (E)}}}}}
%      \ar[r]^{\funbara {\tc {\counita_{\tc {\discr (E)}}}}}
%      & \funbara {\tc {\tc {\discr (E)}}}
%      \ar[r]^{\funbara {\multc {\discr (E)}}}
%      & \funbara {\tc {\discr (E)}}
%      }
%    \]
%  \end{minipage}  
  
  It remains to show that $\dist{} = \funbara {\tc {\counita}}$ is a monad
  morphism from $\tc$ to $\td$.  This is checked using the following diagrams.
  In the left diagram, the top triangle is one of the adjunction laws, the
  bottom square is by naturality of $\funbara {\unitc {}}$; so $\dist A$
  (bottom arrow) composed with $\unitd {\funbara A}$ (leftmost vertical path)
  equals $\funbara {\unitc A}$ (rightmost path from $\funbara A$ to $\funbara
  {\tc A}$).

  \noindent
  \begin{minipage}{4cm}
    In the right diagram, the top square is by naturality of $\funbara {\tc
      \counita}$, the bottom square is by naturality of $\funbara {\multc
      {}}$, so $\dist A$ (bottom arrow) composed with $\multd {\funbara A}$
    (leftmost vertical path) equals $\funbara {\multc A} \circ \dist {\tc A} \circ \td
    {\dist A}$ (the other path from top left to bottom right).  \qed
  \end{minipage}
  \begin{minipage}{8.2cm}
  {\small
    \[
    \xymatrix{
      {\funbara A}
      \ar[d]_{\unita_{\funbara A}}
      \ar[rd]|{\identity {\funbara A}} \\
      {\funbara {\discr {\funbara A}}}
      \ar[r]_{\funbara {\counita_A}}
      \ar[d]_{\funbara {\unitc {\discr {\funbara A}}}}
      &
      {\funbara A}
      \ar[d]_{\funbara {\unitc A}}
      \\
      {\funbara {\tc {\discr \funbara A}}}
      \ar[r]_{\funbara {\tc {\counita_A}}}
      &
      {\funbara {\tc A}}
      }
    %\quad
    \xymatrix{
      {\funbara {\tc {\discr \funbara {\tc {\discr {\funbara A}}}}}}
      \ar[r]^{\funbara {\tc {\discr \funbara {\tc \counita_A}}}}
      \ar[d]_{\funbara {\tc {\counita_{\tc {\discr {\funbara A}}}}}}
      &
      {\funbara {\tc {\discr {\funbara {\tc A}}}}}
      \ar[d]|{\funbara {\tc {\counita_{\tc A}}}}
      \\
      {\funbara {\tc {\tc {\discr {\funbara A}}}}}
      \ar[r]^{\funbara {\tc {\tc \counita_A}}}
      \ar[d]_{\funbara {\multc {\discr {\funbara A}}}}
      &
      {\funbara {\tc {\tc A}}}
      \ar[d]|{\funbara {\multc A}}
      \\
      {\funbara {\tc {\discr {\funbara A}}}}
      \ar[r]_{\funbara {\tc {\counita_A}}}
      &
      {\funbara {\tc A}}
      }
    \]
    }
  \end{minipage}
\end{proof*}

%The proof goes through Eilenberg-Moore algebras.  One might instead use the
%adjunction $\KlF \tc \dashv \KlU \tc$, going through the Kleisli category, or
%we might use any other adjunction $F \dashv U$ whose monad is $(\tc, \unitc{},
%\multc{})$; we let the reader check that the construction of the proof above
%is independent of the adjunction $F \dashv U$, provided its monad is $(\tc,
%\unitc{}, \multc{})$.
Note that we could have checked the required diagrams directly; the proof
would be longer than going through adjunctions, as we did.



\subsection{Monoidal, and Strong Monad Morphisms from Monoidal Adjunctions}
\label{distr.s.monoidal}


We first reproduce the argument of Proposition~\ref{prop:adj:distr:1} in the
monoidal case.  While monads correspond to adjunctions in well-defined ways,
only {\em monoidal\/} monads can be linked to so-called {\em monoidal\/}
adjunctions.  This is the reason why we deal with monoidal monads first.

Let $({\cal C}, I^{\cal C}, \otimes^{\cal C}, \alpha^{\cal C}, \ell^{\cal C},
r^{\cal C})$ and $({\cal D}, I^{\cal D}, \otimes^{\cal D}, \alpha^{\cal D},
\ell^{\cal D}, r^{\cal D})$ be two monoidal categories. Let $F \dashv U$ be an
adjunction, where $F : {\cal C} \to {\cal D}$, $U : {\cal D} \to {\cal C}$,
with unit $\eta$, and counit $\epsilon$.  This is a {\em monoidal
  adjunction\/} if and only if $F$ and $U$ are monoidal functors (with
respective mediating pairs $(\theta^F, \iota^F)$ and $(\theta^U, \iota^U)$),
and the unit $\eta$ and the counit $\epsilon$ are {\em monoidal natural
  transformations}, by which we mean that the following diagrams commute:


\noindent
\begin{minipage}{4.5cm}
  \begin{equation}
    \label{eq:moneta:I}
    \xymatrix{
      I^{\cal C} \ar[r]^{\iota^U}
      \ar[rd]_{\eta_{I^{\cal C}}}
      & U (I^{\cal D}) \ar[d]^{U (\iota^F)}
      \\
      & UF (I^{\cal C})
      }
  \end{equation}
\end{minipage}
\begin{minipage}{7.5cm}
  \begin{equation}
    \label{eq:moneta:tensor}
    \xymatrix@C-55pt@R-10pt{
      A \otimes^{\cal C} B
      \ar[rr]^(.4){\eta_A \otimes^{\cal C} \eta_B}
      \ar[dd]_{\eta_{A \otimes^{\cal C} B}}
      &&
      UF (A) \otimes^{\cal C} UF (B)
      \ar[ld]^(.3){\theta^U_{F(A), F(B)}}
      \\
      & \ \ \ \ \ U (F (A) \otimes^{\cal D} F (B))
      \ar[ld]^(.3){U (\theta^F_{A, B})} &
      \\
      UF (A \otimes^{\cal C} B)
      &&
      }
  \end{equation}
\end{minipage}

\noindent
\begin{minipage}{4.5cm}
  \begin{equation}
    \label{eq:moneps:I}
    \xymatrix@C-10pt{
      I^{\cal D}
      \ar[d]_{\iota^F}
      &
      \\
      F (I^{\cal C})
      \ar[r]_{F (\iota^U)}
      &
      FU (I^{\cal D})
      \ar[lu]_{\epsilon_{I^{\cal D}}}
      }
  \end{equation}
\end{minipage}
\begin{minipage}{7.5cm}
  \begin{equation}
    \label{eq:moneps:tensor}
    \xymatrix@C-55pt@R-10pt{
      &&
      FU (A) \otimes^{\cal D} FU (B)
      \ar[ld]_(.7){\theta^F_{U (A), U (B)}}
      \ar[dd]^{\epsilon_A \otimes^{\cal D} \epsilon_B}
      \\
      &
      F (U (A) \otimes^{\cal C} U (B))
      \ar[ld]_(.7){F \theta^U_{A, B}}
      &
      \\
      FU (A \otimes^{\cal D} B)
      \ar[rr]_{\epsilon_{A \otimes^{\cal D} B}}
      &&
      A \otimes^{\cal D} B
      }
  \end{equation}
\end{minipage}


The value of monoidal adjunctions is their relation with monoidal monads
(Section~\ref{strong.s:monoidal}).  Recall that a monoidal monad on $\cal C$
is a tuple $(T, \eta, \mu, d)$, where $(T, \eta, \mu)$ is a monad on $\cal C$
and $d_{A, B}$ is a natural transformation from $T A \otimes^{\cal C} T B$ to
$T (A \otimes^{\cal C} B)$ such that the following diagrams commute:

\noindent
\begin{minipage}{6cm}
  \[
  \xymatrix@R-12pt{
    I^{\cal C} \otimes^{\cal C} T B
    \ar[rdd]^{\ell^{\cal C}_{T B}}
    \ar[d]_{\eta_{I^{\cal C}} \otimes^{\cal C} \identity {T B}}
    &
    \\
    T I^{\cal C} \otimes^{\cal C} T B
    \ar[d]_{d_{I^{\cal C}, B}}
    &
    \\
    T (I^{\cal C} \otimes^{\cal C} B)
    \ar[r]_(0.7){T \ell^{\cal C}_B}
    &
    T B
    }
  (\ref{eq:monoidal:l})
  \]
\end{minipage}
\begin{minipage}{6cm}
  \[
  \xymatrix@R-12pt{
    T A \otimes^{\cal C} I^{\cal C}
    \ar[rdd]^{r^{\cal C}_{T A}}
    \ar[d]_{\identity {T A} \otimes^{\cal C} \eta_{I^{\cal C}}}
    &
    \\
    T A \otimes^{\cal C} T I^{\cal C}
    \ar[d]_{d_{A, I^{\cal C}}}
    &
    \\
    T (A \otimes^{\cal C} I^{\cal C})
    \ar[r]_(0.7){T r^{\cal C}_A}
    &
    T A
    }
  (\ref{eq:monoidal:r})
  \]
\end{minipage}

\noindent
\[
\xymatrix@R-10pt{
  A \otimes^{\cal C} B
  \ar[r]^{\eta_A \otimes^{\cal C} \eta_B}
  \ar[rd]_{\eta_{A \otimes^{\cal C} B}}
  &
  T A \otimes^{\cal C} T B
  \ar[d]^{d_{A, B}}
  \\
  &
  T (A \otimes^{\cal C} B)
  }
\qquad
(\ref{eq:monoidal:eta})
\]

\noindent
\[
\xymatrix@R-5pt{
  (T A \otimes^{\cal C} T B) \otimes^{\cal C} T C
  \ar[d]^{\alpha^{\cal C}_{T A, T B, T C}}
  \ar[r]^{d_{A, B} \otimes^{\cal C} \identity {T C}}
  &
  T (A \otimes^{\cal C} B) \otimes^{\cal C} T C
  \ar[r]^{d_{A \otimes^{\cal C} B, C}}
  &
  T ((A \otimes^{\cal C} B) \otimes^{\cal C} C)
  \ar[d]^{T \alpha^{\cal C}_{A, B, C}}
  \\
  T A \otimes^{\cal C} (T B \otimes^{\cal C} T C)
  \ar[r]_{\identity {T A} \otimes^{\cal C} d_{B, C}}
  &
  T A \otimes^{\cal C} T (B \otimes^{\cal C} C)
  \ar[r]_{d_{A, B \otimes^{\cal C} C}}
  &
  T (A \otimes^{\cal C} (B \otimes^{\cal C} C))
  }
\ (\ref{eq:monoidal:double})
\]

\noindent
\[
\xymatrix@R-5pt{
  T^2 A \otimes^{\cal C} T^2 B
  \ar[r]^{d_{T A, T B}}
  \ar[d]_{\mu_A \otimes^{\cal C} \mu_B}
  &
  T (T A \otimes^{\cal C} T B)
  \ar[r]^{T d_{A, B}}
  &
  T^2 (A \otimes^{\cal C} B)
  \ar[d]^{\mu_{A \otimes^{\cal C} B}}
  \\
  T A \otimes^{\cal C} T B
  \ar[rr]_{d_{A, B}}
  &
  &
  T (A \otimes^{\cal C} B)
  }
\qquad (\ref{eq:monoidal:mu})
\]

%Observe that for any monoidal category $({\cal C},
%I^{\cal C}, \otimes^{\cal C}, \alpha^{\cal C}, \ell^{\cal C}, r^{\cal C})$,
%its {\em dual\/} $({\cal C}, I^{\cal C}, \otimes^{{\cal C}\;op}, {\alpha^{\cal
%    C}}^{-1}, r^{\cal C}, \ell^{\cal C})$ is also a monoidal category, where
%$A \otimes^{{\cal C}\;op} B = B \otimes^{\cal C} A$.  Given a monad $T$ on
%$\cal C$, call a {\em dual strength\/} any monad strength with respect to the
%dual monoidal category.  In other words, a dual strength is a natural
%transformation $t'_{A, B} : TA \otimes^{\cal C} B \to T (A \otimes^{\cal C}
%B)$ obeying the obvious duals of the strength laws (\ref{eq:strong:l}),
%(\ref{eq:strong:eta}), (\ref{eq:strong:double}), (\ref{eq:strong:mu}).

%Then, a tuple $(T, \eta, \mu, t, t')$ is a {\em monoidal monad\/} on $\cal C$
%if and only if $(T, \eta, \mu)$ is a monad on $\cal C$, $t$ is a strength,
%$t'$ a dual strength, and the following diagram commutes:
%\begin{equation}
%  \label{eq:monoidal}
%  \xymatrix{
%    T A \otimes^{\cal C} T B
%    \ar[rr]^{t_{T A, B}}
%    \ar[dd]_{t'_{A, T B}}
%    &&
%    T (T A \otimes^{\cal C} B)
%    \ar[d]^{T t'_{A, B}}
%    \\
%    &&
%    T^2 (A \otimes^{\cal C} B)
%    \ar[d]^{\mu_{A \otimes^{\cal C} B}}
%    \\
%    T (A \otimes^{\cal C} T B)
%    \ar[r]_{T t_{A, B}}
%    &
%    T^2 (A \otimes^{\cal C} B)
%    \ar[r]_{\mu_{A \otimes^{\cal C} B}}
%    &
%    T (A \otimes^{\cal C} B)
%    }
%\end{equation}
%Call $d_{A, B}$ the common diagonal.  It is easy to check that $t_{A, B} =
%d_{A, B} \circ (\eta_A \otimes^{\cal C} \identity {T B})$, and $t'_{A, B} =
%d_{A, B} \circ (\identity {T A} \otimes^{\cal C} \eta_B)$.  (This uses
%Diagram~(\ref{eq:strong:eta}), the fact that $\eta$ is natural, and $\mu_{A
%  \otimes^{\cal C} B} \circ \eta_{T (A \otimes^{\cal C} B)} = \identity {A
%  \otimes^{\cal C} B}$.)  Therefore, monoidal monads could also be
%characterized as those tuples $(T, \eta, \mu, d)$, where $(T, \eta, \mu)$ is a
%monad and $d_{A, B}$ is a natural transformation (the {\em mediator\/}) from
%$T A \otimes^{\cal C} T B$ to $T (A \otimes^{\cal C} B)$ such that $t = d
%\circ (\eta \otimes^{\cal C} \identity {})$ is a strength and $t' = d \circ
%(\identity {} \otimes^{\cal C} \eta)$ is a dual strength.

%Monoidal monads are related to the more well-known notion of a commutative
%monad: on a {\em symmetric\/} monoidal closed category $({\cal C}, I^{\cal C},
%\otimes^{\cal C}, \alpha^{\cal C}, \ell^{\cal C}, r^{\cal C}, c^{\cal C})$,
%each monad strength $t$ gives rise to a dual strength $t' = T c^{\cal C} \circ
%t \circ c^{\cal C}$.  Then a strong monad $(T, \eta, \mu, t)$ is a {\em
%  commutative monad\/} if and only if $(T, \eta, \mu, t, t')$ is monoidal.

The following lemmas show respectively that every monoidal adjunction gives
rise to a monoidal monad, that every monoidal monad yields a monoidal
adjunction between the base category and the Kleisli category of the monad,
and that monoidal adjunctions compose to yield monoidal adjunctions.  Except
for the first, the arguments are tedious computations, and therefore relegated
to appendices\footnote{These results are folklore, and were confirmed in
  discussions with Paul-Andr\'e Melli\`es, Fran\c cois Lamarche, and Albert Burroni
  notably.  However, we have been unable to find references on this.  We have
  often been directed to the pioneering paper \cite{Street:monads}, but could
  not find the expected results therein.}.

\begin{lemma}
  \label{lemma:unitmon->monoidal}
  Let $F \dashv U$ be a monoidal adjunction, with unit $\eta$ and counit
  $\epsilon$, where $F : {\cal C} \to {\cal D}$, $U : {\cal D} \to {\cal C}$.
  Let $T$ be $UF$, $\mu_A$ be $U \epsilon_{F (A)}$, and $d_{A, B}$ be $U
  \theta^F_{A, B} \circ \theta^U_{F(A), F(B)}$.
% { \small
%    \[
%    \xymatrix@+20pt{
%%      A \otimes^{\cal C} UF (B)
%%      \ar[r]^{\eta_A \otimes^{\cal C} \identity {UF (B)}}
%      %&
%      UF (A) \otimes^{\cal C} UF (B)
%      \ar[r]^{\theta^U_{F(A), F(B)}}
%      & U (F(A) \otimes^{\cal D} F(B))
%      \ar[r]^{U \theta^F_{A, B}}
%      & UF (A \otimes^{\cal C} B)
%      }
%    \]
%    }
%  Let $t_{A, B} = d_{A, B} \circ (\eta_A \otimes^{\cal C} \identity {T
%    B})$, and $t'_{A, B} = d_{A, B} \circ (\identity {T A} \otimes^{\cal C}
%  \eta_B)$.

  Then $(T, \eta, \mu, d)$ is a monoidal monad on $\cal C$.
\end{lemma}
\begin{proof}
  $(T, \eta, \mu)$ is a monad by Proposition~\ref{prop:adj:distr:1}.  We check
  the mediator laws (\ref{eq:monoidal:l}), (\ref{eq:monoidal:r}),
  (\ref{eq:monoidal:eta}), (\ref{eq:monoidal:double}), (\ref{eq:monoidal:mu})
  for $d$.
  
  \paragraph{Diagram~(\ref{eq:monoidal:l})} is obtained by considering the following
  diagram.  The top left triangle is a copy of (\ref{eq:moneta:I}), tensored
  by $UF (B)$ on the right.  The square next to it on its right is a
  naturality square for $\theta^U$.  The next trapezoid on the right (the
  top right trapezoid) is $U$ applied to a coherence square
  (\ref{eq:theta:coh:l}) for $\theta^F$, $\ell^{\cal C}$ and $\ell^{\cal D}$.
  The bottom face, atop the curved arrow $\ell^{\cal C}_{UF (B)}$, is another
  instance of a coherence square (\ref{eq:theta:coh:l}) for $\theta^F$,
  $\ell^{\cal C}$ and $\ell^{\cal D}$.  {\small
    \[
    \xymatrix@R-10pt{
      I^{\cal C} \otimes^{\cal C} UF (B)
      \ar[r]^{\eta_{I^{\cal C}} \otimes^{\cal C} \identity {UF (B)}}
      \ar[rd]|{\iota^U \otimes^{\cal C} \identity {UF (B)}}
      \ar@/_35pt/[ddrrr]^{\ell^{\cal C}_{UF (B)}}
      &
      UF (I^{\cal C}) \otimes^{\cal C} UF (B)
      \ar[r]^{\theta^U_{F (I^{\cal C}), F (B)}}
      &
      U (F (I^{\cal C}) \otimes^{\cal D} F (B))
      \ar[r]^{U (\theta^F_{I^{\cal C}, B})}
      &
      UF (I^{\cal C} \otimes^{\cal C} B)
      \ar[dd]_{UF (\ell^{\cal C}_{B})}
      \\
      &
      U (I^{\cal D}) \otimes^{\cal C} UF (B)
      \ar[u]_{U (\iota^F) \otimes^{\cal C} \identity {UF (B)}}
      \ar[r]_{\theta^U_{I^{\cal D}, F (B)}}
      &
      U (I^{\cal D} \otimes^{\cal D} F (B))
      \ar[u]_{U (\iota^F \otimes^{\cal D} \identity {F (B)})}
      \ar[rd]_{U (\ell^{\cal D}_{F (B)})}
      &
      \\
      &&&
      UF (B)
      }
    \]
    } Now the topmost composition of arrows is $t_{I^{\cal C}, B}$, the
  bottommost arrow from $I^{\cal C} \otimes^{\cal C} UF (B)$ to $UF (B)$ is
  $\ell^{\cal C}_{T B}$, and the rightmost vertical arrow is $T \ell^{\cal
    C}_B$.

  \paragraph{Diagram~(\ref{eq:monoidal:r}).}  This is checked by similar
  arguments, replacing the coherence square (\ref{eq:theta:coh:l}) by
  (\ref{eq:theta:coh:r}).

  \noindent
  \begin{minipage}{5.5cm}
    \paragraph{Diagram~(\ref{eq:monoidal:eta}).}
    This is the diagram on the right, an instance of
    Diagram~(\ref{eq:moneta:tensor}), stating that $\eta$ is a monoidal
    natural transformation.  We recognize $d_{A, B}$ as the rightmost
    composition of vertical arrows, hence the desired
    Diagram~(\ref{eq:strong:eta}).
  \end{minipage}
  \begin{minipage}{6.5cm}
    {\small
      \[
      \xymatrix@R-10pt{
        A \otimes^{\cal C} B
        \ar[r]^{\eta_A \otimes^{\cal C} \eta_B}
        \ar[rdd]_{\eta_{A \otimes^{\cal C} B}}
        &
        UF (A) \otimes^{\cal C} UF (B)
        \ar[d]^{\theta^U (F (A), F (B))}
        \\
        & U (F (A) \otimes^{\cal D} F (B))
        \ar[d]^{U \theta^F_{A, B}}
        \\
        & UF (A \otimes^{\cal C} B)
        }
      \]
      }
  \end{minipage}

  \noindent
  \paragraph{Diagram~(\ref{eq:monoidal:double}).}
  For space reasons, we flip the diagram so that arrows involving strengths
  are vertical, and arrows involving associativities are horizontal.  Also, we
  drop most subscripts, which are inferrable from context.  {\small
    \[
    \xymatrix@R-15pt@C-5pt{
      {\hbox{$
          \begin{array}{c}
            (UF(A) \otimes^{\cal C} UF (B))\\ \otimes^{\cal C} UF (C)
          \end{array}
          $}}
      \ar[rrr]^{\alpha^{\cal C}}
      \ar[d]_{\theta^U \otimes^{\cal C} \identity {UF (C)}}
      \ar@{}[rrrdd]|{\txt{(coherence (\ref{eq:theta:coh:alpha}) for $\theta^U$)}}
      &&&
      {\hbox{$
          \begin{array}{c}
            UF (A) \otimes^{\cal C}\\ (UF (B) \otimes^{\cal C} UF (C))
          \end{array}
          $}}
      \ar[d]^{\identity {UF (A)} \otimes^{\cal C} \theta^U}
      \\
      {\hbox{$
          \begin{array}{c}
            U (F (A) \otimes^{\cal D} F (B))\\ \otimes^{\cal C} UF (C)
          \end{array}
          $}}
      \ar[rd]^{\theta^U}
      \ar[d]_{U \theta^F \otimes^{\cal C} \identity {UF (C)}}
      &&&
      {\hbox{$
          \begin{array}{c}
            UF (A) \otimes^{\cal C}\\ U (F (B) \otimes^{\cal D} F (C))
          \end{array}
          $}}
      \ar[ld]_{\theta^U}
      \ar[d]^{\identity {UF (A)} \otimes^{\cal C} U \theta^F}
      \\
      {\hbox{$
          \begin{array}{c}
            UF (A \otimes^{\cal C} B)\\ \otimes^{\cal C} UF (C)
          \end{array}
          $}}
      \ar[d]_{\theta^U}
      \ar@{}[r]|{\txt{(natur-\\ality of\\$\theta^U$)}}
      \ar@{}[rrrdd]|{\txt{($U$ applied to coherence (\ref{eq:theta:coh:alpha}) for $\theta^F$)}}
      &
      {\hbox{$
          \begin{array}{c}
            U ((F (A)\\ \otimes^{\cal D} F (B))\\ \otimes^{\cal D} F (C))
          \end{array}
          $}}
      \ar[r]^{U \alpha^{\cal D}}
      \ar[ld]^{U (\theta^F \otimes^{\cal D} \identity {F (C)})}
      &
      {\hbox{$
          \begin{array}{c}
            U (F (A) \otimes^{\cal D}\\ (F (B) \otimes^{\cal D}\\ F (C)))
          \end{array}
          $}}
      \ar[rd]_{U (\identity {F (A)} \otimes^{\cal D} \theta^F)}
      \ar@{}[r]|{\txt{(natur-\\ality of\\$\theta^U$)}}
      &
      {\hbox{$
          \begin{array}{c}
            UF (A) \otimes^{\cal C}\\ UF (B \otimes^{\cal C} C)
          \end{array}
          $}}
      \ar[d]^{\theta^U}
      \\
      {\hbox{$
          \begin{array}{c}
            U (F (A \otimes^{\cal C} B)\\ \otimes^{\cal D} F (C))
          \end{array}
          $}}
      \ar[d]_{U \theta^F}
      &&&
      {\hbox{$
          \begin{array}{c}
            U (F (A) \otimes^{\cal D}\\ F (B \otimes^{\cal C} C))
          \end{array}
          $}}
      \ar[d]^{U \theta^F}
      \\
      {\hbox{$
          \begin{array}{c}
            UF ((A \otimes^{\cal C} B)\\ \otimes^{\cal C} C)
          \end{array}
          $}}
      \ar[rrr]_{UF \alpha^{\cal C}}
      &&&
      {\hbox{$
          \begin{array}{c}
            UF (A \otimes^{\cal C}\\ (B \otimes^{\cal C} C))
          \end{array}
          $}}
      }
    \]
    } The vertical arrows on the left compose to form $d_{A \otimes^{\cal C}
    B, C} \circ (d_{A, B} \otimes^{\cal C} \identity {UF (C)})$, while the
  vertical arrows on the right compose to form $d_{A \otimes^{\cal C} B, C}
  \circ (\identity {UF (A)} \otimes^{\cal C} d_{B, C})$, whence the result.

  \paragraph{Diagram~(\ref{eq:monoidal:mu}).}  Similarly, we flip the diagram so
  that vertical arrows become horizontal and conversely: {\small
    \[
    \xymatrix@C+80pt@R-15pt{
      UFUF (A) \otimes^{\cal C} UFUF (B)
      \ar[r]^{U \epsilon_{F (A)} \otimes^{\cal C} U \epsilon_{F (B)}}
      \ar[d]_{\theta^U}
      \ar@{}[rdd]|{\txt{(naturality of $\theta^U$)}}
      &
      UF (A) \otimes^{\cal C} UF (B)
      \ar[dd]^{\theta^U}
      \\
      U (FUF (A) \otimes^{\cal D} FUF (B))
      \ar[rd]|{U (\epsilon_{F (A)} \otimes^{\cal D} \epsilon_{F (B)})}
      \ar[d]_{U \theta^F}
      &
      \\
      UF (UF (A) \otimes^{\cal C} UF (B))
      \ar[d]_{UF \theta^U}
      \ar@{}[r]|{\txt{($U$ applied to (\ref{eq:moneps:tensor}))}}
      &
      U (F (A) \otimes^{\cal D} F (B))
      \ar[dd]^{U \theta^F}
      \\
      UFU (F (A) \otimes^{\cal D} F (B))
      \ar[ru]|{U \epsilon_{F (A) \otimes^{\cal D} F (B)}}
      \ar[d]_{UFU \theta^F}
      &
      \\
      UFUF (A \otimes^{\cal C} B)
      \ar[r]_{U \epsilon_{F (A \otimes^{\cal C} B)}}
      \ar@{}[ruu]|{\txt{(naturality of $U \epsilon$)}}
      &
      UF (A \otimes^{\cal C} B)
      }
    \]
    } We recognize $T d_{A, B} \circ d_{T A, T B}$ as the leftmost composition
  of vertical arrows, and the rightmost vertical composition is $d_{A, B}$.
  Also, the top horizontal arrow is $\mu_A \otimes^{\cal C} \mu_B$, while the
  bottom arrow is $\mu_{A \otimes^{\cal C} B}$.
\end{proof}

\begin{lemma}
  \label{lemma:monoidal->unitmon}
  Let $({\cal C}, I^{\cal C}, \otimes^{\cal C}, \alpha^{\cal C}, \ell^{\cal
    C}, r^{\cal C})$ be a monoidal category, and let $(T, \eta, \mu, d)$ be a
  monoidal monad on $\cal C$.
%  Let $d_{A, B} : \mu_{A \otimes^{\cal C} B}
%  \circ T t'_{A, B} \circ t_{T A, B} = \mu_{A \otimes^{\cal C} B} \circ T
%  t_{A, B} \circ t'_{A, T B} : T A \otimes^{\cal C} T B$.
  
  Let $\cal D$ be the Kleisli category of $T$, $I^{\cal D} = I^{\cal C}$,
  $\otimes^{\cal D}$ be defined on objects by $A \otimes^{\cal D} B = A
  \otimes^{\cal C} B$ and on morphisms by letting $f \otimes^{\cal D} g$ (in
  $\cal D$) be the morphism $d \circ (f \otimes^{\cal C} g)$ in $\cal C$; let
  $\alpha^{\cal D} = \eta \circ \alpha^{\cal C}$, $\ell^{\cal D} = \eta \circ
  \ell^{\cal C}$, $r^{\cal D} = \eta \circ r^{\cal C}$.  Then $({\cal D},
  I^{\cal D}, \otimes^{\cal D}, \alpha^{\cal D}, \ell^{\cal D}, r^{\cal D})$,
  is a monoidal category.
  
  Moreover, $\KlF T \dashv \KlU T$ is a monoidal adjunction.  The mediating
  pairs of $\KlF T$ and $\KlU T$ are $(\theta^{\KlF T}, \iota^{\KlF T})$ and
  $(\theta^{\KlU T}, \iota^{\KlU T})$ respectively, where $\theta^{\KlF T}_{A,
    B} : \KlF T (A) \otimes^{\cal D} \KlF T (B) \to \KlF T (A \otimes^{\cal C}
  B)$ (in $\Kleisli T$) is the morphism $\eta_{A \otimes^{\cal C} B}$ in $\cal
  C$, $\iota^{\KlF T} : I^{\cal D} \to \KlF T (I^{\cal C})$ (in $\Kleisli T$)
  is $\eta_{I^{\cal C}}$, $\theta^{\KlU T}_{A, B} : \KlU T (A) \otimes^{\cal
    C} \KlU T (B) \to \KlU T (A \otimes^{\cal D} B)$ (in $\cal C$) is $d_{A,
    B}$, and $\iota^{\KlU T} : I^{\cal C} \to \KlU T (I^{\cal D})$ (in $\cal
  C$) is $\eta_{I^{\cal C}}$.
  
  Finally, $\KlF T \dashv \KlU T$ generates the monoidal monad, in the sense
  that $\KlU T \KlF T = T$, $\eta$ is the unit of the adjunction and of $T$,
  $\mu_A = \KlU T \epsilon_{F (A)}$ where $\epsilon$ is the counit of the
  adjunction, and $d_{A, B} = \KlU T \theta^{\KlF T}_{A, B} \circ \theta^{\KlU
    T}_{\KlF T (A), \KlF T (B)}$.
\end{lemma}
\begin{proof}
  Tedious.  See Appendix~\ref{app:monoidal->unitmon}.
\end{proof}

\begin{lemma}
  \label{lemma:monadj:comp}
  Let $\xymatrix{\catd \ar@<1ex>[r]^{\discr} & \catc \ar@<1ex>[l]^{\funbar}
    \ar@<1ex>[r]^{F} & {\cal D} \ar@<1ex>[l]^{U}}$ be a diagram of
  functors.  Assume that these functors are monoidal; let $(\tstrna, \tstri)$
  be the mediating pair of $\funbar$, $(\tstrcna, \tstrci)$ that of $\discr$,
  $(\theta^U, \iota^U)$ that of $U$, $(\theta^F, \iota^F)$ that of $F$.
  
  Then $F \discr$ and $\funbara U$ are monoidal functors, with respective
  mediating pairs $(F \tstrcna \circ \theta^F, F \tstrci \circ \iota^F)$ and
  $(\funbara {\theta^U} \circ \tstrna, \funbara {\iota^U} \circ \tstri)$.
  
  Furthermore, if $\discr \dashv \funbar$ and $F \dashv U$ are monoidal
  adjunctions, then $F \discr \dashv \funbara U$ is a monoidal adjunction,
  too.
\end{lemma}
\begin{proof}
  Straightforward.  See Appendix~\ref{app:monadj:comp}.
\end{proof}

The following proposition is then both similar and proved similarly to
Proposition~\ref{prop:adj:distr:1}.
\begin{proposition}
  \label{prop:adj:distr:2}
  Let $(\catc, \tensorc, \Ic, \alphacna, \lc{}, \rc{})$ and $(\catd, \tensord,
  \Id, \alphadna, \ld{}, \rd{})$ be monoidal categories.
  
  Let $(\tc, \unitc{}, \multc{}, \bistrcna)$ be a monoidal monad on $\catc$,
  $\funbar : \catc \to \catd$ and $\discr : \catd \to \catc$ be monoidal
  functors, yielding a monoidal adjunction $\discr \dashv \funbar$.  Let
  $\counita_A : \discr {\funbara A} \to A$ be the counit of the adjunction,
  $\unita_E : E \to \funbara {\discr (E)}$ be the unit of the adjunction.  Let
  $(\tstrna, \tstri)$ be the mediating pair of $\funbar$, $(\tstrcna,
  \tstrci)$ be the mediating pair of $\discr$.
  
  Define $\td {} = \funbar \circ \tc{} \circ \discr = \funbara {\tc \discr}$,
  $\unitd E = \funbara {\unitc {\discr (E)})} \circ \unita_E$, $\multd E =
  \funbara {\multc {\discr (E)} \circ \tc {\counita_{\tc {\discr (E)}}}}$,
  $\bistrd E F = \funbara {\tc \tstrc E F \circ \bistrc {\discr E} {\discr F}}
  \circ \tstr {\tc \discr E} {\tc \discr F}$.  Finally, let $\dist A =
  \funbara {\tc {\counita_A}} : \td {\funbara A} \to \funbara {\tc A}$.  Then
  $(\td {}, \unitd{}, \multd{}, \bistrdna)$ is a monoidal monad on $\catd$ and
  $(\funbar, \dist {})$ is a monoidal monad morphism from $\tc$ to $\td$.
\end{proposition}
\begin{proof}
  Let $F = \KlF \tc$, $U = \KlU \tc$.  By Lemma~\ref{lemma:monoidal->unitmon},
  $F \dashv U$ is a monoidal adjunction which generates the monoidal monad
  $(\tc, \unitc{}, \multc{}, \bistrcna)$.  Compose the monoidal adjunction
  $\discr \dashv \funbar$ with the monoidal adjunction $F \dashv U$, yielding
  the adjunction $F \discr \dashv \funbara U$.  This is also a monoidal
  adjunction by Lemma~\ref{lemma:monadj:comp}.
%, with the obvious mediating
%  pairs $(F \tstrcna \circ \theta^F, F \tstrci \circ \iota^F)$ for $F
%  \discr$ and $(\funbara {\theta^U} \circ \tstrna, \funbara {\iota^U} \circ
%  \tstri)$ for $\funbara U$.
%!!! checked for moneta parts, not moneps (but a symmetry argument says this
 %should work).
  
  By Lemma~\ref{lemma:monoidal->unitmon}, this monoidal adjunction generates a
  monoidal monad, and this is $(\td {}, \unitd{}, \multd{}, \bistrdna)$ as
  stated in the Proposition.  Indeed, all cases except the mediator have
  been dealt with in Proposition~\ref{prop:adj:distr:1}, and the mediator is
  by definition $\funbara {U (F \tstrcna \circ \theta^F)} \circ \funbara
  {\theta^U} \circ \tstrna = \funbara {UF \tstrcna} \circ \funbara {U \theta^F
    \circ \theta^U} \circ \tstrna = \funbara {\tc \tstrcna} \circ \funbara
  {\bistrcna} \circ \tstrna$.
  
  It remains to check the monoidal monad morphism Diagram~(\ref{d_distbistr}).
  This is given by the following diagram: {\small
    \[
    \xymatrix@-5pt{
      {\hbox{$
          \begin{array}{c}
            \funbara {\tc \discr \funbara {A_1}}\\ \tensord \funbara {\tc \discr \funbara {A_2}}
          \end{array}
          $}}
      \ar[r]^{\tstrna}
      \ar[d]|{\funbara {\tc \counita_{A_1}} \tensord \funbara {\tc
          \counita_{A_2}}}
      \ar@{}[rrdd]|{\txt{(naturality of $\funbara {\bistrcna} \circ \tstrna$)}}
      &
      {\hbox{$
          \funbara {
            \begin{array}{c}
              \tc \discr \funbara {A_1}\\\tensorc \tc \discr \funbara {A_2}
            \end{array}
            }
          $}}
      \ar[r]^{\funbara {\bistrcna}}
      &
      {\hbox{$
          \funbara {\tc \left(
              \begin{array}{c}
                \discr \funbara {A_1}\\ \tensorc \discr \funbara {A_2}
              \end{array}
            \right)}
        $}}
      \ar[r]^{\funbara {\tc \tstrcna}}
      \ar[rdd]_{\funbara {\tc (\counita_{A_1} \tensorc \counita_{A_2})}}
      \ar@{}[rd]|{\txt{(\ref{eq:moneps:tensor})}}
      &
      \funbara {\tc \discr (\funbara {A_1} \tensord \funbara {A_2})}
      \ar[d]|{\funbara {\tc \discr \tstrna}}
      \\
      {\funbara {\tc {A_1}} \tensord \funbara {\tc {A_2}}}
      \ar[d]|{\tstrna}
      &
      &
      &
      \funbara {\tc \discr \funbara {A_1 \tensorc A_2}}
      \ar[d]|{\funbara {\tc \counita_{A_1 \tensorc A_2}}}
      \\
      {\funbara {\tc {A_1} \tensorc \tc {A_2}}}
      \ar[rrr]_{\funbara {\bistrcna}}
      &
      &
      &
      {\funbara {\tc (A_1 \tensorc A_2)}}
      }
    \]
    }
\end{proof}

We can in fact prove something similar with just strong monads. Unfortunately,
it seems that we cannot use the nice trick of going through some adjunction
generating the strong monad.  The proof therefore goes through extremely
tedious diagram checking.


\begin{proposition}
  \label{prop:adj:distr:3}
  Let $(\catc, \tensorc, \Ic, \alphacna, \lc{}, \rc{})$ and $(\catd, \tensord,
  \Id, \alphadna, \ld{}, \rd{})$ be monoidal categories.
  
  Let $\funbar$ be a monoidal functor from $\catc$ to $\catd$, with mediating
  pair $(\tstrna, \tstri)$, $\discr$ be a monoidal functor from $\catd$ to
  $\catc$, with mediating pair $(\tstrcna, \tstrci)$, and assume that $\discr
  \dashv \funbar$ is a monoidal adjunction.

  
  Define $\td {} = \funbar \circ \tc{} \circ \discr = \funbara {\tc \discr}$,
  $\unitd E = \funbara {\unitc {\discr (E)})} \circ \unita_E$, $\multd E =
  \funbara {\multc {\discr (E)} \circ \tc {\counita_{\tc {\discr (E)}}}}$,
  $\dist A = \funbara {\tc {\counita_A}} : \td {\funbara A} \to \funbara {\tc
    A}$.
  
  Define also $\strd E F$ as the composite $\funbara {\tc \discr \tstrc E F
    \circ \strc {\discr E} {\discr F}} \circ \tstr {\discr E} {\tc \discr F}
  \circ (\unita_E \tensord \identity {\td F})$.
%  {\small
%    \[
%    \xymatrix{
%      E \tensord \funbara {\tc \discr F}
%      \ar[r]^{\unita_E \tensord \identity {\td F}}
%      &
%      {\funbara {\discr E} \tensord \funbara {\tc \discr F}}
%      \ar[r]^{\tstr {\discr E} {\tc \discr F}}
%      &
%      {\funbara {\discr E \tensorc \tc \discr F}}
%      \ar[r]^{\funbara {\strc {\discr E} {\discr F}}}
%      & 
%      {\funbara {\tc (\discr E \tensorc \discr F)}}
%      \ar[r]^{\funbara {\tc \tstrc E F}}
%      &
%      {\funbara {\tc \discr (E \tensord F)}}
%      }
%    \]
%    }
  
  Then $(\td {}, \unitd{}, \multd{}, \strdna)$ is a strong monad on $\catd$
  and $(\funbar, \dist {})$ is a strong monad morphism from $\tc$ to $\td$.
\end{proposition}
\begin{proof}
  Because of Proposition~\ref{prop:adj:distr:1}, we only have to check the
  strength laws (\ref{eq:strong:l}), (\ref{eq:strong:eta}),
  (\ref{eq:strong:double}), (\ref{eq:strong:mu}) for $\strdna$, and the strong
  monad morphism law (\ref{d_diststr}).  As we said, this is tedious, hence
  relegated to Appendix~\ref{app:adjstrong}.
\end{proof}


==> fun.tex <==

\newcommand\quot[2]{{#1}/{#2}}
\newcommand{\interior}[1]{{\buildrel \circ \over {#1}}}
\newcommand\uuarrow{\rlap{$\uparrow$}\raise.5ex\hbox{$\uparrow$}}%%
\newcommand\ques[1]{\tc (#1)}

\subsection{Fun With Categories~I: Taking $\catc\neq \catset$, the Example of $\Dcpo$}
\label{sec:notset}

The constructions of this paper apparently allow for some considerable
degree of freedom.  We may choose distinct categories for $\catc$ and
$\catd$, different monads $\tc$ and $\td$, several monad morphisms
$\distr$, several mono factorization systems, and so on.

However, the examples we have given until now used none of these
degrees of freedom.  By taking $\catc = \catd = \setcat$ notably, we
have essentially narrowed down our possible choices to just one.  So
let us have fun, trying to vary various parameters, and see what
happens.  We start by keeping $\catc=\catd$, but with categories
$\catc$ other than $\catset$ or presheaf categories.  We shall then
look at several mono factorization systems.

The aim of this section is to show that, at least if we keep $\catc =
\catd$, our freedom is considerably restricted.

Imagine $\catc$ is $\Dcpo$, the category of cpos and continuous maps.
By {\em cpo\/} we mean any ordered set such that any directed family
of elements has a least upper bound.  See
\cite{AJ:domains,GHKLMS:compendium,GHKLMS:contlatt} for background
information on cpos and related topics.
We always assume cpos to be equipped with  their Scott topology.

Imagine the monad we are interested in on $\Dcpo$ is that of demonic
non-determinism, whereby intuitively, non-deterministic choices are in
the hand of a malevolent external adversary.  The traditional monad
$\tc$ modeling this is the {\em Smyth powerdomain\/} construction:
$\tc A = \mathcal Q (A)$ consists of all compact non-empty
upward-closed subsets of $A$, ordered by {\em reverse\/} inclusion
$\supseteq$.  One problem here is that $\mathcal Q (A)$ need not be a cpo.  It
is one if $A$, equipped with its Scott topology, is a {\em sober\/}
topological space; for example, if $A$ is a continuous cpo.  So we
should restrict to some cartesian-closed category consisting of
continuous cpos only.  We know what these categories should be, by
Jung's results \cite{Jung:CCC}, but this is a bit complicated for an
illustration.
\ifmscs
\else
(We shall return to these categories anyway in
Section~\ref{sec:top}, out of necessity, but will avoid them as long
as we can.)
\fi

Instead, take Heckmann's characterization of the upper power domain
\cite{Heckmann:PhD} (without the top element, which would be the empty
compact in $\mathcal Q (A)$ above).  Let $\mathbf 2 = \{0, 1\}$ be the
{\em Sierpi\'nski space\/}, i.e., the two-element cpo with $0 < 1$.  Let
$[A \to \mathbf 2]$ be the set of Scott-continuous functions from $A$ to
$\mathbf 2$; this is canonically isomorphic to the space of Scott
opens of $A$, through the map sending $f \in [A \to \mathbf 2]$ to $f^{-1}
\{1\}$.  Define $\top$ as $\lambda x \cdot 1$ in $[A \to \mathbf 2]$, $\bot$ as $\lambda x \cdot 0$;
least upper bounds $\sqcup$ and greatest lower bounds $\sqcap$ are defined
pointwise.  Following Heckmann, $\mathcal U_* (A)$ is the set of
continuous linear non-trivial second-order predicates, i.e., the set
of Scott-continuous functionals $F$ from $[A \to \mathbf 2]$ to $\mathbf
2$ that preserve $\top$ and meets $\sqcap$ (linearity), and map $\bot$ to $0$
(non-triviality).  (See \cite[Chapter~19]{Heckmann:PhD} for the
rationale behind this construction, and for related theorems.  While
our constructions will work for several other power constructions, we
only take one as illustration.)

$\mathcal U_*$ is a monad $\tc$ on $\Dcpo$.  Its action on morphisms $h
: A \to B$ is given by $\tc (h) = \lambda F \in \mathcal U_* (A), f \in [B \to \mathbf
2] \cdot F (f \circ h)$.  Its unit is given by $\unitc A (x) = \lambda f \in [A \to
\mathbf 2] \cdot f (x)$ ($x \in A$), and its multiplication is given by
$\multc A (G) = \lambda f \in [A \to \mathbf 2] \cdot G (\lambda F \in \mathcal U_* (A) \cdot F
(f))$ ($G \in \mathcal U_*^2 (A)$).  The strength is given by $\strc A B =
\lambda (x, F) \in A \times \mathcal U_* (B) \cdot \lambda f \in [A \times B \to \mathbf 2] \cdot F (\lambda y \in B
\cdot f (x, y))$.  Note that these are the same formulae as those defining
the continuation monad.

It turns out that if $A$ is a continuous cpo, then $\mathcal U_* (A)$
and $\mathcal Q (A)$ are naturally isomorphic.  They key result here
is the Hofmann-Mislove Theorem \cite[Corollary~7.2.10]{AJ:domains}.
The isomorphism maps any upward-closed compact subset $Q$ of $A$ to
the continuous linear functional $\lambda f \in [A \to \mathbf 2] \cdot Q \subseteq f^{-1}
\{1\}$, and conversely, maps any continuous linear functional $F$ to the
intersection of all opens $O$ of $A$ such that $F (\chi_O)=1$.  (The hard
part of the Hofmann-Mislove theorem is to show that this is compact,
as soon as $A$ is sober.)
\ifmscs
\else
While this shows the connection between
$\mathcal U_*$ and $\mathcal Q$, we shall not use this until
Section~\ref{sec:top}.
\fi

To apply our construction of logical relations, we need a mono
factorization system.  In $\Dcpo$, there are at least three:
\begin{itemize}
\item The {\em trivial mono factorization\/}.  Here, relevant monos
  are isos, and pseudoepis are arbitrary morphisms.  This exists in
  every category, and is completely uninteresting in every category:
  given any binary relation $S$ between $A_1$ and $A_2$, i.e.,
  $\xymatrix@-5pt{S \arrmonoxy[r]^m & {A_1 \times A_2}}$, then $S$ is
  in fact the whole of $A_1 \times A_2$ (up to iso).
\item The {\em epi / regular mono factorization\/}.  Recall that a
  mono is {\em regular\/} if and only if it is the equalizer of a
  parallel pair.  Let us describe regular monos more concretely in
  $\Dcpo$.
%   A {\em sub-cpo\/} of a cpo $B$ is a subset of $B$ that is
%   a cpo with the induced ordering; this is usually called an {\em
%     inductive subset\/} of $B$, and is characterized as one that is
%   stable under the formation of least upper bounds of directed
%   subsets.

  A regular mono $m : \xymatrix@-5pt{C \arrmonoxy[r] & B}$ in $\Dcpo$
  is a Scott-closed subset of $B$, up to isomorphism.  More precisely,
  $m$ is the composite of an iso from $C$ to some Scott-closed subset
  $m (C)$ of $B$, with the canonical inclusion of $m (C)$ in $B$.

  An epi is any continuous function $e : \xymatrix@-5pt{A \arrepixy[r]
    & C}$ such that $e (A)$ is {\em dense\/} in $C$, i.e., such that
  $cl (e (A))=C$, where $cl$ denotes the (Scott) topological closure
  operator.  Equivalently, such that $e^{-1} (U) \neq \emptyset$ for any
  non-empty Scott-open $U$ of $C$.

  It is well-known that this yields a mono factorization system on
  $\Dcpo$.  We skip the details, which are not very interesting at
  this point.

\item The {\em extremal epi / mono factorization\/}.  Recall that the
  {\em extremal\/} pseudoepis are the morphisms $\xymatrix@-5pt{A
    \ar[r]^e & B}$ such that, whenever $e$ can be written as the
  composite $\xymatrix@-5pt{A \ar[r] & B' \arrmonoxy[r]^m & B}$ where
  $m$ is mono, then $m$ is actually iso.

  Many categories $\catc$ have a mono factorization system where the
  pseudoepis are the extremal pseudoepis, as shown by Freyd and Kelly:
  by Proposition~2.3.4 of \cite{FK:cont}, this is the case if $\catc$
  has all finite limits and admits intersections of monos (i.e.,
  limits of all classes of monos ${(\xymatrix@-5pt{X_\alpha
      \arrmonoxy[r]^{m_\alpha} & B})}_{\alpha \in \Omega}$); or if $\catc$ has all
  finite colimits and admits colimits of all classes of extremal
  pseudoepis ${(\xymatrix@-5pt{B \arrepixy[r]^{e_\alpha} & Y_\alpha})}_{\alpha \in \Omega}$;
  or if $\catc$ has all finite limits, all finite colimits, and
  composites of coequalizers are coequalizers.  In all these cases,
  extremal pseudoepis are in fact epis; in the third case, they are
  regular, i.e., coequalizers of parallel pairs.  By the way, the
  argument of Freyd and Kelly in fact shows that $\catc$ has a mono
  factorization system as soon as $\catc$ has pullbacks (not
  necessarily all limits) and admits non-empty intersections of monos:
  the factorization of any given morphism $\xymatrix@-5pt{A \ar[r]^f &
    B}$ is the intersection of the class of all monos $m_\alpha$ such that
  $f$ factors through $m_\alpha$, i.e., such that $f$ can be written
  $\xymatrix@-5pt{A \ar[r]^{e_\alpha} & C_\alpha \arrmonoxy[r]^{m_\alpha} & B}$.  (In
  this case, it is unknown whether pseudoepis are epi.)

  While monos in $\Dcpo$ are simple to characterize---they are just
  the injective continuous maps---extremal epis have a much more
  complicated structure, which we therefore elude.
\end{itemize}
It turns out that we have been unable to show that the functor $\tc =
\mathcal U_*$ mapped relevant pseudoepis to pseudoepis, despite our
efforts.  We shall see in the next sections that this is not needed.
All we have to do is make $\catd$ slightly different from $\catc$, and
$\td$ slightly different from $\tc$.

\subsection{Fun With Categories~II: Making $\catc$ and $\catd$
  Distinct, e.g., $\catc = \Dcpo$, $\catd=\ordcat$}
\label{sec:c!=d}

Consider $\catd = \ordcat$, the category of partial orders and
monotonic maps.  There is an obvious forgetful functor $\funbar_0 :
\Dcpo \to \ordcat$.  In the following, if $A \subseteq B$, we write $\uparrow_B A$ the
subset $\{x \in B | \exists y \in A \cdot y \leq x\}$.

In any partial order $A$, say that a subset is {\em finitary\/} if and
only if it is of the form $\uparrow_A E$ with $E$ finite.  In the following,
we take $\td A$ as the space of non-empty finitary subsets of $A$,
ordered by {\em reverse\/} inclusion $\supseteq$.  Why should we take this?
Well, we have seen above that the space $\tc A = \mathcal U_* (A)$ could
be identified with the space of compact non-empty upward-closed
subsets of $A$, ordered by reverse inclusion.  For our construction to
work out, in particular to be able to find a suitable monad morphisms,
$\td$ should in a sense mimic $\tc$ in the category $\catd$.  By going
from $\catc=\Dcpo$ to $\catd=\ordcat$, we keep the ordering but forget
about the (Scott-) topology.  It turns out that, if we just know about
the ordering $\leq$, there are many possible topologies from which it may
arise.  Precisely, there are many topologies with $\leq$ as {\em
  specialization quasi-ordering\/} --- the one defined so that $x$ is
less than or equal to $y$ if and only if every open containing $x$
must also contain $y$.  One is the Scott-topology.  The finest is the
Alexandroff topology, whose opens are all upward-closed subsets.  In
all these topologies, the only subsets that are guaranteed to be
compact upward-closed are the finitary subsets.  The latter then
intuitively form a concept similar to the notion of compact
upward-closed subsets.  This should be checked formally, by verifying
the axioms for monad morphisms, which we do right away.

Note in passing that there is a slightly distinct presentation of $\td
A$, as set of finite non-empty {\em antichains\/} (sets $E$ where no
two distinct elements are comparable), ordered in the {\em Smyth
  ordering\/} $\leq^\sharp$ defined by $E \leq^\sharp E'$ if and only if every element
of $E'$ is greater than or equal to some element of $E$.


For every map $f : A \to B$, $\td f$ maps the finitary subset $\uparrow_A \{x_1,
\ldots, x_n\}$ to $\uparrow_B \{f (x_1), \ldots, f (x_n)\}$.  This defines a monad on
$\ordcat$, together with unit $\unitd A : A \to \td A$ defined by
$\unitd A (x) = \uparrow_A \{x\}$, multiplication $\multd A : \td^2 A \to \td A$
defined by $\multd A (\uparrow_{\td A} \{\uparrow_A E_1, \ldots, \uparrow_A E_n\}) = \uparrow_A \bigcup_{i=1}^n
E_i$.  This is in fact a commutative monad, with mediator $\bistrd A B
: \td A \times \td B \to \td (A \times B)$ defined by $\bistrd A B (\uparrow_A E, \uparrow_B F)
= \uparrow_{A \times B} (E \times F)$.  The corresponding strength maps $(x, \uparrow_B \{y_1,
\ldots, y_m\})$ to $\uparrow_{A \times B} \{(x,y_1), \ldots, (x,y_m)\}$.

The required monad morphism $\dist A^0 : \td {\funbara A_0} \to \funbara
{\tc A}_0$ maps $\uparrow_A E$ to the function $\lambda f \in [A \to \mathbf 2] \cdot E \subseteq
f^{-1} \{1\}$.  (We identify truth with $1$, so that $E \subseteq f^{-1} \{1\}$
denotes $1$ if true, $0$ if false.)  The latter function is
continuous, because $E$ is finite, so this indeed defines a map to
$\funbara {\tc A}_0$.  This is clearly natural in $A$.  Let us check
the monad morphism laws (\ref{d_distlaw}).  First, $\dist A^0 \circ \unitd
{\funbara A_0}$ maps $x \in A$ to $\lambda f \in [A \to \mathbf 2] \cdot \{x\} \subseteq f^{-1}
\{1\} = \lambda f \in [A \to \mathbf 2] \cdot f (x) = \funbara {\unitc A}_0 (x)$.
Second, fix an element $\uparrow_{\td A} \{\uparrow_A E_1, \ldots, \uparrow_A E_n\}$ in $\td^2
\funbara A_0$.  This is mapped by $\td \dist A^0$ to $\uparrow_{\funbara {\tc
    A}_0} \{\lambda f \cdot E_1 \subseteq f^{-1} \{1\}, \ldots, \lambda f \cdot E_n \subseteq f^{-1} \{1\}\}$; then
by $\dist {\tc A}^0$ to $\lambda F \in [\tc A \to \mathbf 2] \cdot \forall i, 1\leq i\leq n \cdot (\lambda
f \cdot E_i \subseteq f^{-1} \{1\}) \subseteq F^{-1} \{1\} = \lambda F \cdot \forall i, 1\leq i\leq n \cdot F (\lambda f \cdot E_i
\subseteq f^{-1} \{1\})=1$; then by $\funbara {\multc A}_0$ to $\lambda f \cdot \forall i, 1\leq i\leq
n \cdot E_i \subseteq f^{-1} \{1\}$.  On the other hand, $\uparrow_{\td A} \{\uparrow_A E_1, \ldots, \uparrow_A
E_n\}$ is mapped by $\multd A$ to $\uparrow_A (E_1 \cup \ldots \cup E_n)$, then by $\dist
A^0$ to $\lambda f \cdot E_1 \cup \ldots \cup E_n \subseteq f^{-1} \{1\}$, so the diagram on the
right of (\ref{d_distlaw}) commutes.

We may also check that $\dist A^0$ is a strong monad morphism.
Diagram (\ref{d_diststr}) states that we may indeed compute the map
sending $(x, \uparrow_{\funbara {A_2}_0} \{y_1, \ldots, y_m\}) \in \funbara {A_1}_0 \times
\td \funbara {A_2}_0$ to $\lambda f \in [A_1 \times A_2 \to \mathbf 2] \cdot \{(x,y_1), \ldots,
(x,y_m)\} \subseteq f^{-1} \{1\}$ in two different ways.

Now we have at least three mono factorization systems on $\ordcat$,
which are much simpler as in $\Dcpo$:
\begin{enumerate}
\item The trivial mono factorization system, which is, as usual,
  uninteresting.
\item The epi / regular mono factorization.  Here the epis are just
  the surjective monotone maps, while the regular monos are
  embeddings, i.e., maps $m$ such that $x \leq y$ if and only if $m (x) \leq
  m (y)$.  

  It is not quite obvious that the epis are the surjective monotone
  maps.  Here is a quick proof of the difficult implication.  Assume
  $e$ epi from $A$ to $C$.  For any two upward-closed subsets $U$, $V$
  of $C$, the characteristic functions $\chi_U, \chi_V : C \to \mathbf 2$ are
  monotone.  If $\chi_U \circ e = \chi_V \circ e$ then $U=V$.  In other words, if $e
  (A) \cap U = e (A) \cap V$ then $U=V$.  Consider any $z \in C$, and build $U
  = \uparrow_C z$, $V = \uparrow_C (e (A) \cap U)$.  It is easy to check that $V \subseteq U$,
  so $e (A) \cap V \subseteq e (A) \cap U$; the converse inclusion is obvious.  So
  $U=V$.  It follows that $z \in V$, i.e., there is an element $z' \leq z$
  such that $z' \in e (A) \cap \uparrow_C z$, whence $z \in e (A)$.

  The factorization of $\xymatrix@-5pt{A \ar[r]^f & B}$ goes through
  the middle object $C$ defined as the image $f (A)$ of $A$ by $f$,
  equipped with the ordering inherited from $B$.

  This is a monoidal mono factorization (condition {\bf (iii.a)}): the
  product of two surjective monotone maps $e_1 : A_1 \to C_1$ and $e_2 :
  A_2 \to C_2$ is clearly again surjective.

  Condition {\bf (vi)}, that $\ihom A \_$ preserves regular monos, is
  obvious from the remark that $\ihom A \_$ is a right-adjoint, so it
  preserves limits, in particular equalizers.

  It remains to show that $\td$ preserves epis (condition {\bf (iv)}).
  Fix an epi $e$ from $A$ to $B$ in $\ordcat$.  It is clear that every
  $\uparrow_B \{y_1, \ldots, y_n\} \in \td B$ is the image of $\uparrow_A \{x_1, \ldots, x_n\} \in \td
  A$ by $\td e$, where for each $i$, $x_i$ is any element such that $e
  (x_i) = y_i$.  So $\td e$ is surjective, that is, epi.

\item The extremal epi / mono factorization.  The monos are just the
  injective monotone maps, while the extremal epis are the quotient
  maps.  A {\em quotient map\/} $\xymatrix@-5pt{A \arrepixy[r]^q & C}$
  is by definition the map sending $x \in A$ to its equivalence class in
  $C = \quot A \equiv$, for some equivalence relation $\equiv$ on $A$.  (This is
  up to post-composition with an iso, naturally.)  The ordering on $C$
  is then given as the smallest transitive relation $\leq_C$ such that $x
  \leq y$ in $A$ implies $q (x) \leq_C q (y)$ in $C$.  Equivalently, $q$ is
  a quotient map if and only if it is surjective and, for every subset
  $V$ of $C$, $V$ is upward-closed in $C$ if and only if $q^{-1} (V)$
  is upward-closed in $A$.  The factorization of $\xymatrix@-5pt{A
    \ar[r]^f & B}$ goes through the middle object $C$ defined as the
  image $f (A)$ of $A$ by $f$, equipped with the ordering $\leq_C$
  defined as the smallest transitive relation such that $x \leq y$ in $A$
  implies $f (x) \leq_C f (y)$ in $C$.

  This is also a monoidal mono factorization (condition {\bf
    (iii.a)}): if $q_1 : A_1 \to \quot {A_1} {\equiv_1}$ and $q_2 : A_2 \to
  \quot {A_2} {\equiv_2}$ are quotient maps, then $q_1 \times q_2$ is the
  quotient map from $A_1 \times A_2$ to $\quot {(A_1 \times A_2)} \equiv$, where
  $(x_1, x_2) \equiv (y_1, y_2)$ if and only if $x_1 \equiv_1 y_1$ and $x_2 \equiv
  y_2$.

  $\td$ also preserves extremal epis (condition {\bf (iv)}).  Indeed,
  let $q : A \to C$ be an extremal epi, that is, a quotient map, for
  some equivalence relation $\equiv$ on $A$.  In particular, $C = \quot A
  \equiv$.  By construction, $q (x) \leq q (x')$ if and only if $x {(\leq \cup \equiv)}^*
  y$, where ${(\leq \cup \equiv)}^*$ is the reflexive transitive closure of the
  union of the two relations $\leq$ and $\equiv$.  For any $y \in C$, let $x$ be
  any element such that $q (x)=y$.  To show that $\td q$ is quotient,
  we must show that for any subset $\mathcal U$ of $\td C$, if ${(\td
    q)}^{-1} (\mathcal U)$ is upward-closed then so is $\mathcal U$.
  Let $\uparrow_C \{y_1, \ldots, y_m\}$ be an element of $\td C$, and $\uparrow_C \{y'_1, \ldots,
  y'_n\}$ any larger element (wrt.\ $\supseteq$, i.e., a smaller subset).  We
  may assume without loss of generality that $\{y_1, \ldots, y_m\}$ and
  $\{y'_1, \ldots, y'_n\}$ are antichains, and that $\{y_1, \ldots, y_m\} \leq_C^\sharp
  \{y'_1, \ldots, y'_n\}$: for each $j$, $1\leq j\leq n$, there is $i$, $1\leq i\leq m$,
  such that $y_i \leq_C y'_j$.  Since $q$ is surjective, write $y_i =
  q(x_i)$, $y'_j = q(x'_j)$.  In particular: $(*)$ for each $j$ there
  is $i$ such that $x_i {(\leq \cup \equiv)}^* x'_j$.  Then ${(\td q)}^{-1} (\uparrow_C
  \{y_1, \ldots, y_m\})$ is the set of elements $x \in A$ such that $x_i {(\leq \cup
    \equiv)}^* x$ for some $i$, $1\leq i\leq m$.  Similarly, ${(\td q)}^{-1} (\uparrow_C
  \{y'_1, \ldots, y'_n\})$ is the set of elements $x \in A$ such that $x'_j {(\leq
    \cup \equiv)}^* x$ for some $j$, $1\leq j\leq n$.  By $(*)$ above, every such
  $x$ is also such that $x_i {(\leq \cup \equiv)}^* x$ for some $i$, $1\leq i \leq m$.
  So ${(\td q)}^{-1} (\uparrow_C \{y_1, \ldots, y_m\})$ contains ${(\td q)}^{-1}
  (\uparrow_C \{y'_1, \ldots, y'_n\})$.  Since ${(\td q)}^{-1} (\mathcal U)$ is
  upward-closed (for the $\supseteq$ ordering), ${(\td q)}^{-1} (\uparrow_C \{y'_1, \ldots,
  y'_n\})$ must also be in ${(\td q)}^{-1} (\mathcal U)$, that is, $\uparrow_C
  \{y'_1, \ldots, y'_n\}$ is in $\mathcal U$.  So $\mathcal U$ is
  upward-closed, and $\td q$ is therefore quotient.

  Explicitly, one can show that the equivalence relation $\equiv'$ defined
  by the quotient map $\td q$ on $\td A$, that is the relation defined
  by $\uparrow_A \{x_1, \ldots, x_m\} \equiv' \uparrow_A \{x'_1, \ldots, x'_n\}$ if and only if $\td q
  (\uparrow_A \{x_1, \ldots, x_m\}) = \td q (\uparrow_A \{x'_1, \ldots, x'_n\})$, can be defined
  equivalently by: for every $i$ there is $j$ such that $x_i {(\leq \cup
    \equiv)}^* x'_j$, and for every $j$ there is $i$ such that $x'_j {(\leq \cup
    \equiv)}^* x_i$.
\end{enumerate}


This much gives us an instance of our construction for logical
predicates, i.e., logical relations of arity one.  As for the
$\setcat$ example, binary predicates are obtained by letting $\catc$
be $\Dcpo \times \Dcpo$, keeping $\catd = \ordcat$, defining $\funbara
{A_1, A_2} = A_1 \times A_2$, $\tc$ as $\td \times \td$, and the monad morphism
$\dist {A_1, A_2}$ by $\dist {A_1, A_2} (\uparrow_{A_1 \times A_2} \{(x_1,y_1), \ldots,
(x_m, y_m)\}) = (\lambda f_1 \in [A_1 \to \mathbf 2] \cdot \{x_1, \ldots, x_m\} \subseteq f_1^{-1}
\{1\}, \lambda f_2 \in [A_2 \to \mathbf 2] \cdot \{y_1, \ldots, y_m\} \subseteq f_2^{-1} \{1\})$.  Take
for mediating pair $\tstr {A_1, A_2} {B_1, B_2} : \funbara {A_1, A_2}
\tensord \funbara {B_1, B_2} \to \funbara {(A_1, A_2) \times (B_1, B_2)}$
defined as mapping $((x_1,x_2),(y_1,y_2))$ to $((x_1,y_1),(x_2,y_2))$,
and the obvious morphism $\tstri : \mathbf 1 \to \funbara {\mathbf 1}$.
Then checking that $\distr$ is a strong monad morphism presents no
difficulty.

\vskip1em

Let's now look at the form of the binary logical relations we get in
this setting, depending on the mono factorization system we consider.

\textbf{Epi / regular mono factorization, binary case.}  In this
setting, a binary relation $\xymatrix@-5pt{S \arrmonoxy[r]^m & {A_1 \times
    A_2}}$ between $A_1$ and $A_2$ is just a subset $S$ of $A_1 \times
A_2$, up to iso.  The ordering on $S$ is inherited from that on $A_1 \times
A_2$.

Given such a subset $S \subseteq A_1 \times A_2$, with inclusion embedding $m$, our
construction first builds $\dist {A_1, A_2} \circ \td m$: this maps any
finitary subset $\uparrow_S \{(x_1,y_1), \ldots, (x_m,y_m)\} \in \td S$ (i.e., where
$(x_i, y_i) \in S$ for every $i$) to $(\lambda f_1 \in [A_1 \to \mathbf 2] \cdot \{x_1,
\ldots, x_m\} \in f_1^{-1} \{1\}, \lambda f_2 \in [A_1 \to \mathbf 2] \cdot \{y_1, \ldots, y_m\} \in
f_2^{-1} \{1\})$.  Then factor this arrow through an object $\lift S$,
which embeds into $\tc {A_1} \times \tc {A_2}$: $\lift S$ is the subset of
all $(F_1, F_2) \in \tc {A_1} \times \tc {A_2}$ such that there are finitely
many pairs of related elements $(x_1,y_1) \in S$, \ldots, $(x_m,y_m) \in S$
having the property that $F_1 (f_1)=1$ if and only if $f_1$ maps every
$x_i$ to $1$, and $F_2 (f_2)=1$ if and only if $f_2$ maps every $y_i$
to $1$.

% !!! explain what kind of logical relation this defines.

\textbf{Extremal epi / mono factorization, binary case.}  In this
framework, and up to iso, a binary relation $\xymatrix@-5pt{S
  \arrmonoxy[r]^m & {A_1 \times A_2}}$ between $A_1$ and $A_2$ is again a
subset $S$ of $A_1 \times A_2$, {\em together\/} with an ordering $\preceq$ such
that $(x_1,x_2) \preceq (y_1,y_2)$ implies $x_1 \leq y_1$ and $x_2 \leq y_2$.
Call $(S, \preceq)$ a {\em sub-order\/} of $A_1 \times A_2$.

Given such a sub-order, it can be checked that $\lift S$ relates
exactly the same functions as with the epi / regular mono
factorization.  Only the ordering on $\lift S$ changes: instead of
being inherited from that on $\tc {A_1} \times \tc {A_2}$, it is the
ordering $\leq_C$ defined above, with $C = \lift S$.  In other words,
$\leq_{\lift S}$ is the smallest transitive relation such that $(\lambda f_1 \in
[A_1 \to \mathbf 2] \cdot \{x_1, \ldots, x_m\} \in f_1^{-1} \{1\}, \lambda f_2 \in [A_1 \to
\mathbf 2] \cdot \{y_1, \ldots, y_m\} \in f_2^{-1} \{1\}) \leq_{\lift S} (\lambda f_1 \in [A_1 \to
\mathbf 2] \cdot \{x'_1, \ldots, x'_n\} \in f_1^{-1} \{1\}, \lambda f_2 \in [A_1 \to \mathbf 2]
\cdot \{y'_1, \ldots, y'_n\} \in f_2^{-1} \{1\})$ whenever ${\uparrow_S} \{(x_1,y_1), \ldots,
(x_m,y_m)\} \supseteq {\uparrow_S} \{(x'_1,y'_1), \ldots, (x'_n,y'_n)\}$, that is whenever
for every $j$, $1\leq j\leq n$, there is an $i$, $1\leq i\leq m$, such that
$(x_i,y_i) \preceq (x'_j,y'_j)$.

% !!!, explain what kind of logical relation this defines.

We now make two %three
remarks.

\textbf{Remark.}  Comparing the effect of the two mono factorizations
above, it is clear that they define exactly the same relations, i.e.,
the same sets underlying the space $\lift S$.  The two constructions
only differ in the orderings on $\lift S$.  This is due to the fact
that the set underlying the middle object $C$ in a factorization
$\xymatrix@-5pt{A \arrepixy[r]^e & C \arrmonoxy[r]^m & B}$ of a map $f
: A \to B$ is the image of $A$ under $f$ in both cases.  This need not
be the case in all categories, see the epi / regular mono case in
$\Dcpo$ (Section~\ref{sec:notset}).

% \textbf{Remark.}  The constructions above are instances of those of
% Section~\ref{distr.s}.  Indeed, $\funbar_0$ is right-adjoint to a
% functor $\discr_0 : \ordcat \to \Dcpo$.  We only sketch the argument.

% For every partial order $A$, $\discr_0 A$ is the {\em free cpo\/} over
% $A$.  It is built by freely adding all suprema of directed families in
% $A$.  Formally, $\discr_0 A$ can be built as the set of all
% downward-closed directed families of $A$, ordered by inclusion: think
% of a downward-closed directed family $D$ as coding the supremum of
% $D$, which may be missing from $A$.  The counit of the adjunction, $\counita_A : \discr {\funbara A} \to A$, maps
% any (downward-closed) directed family $D$ of the cpo $A$ to its supremum in $A$.
% The unit $\unita_A : A \to \funbara {\discr (A)}$ maps every element $x$ of
% the partial order $A$ to $\downarrow_A x$.  It is well-known that $\discr_0 A$ is
% then an algebraic cpo, and its compact elements are just those of the form
% $\downarrow_A x$, $x \in A$.
% %  For ease of notation, we equate $\downarrow_A x$ with $x$, which
% %allows us to see $A$ as a subset of $\discr_0 A$.
% Then $[\discr_0 A \to \mathbf 2]$ is naturally isomorphic to the space
% $(A \to \mathbf 2)$ of monotonic, not necessarily continuous functions
% from $A$ to $\mathbf 2$: in the difficult direction, given any
% monotonic function $f$ from $A$ to $\mathbf 2$, extend it to a
% continuous function from $\discr_0 A$ to $\mathbf 2$ by sending $D$ to
% the supremum of all $f (x)$, $x \in D$.  In turn, $(A \to \mathbf 2)$ is
% naturally isomorphic to the space of Alexandroff opens of $A$, and the
% space $\funbara {\tc {\discr_0 A}}_0$ can be identified with the space
% of all Scott-continuous non-trivial filters of Alexandroff opens of
% $A$.  (By non-trivial we mean distinct from the filter of all
% Alexandroff opens.)  One can check, either by elementary calculation,
% or by using the Hofmann-Mislove theorem, that this is naturally
% isomorphic to the space of all finitary non-empty subsets of $A$.
% Explicitly, the isomorphism sends any linear map $F$ from $[\discr_0 A
% \to \mathbf 2]$ to $\mathbf 2$, to the subset $\{x \in A | \forall f \in [\discr_0
% A \to \mathbf 2] \cdot F (f) = 1 \Rightarrow f (\downarrow_A x) = 1\}$, which is upward-closed,
% and finitary (by Hoffman-Mislove); conversely, any finitary subset
% $\uparrow_A \{x_1, \ldots, x_m\}$ is mapped to $\lambda f \in [\discr_0 A \to \mathbf 2] \cdot \forall i
% \cdot f (\downarrow_A x_i)=1$.  Modulo this isomorphism, $\funbara {\tc {\discr_0
%     A}}_0$ is exactly $\td A$, as introduced above.  It is of course
% simpler to reason about the direct definition of $\td$ in terms of
% finitary subsets; however, {\em finding\/} $\td$ itself can be done
% profitably with the help of an adjunction such as $\discr_0 \dashv
% \funbar_0$, and then simplifying the presentation---what we did here.

% % ->: given F continuous linear from (A \to \mathbf 2) to \mathbf 2,
% % define Scott-open filter of upward-closed subsets $U$:
% % \{U | F (\chi_U)=1\}.  Its intersection is \{x | \forall U \cdot F (\chi_U)=1 \Rightarrow x \in U\}$.

% % <-: given finitary compact $Q = \uparrow_A \{x_1,\ldots,x_m\}$,
% % build Scott-open filter of all
% % upward-closed subsets $U$ containing $Q$, $\{U | Q \subseteq U\}$.
% % As a functional, F maps $\chi_U$ to 1 iff $Q \subseteq U$,
% % iff \forall i \cdot x_i \in U$.

\textbf{Remark.}  The binary relation $\lift S$ that we got above, for
whichever of the two mono factorizations we examined, is a bit
disappointing.  Indeed, it only relates functionals of the form $\lambda f \in
[A \to \mathbf 2] \cdot \{x_1, \ldots, x_m\} \in f^{-1} \{1\}$, where $A$ is $A_1$ or
$A_2$; equivalently, of the form $\lambda f \in [A \to \mathbf 2] \cdot \forall i \cdot f
(x_i)=1$.  The latter only encodes {\em finite\/} non-deterministic
choice, among $x_1$, \ldots, $x_m$, while elements of $\tc A$ encode
general non-deterministic choice, typically among the elements of a
compact saturated subset, which is not necessarily finitary.  $\lift
S$ does not relate any element of $\tc A$ to any other, unless it
encodes finite non-determinism.  The core of the problem is our choice
of the category $\catd$ as $\ordcat$, which keeps all ordering
information, but forgets about all continuity properties.
\ifmscs
Possible ways of getting around this problem are explored in the full version \cite{GLN02}.
\else
\fi

% One can get out of this by choosing another monad $\td$ on $\ordcat$.
% Take now $\td A$ to be the set of {\em all\/} upward-closed subsets of
% $A$, not just the finitary subsets, and $\td f (U) = \uparrow_B f (U)$ for
% any $f : A \to B$.  $\td$ again defines a strong monad on $\ordcat$.
% One may check that $\td$ preserves pseudoepis again:
% \begin{itemize}
% \item In the epi / regular mono case, we must show that $\td e$ is
%   surjective as soon as $e : A \to C$ is.  Let $V$ be any element of
%   $\td C$, that is, any upward-closed subset of $C$.  Let $U = e^{-1}
%   (V)$: $U$ is upward-closed in $A$.  We claim that $\td e (U) = V$.
%   Clearly $\td e (U) \subseteq V$: if $y \in \td e (U)$, there is an $x \in U$
%   such that $e (x) \leq y$; $e (x)$ is in $V$ since $x \in e^{-1} (V)$, so
%   that $y \in V$ because $V$ is upward-closed.  Conversely, every $y \in
%   V$ can be written as $e (x)$ with $x \in U$, since $e$ is surjective,
%   hence is in $e (U) \subseteq \uparrow_C e (U)$.
% \item In the extremal epi / mono case, we must show that for any
%   subset $\mathcal U$ of $\td (\quot C \equiv)$, if ${(\td q)}^{-1}
%   (\mathcal U)$ is upward-closed then so is $\mathcal U$.  Let $U$ be
%   any element of $\mathcal U$, and $U$ be lower than $U'$ (in the $\supseteq$
%   ordering), i.e., $U' \subseteq U$.  Since, as we have seen earlier, $\td q$
%   is surjective, there are two upward-closed subsets of $A$ such that
%   $\td q (V) = U$ and $\td q (V') = U'$.  Recall that we could in fact
%   define $V = q^{-1} (U)$, $V' = q^{-1} (U')$.  Then $V' \subseteq V$.  Since
%   $V$ is in ${(\td q)}^{-1} (\mathcal U)$, and the latter is
%   upward-closed (in the $\supseteq$ ordering), $V'$ is also in ${(\td q)}^{-1}
%   (\mathcal U)$.  This means that $\td q (V')$ is in $\mathcal U$,
%   therefore $\mathcal U$ is upward-closed.
% \end{itemize}
% Define the strong monad morphism as mapping $U \in td {\funbara A_0}$ to
% $\lambda f \cdot [A \to \mathbf 2] \cdot U \Subset f^{-1} (1)$, where $U \Subset V$ if
% and only if $U \subseteq \uparrow_A E \subseteq V$ for some finitary subset $\uparrow_A E$ of $A$.
% We let the interested reader check all the details.  The role of $\uparrow_E
% E$ in the definition is to make the above functional continuous.
% It can be checked that $\lift S$ now relates %!!!
% % $U$ is mapped to 

\ifmscs
\else

\subsection{Fun With Categories~III: The Case $\catc=\FS$, $\catd=\Top$}
\label{sec:top}

This can be repaired by choosing another category for $\catd$, which
will keep all necessary information related to continuity.  The
obvious choice is $\Top$, the category of topological spaces.  One of
the novelties here is that for one choice of mono factorization, the
pseudoepis won't be surjective maps.  Another one is that we shall see
cases where $\td$ maps relevant pseudoepis to pseudoepis but does not
preserve pseudoepis.

Before we delve into the subject proper, we must note that choosing
$\catd=\Top$ incurs several problems.

First, $\Top$ is not cartesian closed.  This is not too serious.  We
can for example define a logical relation at arrow types $\tau_1 \to \tau_2$
that would be defined only when the denotation of $\tau_1$ is {\em
  exponentiable\/}.  Recall that a topological space $X$ is
exponentiable if and only if the exponential object $\ihom X Y$ exists
for every topological space $Y$.  It is well-known that the
exponentiable spaces are exactly the {\em core-compact\/} spaces
\cite{EH:topfun}, i.e., those whose lattice of opens is continuous.
In particular, every continuous cpo is locally compact, hence
core-compact, when seen as a topological space.  Another possibility
is to replace $\Top$ by one of its cartesian-closed subcategories
$\Top_{\mathcal C}$, of which there are many: Day's Theorem indeed
states that, given any class $\mathcal C$ of topological spaces, the
category $\Top_{\mathcal C}$ of so-called $\mathcal C$-generated
spaces, with continuous maps as morphisms, is cartesian-closed as soon
as $\mathcal C$ is a productive class.  See \cite{ELS:CCC:Top} for
details.  Examples of productive classes include continuous cpos ({\em
  domain generated spaces\/}), or compact spaces ({\em compactly
  generated spaces\/}).  In all these cases, $\Top_{\mathcal C}$ is
coreflective in $\Top$, meaning that there is a functor $\mathcal C :
\Top \to \Top_{\mathcal C}$ that is right adjoint to the inclusion
functor $\subseteq$ from $\Top_{\mathcal C}$ into $\Top$.  This immediately
implies that any mono factorization system on $\Top$ transports to one
on $\Top_{\mathcal C}$: if $\xymatrix@-5pt{A \ar[r]^f & B}$ in
$\Top_{\mathcal C}$ factors as $\xymatrix@-5pt{A \arrepixy[r]^e & C
  \arrmonoxy[r]^m & B}$ in $\Top$, then it factors as
$\xymatrix@-5pt{A \arrepixy[r]^e & {\mathcal C} (C) \arrmonoxy[r]^m &
  B}$ in $\Top_{\mathcal C}$, and $m$ is clearly again a mono in
$\Top_{\mathcal C}$.  Since product $\times_{\mathcal C}$ in
$\Top_{\mathcal C}$ is given by $A \times_{\mathcal C} B = \mathcal C (A \times
B)$ \cite[Section~5]{EH:topfun}, the adjunction $\subseteq \dashv \mathcal C$ is
monoidal: $\mathcal C$ preserves product on the nose.  It follows that
we can transport a strong monad on $\Top$ to one on $\Top_{\mathcal
  C}$, gaining a cartesian-closed structure along the way.
\ifmscs
(This is made explicit in \cite[Section~8]{GLN02}.)
\else
\fi

We will refrain from doing so {\em explicitly\/}, since we wouldn't
learn much.  We shall therefore concentrate on the $\Top$ case.  Note
in passing that, taking $\mathcal C$ consisting of just the Sierpi\'nski
space $\mathbf 2$, $\Top_{\mathcal C}$ will be the category of
Alexandroff spaces \cite[Example (2)]{EH:topfun}, which is equivalent
to $\ordcat$; in other words, taking $\mathcal C = \{\mathbf 2\}$ gives
back the construction of Section~\ref{sec:c!=d}.

% example: types arising from a CPS?
% otherwise, use a coreflective subcategory of \Top which is CCC.

Second, the product of cpos in $\Top$ does not coincide with their
product in $\Dcpo$.  Precisely, any cpo $A$ defines a topological
space $\funbara A$, where $A$ is equipped with its Scott topology.
But the product topology, i.e., that of $\funbara A \times \funbara B$, is
in general strictly coarser than the Scott topology on the product,
i.e., the topology on $\funbara {A \times B}$.  The obvious choice of
mediating morphism $\tstr A B : \funbara A \times \funbara B \to \funbara {A
  \times B}$, namely the identity map, will therefore fail to be continuous
in general.  We repair this by considering $\catc$ to be some
cartesian-closed subcategory of continuous cpos, instead of the whole
of $\Dcpo$.  Indeed, in this case it is well-known that the Scott
topology and the product topologies agree: $\funbara A \times \funbara B =
\funbara {A \times B}$.

There are many choices for $\catc$, then.  The first, historically, is
the category of Scott domains, i.e., algebraic bounded-complete cpos.
Other candidates are Jung's category $\FS$ of FS-domains, or that
$\CL$ of continuous L-domains \cite{Jung:CCC}.  We observe that $\tc
A$ is an FS-domain as soon as $A$ is, because $\tc A$ is a closed
subset of $[[A \to \mathbf 2] \to \mathbf 2]$, and closed subsets of
FS-domains are again FS-domains.  So $\tc$ defines a monad on $\FS$.
We shall therefore use $\catc=\FS$ is the rest of this section.  It
won't be necessary to know exactly what FS-domains really are.  The
interested reader is refered to \cite{Jung:CCC}.
%  Another argument
%is that since $A$ is a continuous cpo, $\funbara A$ is a sober topological space

We take the corresponding monad $\td$ on $\catd = \Top$ as follows.
Let $\td A$ be the set of continuous linear non-trivial second-order
predicates on $A$, just as $\tc A$, but equipped with the weak
topology instead of the Scott topology.  The {\em weak topology\/} is
the topology generated by the basis of opens $\Box O = \{F \in \td A | F
(\chi_O) = 1\}$, where $\chi_O$ is the indicator function of the open $O$ of
$A$.  Note in passing that {\em any\/} $f \in [A \to \mathbf 2]$ must be
of the form $\chi_O$ for some open $O$ of $A$.  Our choice of the weak
topology is justified by the fact that $\td$ will preserve pseudoepis
(condition {\bf (iv)}), see below.

The weak topology is in general coarser than the Scott topology, which
thwarts the existence of a monad morphism $\dist A : \td {\funbara A}
\to \funbara {\tc A}$.  (The identity map does not fit, as it would fail
to be continuous.)  However, when $A$ is a continuous cpo, the two
topologies coincide---another good reason to take $\catc$ to consist
solely of continuous cpos.  The classical argument is as follows.
Since $\tc A$ is a continuous cpo, its Scott topology has a basis
consisting of opens of the form $\uuarrow F$, where $F \in \tc A$,
$\uuarrow F = \{G \in \tc A | F \ll G\}$, and $\ll$ is the usual way-below
relation: $F \ll G$ if and only if every directed family whose supremum
is above $G$ contains an element above $F$.  By the Hoffman-Mislove
theorem, we may equate linear functionals with upward-closed compacts,
and then $Q \ll Q'$ if and only if the interior $\interior Q$ of $Q$
contains $Q'$.  Then $\uuarrow Q = \{Q' | Q' \subseteq \interior Q\} = \Box
\interior Q$ is a weak open.
%   A more direct proof, not going through
% the Hofmann-Mislove theorem, proceeds as follows.  Write $\interior F$
% the union of all opens $O$ of $A$ such that $O \subseteq O'$ for every open
% $O'$ such that $F (\chi_{O'})=1$.  We claim that: $(*)$ $F \ll G$ if and
% only if $G (\chi_{\interior F})=1$.  The if direction is clear: if the
% supremum of the directed family ${(F_i)}_{i\in I}$ is above $G$, then
% for some $i \in I$, $F_i (chi_{\interior F})=1$; so for all opens $O'$
% of $A$, if $F (\chi_{O'})=1$, that is if $\interior F \subseteq O'$, then $F_i
% (\chi_{O'})=1$; in other words, $F \leq F_i$, so $F \ll G$.  Conversely,
% assume $F \ll G$ and consider the family of functions $F_O$
% defined as mapping $\chi_{O'}$ to $1$ if and only if $O \subseteq O'$.
% Consider
%the directed family of all opens $O'$ such that $F (\chi_{O'}) = 1$.
It follows that, when $A$ is continuous, the identity map from $\td
{\funbara A}$ to $\funbara {\tc A}$ is continuous, and therefore
defines a monad morphism from $\tc$ to $\td$.

Now we have at least {\em four\/} mono factorization systems on
$\Top$:
\begin{enumerate}
\item The trivial mono factorization system, which is, as usual,
  uninteresting.
\item The epi / regular mono factorization.  This is close to the
  corresponding one in $\Dcpo$ or in $\ordcat$: regular monos are
  embeddings of closed subsets (i.e., $m : \xymatrix@-5pt{C
    \arrmonoxy[r] & B}$ is a regular mono if and only if $m$ is a
  homeomorphism onto a closed subset of $B$), and epis are continuous
  maps with dense image.  Note that $e : A \to C$ is epi if and only if
  $C$ equals the closure of $e (A)$ in $C$, or equivalently, $e^{-1}
  (V)$ is non-empty for every non-empty open $V$ of $C$.
\item The extremal epi / mono factorization.  This is much simpler to
  describe as in $\Dcpo$, and is similar to $\ordcat$.  The monos are
  just the injective continuous maps, while the extremal epis are the
  quotient maps.  A {\em quotient map\/} $\xymatrix@-5pt{A
    \arrepixy[r]^q & C}$ is by definition the map sending $x \in A$ to
  its equivalence class in $C = \quot A \equiv$, for some equivalence
  relation $\equiv$ on $A$.  (Again, up to postcomposition with isos.)
  Equivalently, $q$ is a quotient map if and only if $q$ is surjective
  and, for every subset $V$ of $C$, $V$ is open in $C$ if and only if
  $q^{-1} (V)$ is open in $A$.
% This implies that q is surjective: no, take A = \{*\}, C = \{1, 2\},
% with the discrete topologies, and q map * to 1.
%% If y in C, and y \not\in q(A), then q^{-1} \{y\} is empty hence open,
%% so \{y\} is open in C.
%% if y \leq y' then y'=y, so y is maximal in C.
%% The complement of q(A) is the union of \{y\}s, so is open.  So q(A) is closed in C.
%% On the other hand, q^{-1} (q (A)) = A is open, so q(A) is open in C.
\item What we shall call the {\em intermediate\/} mono factorization:
  the pseudoepis are the continuous surjective maps, and the relevant
  monos are the embeddings of subspaces (i.e., $m : \xymatrix@-5pt{C
    \arrmonoxy[r] & B}$ is an embedding, that is, a homeomorphism onto
  some subspace, not necessarily closed, of $B$).
\end{enumerate}


All of these are candidates for our construction.  As usual, the main
property to check is that $\td$ should preserve pseudoepis, or at
least map relevant pseudoepis to pseudoepis.

\textbf{Epi / regular mono factorization.}  Let $e$ be a pseudoepi
from $A$ to $C$, that is, an epi: for every non-empty open $V$ of $C$,
$e^{-1} (V)$ is non-empty.  It suffices to show that ${\td e}^{-1} (\Box
O)$ is non-empty for any non-empty open $O$ of $C$.  (This is the
point in choosing to equip $\td C$ with the weak topology.)  Now ${\td
  e}^{-1} (\Box O)$ is the set of all $F \in \td A$ such that $\lambda f \in [C \to
\mathbf 2] \cdot F (f \circ e)$ is in $\Box O$, i.e., such that $F (\chi_O \circ e) =
1$, or equivalently $F (\chi_{e^{-1} (O)}) = 1$.  By assumption, $e^{-1}
(O)$ is non-empty: let $x \in e^{-1} (O)$, then $F = \unitd A (x) = \lambda f
\in [A \to \mathbf 2] \cdot f (x)$ is in ${\td e}^{-1} (\Box O)$.

Condition {\bf (iv)} obtains.  We also have to check condition {\bf
  (iii.a)}, that this mono factorization system is monoidal.  But
products of epis are always epi, so this is clear.

\textbf{Intermediate mono factorization.}  Here pseudoepis are
surjective continuous maps.  This is one case where $\td$ does {\em
  not\/} preserve pseudoepis.  Take $A=\nat$ with the discrete
topology, and $C=\nat$ with the cofinite topology, whose opens are $\emptyset$
and all complements of finite sets of integers.  Now consider $e : A \to
C$ the identity map.  Since the topology of $A$ is finer than that of
$C$, $e$ is continuous; $e$ is also clearly surjective.  We claim that
$\td e$ is not surjective.  It is an easy exercise to show that the
elements of $\td A$ are all of the form $\lambda f \in [A \to \mathbf 2] \cdot E \subseteq
f^{-1} \{1\}$, where $E$ is some finite non-empty subset of $A$.  (And
this comes from free if we consider that $A$ is sober, from the
correspondence between $\td A$ and $\mathcal Q (A)$, and the fact
that the upward-closed compacts of $A$ are the finite subsets $E$ of
$A$.)  Now consider the functional $G \in \td C$ that maps $f \in [C \to
\mathbf 2]$ to $1$ if $f$ is not identically $0$, and maps the zero
function to $0$.  $G$ is trivially continuous, and preserves $\top$.
That $G$ preserves binary infima rests on the fact that the
intersection of any two non-empty opens is again non-empty in $C$.
Assume now that $G$ is the image by $\td e$ of some functional $\lambda f \in
[A \to \mathbf 2] \cdot E \subseteq f^{-1} \{1\}$, in other words, $G = \lambda g \in [C \to
\mathbf 2] \cdot E \subseteq {(g \circ e)}^{-1} \{1\}$.  For any integer $n \in \nat$, $G
(\chi_{C \setminus \{n\}})=1$, so $E$ cannot contain $n$; i.e., $E$ is empty, a
contradiction.
%; but then $G (\chi_\emptyset)$ would equal $1$, not $0$.

However, $\td$ maps {\em relevant\/} pseudoepis to pseudoepis.  The
crucial, albeit trivial, observation is:
\begin{fact}
  \label{fact:td:relmono}
  If $\td$ preserves relevant monos and $\dist A$ is a relevant mono,
  then all relevant pseudoepis are iso.  In particular, $\td$ maps
  relevant pseudoepis to isos, hence to pseudoepis.
\end{fact}
Indeed, a relevant pseudoepi is the pseudoepi part of the
factorization of $\dist A \circ \td m$, where $m$ is a relevant mono.
Since by assumption $\dist A \circ \td m$ is a relevant mono, we conclude
by uniqueness of factorizations up to iso.

In our case, $\dist A$ is the identity map between $\td {\funbara A}$
and $\funbara {\tc A}$; remember these two coincide because the Scott
topology agrees with the weak topology on continuous cpos.  It remains
to show that $\td m$ is a relevant mono as soon as $m : C \to B$ is.
Remember that a relevant mono $m$ is a homeomorphism onto its image,
i.e., an injective, continuous and open map.  $\td m$ is continuous.
It is injective, too: if $\td m (F) = \td m (F')$, then for every open
$O'$ of $A$, $F (\chi_{0'} \circ m) = F' (\chi_{0'} \circ m)$.  In particular, for
every open $O$ of $C$, taking $O' = m (O)$ (since $m$ is an open map),
$F (\chi_{m (O)} \circ m) = F' (\chi_{m (O)} \circ m)$.  Now $\chi_{m (O)} \circ m =
\chi_{m^{-1} (m (O))} = \chi_O$ since $m$ is injective, so $F (\chi_0) = F'
(\chi_O)$: so $F=F'$.  Finally, $\td m$ is open.  Since $\Box O \cap \Box O' = \Box
(O \cap O')$, the sets $\Box O$ form a basis of the weak topology, that is,
every open subset of $\td C$ is a union $\bigcup_{i\in I} \Box O_i$.  It is easy
to check that $\td m (\bigcup_{i\in I} \Box O_i)$ equals $\bigcup_{i\in I} \Box m (O_i)$,
which is clearly open.  So $\td m$ is a relevant mono.

We have therefore established condition {\bf (iv)}: $\td$ maps
relevant pseudoepis to pseudoepis, although $\td$ does not map
pseudoepis to pseudoepis.

To lift the cartesian structure to the subscone, we also have to check
condition {\bf (iii.a)}, that this mono factorization system is
monoidal.  This is again clear: the product of two surjective
continuous maps is again surjective and continuous.

%!!! Note that this won't work in the binary case.

\textbf{Extremal epi / mono factorization.}  Since $\td$ does not
preserve surjective maps, it is unlikely that it will preserve
extremal epis.  Moreover, Fact~\ref{fact:td:relmono} does not apply,
since $\td$ does not preserve injective maps.  Take indeed $m : C \to B$
be the identity from $C=\nat$ with the discrete topology, to $B=\nat$
with its Alexandroff topology.  Then $\td m$ maps $\lambda f \cdot \{2\} \subseteq f^{-1}
\{1\}$ and $\lambda f \cdot \{2,3\} \subseteq f^{-1} \{1\}$ to the same element $\lambda g \cdot \{2\} \subseteq
g^{-1} \{1\}$, because for any Alexandroff-continuous (i.e., monotone)
function $g : B \to \mathbf 2$, $g (2)=1$ if and only if $g (2)=g(3)=1$.

% However we can again conclude that $\td$ will map
% relevant pseudoepis to pseudoepis, by Fact~\ref{fact:td:relmono}.  So
% condition {\bf (iv)} again holds.

% The problematic condition in the extremal epi / mono setting is
% condition {\bf (iii.a)}, that products of pseudoepis should be
% pseudoepi.  It is well-known that this is equivalent to the condition
% that products of a pseudoepi with an identity map should be pseudoepi
% \cite[Definition~5.2.1]{SJA:thesis}.  In $\Top$, this would mean that
% $q \times \identity B : A \times B \to C \times B$ should be quotient whenever $q : A \to C$ is
% quotient.  However this property is actually equivalent to $B$ being
% exponentiable, that is, core compact.  See for example
% \cite[Lemma~2.6]{ELS:CCC:Top}.  This is easily repaired by considering
% $\catd$ to be the CCC $\Top_{\mathcal C}$ instead of $\Top$ (where
% $\mathcal C$ is productive): by \cite[Theorem~5.4, (i)]{ELS:CCC:Top},
% for every $\mathcal C$-generated spaces $A$, $B$, $C$, if $q : A \to C$
% is quotient (in $\Top$) then $q \times \identity B : A \times_{\mathcal C} B \to C
% \times_{\mathcal C} B$ is quotient.  Now we recall that, in $\Top_{\mathcal
%   C}$, pseudoepis are of the form $\xymatrix@-5pt{A \arrepixy[r]^q &
%   {\mathcal C} (C)}$ where $q$ is an extremal epi, i.e., a quotient
% map (in $\Top$).  By definition $C$ is a quotient of a $\mathcal
% C$-generated space, so it is $\mathcal C$-generated by
% \cite[Lemma~3.2, (ii)]{ELS:CCC:Top}, therefore ${\mathcal C} (C) = C$.
% We have just shown that pseudoepis in $\Top_{\mathcal C}$ were just
% quotients (in $\Top$), and that the resulting quotient / continuous
% injection factorization on $\Top_{\mathcal C}$ is monoidal.

% In other words, working in $\Top_{\mathcal C}$ instead of $\Top$
% solves many problems, at the price of some complications.

\vskip1em

Let us now consider the form of binary logical relations in the above
topological settings.  Again, we look at each available mono
factorization.  We will not consider the extremal epi / mono
factorization.  We will in fact also avoid the intermediate mono
factorization system.  In the intermediate system, $\td$ does not
preserve pseudoepis, and Fact~\ref{fact:td:relmono} does not apply,
because $\dist {A_1, A_2}$ will not be a relevant mono in general.

In the binary case, $\funbara {A_1, A_2} = A_1 \times A_2$ (there is no
ambiguity in writing $\times$ here, as products of continuous cpos coincide
with topological products), and for every FS-domains $A_1$ and $A_2$,
$\dist {A_1, A_2}$ maps $F \in \td (A_1 \times A_2)$ to the pair of maps $\lambda
f_1 \in [A_1 \to \mathbf 2] \cdot F (f_1 \circ \pi_1)$ and $\lambda f_2 \in [A_2 \to \mathbf
2] \cdot F (f_2 \circ \pi_2)$.  Here $\pi_1$ and $\pi_2$ denote first and second
projections, respectively.

\textbf{Epi / regular mono factorization, binary case.}  A binary
relation $\xymatrix@-5pt{S \arrmonoxy[r]^m & {A_1 \times A_2}}$ between
$A_1$ and $A_2$ is, up to iso, a closed subset $S$ of $A_1 \times A_2$.  It
is easy to check that our construction builds a lifted relation $\lift
S$ between $\td A_1$ and $\td A_2$ defined by $(F_1, F_2) \in \lift S$
if and only if $(F_1, F_2)$ is in the closure of the set
\begin{eqnarray}
  \label{eq:liftS0}
  \lift S_0 & = &
  \Bigg\{(G_1, G_2) \in \td A_1 \times \td A_2 | \exists G \in \td S \cdot \\\nonumber
  && \qquad \phantom{\land}
  \forall f_1 \in [A_1 \to \mathbf 2] \cdot G_1 (f_1) = G (\lambda (x_1, x_2) \in S \cdot f_1 (x_1)) \\\nonumber
  && \qquad \land
  \forall f_2 \in [A_2 \to \mathbf 2] \cdot G_2 (f_2) = G (\lambda (x_1, x_2) \in S \cdot f_2 (x_2))
  \Bigg\}
\end{eqnarray}
It is easier to understand this through the Hofmann-Mislove isomorphism.
Any element $G_i$ of $\td A_i$ can be written as $\lambda \chi_O \cdot Q_i \subseteq O$
for some non-empty compact upward-closed subset $Q_i$ of $A_i$, $i=1,2$.
Similarly $G$ corresponds to some non-empty compact upward-closed subset $Q$ of $S$.
% Since $S$ is closed, the latter are exactly the non-empty intersections $Q \cap S$ of
% compact upward-closed subsets $Q$ of $A_1 \times A_2$ with $S$.
The condition $\forall f_1 \in [A_1 \to \mathbf 2] \cdot G_1 (f_1) = G (\lambda (x_1, x_2)
\in S \cdot f_1 (x_1))$ is then equivalent to: for every open subset $O_1$
of $A_1$, $Q_1 \subseteq O_1$ if and only if $Q \subseteq (O_1 \times A_2) \cap S$.  Since the
upward-closed subsets of a topological space are exactly those that
are the intersection of all opens containing them, this is equivalent
to $Q \subseteq (Q_1 \times A_2) \cap S$.  Summing this up,
\begin{eqnarray*}
  \lift S_0 & = & \{(\lambda \chi_O \cdot Q_1 \subseteq O, \lambda \chi_O \cdot Q_2 \subseteq O) | \\
  && \quad \exists Q \mbox{ non-empty compact upward-closed subset of }S
  \cdot Q \subseteq (Q_1 \times Q_2) \cap S\}
\end{eqnarray*}
By Tychonoff's Theorem, $Q_1 \times Q_2$ is compact, so $(Q_1 \times Q_2) \cap S$
is compact since $S$ is closed.  Since $Q_1 \times Q_2$ is upward-closed in
$A_1 \times A_2$, $(Q_1 \times Q_2) \cap S$ is upward-closed in $S$, so in fact
$\lift S_0$ consists of those pairs $(\lambda \chi_O \cdot Q_1 \subseteq O, \lambda \chi_O \cdot Q_2 \subseteq
O)$ such that $(Q_1 \times Q_2) \cap S$ is non-empty.  In other words, and up
to the Hofmann-Mislove Theorem, $\lift S_0$ relates those compacts
$Q_1$ and $Q_2$ such that $Q_1$ contains an element $x_1$ and $Q_2$
contains $x_2$ so that $(x_1, x_2)$ are related by $S$.

Remember, then, that $\lift S$ is the topological closure of $\lift
S_0$.  However, we claim that $\lift S_0$ is closed in the weak
topology.  To show this, it is enough to show that $\lift S_0$ is
Scott-closed, since the weak topology and the Scott topology coincide
on $\td A$ for any continuous cpo $A$.  First, $\lift S_0$ is
downward-closed (with respect to the product $\supseteq \times \supseteq$ of reversed
inclusion).  Second, if $(Q_{1i}, Q_{2i})$, $i\in I$, forms a directed
family (wrt.\ $\supseteq$) of pairs of non-empty compact upward-closed subsets
such that $(Q_{1i} \times Q_{2i}) \cap S \neq \emptyset$ for all $i$, we note that
${((Q_{1i} \times Q_{2i}) \cap S)}_{i\in I}$ forms a directed family of
non-empty compact subsets of $A_1 \times A_2$, because $S$ is closed in
$A_1 \times A_2$.  Since $A_1 \times A_2$ is sober, its least upper bound (its
intersection) is again non-empty and compact, see e.g.,
\cite[Corollary~7.2.11]{AJ:domains}.  It follows that $\left(\bigcap_{i\in I}
  Q_{1i} \times \bigcap_{i\in I} Q_{2i}\right) \cap S = \bigcap_{i\in I} (Q_{1i} \times Q_{2i}) \cap
S$, so the least upper bound $\bigcap_{i\in I} Q_{1i} \times \bigcap_{i\in I} Q_{2i}$ is
again in $\lift S_0$.  We conclude that $\lift S_0$ is Scott-closed,
hence closed, so that $\lift S = \lift S_0$.

Note that $\lift S$ does {\em not have the form of a bisimulation
  relation\/}; rather, $Q_1$ and $Q_2$ are related by $\lift S$ if and
only if $Q_1$ and $Q_2$ have related refinements, where a {\em
  refinement\/} $x$ of a compact $Q$ is an element $x \in Q$, i.e., if
$\uparrow x$ is an element above $Q$ in $\mathcal Q (X)$.

Transposing this back to the realm of functionals, we see that $(G_1,
G_2) \in \lift S$ if and only if there is a refinement $x_1$ of $G_1$,
i.e., an element $x_1$ of $A_1$ such that $G_1 \leq \unitd {A_1} (x_1)$,
and a refinement $x_2$ of $G_2$ such that $(x_1, x_2) \in S$.

It would have been tempting to guess that $\lift S$ would be
characterized by the following relation $\widehat{\widehat S}$, in the
style of observational equivalence.  Define $\widehat S$ as the set of
all $(f_1, f_2)$ such that whenever $(x_1, x_2) \in S$ then $f_1 (x_1) =
f_2 (x_2)$; then $\widehat {\widehat S}$ is the set of $(G_1, G_2)$
such that whenever $(f_1, f_2) \in \widehat S$, $G_1 (f_1)=G_2 (f_2)$.
Clearly, $(G_1, G_2) \in \lift S_0$ implies $(G_1, G_2) \in
\widehat{\widehat S}$.  However, the converse does not seem to hold.


% Conversely, if $(G_1, G_2) \in
% \widehat{\widehat S}$, then writing $G_1$ as $\lambda \chi_O \cdot Q_1 \subseteq O$ and
% $G_2$ as $\lambda \chi_O \cdot Q_2 \subseteq O$, whenever $(\chi_{O_1}, \chi_{O_2}) \in \widehat S$,
% then $Q_1 \subseteq O_1$ if and only if $Q_2 \subseteq O_2$.



% An alternative characterization of $\lift S_0$ is as we should expect:
% define   The difficult direction is that show that if $G_1
% (f_1)=G_2 (f_2)$ for every $(f_1, f_2) \in \widehat S$, then $(G_1, G_2)
% \in \lift S_0$.  The easiest way is to rely on the Hofmann-Mislove
% theorem again.  Let $Q_1$, $Q_2$ the non-empty compact upward-closed
% subsets associated with $G_1$, $G_2$ respectively: $Q_i =
% \bigcap_{\substack{O\mbox{\footnotesize{} open of }A_i\\G_i (\chi_O)=1}} O$,
% and conversely $G_i$ maps $\chi_{O_i} \in [A_i \to \mathbf 2]$ to the
% truth-value of $Q_i \subseteq O_i$.  By Tychonoff's theorem, $Q_1 \times Q_2$ is
% compact, so $Q = (Q_1 \times Q_2) \cap S$ is compact, since $S$ is closed.
% Let $G \in \td S$ map $\chi_O \in [S \to \mathbf 2]$ to the truth-value of $Q \subseteq
% O$.

% To show that $G$ fits, we observe that for every $x_1 \in Q_1$, there is $x_2 \in Q_2$ such that $(x_1, x_2) \in S$.

% For every $f_1 = \chi_{O_1} \in [A_1 \to \mathbf 2]$, $G_1 (f_1)=1$
% if and only if $Q_1 \subseteq O_1$.  On the other hand, $G (\lambda (x_1, x_2) \in S \cdot f_1 (x_1))=1$
% if and only if $Q \subseteq (O_1 \times A_2) \cap S$.


% follows.  Fix any $f = \chi_O \in [S \to \mathbf 2]$,
% where $O$ is an open subset of $S$.  Since the inclusion $S \subseteq A_1 \times A_2$ is an embedding,
% $O$ is of the form $O' \cap S$ for some open $O'$ of $A_1 \times A_2$.
% Since $A_1$ and $A_2$ are continuous cpos, the Scott-topology on $A_1 \times A_2$ agrees with the product topology,
% so $O'$ is a union $\bigcup_{i\in I} O_{1i} \times O_{2i}$ of products of opens of $A_1$ and of $A_2$ respectively.
% Define $G (f)$ as $1$ if and only if 

% \textbf{Intermediate mono factorization.}  Here pseudoepis are
% surjective, so we do not need to mess around with closures.  In other
% words, $\lift S$ is directly given by the formula (\ref{eq:liftS0})
% above.  However, $S$ is no longer a closed subset of $A_1 \times A_2$ in
% general: in the intermediate mono factorization, relations $S$ are any
% subsets, not necessarily closed, with the topology induced by $A_1 \times
% A_2$ (up to iso).  Remember that the fact that $S$ was closed was
% crucial in our above argument that $(G_1, G_2) \in \lift S$ meant the
% existence of $S$-related refinements for $G_1$ and $G_2$.

% But we are going too fast.  To merely show that our construction
% applies again, we should check condition {\bf (iv)}, namely that $\td$
% maps relevant pseudoepis to pseudoepis.  We have seen that $\td$ did
% not preserve pseudoepis in general.  Moreover, $\dist {A_1, A_2}$ is
% not a relevant mono in general, so Fact~\ref{fact:td:relmono} does not
% apply.  We need another argument.

% Recall that by the Hofmann-Mislove theorem, we may equate continuous
% linear functionals $F$ with upward-closed compact subsets $Q$ of $A$.
% Through this isomorphism, the image of $Q$ by $\td e$, where $e : A \to
% C$, is $\uparrow_C e (Q)$.  When $e$ is surjective, it is tempting to attempt
% to show that $\td e$ is surjective by taking as antecedent of the
% upward-closed compact subset $Q'$ of $C$, the subset $e^{-1} (Q')$.
% However, there is no reason why this should be compact, unless $e$ is
% proper.

% However, we claim that $\td$ maps {\em relevant\/} pseudoepis to
% pseudoepis.  This requires some domain theory.  Let $\Subset$ denote
% the way-below relation on Scott-open subsets of a cpo $A$.  By
% \cite[Proposition~4.2.15]{AJ:domains}, if $A$ is a continuous cpo,
% then $O \Subset O'$ if and only if $O \subseteq Q \subseteq O'$ for some upward-closed
% compact subset $Q$ of $A$.  Also, FS-domains are coherent
% \cite[Theorem~4.2.18]{AJ:domains}, i.e., $O \Subset O_1 \cap O_2$ if and
% only if $O \Subset O_1$ and $O \Subset O_2$.

% Let $e : \td S \to \lift S$
% be a relevant pseudoepi.  This means
% that there is an FS-domain $A$,
% and an embedding $f$ of $S$ into $\funbara A$,
% such that $e$ is the pseudoepi part
% of a factorization of $\dist A \circ \td f : \td S \to 
% \funbara {\tc A}$.  Up to iso, equate $S$ with a subset of $\funbara A$, equipped
% from the topology inherited from $A$: the open subsets $U$ of $S$ are exactly
% the intersections $O \cap S$, where $O$ ranges over the open subsets of $A$.
% For any %!!!

% Let then $e : A \to C$ be a relevant pseudoepi in $\Top$.  In
% particular, $A$ is an FS-domain

% %Lawson-compact \cite[Text before Theorem~4]{Jung:CCC2},
% and that 

% Let $e$ be a continuous
% surjective map.  Let %!!!

% %!!! FS-domains are Lawson-compact \cite{Jung:CCC2}, just before Theorem~4.
% % And Lawson-compact = stably compact for a domain (continuous cpo).

% Let $G$ be any element of $\td C$, and define $F$ by
% $F (\chi_O) = \sup_{V / e^{-1} (V) \subseteq O} G (\chi_V)$, i.e., $F$ maps $\chi_O$ to
% $1$ if and only if $G (\chi_V)$ for some open $V$ of $C$ such that
% $e^{-1} (V) \subseteq O$.  We claim that $F$ is in $\td A$ and $\td e (F) =
% G$, which will show that $\td e$ is surjective, too.
% First, $F \in \td A$.

% $\td e$ maps $F \in \td A$ to $\lambda f \in [C \to
% \mathbf 2] \cdot F (f \circ e)$

% %!!!

% However, $(*)$ helps in showing that $\td q$ is, indeed, surjective.

% %!!!

% However, we claim that, given that $q$ is continuous, $q$ is quotient
% if and only if $q$ is {\em epi\/} and satisfies $(*)$.  Since every
% surjective map is epi, we have to show that $q$ is surjective whenever
% $q$ is epi and satisfies $(*)$.  That $q$ is epi means that the
% closure $cl (q (A))$ in $C$ is the whole of $C$.  Consider the
% complement $V$ of $q (A)$ in $C$.  Clearly $q^{-1} (V)$ is empty,
% hence open.  By $(*)$, $V$ is open, hence $q (A)$ is closed in $C$.
% So $cl (q (A)) = q (A)$.  It follows that $q (A)=C$, so $q$ is
% surjective.

% We already know (see above) that $\td$ maps epis to epis.  To show
% that $\td$ maps pseudoepis to pseudoepis, let $q$ be quotient, let
% $\mathcal V$ be any subset of $\tc C$ such that ${(\td q)}^{-1}
% (\mathcal V)$ is open in $\td A$.  So ${(\td q)}^{-1} (\mathcal V)$ is
% a union $\bigcup_{i\in I} \Box O_i$, where $O_i$ is open in $A$.  Then for every
% $F \in \td A$, $\td q (F) \in \mathcal V$ if and only if $F (\chi_{O_i})=1$
% for some $i \in I$.

%!!!


\subsection{Fun With Categories~IV: Metric Spaces}
\label{sec:metric}

Among the degrees of freedom afforded by our constructions, observe
that we have the option to consider categories that are not
cartesian-closed, but, say, just symmetric monoidal closed.

The categories of ultrametric spaces, and of complete ultrametric
spaces, are cartesian-closed.  It is even possible to equip these
categories with a probability monad.  The main difficulty is to show
that the space of all probability measures on an ultrametric space can
be equipped with a distance that makes it ultrametric.  See
\cite[Lemma~4.3]{dVR:proba:bisim}.  Let us take the stance of working
inside the larger category $\Met$ of metric spaces---for whatever
practical reason.  Our reason is to provide an example: we wish to
show how our construction works on the symmetric monoidal closed, but
not cartesian-closed, category $\Met$.

Precisely, we consider the category $\Met$ of metric spaces and
non-expansive maps. We write $d_A$ for the distance on $A$, and allow
distances to take the value $+\infty$.  (This is as in
\cite{Lawvere:metric}, who considers additional relaxations on the
notion of distance.)
In other words, a distance $d_A$ on $A$ is any function from $A$ to $\real_+
\cup \{+\infty\}$, such that $d_A (x,y) = 0$ if and only if $x=y$, for every
$x,y \in A$; $d_A (x,y) = d_A (y,x)$ for every $x,y\in A$; and $d_A (x,z) \leq
d_A (x,y) + d_A (y,z)$ for every $x,y,z \in A$.  A map $f$ is {\em
  non-expansive\/} from $A$ to $B$ if and only if $d_B (f (x), f (x')) \leq
d_A (x, x')$ for every $x, x' \in A$.

Every metric space $A$ has a topology, generated by its open balls
$\OBall x \epsilon = \{y | d_A (x, y) < \epsilon\}$, for which it is Hausdorff.  There
is a cartesian product on $\Met$: $A \times B$ is the set of pairs $(x,
y)$, $x \in A$, $y \in B$, with distance $d_{A \times B}$ defined by $d_{A \times B}
((x, y), (x', y')) = \max (d_A (x, x'), d_B (y, y'))$.  There is no
corresponding notion of exponential.

On the other hand, $\Met$ is symmetric monoidal closed.  The tensor
product $A \tensorc B$ is the set of pairs $(x, y)$, $x \in A$, $y \in B$,
with distance $d_{A \tensorc B}$ defined by $d_{A \tensorc B} ((x, y),
(x', y')) = d_A (x, x') + d_B (y, y')$.  The exponential $\ihom B C$
is the set of non-expansive maps $f$ from $B$ to $C$, with distance
$d_{\ihom B C} (f, f') = \sup_{x \in B} d_C (f (x), f' (x))$. (This is
well-defined because we allow distances to take the value $+\infty$.) The
underlying topology of $A \tensorc B$, as well as of $A \times B$, is the
product topology of $A$ and $B$.

As far as monads are concerned, we shall look at the probability monad
on $\Met$.  I.e., we consider general, not just discrete
probabilities.  This will provide a non-trivial example of our
construction.  A {\em measure\/} on $A$ is by convention a measure on
the Borel $\sigma$-algebra of its topology.  A {\em probability\/} measure
maps $A$ to $1$.  A natural choice for a probability monad $\mathcal
M_1$ on $\Met$ is to let $\mathcal M_1 (A)$ be the set of all
probability measures on $A$, equipped with the {\em Hutchinson
  metric\/}:
\[
d_{\tc A} (\pmb{\nu}, \pmb{\xi}) = \sup_{g \in \homset \Met A {[0, 1]}}
\left|
  \int_{x \in A} g (x) d\pmb{\nu} - \int_{x\in A} g (x) d\pmb{\xi}
\right|
\]
making $\mathcal M_1 (A)$ a metric space.  (Some call it the
Kantorovitch metric; one may also call it the $L^1$ metric.)  It can
be checked that $\mathcal M_1$ gives rise to a monoidal monad.  We
skip the details.

Now take $\catd = \catc = \Met$.  There is a natural epi-mono
factorization on $\Met$: relevant monos are {\em isometric
  embeddings}, that is, maps $m : C \to B$ such that $d_B (m (x), m (y))
= d_C (x, y)$ for all $x, y\in C$.  Pseudoepis from $A$ to $C$ are {\em
  surjective\/} non-expansive maps from $A$ to $C$. It is fairly easy
to see that this yields a monoidal mono factorization system on
$\Met$.

It is then tempting to choose $\td$ and $\tc$ to be $\mathcal M_1$,
but this would expose some difficulties.  Indeed, we know that
$\mathcal M_1$ preserves pseudoepis (condition {\bf (iv)}), that is,
surjective non-expansive maps, in some cases but not in general.
E.g., if $f$ is continuous surjective from $A$ to $B$, and both $A$
and $B$ are compact Hausdorff, then $\mathcal M_1 (f)$ is surjective
\cite[2.4, Lemma~1]{Bourbaki:int:IX}; similarly if the underlying
topological space of $A$ is an analytic space \cite[2.4,
Proposition~9]{Bourbaki:int:IX}.

Instead, we choose $\td$ as a continuation-like monad that is as close
to $\mathcal M_1$ as possible.  (Remember the $\mathcal Q$ and
$\mathcal U_*$ monads in $\Top$.)  Let $\cbf A$ be the vector space of
all bounded non-expansive functions from the metric space $A$ to
$\real$, with the sup norm: for all $g \in \cbf A$, $||g|| = \sup_{x\in A}
|g (x)|$.  Let ${\cal L}_A$ be the vector space of all continuous
linear forms on $\cbf A$, that is, of all continuous linear functions
$F : \cbf A \to \real$.  Recall that a linear function $F$ from $\cbf A$
to $\real$ is continuous if and only if it is Lipschitz, i.e., if and
only if $||F|| = \sup_{||g|| = 1} |F (g)|$ is a well-defined real
(i.e., not $+\infty$).  Then $||F||$ is called the {\em norm\/} of $F$.
Let ${\cal L}^1_A$ be the subset of those $F$ in ${\cal L}_A$ of norm
$1$.  Finally, let $\td A$ be the subset of those $F$ in ${\cal
  L}^1_A$ which are positive, i.e., such that $g \geq 0$ implies $F (g) \geq
0$.  Both ${\cal L}^1_A$ and $\td A$ inherit the distance on ${\cal
  L}_A$ that is induced by norm.  Equivalently, $\td A$ is a metric
space whose distance is defined by $d_{\td A} (F, G) = \sup_{g \in
  \homset \Met A {[-1, 1]}} |F (g) - G (g)|$.  $\td$ then defines an
endofunctor on $\Met$ by letting $\td f$ map $F \in \td A$ to $\lambda g \in
\cbf B \cdot F (g \circ f)$, for every non-expansive map $f$ from $A$ to $B$.

The space $\mathcal M_1 (A)$ of all probability measures on $A$ embeds
in $\td A$ by $\pmb{\nu} \mapsto \lambda g \in \cbf A \cdot \int_{x\in A} g (x) d\pmb{\nu}$.  In
fact, the distance on probability measures on $A$ inherited from the
metric structure on $\td A$ is a slight variant of the Hutchinson
metric introduced above.  Moreover, if $A$ is compact, then every
element of $\td A$ arises from a probability measure in this way, by
the Riesz Representation Theorem.  This makes $\td A$ a metric space
that is arguably close enough to a space of probability measures.

The point of this definition of $\td$ is that $\td$ preserves pseudoepis in
$\Met$.  The proof is similar to that of \cite[2.4, Lemma~1]{Bourbaki:int:IX}.
\begin{lemma}
  \label{lemma:td:met}
  If $f$ is any surjective non-expansive map from $A$ to $B$, then $\td f$ is
  surjective from $\td A$ to $\td B$.
\end{lemma}
\begin{proof}
  Let $\lambda_f$ be the function mapping $g \in \cbf B$ to $g \circ f$.  Note
  that $\lambda_f (g)$ is bounded and non-expansive, hence in $\cbf A$.  Also,
  $||\lambda_f (g)|| = \sup_{x \in A} |g (f (x))| = \sup_{y \in B} |g (y)|$
  (since $f$ is surjective) $= ||g||$, so that $\lambda_f$ is an isometric
  embedding of $\cbf B$ into $\cbf A$.
  
  Let $H$ be the range of $\lambda_f$ in $\cbf A$.  $H$ is a linear subspace
  of $\cbf A$, which is by construction isometrically isomorphic to $\cbf B$.
  In particular, $\lambda_f^{-1}$ is a continuous linear map from $H$ to $\cbf
  B$.
  
  Given $G \in \td B$, $G \circ \lambda_f^{-1}$ is therefore a continuous
  linear form on $H$.  By the Hahn-Banach Theorem, $G \circ \lambda_f^{-1}$
  can be extended to a continuous linear form $F$ on $\cbf A$, with the same
  norm, i.e., $||F|| = ||G \circ \lambda_f^{-1}||$.  The latter means that
  $||F|| = \sup_{h \in \cbf A, ||h||=1} |F (h)| = \sup_{h \in H, ||h||=1} |G
  (\lambda_f^{-1} (h))| = \sup_{g \in \cbf B, ||g \circ f|| = 1} |G (g)| =
  ||G|| = 1$.
  
  As far as positivity is concerned, we first note that $||G|| = G (\lambda y
  \in B \cdot 1)$.  Indeed, first, $||\lambda y \in B \cdot 1|| = 1$, so
  $||G|| \geq G (\lambda y \in B \cdot 1)$.  To show the converse inequality,
  note first that for every $g \in \cbf B$, we may write $g$ as the difference
  $g_+ - g_-$ of two positive functions, so $|G (g)| = |G (g_+) - G (g_-)|
  \leq \max (G (g_+), G (g_-))$ (since $G (g_+), G (g_-) \geq 0$); if
  $||g||=1$, then $g_+ (y) \leq 1$ and $g_- (y) \leq 1$ for all $y\in B$, so
  $|G (g)| \leq G (\lambda y \in B \cdot 1)$; taking the sup over all $g$,
  $||G|| \leq G (\lambda y \in B \cdot 1)$.
  
  Then $F (\lambda x \in A \cdot 1) = F (\lambda_f (\lambda y \in B \cdot 1))
  = G (\lambda y \in B \cdot 1)$.  So $F (\lambda x \in A \cdot 1) = ||G|| =
  ||F||$.  If $F$ was not positive, there would be some $g \in \cbf A$, $g
  \geq 0$, with $F (g) < 0$.  We may assume without loss of generality that $g
  \leq 1$, so $\lambda x \in A \cdot 1-g(x)$ is of norm at most $1$.  But then
  $||F|| \geq F (\lambda x \in A \cdot 1-g(x)) = F (\lambda x \in A \cdot 1) -
  F (g) > F (\lambda x \in A \cdot 1)$, a contradiction.  So $F$ is positive.

  Finally, $\td f (F) = \lambda g \in \cbf B \cdot F (g \circ f) = \lambda g
  \in \cbf B \cdot G (\eta (g \circ f)) = \lambda g \in \cbf B \cdot G (g) =
  G$.  Since $G$ is arbitrary, $\td f$ is surjective.
\end{proof}

$\td$ can be used to form a monoidal monad on $\Met$.  Define $\unitd
A$ as the function mapping $x \in A$ to $\lambda g \in \cbf A \cdot g (x)$.  This is
natural in $A$, and non-expansive in $x$.  Define $\multd A$ as
mapping $F \in \td^2 A$ to $\lambda g \in \cbf {\td A} \cdot F (\lambda G \in \td A \cdot G
(g))$.  It requires a bit more work to show that $\multd A$ is
well-defined and non-expansive in $F$; it is however clear that this
is natural in $A$.  Furthermore, the monad laws are satisfied, so that
$(\td, \unitd{}, \multd{})$ is a monad on $\Met$.  The strength $\strd
A B$ maps $(x, G) \in A \tensord \td B$ to $\lambda h \in \cbf {A \tensord B} \cdot
G (\lambda y \in B \cdot h (x, y))$.

\vskip1em

To define a notion of binary metric logical relations, we take $\catc = \Met
\times \Met$, define a monad $\tc$ on $\catc$ pointwise (i.e., $\tc (A_1, A_2)
= (\td A_1, \td A_2)$).  It remains to define a monad morphism from $\tc$ to
$\td$.

Define $\funbara {A_1, A_2}$ as the cartesian product $A_1 \times A_2$, much
as in $\catset$.  Note that the only difference between cartesian product and
tensor product is that their distances differ: $d_{A_1 \times A_2} ((x, y),
(x', y'))$ is the max of the distances $d_{A_1} (x, x')$ and $d_{A_2} (y,
y')$, while $d_{A_1 \tensord A_2} ((x, y), (x', y'))$ is the sum of the same
distances.

Similarly as in $\catset$, define the monad morphism $\dist {A_1,
  A_2}$ as $\langle \td \pi_1, \td \pi_2 \rangle$.  That is, for every $F \in \td (A_1 \times
A_2)$, $\dist {A_1, A_2} (F) = (\lambda g_1 \in \cbf {A_1} \cdot F (\lambda (x, y) \cdot g_1
(x)), \lambda g_2 \in \cbf {A_2} \cdot F (\lambda (x, y) \cdot g_2 (y)))$.  We let the
reader check all required properties.  Then $(\funbar, \dist{})$ is a
monoidal monad morphism.  It is also easy to check that $\Met$ has
pullbacks: the pullback of $f : A \to C$ and $g : B \to C$ is the subspace
of $A \times B$ consisting of all $(x, y)$ such that $f (x) = g (y)$; and
$\ihom A \_$ preserves relevant monos: $\ihom A \_$ maps $f : B \to C$ to
$\lambda g \in \ihom A B \cdot f \circ g$, which is an isometric embedding as soon as
$f$ is.

This yields the following notion of binary metric logical relation
$\Eval \tau$ between metric spaces $\Eval \tau_1$ and $\Eval \tau_2$ indexed by
types in a linear version of Moggi's meta-language.  The types are:
\[
\tau ::= b | 1 | \tau \otimes \tau | \tau \llimp \tau | \ques \tau
\]
where $b$ ranges over base types, $\llimp$ is linear implication, and
$\ques$ is a syntactic, strong monad.  It is easy to craft a calculus
based on this type algebra.  The linear $\lambda$-terms are given by:
\begin{eqnarray*}
  s, t, u, v, ... & ::= & x | * | \letin {* = s} t | s \otimes t | \letin {x \otimes y =
    s} t | st | \lambda x \cdot s \\
  && | \valu s | \letin {\valu x = s} t
\end{eqnarray*}
The typing rules are those of Moggi's calculus, except for its linear
flavor.  Contexts $\Gamma$ are multisets of bindings $x:\tau$, with pairwise
distinct variable parts $x$, and comma denotes multiset union.
\begin{eqnarray*}
  \begin{prooftree}
    \justifies
    x:A \vdash x:A
    \using (Var)
  \end{prooftree}
  &&
  \\
  \begin{prooftree}
    \Gamma \vdash s : 1 \quad
    \Delta, x:1 \vdash t : \tau
    \justifies
    \Gamma, \Delta \vdash \letin {* = s} t : \tau
    \using (1\mathcal E)
  \end{prooftree}
  &&
  \begin{prooftree}
    \justifies
    \vdash * : 1
    \using (1)
  \end{prooftree}
  \\
%  \begin{prooftree}
%    \Gamma \vdash s : \tau \otimes \tau' \quad
%    \Delta, x:\tau, y:\tau' \vdash t : \tau''
%    \justifies
%    \Gamma, \Delta \vdash t [x:=\pi_1 s, y:=\pi_2 s]
%    \using (Proj)
%  \end{prooftree}
  \begin{prooftree}
    \Gamma \vdash s : \tau \otimes \tau' \quad
    \Delta, x : \tau, y : \tau' \vdash t : \tau''
    \justifies
    \Gamma, \Delta \vdash \letin {x \otimes y = s} t : \tau''
    \using (\otimes\mathcal E)
  \end{prooftree}
  &&
  \begin{prooftree}
    \Gamma \vdash s : \tau \quad
    \Delta \vdash t : \tau'
    \justifies
    \Gamma, \Delta \vdash s \otimes t : \tau \otimes \tau'
    \using (Pair)
  \end{prooftree}
  \\
  \begin{prooftree}
    \Gamma \vdash s : \tau \llimp \tau' \quad
    \Delta \vdash t : \tau
    \justifies
    \Gamma, \Delta \vdash st : \tau'
    \using (App)
  \end{prooftree}
  &&
  \begin{prooftree}
    \Gamma, x : \tau \vdash s : \tau'
    \justifies
    \Gamma \vdash \lambda x \cdot s : \tau \llimp \tau'
    \using (Abs)
  \end{prooftree}
  \\
  \begin{prooftree}
    \Gamma \vdash s : \ques \tau \quad
    \Delta, x:\tau \vdash t : \ques {\tau'}
    \justifies
    \Gamma, \Delta \vdash \letin {\valu x=s} t : \ques {\tau'}
    \using (Let)
  \end{prooftree}
  &&
  \begin{prooftree}
    \Gamma \vdash s : \tau
    \justifies
    \Gamma \vdash \valu s : \ques \tau
    \using (Val)
  \end{prooftree}
\end{eqnarray*}
Conversion rules are given by judgments $\Gamma \vdash s \to t : \tau$ (which we write $s \to
t$ when $\Gamma$ and $\tau$ are clear or irrelevant), of which the most important are:
\begin{eqnarray*}
  \letin {* = *} s \to s
  %\Gamma \vdash s \to * : 1
  &&
  \vdash s \to * : 1
  \\
  \letin {x \otimes y = s \otimes t} u \to u [x:=s, y:=t] &&
  \letin {x \otimes y = s} {x \otimes y} \to s
%  \pi_1 \langle s, t \rangle \to s \quad
%  & \pi_2 \langle s, t \rangle \to t &
%  \quad
%  \langle \pi_1 s, \pi_2 s\rangle \to s
  \\
  (\lambda x \cdot s) t \to s[x:=t] && \lambda x \cdot sx \to s \quad
  \mbox{($x$ not free in $s$)} \\
  \letin {\valu x = \valu s} t \to t[x:=s] &&
  \letin {\valu x = s} {\valu x} \to s \\
  \letin {\valu x = \letin {\valu y = s} t} u
  & \to & \letin {\valu y=s} {\letin {\valu x = t} u}
\end{eqnarray*}
There are other rules, notably the infamous commutative conversion
rules---which originate in \cite{Prawitz:natdeduc}---and which we won't state.
The interpretation in symmetric monoidal closed categories follows the same
lines as those of the ordinary $\lambda$-calculus with a monadic type, replacing
cartesian products by tensor products. Our constructions then yield a notion
of subscone for this kind of calculus and models, requiring
conditions {\bf (i.b)}, {\bf (iii.a)}, {\bf (iv)}, {\bf (v)}, and {\bf (vi)}.

Note that $\Eval {\tau \otimes \tau'}_i = \Eval \tau_i \tensord \Eval {\tau'}_i$, $\Eval
{\tau \llimp \tau'}_i = \ihom {\Eval \tau_i} {\Eval {\tau'}_i}$, $\Eval {\ques \tau}_i =
\td \Eval \tau_i$.  Then the definition of the subscone specializes to:
\begin{eqnarray*}
  (f_1, f_2) \in \Eval {\tau \llimp \tau'} & \iff &
  \forall a_1 \in \Eval \tau_1, a_2 \in \Eval \tau_2 \cdot
  \\
  && \quad (a_1, a_2) \in \Eval \tau \Rightarrow (f_1 (a_1), f_2 (a_2)) \in \Eval {\tau'}
  \\
  ((a_1, a'_1), (a_2, a'_2)) \in \Eval {\tau \otimes \tau'} & \iff &
  (a_1, a_2) \in \Eval {\tau} \land (a'_1, a'_2) \in \Eval {\tau'}
\end{eqnarray*}
Finally, $(F_1, F_2) \in \Eval {\ques \tau}$ if and only if there is $F \in \td
\Eval \tau$ such that
\begin{eqnarray*}
  F_1 (g_1) & = & F (\lambda (x, y) \in \Eval \tau \cdot g_1 (x))
  \mbox{ for every }g_1 \in \cbf {\Eval \tau_1} \\
  F_2 (g_2) & = & F (\lambda (x, y) \in \Eval \tau \cdot g_2 (y))
  \mbox{ for every }g_2 \in \cbf {\Eval \tau_2}
\end{eqnarray*}
(Up to isomorphism, relevant monos are inclusions, so we may consider
that $\Eval \tau \subseteq \Eval \tau_1 \times \Eval \tau_2$.)  This condition implies that,
if $(F_1, F_2) \in \Eval {\ques \tau}$, then for every $g_1 \in \cbf {\Eval \tau_1}$
and $g_2 \in \cbf {\Eval \tau_2}$ such that $g_1 (a_1) = g_2 (a_2)$ for
every $(a_1, a_2) \in \Eval \tau$, then $F_1 (g_1) = F_2 (g_2)$.  It turns
out that this is equivalent to it, just as in the case of the
continuation monad: $(F_1, F_2) \in \Eval {\ques \tau}$ if and only if, for
every $g_1 \in \cbf {\Eval \tau_1}$ and $g_2 \in \cbf {\Eval \tau_2}$ such that
$g_1 (a_1) = g_2 (a_2)$ for every $(a_1, a_2) \in \Eval \tau$, then $F_1
(g_1) = F_2 (g_2)$.

The difficult if direction is proved as follows.  Assume that $F_1
(g_1) = F_2 (g_2)$ for every $g_1 \in \cbf {\Eval \tau_1}$ and $g_2 \in \cbf
{\Eval \tau_2}$ such that $g_1 (a_1) = g_2 (a_2)$ for every $(a_1, a_2) \in
\Eval \tau$.  Let $S$ be $\Eval \tau$, and $H$ be the subspace of $\cbf S$
of those functions of the form $\lambda (x, y) \in S \cdot g_1 (x)+g_2 (y)$, where
$g_1$ ranges over $\cbf {\Eval \tau_1}$, $g_2$ ranges over $\cbf {\Eval
  \tau_2}$.  Let $F_0 (g)$ be defined as $F_1 (g_1) + F_2 (g_2)$ for
every $g = \lambda (x, y) \in S \cdot g_1 (x)+g_2 (y)$ in $H$.  This is
independent of the choice of $g_1$ and $g_2$, since if $g$ can also be
written as $\lambda (x, y) \in S \cdot g'_1 (x)+g'_2 (y)$, then by construction
$g_1 (a_1) - g'_1 (a_1) = g'_2 (a_2) - g_2 (a_2)$ for every $(a_1,
a_2) \in S = \Eval \tau$, so $F_1 (g_1-g'_1) = F_2 (g'_2-g_2)$, which
implies $F_1 (g_1) + F_2 (g_2) = F_1 (g'_1) + F_2 (g'_2)$.  It is easy
to see that $F_0$ is a continuous linear form, so it extends to a
continuous linear form $F$ with the same norm on the whole of $\cbf
S$, by the Hahn-Banach Theorem.  By the same argument as in
Lemma~\ref{lemma:td:met}, $F$ is a positive linear form.  Clearly $F_1
(g_1) = F (\lambda (x, y) \in \Eval \tau \cdot g_1 (x))$ for every $g_1 \in \cbf {\Eval
  \tau_1}$, and $F_2 (g_2) = F (\lambda (x, y) \in \Eval \tau \cdot g_2 (y))$ for every
$g_2 \in \cbf {\Eval \tau_2}$, whence the claim.

In other words, the logical relation at $\ques \tau$ types is defined by a
formula in the style of observational equivalence.

It is reasonable to represent the set of probabilistic transition
systems on a metric space $A$ as the metric space $\ihom A {\td A}$ of
all non-expansive maps from the set of states $A$ to the set of
probability measures on $A$. The subscone construction provides a
condition when two such probabilistic transition systems are related.
Given any relation $S$ on $A$ (defining a metric subspace of $A \times A$),
define the relation $\lift S$ on $\ihom A {\td A}$ by: for any
non-expansive maps $f_1, f_2$ from $A$ to $\td A$, $(f_1, f_2) \in \lift
S$ if and only if, for every $(a_1, a_2) \in S$, there is $F \in \td S$
such that
\begin{eqnarray*}
  f_1 (a_1) (g_1) & = & F (\lambda (x, y) \in S \cdot g_1 (x))
  \mbox{ for every }g_1 \in \cbf A \\
  f_2 (a_2) (g_2) & = & F (\lambda (x, y) \in S \cdot g_2 (y))
  \mbox{ for every }g_2 \in \cbf A
\end{eqnarray*}
or, equivalently, for every $g_1, g_2 \in \cbf A$ such that $g_1 (x) =
g_2 (y)$ for every $(x, y) \in S$, then $f_1 (a_1) (g_1) = f_2 (a_2)
(g_2)$.  In case $A$ is compact, by the Riesz Representation Theorem,
we may replace positive continuous linear functionals on $\cbf A$ by
probability measures.  Rephrasing the above, we get: for any
non-expansive maps $f_1, f_2$ from $A$ to the space of probability
measures on $A$, $(f_1, f_2) \in \lift S$ if and only if, for every
$(a_1, a_2) \in S$, there is a probability measure $\nu$ on $S$ such that
\begin{eqnarray*}
  f_1 (a_1) (X_1) & = & \nu ((X_1 \times A) \cap S)
  \mbox{ for every measurable subset }X_1\mbox{ of }A
  \\
  f_2 (a_2) (X_2) & = & \nu ((A \times X_2) \cap S)
  \mbox{ for every measurable subset }X_2\mbox{ of }A
\end{eqnarray*}
We retrieve a notion of probabilistic bisimulation: $S$ is a {\em
  bisimulation\/} on the space $A$ of states between the transition
systems $f_1$ and $f_2$ if and only if $\lift S$ relates $f_1$ and
$f_2$.

In passing, we have just shown that the
observational-equivalence-style definition of $\lift S$ coincides with
the bisimulation-style definition, using the Riesz Representation
Theorem.  This can be seen as a form of a completeness theorem.

The notion above is formally analogous to the notion of probabilistic
bisimulation of \cite{DEP:markov:bisim}; i.e., the formulas we use and
theirs for defining bisimulations is the same.  This is also formally
analogous to metric bisimulations as introduced by de Vink and Rutten
\cite{dVR:proba:bisim} for ultrametric spaces, and extended by Worrell
\cite{Worrell:PhD} to generalized metric spaces.  A difference is that
the latter authors use a coalgebraic approach; in particular, their
construction requires a $\td$ functor that preserves isometric
embeddings (our relevant monos), while we require it to preserve
pseudoepis (surjective non-expansive maps).

\fi


==> lifting.tex <==
%\documentclass[11pt]{llncs}

%\usepackage{amsmath,amscd,amssymb,amsfonts,latexsym}
%\usepackage{diagrams}
%\usepackage{xypic,xy}
%\xyoption{all}

%\begin{document}

\iflong%
\section{Preliminaries}
\label{prelim.s}

\else%
\fi%

\noindent
\begin{minipage}{8.5cm}
  \iflong%
  \relax%
  \else%
  \smallskip\hspace{0.5cm}{\bf Preliminaries.}
  \fi%
  Fix two categories $\catc$ and $\catd$ and a functor $\funbar : \catc \to
  \catd$. Consider the comma category $\comma{\catd}{\funbar}$, whose objects
  are tuples $\langle S, f, A \rangle$, with $f : S \to \funbara{A}$ in
  $\catd$ and whose morphisms are pairs $\langle g, h \rangle : \langle S, f,
  A \rangle \to \langle S', f', A' \rangle$, $g : S \to S'$ in $\catd$ and $h
  : A \to A'$ in $\catc$, such that the diagram on the right commutes in $\catd$.
\end{minipage}
\begin{minipage}{3.5cm}
  \begin{equation}
    \label{d_morph}
    \xymatrix@-5pt{
      S \ar[d]_{g} \ar[r]^{f} & \funbara{A} \ar[d]^{\funbara{h}} \\
      S' \ar[r]_{f'} & \funbara{A'}
      }
  \end{equation}
\end{minipage}

\noindent
This category is the {\em scone of $\catc$ over $\catd$} via $\funbar$, {\em
  $\scone{\catc}{\catd}{\funbar}$}.  (We extend here terminology of
\cite{MS93}, where the name {\em scone} was reserved to the case $\catd =
\catset$, $\funbar = \homset {\catc} {\termobj} \_$ only.)  The projection
functor $\forfun : \comma{\catd}{\funbar} \to \catc$ maps $\langle S, f, A \rangle$ to $A$
and the morphism $\langle g,h \rangle$ to $h$.

In the sequel we shall be especially interested in the case where $\catd =
\catset$, and $\funbar = \homset{\catc}{\termobj}{\_}$ is the {\em global
  section\/} functor, where $\termobj$ is terminal in $\catc$. Another
interesting situation arises when $\catc = \catd {\times} \catd$ and
$\funbara{(A,B)} = A {\times} B$, assuming that $\catd$ has finite products.
Objects of the scone then represent binary relations between objects in
$\catd$. In this case, given two functors $\funbar_1 : \catc_1 \to \catd$ and
$\funbar_2 : \catc_2 \to \catd$, we may define $\funbar : \catc \to \catd$,
for $\catc = \catc_1 {\times} \catc_2$, by $\funbara{(A_1, A_2)}
= \funbaraa{1}{A_1} {\times} \funbaraa{2}{A_2}$.

Further assume we are given a monad $( \tc, \unitc{}, \multc{} )$ on $\catc$.
When $\catc = \catc_1 {\times} \catc_2$, the monad $\tc$ on $\catc$ will be usually
defined pointwise, by two monads $\tc_1$ and $\tc_2$ on $\catc_1$ and
$\catc_2$, respectively: $\tc(A_1, A_2) = (\tc_1(A_1), \tc_2(A_2))$.

\section{Lifting of a Monad to a Scone}
\label{scone.s}

\iflong By {\em lifting of a monad $(\tc, \unitc{}, \multc{})$} to the scone
$\scone \catc \catd \funbar$ of $\catc$ over $\catd$ we mean a monad $(\tS,
\unitS{}, \multS{})$ on $\scone{\catc}{\catd}{\funbar}$ such that the diagram
\begin{equation}
\label{d_lifting1}
\xymatrix@-5pt{
\scone{\catc}{\catd}{\funbar} \ar[r]^{\tS} \ar[d]_{\forfun} & 
\scone{\catc}{\catd}{\funbar} \ar[d]^{\forfun} \\
\catc \ar[r]_{\tc} & \catc
}
\end{equation}
commutes, i.e.~$\forfun \circ \tS = \tc \circ \forfun$ 
and moreover
\begin{equation}
\label{e_lifting2}
\forfun \unitS{} = \unitc{\forfun} \ \ \mbox{and} \ \ 
\forfun \multS{} = \multc{\forfun}.
\end{equation}
\else
\noindent
\begin{minipage}{7.1cm}
  By {\em lifting of a monad $(\tc, \unitc{}, \multc{})$} to the scone of
  $\catc$ over $\catd$ we mean a monad $(\tS, \unitS{}, \multS{})$ on
  $\scone{\catc}{\catd}{\funbar}$ such that the diagram on the right commutes.
  That is, $\forfun \circ \tS = \tc \circ \forfun$ and moreover
\end{minipage}
\begin{minipage}{4.9cm}
  \begin{equation}
    \label{d_lifting1}
    \xymatrix@-5pt{
      \scone{\catc}{\catd}{\funbar} \ar[r]^{\tS} \ar[d]_{\forfun} & 
      \scone{\catc}{\catd}{\funbar} \ar[d]^{\forfun} \\
      \catc \ar[r]_{\tc} & \catc
      }
  \end{equation}
\end{minipage}

\begin{equation}
\label{e_lifting2}
\forfun \unitS{} = \unitc{\forfun} \ \ \mbox{and} \ \ 
\forfun \multS{} = \multc{\forfun}.
\end{equation}
\fi

\noindent
\begin{minipage}[t]{5.5cm}
  By $\forfun \unitS{}$ and $\unitc{\forfun}$ we mean the two possible
  compositions of a natural transformation with $\forfun$, similarly $\forfun
  \multS{}$ and $\multc{\forfun}$.  The equations~(\ref{e_lifting2}) amount to
  the requirement that the two diagrams on the right commute, for all objects
  $X$ in $\scone{\catc}{\catd}{\funbar}$:
\end{minipage}
\begin{minipage}[t]{6.5cm}
  \small
  \hfill$
  \xymatrix@-5pt{
    & 
    &
    &
    \tc^2 \forfun X \ar@{=}[d]^{\mbox{(\ref{d_lifting1})}} 
    \ar[ld]_{\multc{\forfun X}} \\
    & 
    \tc \forfun X \ar@{=}[d]^{\mbox{(\ref{d_lifting1})}} &
    \tc \forfun X \ar@{=}[d]^{\mbox{(\ref{d_lifting1})}} &
    \tc \forfun \tS X \ar@{=}[d]^{\mbox{(\ref{d_lifting1})}} \\
    \forfun X \ar[r]_{\forfun \unitS{X}} \ar[ru]^{\unitc{\forfun X}} &
    \forfun \tS X &
    \forfun \tS X &
    \forfun \tS^2 X \ar[l]^{\forfun \multS{X}} 
    }
  $
\end{minipage}

In other words, the functor $\forfun$ together with the identity natural
transformation is a morphism of monads from $\tS$ to $\tc$.  (We recall monad
morphisms shortly.)  Note that the equations~(\ref{e_lifting2}) determine the
$\catc$-components of $\unitS{}$ and $\multS{}$ unambiguously. Moreover,
diagram~(\ref{d_lifting1}) determines the $\catc$-component of the action of
$\tS$ on objects and morphisms, i.e.\ $\langle S, f, A \rangle$ is necessarily
mapped to $\langle \lift{S}, \lift{f}, \tc A \rangle$, for some $\lift{S},
\lift{f}$ and a morphism $\langle g, h \rangle$ is necessarily mapped to
$\langle \lift{g}, \tc h \rangle$, for some $\lift{g}$.

\iflong
Our notion of lifting could be stated more
generally, for an arbitrary pair of categories, a functor 
from the first one to the second one and a monad on 
the second category.
In fact, in the next section we consider a lifting
of $\tc$ to another category, namely a suitable subcategory of 
$\scone{\catc}{\catd}{\funbar}$.
\else
\fi

To be able to give an appropriate lifting we assume another monad $( \td,
\unitd{}, \multd{} )$ on $\catd$ such that the two monads $\tc$ and $\td$ are
related by a {\em monad morphism\/} from $\tc$ to $\td$, i.e.\ a natural
transformation
\[
\dist{} : \td \funbar \ \ \natto \ \  \funbara{\tc}
\]
making the following two diagrams commute, for each object $A$
in $\catc$:
\begin{equation}
\label{d_distlaw}
\xymatrix@-5pt{
 & & &
\td^2 \funbara{A} \ar[ld]_{\multd{\funbara{A}}} 
                  \ar[d]^{\td \dist{A}} \\
 & \td \funbara{A} \ar[d]^{\dist{A}} & 
   \td \funbara{A} \ar[d]^{\dist{A}} & 
\td \funbara{\tc A } \ar[d]^{\dist{\tc A}} \\
\funbara{A} \ar[ru]^{\unitd{\funbara{A}}} 
            \ar[r]_{\funbara{\unitc{A}}} & 
\funbara{\tc A } & 
\funbara{\tc A } & 
\funbara{\tc^2 A} \ar[l]^{\funbara{\multc{A}}}
}
\end{equation}
To be formal, a monad morphism is a {\em pair\/} $(\funbar, \dist{})$
satisfying the equations above.  We shall however continue to say that
$\dist{}$ is a monad morphism, when $\funbar$ is understood.

Having $\dist{}$, we define $\tS$ on objects by
\[
\xymatrix@-5pt{
\langle S, f, A \rangle  &  \ar@{|->}[r] & &
\langle \td S, \dist{A} \circ \td f, \tc A \rangle 
}
\]
exploiting that if \smash{$\xymatrix@-5pt{S \ar[r]^{f} &\funbara{A}}$}
then \smash{$\xymatrix@-5pt{\td S \ar[r]^{\td f} & {\td \funbara{A}} \ar[r]^{\dist{A}} &
    \funbara{\tc A}}
  $} is a morphism.
\iflong
On morphisms we define $\tS$ by
\[
\xymatrix@-5pt{
\langle g, h \rangle  &  \ar@{|->}[r] & &
\langle \td g, \tc h \rangle 
}
\]
since from \raisebox{2em}{ $ \xymatrix@-5pt{
    S \ar[r]^{f} \ar[d]_{g} & \funbara{A} \ar[d]^{\funbara{h}} \\
    S' \ar[r]_{f'} &\funbara{A'} } $ } we deduce that \raisebox{2em}{ $
  \xymatrix@-5pt{ \td S \ar[r]^{\td f} \ar[d]_{\td g} & {\td \funbara{A}}
    \ar[r]^{\dist{A}} &
    \funbara{\tc A} \ar[d]^{\funbara{\tc h}} \\
    \td S' \ar[r]_{\td f'} & {\td \funbara{A'}} \ar[r]_{\dist{A'}} &
    \funbara{\tc A'} } $ } commutes, by naturality of $\dist{}$.
\else
On morphisms, note that \raisebox{2em}{ $ \xymatrix@-5pt{ \td S \ar[r]^{\td f}
    \ar[d]_{\td g} & {\td \funbara{A}} \ar[r]^{\dist{A}} &
    \funbara{\tc A} \ar[d]^{\funbara{\tc h}} \\
    \td S' \ar[r]_{\td f'} & {\td \funbara{A'}} \ar[r]_{\dist{A'}} &
    \funbara{\tc A'} } $ } commutes since \raisebox{2em}{ $ \xymatrix@-5pt{
    S \ar[r]^{f} \ar[d]_{g} & \funbara{A} \ar[d]^{\funbara{h}} \\
    S' \ar[r]_{f'} &\funbara{A'} } $ } commutes and $\dist{}$ is natural.  So
we define $\tS$ by $ \xymatrix@-5pt{ \langle g, h \rangle \ar@{|.>}[r] &
  \langle \td g, \tc h \rangle } $. \fi
%
Moreover, we put
\iflong
\[
\unitS{\langle S,f,A \rangle} = \langle \unitd{S}, \unitc{A} \rangle  
\ \ \mbox{and} \ \ 
\multS{\langle S,f,A \rangle} = \langle \multd{S}, \multc{A} \rangle.\\
\]
\else
$
\unitS{\langle S,f,A \rangle} = \langle \unitd{S}, \unitc{A} \rangle  
\ \ \mbox{and} \ \ 
\multS{\langle S,f,A \rangle} = \langle \multd{S}, \multc{A} \rangle.\\
$
\fi

\noindent
\begin{minipage}[t]{7cm}
  Checking that this defines a monad is straightforward. First, to check that
  unit and multiplication are well defined it is sufficient to merge the
  commuting diagrams~(\ref{d_distlaw}) and complete them with naturality
  squares for $\unitd{}$ and $\multd{}$ as shown on the right.
  
  Unit $\unitS{}$ and multiplication $\multS{}$ are natural since they are
  defined pointwise and $\unitc{}$, $\multc{}$, $\unitd{}$ and $\multd{}$ are.
  Verifying monad laws is immediate, by the same argument.
\end{minipage}
\begin{minipage}[t]{5cm}
  \hfill
  $
  \xymatrix@-5pt{
    S \ar[ddd]_{f} \ar[r]^{\unitd{S}} & 
    \td S \ar[dd]_{\td f} & 
    \td^2 S \ar[d]^{\td^2 f} \ar[l]_{\multd{S}} \\
    & & 
    \td^2 \funbara{A} \ar[ld]_{\multd{\funbara{A}}} 
    \ar[d]^{\td \dist{A}} \\
    & \td \funbara{A} \ar[d]^{\dist{A}} & 
    \td \funbara{\tc A } \ar[d]^{\dist{\tc A}} \\
    \funbara{A} \ar[ru]^{\unitd{\funbara{A}}} 
    \ar[r]_{\funbara{\unitc{A}}} & 
    \funbara{\tc A } & 
    \funbara{\tc^2 A} \ar[l]^{\funbara{\multc{A}}}
    }
  $
  \hfill\strut
\end{minipage}

\noindent

\iflong The monad morphism (\ref{d_distlaw}) can be equivalently given by a
lifting of $\funbar$ to the categories of algebras of the monads, i.e.\ by a
functor $\lift{\funbar} : \catalg{\catc}{\tc} \to \catalg{\catd}{\td}$ making
the diagram commute:
\[
\xymatrix@-5pt{
\catalg{\catc}{\tc} \ar[r]^{\lift{\funbar}} \ar[d]_{\forfunalg{\tc}} & 
\catalg{\catd}{\td} \ar[d]^{\forfunalg{\td}} \\
\catc \ar[r]_{\funbar} & \catd
}
\]
where $\catalg{\catc}{\tc}$ and $\catalg{\catd}{\td}$ denote categories of
algebras of the monads and $\forfunalg{\tc}$ and $\forfunalg{\td}$ denote the
obvious forgetful functors. In fact, for fixed monads $\tc$ and $\td$ and a
fixed functor $\funbar$, there is a one-to-one correspondence between the
monad morphisms $\dist{}$ and liftings of $\funbar$ to algebras. The proof of
this fact can be found in~\cite{App65} or in \cite{John75}.
\fi%

\section{Lifting of a Monad to a Subscone}
\label{subscone.s}
\label{s_liftsubscone}

%The {\em subscone\/} is defined in \cite{MS93} just like the scone, except
%objects $\langle S, f, A \rangle$ are now restricted so that $f$ is {\em
%  mono}.
Following, and slightly extending \cite{MS93}, we may call the {\em subscone
  of $\catc$ over $\catd$} the full subcategory
$\subscone{\catc}{\catd}{\funbar}$ of $\scone{\catc}{\catd}{\funbar}$
consisting of all objects $\langle S, f, A \rangle$ with $f$ a mono, written
$\xymatrix@-5pt{S \arrnotrelmonoxy[r]^f & \funbara{A}}$.  (We shall actually
define the subscone slightly differently below.)

When $\catd = \catset$ and $\funbara{A}$ is given by
$\homset{\catc}{\termobj}{A}$, each object $\xymatrix@-5pt{S
  \arrnotrelmonoxy[r] & \funbara{A}}$ in the subscone represents a subset of
global elements of $A$. In the binary case, i.e. when $\catc = \catc_1
{\times} \catc_2$ and $\funbara{(A_1, A_2)} =
\homset{\catc_1}{\termobj_1}{A_1} \times \homset{\catc_2}{\termobj_2}{A_2}$,
$\xymatrix@-5pt{S \arrnotrelmonoxy[r] & \funbara{(A_1, A_2)}}$
corresponds to a binary relation on global elements of $A_1$ and $A_2$---when
$A_1$ and $A_2$ are the respective denotations of type $\tau$ in two given
models, this will be the logical relation at type $\tau$.

For technical reasons, 
% we need to further restrict $f$ to be a {\em relevant mono}.  Precisely, 
we require that $\catd$ has a {\em mono factorization
  system}.  This is essentially an epi-mono factorization~\cite{AHS}, except
we relax part of the definition: we keep the mono part but do not require the
epis in the sequel.  Alternately, this is a factorization system where one of
the classes of morphisms is required to consist of monos only.
%  Our definition is a minor modification of definition of factorization system in~\cite{AHS}.

Formally, a mono factorization system is given by two distinguished subclasses
of morphisms in $\catd$, the so-called {\em pseudoepis\/}
$\xymatrix@-5pt{\arrepixy[r]&}$ and the so-called {\em relevant monos\/}
$\xymatrix@-5pt{\arrmonoxy[r]&}$. The latter must be monos, while the former
are not required to be epis.  
Both classes must 
% contain all isomorphisms and
be closed under composition with isomorphisms.
%\iflong%
%\footnote{ In particular, we do not need pseudoepis to be closed under
%  composition, which holds true for an epi-mono factorization system, see
%  e.g.~\cite{AHS}, Chapter 14.  }
%\else%
%\fi%

\noindent
\begin{minipage}{9cm}
Each morphism $f$ in $\catd$ must factor as
%\begin{equation*}
%\label{e_emfactor}
$f = m \circ e$
%\end{equation*}
for some pseudoepi $e$ and some relevant mono $m$; and each commuting
square~(\ref{d_factor}) has a diagonal making both triangles commute as
in~(\ref{d_factordiag}). We call this diagonal morphism the {\em diagonal
  fill-in}. Note that the diagonal fill-in is necessarily unique and that
whenever the lower-right triangle commutes, the upper-left triangle does too.
Furthermore, the latter property guarantees that the factorization
$f = m \circ e$  %~(\ref{e_emfactor})
is unique up to iso.
\end{minipage}
  \begin{minipage}{     3cm}
    \begin{equation}
      \label{d_factor}
      \xymatrix@-5pt{
        \cdot \arrepixy[r] \ar[d] & \cdot \ar[d] \\
        \cdot \arrmonoxy[r] & \cdot
        }
    \end{equation}
    \begin{equation}
      \label{d_factordiag}
      \xymatrix@-5pt{
        \cdot \arrepixy[r] \ar[d] & \cdot \ar[d] \ar@{.>}[ld] \\
        \cdot \arrmonoxy[r] & \cdot
        }
    \end{equation}
\ \\
  \end{minipage}

\noindent
In particular, we do not require neither pseudoepis nor relevant monos to be
closed under composition, which holds true for an epi-mono factorization
system, see e.g.~\cite[Chapter 14]{AHS}. But it is easy to deduce from the
diagonal fill-in property that a composition of two pseudoepis is pseudoepi
indeed, and similarly a composition of two relevant monos is a relevant mono,
see e.g.~\cite{Barr98}. It is also proved there that both classes contain all
isomorphisms.

In fact, the factorization of $f$ as $m \circ e$ determines uniquely a
so-called {\em relevant subobject\/} of the codomain, defined as follows.  Two
relevant monos in $\catd$ with the same codomain, $\xymatrix@-5pt{S_1
  \arrnotrelmonoxy[r]^{f_1} & S}$ and $\xymatrix@-5pt{S_2
  \arrnotrelmonoxy[r]^{f_2} & S}$ are called equivalent if and only if there
exist $g_1$ and $g_2$ making the two triangles commute:
\[
\xymatrix@-5pt{
S_1 \ar@<0.5ex>[rr]^{g_2} \arrnotrelmonoxy[rd]_{f_1} & 
&
S_2 \ar@<0.5ex>[ll]^{g_1} \arrnotrelmonoxy[ld]^{f_2} \\
& S &
}
\]
i.e., $f_1 \circ g_1 = f_2$ and $f_2 \circ g_2 = f_1$. A {\em relevant
  subobject\/} of $S$ is an equivalence class of relevant monos with codomain
$S$. Equivalently, we could take as objects of the subscone all relevant
subobjects of $\funbara{A}$, for all objects $A$ in $\catc$.  We prefer to
keep the simpler presentation, despite the fact that this implies that some
constructions in the sequel are only determined up to isomorphism, e.g.,
(\ref{d_tsonobj}) below.

We come back to the definition of the subscone:
\begin{definition}
  \label{defn:subscone}
  Given two categories $\catc$, $\catd$, a functor $\funbar : \catc \to \catd$,
  and a mono factorization system on $\catd$, the {\em subscone of $\catc$
    over $\catd$} is the full subcategory $\subscone{\catc}{\catd}{\funbar}$
  of $\scone{\catc}{\catd}{\funbar}$ consisting of all objects $\langle S, f, A \rangle$
  with $f$ a relevant mono $\xymatrix@-5pt{S \arrnotrelmonoxy[r]^f &
    \funbara{A}}$.
\end{definition}
It may seem that the notation $\subscone{\catc}{\catd}{\funbar}$ is too vague,
as it does not mention $\catc$
%$\funbar$
%@@@
or the mono factorization system explicitly. It will be clear that making all
parameters explicit would make the notation extremely heavy.

Additionally, we shall assume that $\td e$ is pseudoepi for every morphism $e$
in a subclass of all pseudoepis called {\em relevant pseudoepis}, which we
shall define shortly.  This will be used in Diagram~(\ref{d_mults}) below.  In
most applications, it will suffice to check that $\td$ preserves pseudoepis.
%; in fact, in this diagram only.
%  Preserving pseudoepis is actually not
%necessary, and we shall give a more refined, but more complex condition in
%Section~\ref{sec:mult:subscone}.

Note the following simple and important fact:
\begin{fact}
\label{f_determ}
The first component $g$ of a morphism $\langle g, h \rangle$ (recall that
\raisebox{2em}{ $ \xymatrix@-5pt{
    S \ar[d]_{g} \arrnotrelmonoxy[r] & \funbara{A} \ar[d]^{\funbara{h}} \\
    S' \arrnotrelmonoxy[r] & \funbara{A'} } $} commutes) in a subscone is
uniquely determined by the second component $h$.
\end{fact}
This is because the bottom arrow is now mono.
% This will allow us to reduce the
%commutativity of diagrams in the subscone to the commutativity of diagrams
%involving only the $h$ parts, i.e., to the commutativity of the corresponding
%diagrams in $\catc$.  In other words, it will suffice to construct objects and
%morphisms in the subscone so that applying $\forfun$ to them gives the expect
%objects and morphisms in $\catc$, then all necessary diagrams will commute: we
%won't have to check any.
%These property will be of great use in the sequel.


Let us define a lifting of the monad to the subscone by analogy with
(\ref{d_lifting1}) and (\ref{e_lifting2}) for the scone. In the binary case
mentioned at the beginning of this section, this corresponds to a lifting of a
monad to the category of binary relations (as objects) and relation preserving
functions (as morphisms).

\noindent
\begin{minipage}{7cm}
  \subsection{$\tS$ on objects.}
  The lifting $\tS$ on objects is given by the mono part of the mono
  factorization of the lifting of the previous section: $\langle S, f, A
  \rangle$
                                % $\xymatrix@-5pt{S \arrmonoxy[r]^{f} & \funbara{A}}$ 
  is taken to
                                % $\xymatrix@-5pt{\lift{S} \arrmonoxy[r] & \funbara{\tc A}}$
  $\langle \lift{S}, m, \tc A \rangle$ given by the diagram on the right.
\end{minipage}
\begin{minipage}{5cm}
  \begin{equation}
    \label{d_tsonobj}
    \xymatrix@-5pt{
      \td S \ar[r]^{\td f} \arrepixy[d]_{e} & 
      \td \funbara{A} \ar[d]^{\dist{A}} \\
      \lift{S} \arrmonoxy[r]_{m} & \funbara{\tc A}
      }
  \end{equation}
\end{minipage}

\noindent
We call pseudoepis $e$ arising in this way {\em $\td, \dist{}$-relevant
  pseudoepis}.  That is, a $\td, \dist{}$-relevant pseudoepi is the pseudoepi
part of a factorization of a morphism of the form $\dist A \circ \td f$, where
$f$ is a relevant mono.  For short, we shall call them {\em relevant
  pseudoepis\/} when $\td$ and $\dist{}$ are clear from context.

\noindent
Clearly $\tS$ is defined only up to iso. Formally, the construction would be
unambiguous if we worked with subobjects of $\funbara{\tc A}$, which are
determined uniquely.\\

\noindent
\begin{minipage}{7.4cm}
  \subsection{$\tS$ on morphisms.}
  Given a morphism $\langle g, h \rangle$, the diagram on the right commutes.
  Then the action of $\tS$ on $\langle g, h \rangle$ will be obtained from the
  unique diagonal guaranteed by (\ref{d_factordiag}).  We construct diagram
  (\ref{d_tsonmor}) below from two copies of~(\ref{d_tsonobj}).
\end{minipage}
\begin{minipage}{4.6cm}
  \begin{equation}
    \label{d_morphagain}
    \xymatrix@-15pt{
      S \ar[dr]_{g} \arrnotrelmonoxy[rr]^{f} & & \funbara{A} \ar[dr]^{\funbara{h}} & \\
      & S' \arrmonoxy [rr]_{f'} & & \funbara{A'}
      }
  \end{equation}
\end{minipage}

\noindent
\begin{minipage}{6cm}
  All four given faces of the cube commute. Both front and back faces commute
  by definition of $\tS$ on objects: they are copies of
  diagram~(\ref{d_tsonobj}). The right-hand face is a naturality square of
  $\dist{}$; the top face is by application of $\td$ to
  diagram~(\ref{d_morphagain}), hence commutes by definition of morphisms in
  the subscone.
\end{minipage}
\begin{minipage}{6cm}
  \begin{equation}
    \label{d_tsonmor}
    \xymatrix@-15pt{
      \td S \ar[rr]^{\td f} \arrepixy[dd]_{e} \ar[rd]_{\td g}& 
      &
      \td \funbara{A} \ar'[d][dd]^{\dist{A}} \ar[rd]^{\td \funbara{h}}&
      \\
      &
      \td S' \ar[rr]^(.35){\td f'} \arrepixy[dd]^(.7){e'} &
      &
      \td \funbara{A'} \ar[dd]^{\dist{A'}} \\
      \lift{S} \arrmononotmovedxy'[r]^{m}[rr] &
      &
      \funbara{\tc A} \ar[rd]^{\funbara{\tc h}} &
      \\
      & 
      \lift{S'} \arrmononotmovedxy[rr]_{m'} & 
      & 
      \funbara{\tc A'} \\
      }
  \end{equation}
\end{minipage}

\noindent
Now, an instance of diagram~(\ref{d_factor}) can be found in (\ref{d_tsonmor})
by two walks %along the main diagonal
from $\td S$ to $\funbara{\tc A'}$: one starts with the pseudoepi
\smash{$\xymatrix@-5pt{\td S \arrepixy[r]^{e} & \lift{S}}$}, the other ends
with the relevant mono \smash{$\xymatrix@-5pt{\lift{S'} \arrmonoxy[r]^{m'} &
    \funbara{\tc A'}}$}. Since all faces commute, there is an arrow
\smash{$\xymatrix@-5pt{\lift{S} \ar@{.>}[r] & \lift{S'}}$} as in
diagram~(\ref{d_factordiag}), making the two newly created faces of the cube
commute.  This arrow is unique by Fact~\ref{f_determ}.  Now $\tS \langle g, h
\rangle$ is given by the bottom face.
Functoriality follows immediately from uniqueness of the diagonal arrow
in~(\ref{d_factordiag}).
\medskip

\noindent
\begin{minipage}{7cm}
  \subsection{Unit $\unitS{}$.}
  The ($\catd$-component of the) unit $\unitS{\langle S, f, A \rangle}$ is
  defined by post-composing $\unitd{S}$ with the pseudoepi part of the mono
  factorization in~(\ref{d_tsonobj}). This is well-defined since everything in
  sight in the diagram on the right commutes.  Indeed, the right triangle is
  the monad morphism diagram (\ref{d_distlaw}) (left), the upper square is the
  naturality of $\unitd{}$ while the lower one is a copy of~(\ref{d_tsonobj}).
\end{minipage}
\begin{minipage}{5.7cm}
  \begin{equation}
    \label{d_units}
    \xymatrix@-5pt{
      S \arrnotrelmonoxy[rr]^{f} \ar[d]_{\unitd{S}} & 
      & 
      \funbara{A} \ar[dd]^{\funbara{\unitc{A}}} \ar[ld]_{\unitd{\funbara{A}}} \\
      \td S \ar[r]^{\td f} \arrepixy[d]_{e} & 
      \td \funbara{A} \ar[dr]^{\dist{A}} & 
      \\
      \lift{S} \arrmonoxy[rr]_{m} & & \funbara{\tc A}
      }
  \end{equation}
\end{minipage}

\noindent
\subsection{Multiplication $\multS{}$.}
The ($\catd$-component of the) multiplication $\multS{\langle S, f, A
  \rangle}$ will be induced by a diagram similar to~(\ref{d_tsonmor}) (below).

\noindent
\begin{minipage}{6cm}
  Again, all the faces not having the dashed arrow or the required dotted
  arrow as edge commute.  The front face and the lower half of the back face
  are instances of (\ref{d_tsonobj}), defining $\tS \langle S, f, A \rangle$ and $\tS^2 \langle
  S, f, A \rangle$, respectively. The upper half of the back face is by application
  of $\td$ to the front face. The right-hand face is the other monad morphism
  diagram (\ref{d_distlaw}) (right), which we had not used yet, while the
  upper one is a naturality square for $\multd{}$.
\end{minipage}
\begin{minipage}{6.5cm}
  \begin{equation}
    \label{d_mults}
    \xymatrix@-10pt{
      \td^2 S \ar[rr]^{\td^2 f} \arrepixy[d]_{\td e} \ar[rdd]^(.3){\multd{S}} &
      &
      \td^2 \funbara{A} \ar[d]_{\td \dist{A}} \ar[rdd]^{\multd{\funbara{A}}} &
      \\
      \td \lift{S} \ar[rr]|(.23)\hole ^{\td m} \arrepixy[dd]_{\lift{e}} 
      \ar@{-->}[rddd] & 
      &
      \td \funbara{\tc A} \ar'[d][dd]^{\dist{\tc A}} &
      \\
      &
      \td S \ar[rr]^(.35){\td f} \arrepixy[dd]^(.7){e} &
      &
      \td \funbara{A} \ar[dd]^{\dist{A}} \\
      \lift{\lift{S}} \arrmononotmovedxy'[r]|(.63)\hole[rr]^(.4){\lift{m}} 
      \ar@{.>}[rd]_{!} &
      &
      \funbara{\tc^2 A} \ar[rd]^{\funbara{\multc{A}}} &
      \\
      & 
      \lift{S} \arrmononotmovedxy[rr]_{m} & 
      & 
      \funbara{\tc A} \\
      }
  \end{equation}
\end{minipage}
\medskip

\noindent
Note that $\td e$ is a pseudoepi, since $e$ is a relevant pseudoepi by
construction, and $\td$ maps relevant pseudoepis to pseudoepis. The
composition $\lift{e} \circ \td e$ is necessarily a pseudoepi as well
\cite{Barr98}. We may use this result, or use a diagonal~(\ref{d_factordiag})
twice.  Here, and in some other cases later, we prefer to do so.

First, similarly as in diagram~(\ref{d_tsonmor}) we find an instance of
diagram~(\ref{d_factor}) by two walks from $\td^2 S$ to $\funbara{\tc A}$, one
starting with $\td e$ and the other ending with $m$.  Hence, the unique dashed
arrow exists and makes the two triangles commute. One of them, involving the
pseudoepi $\td e$, is the upper part of the left-hand side. The other one,
namely that involving the relevant mono $m$, allows us to
apply~(\ref{d_factor}) again, since the following two walks from $\td
\lift{S}$ to $\funbara{\tc A}$ commute: one starting with the pseudoepi
$\lift{e}$ and the other consisting of the dashed arrow followed by $m$.
Hence, the unique dotted arrow exists and makes the bottom face as well as the
triangle in the left-hand face commute. The multiplication $\multS{\langle S, f, A
  \rangle}$ is then defined by the bottom face of the cube.

%Now, having the full monad $(\tS, \unitS{}, \multS{})$,
Verification of the monad laws is a formality due to the following:
\begin{fact}
  \label{f_eq}
  Given two parallel arrows in $\subscone{\catd}{\catc}{\funbar}$, say $\langle g_1,
  h_1 \rangle$ and $\langle g_2, h_2 \rangle$, they are equal whenever the second components
  $h_1$ and $h_2$ are.
\end{fact}
The proof is immediate by Fact~\ref{f_determ}. Using this fact, and knowing
that second components of $\unitS{}$ and $\multS{}$ satisfy the monad laws (as
they are unit and multiplication of $\tc$, respectively), we deduce
immediately that $\unitS{}$ and $\multS{}$ satisfy the monad laws too.
Similarly one proves naturality of $\unitS{}$ and $\multS{}$.  We shall use
this argument extremely often in the sequel.

It is useful to summarize the ingredients we have used here.  To lift a monad
$(\tc, \unitc{}, \multc{})$ on $\catc$ to $\subscone{\catc}{\catd}{\funbar}$, we need: \\

\begin{tabular}{|l|}
  \hline
  {\bf (i)}\ a category $\catd$ and a functor $\funbar : \catc \to \catd$,
  \\
  {\bf (ii)}\ a monad $( \td, \unitd{}, \multd{} )$ on $\catd$,\\
  \qquad related to $(\tc, \unitc{}, \multc{})$ by a monad morphism $(\funbar,
  \dist{})$ from $\tc$ to $\td$,\\
  {\bf (iii)}\ a mono factorization system on $\catd$,\\
  {\bf (iv)}\ $\td$ maps relevant pseudoepis to pseudoepis.\\
  \hline
\end{tabular}\\

Recall that to lift the CCC structure of $\catc$ to the subscone, we
additionally require $\catd$ to be a CCC with pullbacks, and $\funbar$ to
preserve finite products \cite{MS93}. Description of the construction can be
found e.g., in~\cite{GG01}, Section~5.4.  We shall see in Section~\ref{ccc.s}
that the existence of a mono factorization system on $\catd$ allows us to
relax the requirements on $\funbar$ somewhat.

%\subsubsection*{Summary of assumptions}

%\begin{itemize}
%\item
%We are given two categories,
%$\catc$ and $\catd$ together with a functor 
%$\funbar : \catc \to \catd$.

%\item
%We are given two monads, $( \tc, \unitc{}, \multc{} )$
%on $\catc$
%and $( \td, \unitd{}, \multd{} )$ on $\catd$,
%related by a distributivity law $\dist{}$.

%\item
%Category $\catd$ has a mono factorization system.

%\item
%Functor $\td$ preserves
%pseudoepis.

%\end{itemize}



\section{Lifting of a Monad to Relations}
\label{relations.s}

Recall that we would like to lift monads to categories of binary relations as objects.
%The main motivation is to consider a lifting
%of a construction, given by a monad, to category of
%binary relations.
Hence, assume in this section that $\catc$ is a product category, $\catc =
\catc_1 {\times} \catc_2$ and that both $\catc_1$ and $\catc_2$ are equipped
with monads $\tc_1$ and $\tc_2$, and functors $\funbar_1 : \catc_1 \to \catd$
and $\funbar_2 : \catc_2 \to \catd$.  A monad $\tc$ on $\catc$ can be defined
pairwise: $\tc \langle A_1, A_2 \rangle = \langle \tc_1 A_1, \tc_2 A_2
\rangle$ and similarly we define $\funbar : \catc \to \catd$ by
$\funbara{(A_1, A_2)} = \funbaraa{1}{A_1} {\times}
\funbaraa{2}{A_2}$.

\noindent
\begin{minipage}{6cm}
  To this aim we assume binary products in $\catd$, i.e., for each pair of objects
  $A_1$, $A_2$ of $\catd$, an object $A_1 \times A_2$ in $\catd$, together
  with two morphisms $\pi_1 : A_1 \times A_2 \to A_1$ and $\pi_2 : A_1 \times
  A_2 \to A_2$ satisfying the requirement that for every morphisms $f_1$ and
  $f_2$,
% making the diagram of solid arrows (right) commute, 
  there is a unique morphism $h$ making the whole diagram commute.
  We write $\pair {f_1} {f_2}$ for $h$.  
\end{minipage}
\begin{minipage}{6cm}
  \[
  \xymatrix{
    C
    \ar[rrd]^{f_1}
    \ar@{.>}[rd]|{h}
    \ar[rdd]_{f_2}
    &&
    \\
    & A_1 \times A_2
    \ar[r]^{\pi_1}
    \ar[d]_{\pi_2}
    & A_1
    \\
    & A_2
    &
    }
  \]
\end{minipage}

In the same vein monad morphisms from $\tc_1$ to $\td$ and from $\tc_2$ to
$\td$ induce a monad morphism from $\tc$ to $\td$.  Indeed, given any two
monad morphisms
%distributivity laws for $\catc_1$
%and $\catc_2$ induce a distributivity law for $\catc$.
%Assumed two distributivity laws,
\[
\disttwoarg{}{1} : \td \funbar_1 \ \ \natto \ \  \funbaraa{1}{\tc_1}
\ \ \ \ \mbox{and} \ \ \ \ 
\disttwoarg{}{2} : \td \funbar_2 \ \ \natto \ \  \funbaraa{2}{\tc_2},
\]
we can define 
$\dist{(A_1, A_2)} : 
\td (\funbaraa{1}{A_1} {\times} \funbaraa{2}{A_2}) \to 
\funbaraa{1}{\tc_1 A_1} {\times} \funbaraa{2}{\tc_2 A_2}$ by
\begin{equation}
\label{e_distprod}
\dist{(A_1, A_2)} = \pair
{\disttwoarg{A_1}{1} \circ \td \proj_1}
{\disttwoarg{A_2}{2} \circ \td \proj_2},
\end{equation}
where $\proj_1$ and $\proj_2$ denote the projections
from $\funbaraa{1}{A_1} {\times} \funbaraa{2}{A_2}$.

The situation gets much simpler when $\catd = \catset$, $\funbar_1 =
\homset{\catc_1}{\termobj_1}{\_}$ and $\funbar_2 =
\homset{\catc_2}{\termobj_2}{\_}$, where we assume that $\catc_1$ and
$\catc_2$ have terminal objects, $\termobj_1$ and $\termobj_2$ respectively.
Each object $\xymatrix@-5pt{S \arrnotrelmonoxy[r] & \funbara{(A_1, A_2)}}$
in the subscone defines a binary relation (again noted $S$) on
global elements of $A_1$ and $A_2$. Obviously $\catset$ satisfies all
requirements from previous sections, with surjections as pseudoepis and
injections as relevant monos.

For a moment imagine that $\tc_1$ and $\tc_2$ are {\em strong}
monads and that we are able to lift strong monads to subscones --
this will be tackled in detail in the following 
Sections~\ref{sec:monoidal} and~\ref{strong.s}.
Given two CCCs $\catc_1$ and $\catc_2$ with respective strong monads $\tc_1$
and $\tc_2$, the fact that $\comp$ is the free CCC with strong monad on the
set $B$ of base types means that there are two representations of
CCCs-with-strong-monads, $\Eval\__1$ and $\Eval\__2$, from $\comp$ to
$\catc_1$ and $\catc_2$ respectively: they are the natural meaning functions
for monadic types and computational $\lambda$-terms.  \\

\noindent
\begin{minipage}{6.5cm}
  
  Our construction of a lifting together with standard constructions on
  subscones \cite{MS93} yield another representation of
  CCCs-with-strong-monads $\Eval\_$ from $\comp$ to $\subscone{\catc_1 \times
    \catc_2}{\setcat}{\funbar}$.  That $\Eval\_$ is a lifting means that
  $\forfun \circ \Eval\_ = \pair {\Eval\__1} {\Eval\__2}$, i.e., the diagram on the
  right commutes.  When $\catc_1$ and $\catc_2$ are concrete categories, this
  means that
\end{minipage}
\begin{minipage}{5.5cm}
  \[
\ \ \ \ 
 \xymatrix@-10pt{
 & & \subscone{\catc_1 \times \catc_2}{\setcat}{\funbar} \ar[d]^{\forfun} \\
\comp \ar[rru]^{\Eval\_} \ar[rr]_{\langle \Eval\__1, \Eval\__2 \rangle} 
 & & 
\catc_1 \times \catc_2
  }
  \]
\ \\    
\end{minipage}

\begin{equation}
  \label{eq:basic}
  \forall a_1 \in \Eval \Gamma_1, a_2 \in \Eval \Gamma_2 .
  (a_1, a_2) \in \Eval \Gamma \Rightarrow (\Eval t_1 (a_1), \Eval t_2 (a_2)) \in
  \Eval {\tau}
\end{equation}
for all terms $t$ of type $\tau$ in the context $\Gamma = x_1:\tau_1, \ldots,
x_n:\tau_n$; representations of $\Gamma$ are taken to be products of the
representations of $\tau_1$, \ldots, $\tau_n$; $\Eval \tau$ is a relation
between $\Eval \tau_1$ and $\Eval \tau_2$, defined by induction on types
$\tau$ (the case where $\tau$ is a base type is arbitrary):
\[
\begin{array}{c}
  (f_1, f_2) \in \Eval {\tau \to \tau'} \iff \forall (a_1, a_2) \in \Eval \tau .
  (f_1(a_1), f_2(a_2)) \in \Eval {\tau'} \\
  ((a_1, a'_1), (a_2,a'_2)) \in \Eval {\tau \times \tau'} \iff (a_1, a_2) \in \Eval \tau \land
  (a'_1, a'_2) \in \Eval {\tau'} \\
  (B_1, B_2) \in \Eval {\tc \tau} \iff (B_1, B_2) \in \tS {\Eval \tau}
\end{array}
\]
These equations (except possibly the last one) are the standard definition of
a {\em logical relation}. (\ref{eq:basic}) is the already cited {\em Basic
  Lemma}.

Further simplification is gained when $\catc_1 = \catc_2 = \catset$, the three
monads $\tc_1$, $\tc_2$ and $\td$ are identical and both $\funbar_1$ and
$\funbar_2$ are identity functors.  The monad morphism $\dist{}$ reduces to
distributivity of the monad $\td$ over binary product, and (\ref{e_distprod})
rewrites to \iflong
\[
\dist{(A_1, A_2)} = \pair
{\td \proj_1} {\td \proj_2} : 
\td (A_1 {\times} A_2) \to \td A_1 {\times} \td A_2
\]
\else
$\dist{(A_1, A_2)} = \langle
\td \proj_1, \td \proj_2 \rangle : 
\td (A_1 {\times} A_2) \to \td A_1 {\times} \td A_2$, 
\fi 
where by $\td$ we denote a given single monad on $\catset$.
This is a particularly important special case, so we study it in more
detail.

Every binary relation $S \subseteq A_1 \times A_2$ has a representation
$\xymatrix@-5pt{S \arrnotrelmonoxy[rr]^(.4){\pair {\projrel_1} {\projrel_2}} 
& & A_1 {\times} A_2}$ where the arrow is the inclusion induced
by two projections $\projrel_1 : S \to A_1$ and $\projrel_2 : S \to A_2$. In
fact, the full subcategory of the subscone consisting exclusively of
inclusions instead of all injections is equivalent to the whole subscone, so
without loss of generality we consider only inclusions in the rest of this
section.

\noindent
\begin{minipage}{6cm}
  Recall the action of a lifted monad $\tS$ on a relation $\xymatrix@-5pt{S
    \arrnotrelmonoxy[rr]^(.4){\pair {\projrel_1} {\projrel_2}} & & A_1
    {\times} A_2}$:
\end{minipage}
\begin{minipage}{6cm}
  \[
  \xymatrix@-10pt{
    \td S \ar[rr]^(.4){\td {\pair {\projrel_1} {\projrel_2}}} 
    \arrepixy[d] & &
    \td(A_1 {\times} A_2) \ar[d]^{\dist{(A_1,A_2)}} \\
    \lift{S} \arrmonoxy[rr] & & \td A_1 {\times} \td A_2
    }
  \]
\end{minipage}
% If $\td$ preserves also monos, which is often
% the case, 

\iflong%
\noindent
The functor $\tS$ maps a relation $S$ to the relation between sets $\td A_1$
and $\td A_2$ defined as the direct image of the function $\pair {\td
\projrel_1} {\td \projrel_2} : TS \to \td A_1 {\times} \td A_2$, since
the middle (dashed) triangle in the following diagram commutes by the
universal property of product (together with all other triangles):
\[
\xymatrix@-5pt{
  & & & & \td S 
  \ar@{-->}[dd]|{\td \pair {\projrel_1} {\projrel_2}} 
  \ar@/_/@{-->}[lddd]|{\pair {\td \projrel_1} {\td \projrel_2}}
  \ar@/_/[llllddd]_{\td \projrel_1} \ar@/^/[rddd]^{\td \projrel_2} & \\
  & & & & & \\
  & & & & \td (A_1 {\times} A_2) 
  \ar[lllld]|(.33)\hole _{\td \proj_1}  
  \ar@{-->}[ld]|{\pair {\td \proj_1} {\td \proj_2}}
  \ar[rd]_{\td \proj_2} & \\
  \td A_1 & & & \td A_1 {\times} \td A_2 \ar[lll]^{\proj'_1} 
  \ar[rr]_{\proj'_2} & & \td A_2
  }
\]
where by $\proj'_1$ and $\proj'_2$ we denote two
projections from $\td A_1 {\times} \td A_2$.

It is instructive to look at some concrete example before going to more
technical Sections~\ref{sec:monoidal} and ~\ref{strong.s}. Further examples
are presented in more detail in Section~\ref{examples.s}. Consider $\td A =
\pfin{A}$, the finite powerset monad on $\catset$. If we assume for simplicity
that $\projrel_1$ and $\projrel_2$ are simply inclusions, then the function
$\td \projrel_1$ takes a finite relation $R \subset S$ to its domain, i.e. $\{x | \exists y
\cdot (x, y) \in R\}$, and $\td \projrel_2$ takes $R$ to its codomain, i.e., $\{y | \exists
x \cdot (x, y) \in R\}$. Hence, the image of the function $\pair {\td \projrel_1}
{\td \projrel_2}$ is a relation $\lift{S}$ between finite subsets of $A_1$ and
$A_2$ that contains precisely domain-codomain pairs of finite relations $R \subseteq
S$. Hence $(B_1, B_2) \in \lift{S}$ iff
\[
\forall b_1 \in B_1 . \exists b_2 \in B_2 . (b_1, b_2) \in S 
\ \ \ \  \land 
\ \ \ \ 
\forall b_2 \in B_2 . \exists b_1 \in B_1 . (b_1, b_2) \in S.
\]
\else%
The functor $\tS$ maps a relation $S$ to the relation between sets $\td A_1$
and $\td A_2$ defined as the direct image of the function $\langle \td
\projrel_1, \td \projrel_2 \rangle : TS \to \td A_1 {\times} \td A_2$,
since $\langle \td \projrel_1, \td \projrel_2 \rangle =
\langle \td \proj_1, \td \proj_2 \rangle \circ 
\td \langle \projrel_1, \projrel_2 \rangle$.

\comment{

not really necessary  (SL, 18.06.2002)


\noindent
\begin{minipage}{4cm}
  Indeed the middle (dashed) triangle in the diagram on the right commutes by
  the universal property of product (together with all other triangles).  By
  $\proj'_1$ and $\proj'_2$ we denote two projections from $\td A_1 {\times}
  \td A_2$.
\end{minipage}
\begin{minipage}{8cm}
  \tiny
  \[
  \xymatrix@-5pt{
    & & & & \td S 
    \ar@{-->}[dd]|{\td \langle \projrel_1, \projrel_2 \rangle} 
    \ar@/_/@{-->}[lddd]|{\langle \td \projrel_1, \td \projrel_2 \rangle}
    \ar@/_/[llllddd]_{\td \projrel_1} \ar@/^/[rddd]^{\td \projrel_2} & \\
    & & & & & \\
    & & & & \td (A_1 {\times} A_2) 
    \ar[lllld]|(.33)\hole _{\td \proj_1}  
    \ar@{-->}[ld]|{\langle \td \proj_1, \td \proj_2 \rangle}
    \ar[rd]_{\td \proj_2} & \\
    \td A_1 & & & \td A_1 {\times} \td A_2 \ar[lll]^{\proj'_1} 
    \ar[rr]_{\proj'_2} & & \td A_2
    }
  \]
\end{minipage}

}

\fi%

\cite{Pit96} also considers lifting of certain constructions on
objects to corresponding constructions on relations over these
objects. The concept of lifting is similar to ours, although
technically different.
The notion of ''relation'' used in the paper is given by a so called
\emph{relational structure} on a category, and is fairly abstract.
On the other hand, Pitts restricts to categories of domains, usually 
defined as least solutions of recursive domain equations.
The interest of the author is mainly in questions related to domain theory.
One of main results gives conditions for existence of lifting of 
the solution of an equation in the following sense:
given a domain defined by $D = \Phi(D)$, is there a relation $\Delta$ on
$D$ such that $\Delta = \Phi(\Delta)$?
Strong monads and their liftings are not considered in the work of Pitts.
Although, for certain types of relational structures the approach
of Pitts seems to yield similar liftings as ours. E.g., in the case
of binary relations, the function space is lifted precisely as
logical relations are usually defined on a function type, and hence
exactly like in the case of lifting to subscones.



\section{Lifting Monoidal Structures}
\label{sec:monoidal}



\subsection{Monoidal Categories}
\label{sec:monoidal:1}


In this section, and the following ones, we assume that each of the categories
$\catc$ and $\catd$ is equipped with a monoidal structure. 
In other words, we
assume that $(\catc, \tensorc, \Ic, \alphacna, \lc{}, \rc{})$ and $(\catd,
\tensord, \Id, \alphadna, \ld{}, \rd{})$ are {\em monoidal categories\/}
\cite{McLane:cat:math}.
This will allow us to extend our lifting of a monad to one of a strong
monad in the following Section~\ref{strong.s}.


This means that $\Id$ is an object of $\catd$, $\tensord$ is a functor from
$\catd \times \catd$ to $\catd$, and $\alphad A B C : (A \tensord B) \tensord
C \to A \tensord (B \tensord C)$, $\ld A : \Id \tensord A \to A$, $\rd A : A
\tensord \Id \to A$ are natural isomorphisms called the associativity, the
left unit and the right unit laws respectively, making the following squares
commute.
%!!! ca marche aussi si ce sont juste des transformations naturelles, mais
 %Ambler (3.1, p.35) dit que ce sont des isos.
\begin{equation}
  \label{eq:alpha:coh1}
  \xymatrix@C-5pt{
    ((A \tensord B) \tensord C) \tensord D \ar[r]^{\alphad {A \tensord B} C D}
    \ar[d]^{\alphad A B C \tensord \identity D}
    & (A \tensord B) \tensord (C \tensord D) \ar[r]^{\alphad A B {C \tensord
        D}}
    & A \tensord (B \tensord (C \tensord D)) \\
    (A \tensord (B \tensord C)) \tensord D \ar[rr]_{\alphad A {B \tensord C} D}
    && A \tensord ((B \tensord C) \tensord D)
    \ar[u]^{\identity A \tensord \alphad B C D}
    }
\end{equation}

% d'apres Simon Ambler, 3.1, p.35, on n'a pas ces deux-la?
% d'apres MacLane, ils sont deductibles de l_I=r_I; d'apres David, meme ce
 % dernier est deductible.
%\begin{minipage}{5.5cm}
%  \begin{equation}
%    \label{eq:alpha:cohll}
%    \xymatrix@-10pt{
%      (\Id \tensord A) \tensord B \ar[r]^{\alphad \Id A B}
%      \ar[rd]_{\ld A \tensord \identity B}
%      & \Id \tensord (A \tensord B) \ar[d]^{\ld {A \tensord B}}
%      \\
%      & A \tensord B
%      }
%  \end{equation}
%\end{minipage}
%\qquad
%\begin{minipage}{5.5cm}
%  \begin{equation}
%    \label{eq:alpha:cohrr}
%    \xymatrix@-10pt{
%      (A \tensord B) \tensord \Id \ar[r]^{\alphad A B \Id}
%      \ar[d]_{\rd {A \tensord B}}
%      & A \tensord (B \tensord \Id)
%      \ar[ld]^{\identity A \tensord \rd B}
%      \\
%      A \tensord B
%      }
%  \end{equation}
%\end{minipage}

\noindent
\begin{equation}
  \label{eq:alpha:cohlr}
  \xymatrix{
    (A \tensord \Id) \tensord B \ar[rr]^{\alphad A \Id B}
    \ar[rd]_{\rd A \tensord \identity B}
    && A \tensord (\Id \tensord B)
    \ar[ld]^{\identity A \tensord \ld B}
    \\
    & A \tensord B &
    }
\end{equation}
And similarly for $\Ic$, $\tensorc$, $\alphacna$, $\lc{}$, $\rc{}$.

We prefer to work
in a slightly more general setting compared to~\cite{MS93}, where cartesian structure
was assumed.
\ifmscs
\else
In Section~\ref{ccc.s} we show how this added generality can be exploited
for a fragment of linear lambda calculus.
\fi
Typically, our categories will have finite products, then $\Id$ will be a
terminal object, $\tensord$ will be binary product, and $\alphadna$, $\ld{}$
and $\rd{}$ will be the obvious isomorphisms.


%products given explicitly. By the same symbol $\termobj$ we denote the
%terminal object both in $\catc$ and $\catd$. Moreover we assume that
%natural isomorphisms are given:
%\begin{align}
%\label{e_natisos}
%\begin{aligned}
%  \rc{A} : \termobj {\times} A \to A   & & 
%  \alphac{A}{B}{C} : (A {\times} B) {\times} C \to A {\times} (B {\times} C) &
%  &
%  \mbox{in $\catc$} \\
%  \rd{S} : \termobj {\times} S \to S   & &
%  \alphad{S}{R}{Q} : (S {\times} R) {\times} Q \to S {\times} (R {\times} Q)
%  &&
%  \mbox{in $\catd$}
%\end{aligned}
%\end{align}

We also assume that $\funbar$ is a {\em monoidal functor\/}
\cite{EK:closed:cat}.  That is, there is a {\em mediating pair\/} $(\tstrna,
\tstri)$, composed of a natural transformation $\tstr A B : \funbara A
\tensord \funbara B \to \funbara {A \tensorc B}$ and a morphism $\tstri : \Id
\to \funbara \Ic$ satisfying the following {\em coherence conditions}:
\begin{equation}
  \label{eq:theta:coh:alpha}
  \xymatrix@C+20pt{
    (\funbara A \tensord \funbara B) \tensord \funbara C
    \ar[r]^{\alphad {\funbara A} {\funbara B} {\funbara C}}
    \ar[d]_{\tstr A B \tensord \identity {\funbara C}}
    &
    {\funbara A \tensord (\funbara B \tensord \funbara C)}
    \ar[d]^{\identity {\funbara A} \tensord \tstr B C}
    \\
    {\funbara {A \tensorc B} \tensord \funbara C}
    \ar[d]_{\tstr {A \tensorc B} C}
    &
    {\funbara A \tensord \funbara {B \tensorc C}}
    \ar[d]^{\tstr A {B \tensorc C}}
    \\
    {\funbara {(A \tensorc B) \tensorc C}}
    \ar[r]_{\funbara {\alphac A B C}}
    &
    {\funbara {A \tensorc (B \tensorc C)}}
    }
\end{equation}

\noindent
\begin{minipage}{5.5cm}
  \begin{equation}
    \label{eq:theta:coh:l}
    \xymatrix{
      {\Id \tensord \funbara A}
      \ar[d]_{\tstri \tensord \identity {\funbara A}}
      \ar[rd]^{\ld {\funbara A}}
      \\
      {\funbara \Ic \tensord \funbara A}
      \ar[d]_{\tstr \Ic A}
      &
      {\funbara A}
      \\
      {\funbara {\Ic \tensorc A}}
      \ar[ru]_{\funbara {\lc A}}
      }
  \end{equation}
\end{minipage}
\qquad
\begin{minipage}{5.5cm}
  \begin{equation}
    \label{eq:theta:coh:r}
    \xymatrix{
      {\funbara A \tensord \Id}
      \ar[d]_{\identity {\funbara A} \tensord \tstri}
      \ar[rd]^{\rd {\funbara A}}
      \\
      {\funbara A \tensord \funbara \Ic}
      \ar[d]_{\tstr A \Ic}
      &
      {\funbara A}
      \\
      {\funbara {A \tensorc \Ic}}
      \ar[ru]_{\funbara {\rc A}}
      }
  \end{equation}
\end{minipage}

\noindent
Finally, we assume that pseudoepis and relevant monos form a so-called {\em
  monoidal mono factorization system}, i.e., for every two pseudoepis $e_1$,
$e_2$, then $e_1 \tensord e_2$ is again a pseudoepi.  This name stems from
\cite{SJA:thesis}, Definition~5.2.1, p.91.

We define below a lifting of the monoidal structure to the subscone: we show
that the subscone is a monoidal category $(\subscone \catc \catd \funbar,
\tensorS, \IS, \alphaSna, \lS{}, \rS{})$ in such a way that $\forfun (\lift A
\tensorS \lift B) = \forfun {\lift A} \tensorc \forfun {\lift B}$, $\forfun
\IS = \Ic$, $\forfun \alphaS {\lift A} {\lift B} {\lift C} = \alphac {\forfun
  {\lift A}} {\forfun {\lift B}} {\forfun {\lift C}}$, $\forfun {\lS {\lift
    A}} = \lc {\forfun {\lift A}}$, $\forfun {\rS {\lift A}} = \rc {\forfun
  {\lift A}}$. Lifting to scones is omited here but can be easily extracted
from diagrams below by dropping all factorizations.

\noindent
\begin{minipage}{8.5cm}
  \subsection{Unit element $\IS$.}
  Let $\IS$ be the triple $\langle \overline I, \overline \tstri, \Ic\rangle$
  as built from the diagram on the right, obtained from a factorization of
  $\tstri$.
\end{minipage}
\begin{minipage}{3.5cm}
  \begin{equation}
    \label{d_IS}
    \xymatrix@-5pt{
      {\Id}
      \ar[rd]^{\tstri}
      \arrepixy[d]_{e_I}
      & \\
      {\overline I}
      \arrmonoxy[r]_{\overline \tstri}       % {m_I}
      &
      {\funbara \Ic}
      }
  \end{equation}
\end{minipage}

\noindent
\subsection{Tensor product $\tensorS$.}  We build the tensor product $\langle
S_1, m_1, A_1\rangle \tensorS \langle S_2, m_2, A_2 \rangle$ in the obvious
way: compose $m_1 \tensord m_2$ with the mediating natural transformation
$\tstrna$, and factorize.

\noindent
\begin{minipage}{6cm}
  The tensor product is then given by $\langle S_{12}, m_{12}, A_1 \tensorc
  A_2\rangle$ on the right.  This is similar to the construction of $\tS$.
\end{minipage}
\begin{minipage}{6cm}
  \begin{equation}
    \label{d_tensorS}
    \xymatrix@C+10pt{
      S_1 \tensord S_2
      \ar[r]^{m_1 \tensord m_2}
      \arrepixy[d]_{e_{12}}
      &
      {\funbara {A_1} \tensord \funbara {A_2}}
      \ar[d]_{\tstr {A_1} {A_2}}
      \\
      S_{12}
      \arrmonoxy[r]_{m_{12}}
      &
      {\funbara {A_1 \tensorc A_2}}
      }
  \end{equation}
\end{minipage}

\noindent
\subsection{Associativity $\alphaSna$.}
This is more involved, but basically similar to the construction of the
multiplication of the monad in the subscone.  In the diagram below, $e_{12}
\tensord \identity {S_3}$ is pseudoepi because both $e_{12}$ (given by
Diagram~\ref{d_tensorS}) and $\identity {S_3}$ are pseudoepis, and because our
mono factorization system is monoidal.  The two front faces and the two back
faces are derived from the definition of $\tensorS$, the top face is a
naturality square for $\alphadna$, the right face is the coherence
condition~(\ref{eq:theta:coh:alpha}).  The dashed arrow, and then the dotted
arrow $\widehat \alpha$, are by the diagonal fill-in property of our
factorization system.  The desired associativity morphism is then the pair
$(\widehat \alpha, \alphac {A_1} {A_2} {A_3})$ (bottom face).

\begin{equation}
  \label{d_alphaS}
  \xymatrix@C-28pt@R-10pt{
    (S_1 \tensord S_2) \tensord S_3
    \ar[rr]^{(m_1 \tensord m_2) \tensord m_3}
    \arrepixy[dd]_{e_{12} \tensord \identity {S_3}}
    \ar[rd]^{\alphad {S_1} {S_2} {S_3}}
    &
    &
    (\funbara {A_1} \tensord \funbara {A_2}) \tensord \funbara {A_3}
    \ar[dd]|\hole_(0.7){\tstr {A_1} {A_2} \tensord \identity {A_3}}
    \ar[rd]^{\alphad {\funbara {A_1}} {\funbara {A_2}} {\funbara {A_3}}}
    &
    \\
    &
    S_1 \tensord (S_2 \tensord S_3)
    \ar[rr]^(0.65){m_1 \tensord (m_2 \tensord m_3)}
    \ar[dd]_(0.7){\identity {S_1} \tensord e_{23}}
    &
    &
    {\funbara {A_1} \tensord (\funbara {A_2} \tensord \funbara {A_3})}
    \ar[dd]_(0.3){\identity {\funbara {A_1}} \tensord \tstr {A_2} {A_3}}
    \\
    S_{12} \tensord S_3
    \ar[rr]|(0.47)\hole^(0.3){m_{12} \tensord m_3}
    \arrepixy[dd]_{e_{(12)3}}
    \ar@{-->}[rddd]
    &
    &
    {\funbara {A_1 \tensorc A_2} \tensord \funbara {A_3}}
    \ar[dd]|\hole_(0.7){\tstr {A_1 \tensorc A_2} {A_3}}
    &
    \\
    &
    S_1 \tensord S_{23}
    \ar[rr]^(0.6){m_1 \tensord m_{23}}
    \ar[dd]^(0.7){e_{1(23)}}
    &
    &
    {\funbara {A_1} \tensord \funbara {A_2 \tensorc A_3}}
    \ar[dd]_(0.3){\tstr {A_1} {A_2 \tensorc A_3}}
    \\
    S_{(12)3}
    \arrmonoxy[rr]|(0.47)\hole_(0.7){m_{(12)3}}
    \ar@{.>}[rd]_{\widehat \alpha}
    &
    &
    {\funbara {(A_1 \tensorc A_2) \tensorc A_3}}
    \ar[rd]_{\funbara {\alphac {A_1} {A_2} {A_3}}}
    &
    \\
    &
    S_{1(23)}
    \arrmonoxy[rr]_{m_{1(23)}}
    &
    &
    {\funbara {A_1 \tensorc (A_2 \tensorc A_3)}}
    }
\end{equation}

\ifmscs
The inverse is given by a very similar diagram.
\else
The inverse is given by a very similar diagram (below).

\begin{equation}
  \label{d_alphaS-1}
  \xymatrix@C-28pt@R-10pt{
    (S_1 \tensord S_2) \tensord S_3
    \ar[rr]^{(m_1 \tensord m_2) \tensord m_3}
    \ar[dd]_{e_{12} \tensord \identity {S_3}}
    &
    &
    (\funbara {A_1} \tensord \funbara {A_2}) \tensord \funbara {A_3}
    \ar[dd]|\hole_(0.7){\tstr {A_1} {A_2} \tensord \identity {A_3}}
    &
    \\
    &
    S_1 \tensord (S_2 \tensord S_3)
    \ar[rr]^(0.65){m_1 \tensord (m_2 \tensord m_3)}
    \arrepixy[dd]_(0.7){\identity {S_1} \tensord e_{23}}
    \ar[lu]_{\alphad {S_1} {S_2} {S_3}^{-1}}
    &
    &
    {\funbara {A_1} \tensord (\funbara {A_2} \tensord \funbara {A_3})}
    \ar[dd]_(0.3){\identity {\funbara {A_1}} \tensord \tstr {A_2} {A_3}}
    \ar[lu]_{\alphad {\funbara {A_1}} {\funbara {A_2}} {\funbara {A_3}}^{-1}}
    \\
    S_{12} \tensord S_3
    \ar[rr]|(0.47)\hole^(0.3){m_{12} \tensord m_3}
    \ar[dd]_{e_{(12)3}}
    &
    &
    {\funbara {A_1 \tensorc A_2} \tensord \funbara {A_3}}
    \ar[dd]|\hole_(0.7){\tstr {A_1 \tensorc A_2} {A_3}}
    &
    \\
    &
    S_1 \tensord S_{23}
    \ar[rr]^(0.6){m_1 \tensord m_{23}}
    \arrepixy[dd]^(0.7){e_{1(23)}}
    \ar@{-->}[ld]
    &
    &
    {\funbara {A_1} \tensord \funbara {A_2 \tensorc A_3}}
    \ar[dd]_(0.3){\tstr {A_1} {A_2 \tensorc A_3}}
    \\
    S_{(12)3}
    \arrmonoxy[rr]|(0.47)\hole_(0.7){m_{(12)3}}
    &
    &
    {\funbara {(A_1 \tensorc A_2) \tensorc A_3}}
    &
    \\
    &
    S_{1(23)}
    \arrmonoxy[rr]_{m_{1(23)}}
    \ar@{.>}[lu]^{\widehat \alpha^{-1}}
    &
    &
    {\funbara {A_1 \tensorc (A_2 \tensorc A_3)}}
    \ar[lu]^{\funbara {\alphac {A_1} {A_2} {A_3}^{-1}}}
    }
\end{equation}

\fi

\subsection{Left unit $\lS{}$.}
Let $\langle S, m, A \rangle$ be any object of the subscone.  We build the
diagram below.  The left triangle in the upper back face is the definition of
$\IS$, the rest of this face corresponds to two ways of writing $\tstri
\tensord m$, the lower back face is the definition of $\IS \tensorS \langle S,
m, A\rangle$.  The upper, slanted face is a naturality square for $\ld{}$.

\noindent
\begin{minipage}{3cm}
  Finally, the rightmost triangle is the coherence
  condition~(\ref{eq:theta:coh:l}).
  
  As usual, we first derive the dashed, then the dotted arrow $\widehat
  {\ld{}}$ by diagonal fill-ins.  The desired left unit is $(\widehat {\ld{}},
  \lc A)$.
\end{minipage}
\begin{minipage}{9cm}
\begin{equation}
  \label{d_lS}
  \xymatrix@H-25pt{
    {\Id \tensord S}
    \ar[rr]^{\identity \Id \tensord m}
    \ar[rd]^{\tstri \tensord \identity S}
    \arrepixy[d]_{e_I \tensord \identity S}
    \ar[rddd]^{\ld S}
    &
    &
    {\Id \tensord \funbara A}
    \ar[d]^{\tstri \tensord \identity {\funbara A}}
    \ar[rddd]^{\ld {\funbara A}}
    &
    \\
    {\overline \Ic \tensord S}
    \ar[r]|(0.33)\hole^{\overline \tstri \tensord \identity S}
    \arrepixy[d]_{e_{12}}
    \ar@{-->}[rdd]
    &
    {\funbara \Ic \tensord S}
    \ar[r]^{\identity {\funbara \Ic} \tensord m}
    &
    {\funbara \Ic \tensord \funbara A}
    \ar[d]^{\tstr \Ic A}
    &
    \\
    S_{12}
    \arrmonoxy[rr]|(0.33)\hole_{m_{12}}
    \ar@{.>}[rd]_{\widehat {\ld{}}}
    &
    &
    {\funbara {\Ic \tensorc A}}
    \ar[rd]^{\funbara {\lc A}}
    &
    \\
    &
    S
    \arrmonoxy[rr]_{m}
    &
    &
    {\funbara A}
    }
\end{equation}
\end{minipage}

\noindent
The inverse to $\widehat {\ld{}}$ is also given by a diagonal fill-in.  Start
from $S$, then go to $S$ (again) by the identity morphism---this is a
pseudoepi---, then follow $m$, $\funbara {\lc A^{-1}}$ to $\funbara {\Ic
  \tensorc A}$; or start from $S$, climb along $\ld S^{-1}$, then follow $e_I
\tensord \identity S$, $e_{12}$, $m_{12}$ (a mono) to $\funbara {\Ic \tensorc
  A}$.  The diagonal fill-in is then an arrow from $S$ to $S_{12}$, which is
inverse to $\widehat {\ld{}}$ by Fact~\ref{f_eq}.

\noindent
\begin{minipage}{3cm}
  \subsection{Right unit $\rS{}$.}
  This works exactly as for the left unit, see diagram on the right.  The
  right triangle is the coherence condition~(\ref{eq:theta:coh:r}).  The
  desired right unit is given by $(\widehat {\rd{}}, \rc A)$.
  
  The inverse of $\widehat {\rd{}}$ is built as for $\widehat {\ld{}}$.
\end{minipage}
\begin{minipage}{9cm}
\begin{equation}
  \label{d_rS}
  \xymatrix@H-25pt{
    S \tensord \Id
    \ar[rr]^{m \tensord \identity \Id}
    \ar[rd]^{\identity S \tensord \tstri}
    \arrepixy[d]_{\identity S \tensord e_I}
    \ar[rddd]^{\rd S}
    &
    &
    {\funbara A \tensord \Id}
    \ar[d]^{\identity {\funbara A} \tensord \tstri}
    \ar[rddd]^{\rd {\funbara A}}
    &
    \\
    S \tensord \overline \Ic
    \ar[r]|(0.33)\hole^{\identity S \tensord \overline \tstri}
    \arrepixy[d]_{e_{12}}
    \ar@{-->}[rdd]
    &
    S \tensord \funbara \Ic
    \ar[r]^{m \tensord \identity {\funbara \Ic}}
    &
    {\funbara A \tensord \funbara \Ic}
    \ar[d]^{\tstr A \Ic}
    &
    \\
    S_{12}
    \arrmonoxy[rr]|(0.33)\hole_{m_{12}}
    \ar@{.>}[rd]_{\widehat {\rd{}}}
    &
    &
    {\funbara {A \tensorc \Ic}}
    \ar[rd]^{\funbara {\rc A}}
    &
    \\
    &
    S
    \arrmonoxy[rr]_{m}
    &
    &
    {\funbara A}
    }
\end{equation}
\end{minipage}

Finally, all required naturality, isomorphism, and coherence conditions hold
by Fact~\ref{f_eq}.

We recap what we need to lift monoidal structure to the subscone:

\begin{tabular}{|l|}
  \hline
  {\bf (i.a)} monoidal categories $(\catc, \tensorc, \Ic, \alphacna, \lc{},
  \rc{})$ and $(\catd, \tensord, \Id, \alphadna, \ld{}, \rd{})$, \\
  \qquad and a monoidal functor $\funbar : \catc \to \catd$,\\
  {\bf (iii.a)} a monoidal mono factorization system on $\catd$.\\
  \hline
\end{tabular}


\subsection{Symmetric Monoidal Categories}
\label{sec:monoidal:sym}


We now assume that we have got, and want to preserve {\em symmetric\/}
monoidal structure.  Recall that a symmetric monoidal category $(\catd,
\tensord, \Id, \alphadna, \ld{}, \rd{}, \cdna)$ is a monoidal category
$(\catd, \tensord, \Id, \alphadna, \ld{}, \rd{})$, together with a {\em
  commutativity\/} natural transformation $\cd A B : A \tensord B \to B
\tensord A$ obeying the following coherence conditions.

The first coherence condition is $\cd B A \circ \cd A B = \identity {A
  \tensord B}$, which implies that $\cdna$ is actually a natural isomorphism.
The others are:
\begin{equation}
  \label{eq:alpha:coh:c}
  \xymatrix@C+10pt{
    (A \tensord B) \tensord C
    \ar[r]^{\cd A B \tensord \identity C}
    \ar[d]_{\alphad A B C}
    & (B \tensord A) \tensord C
    \ar[d]^{\alphad B A C}
    \\
    A \tensord (B \tensord C)
    \ar[d]_{\cd A {B \tensord C}}
    & B \tensord (A \tensord C)
    \ar[d]^{\identity B \tensord \cd A C}
    \\
    (B \tensord C) \tensord A
    \ar[r]_{\alphad B C A}
    & B \tensord (C \tensord A)
    }
\end{equation}

\begin{equation}
  \label{eq:c:cohlr}
  \xymatrix{
    {\Id \tensord A}
    \ar[rr]^{\cd \Id A}
    \ar[rd]_{\ld A}
    &&
    A \tensord \Id
    \ar[ld]^{\rd A}
    \\
    & A &
    }
\end{equation}

We now need $\funbar$ to be a {\em symmetric\/} monoidal functor, that is, it
should be monoidal and satisfy the extra coherence condition:
\begin{equation}
  \label{eq:theta:coh:c}
  \xymatrix@C+10pt{
    {\funbara {A_1} \tensord \funbara {A_2}}
    \ar[r]^{\cd {\funbara {A_1}} {\funbara {A_2}}}
    \ar[d]_{\tstr {A_1} {A_2}}
    &
    {\funbara {A_2} \tensord \funbara {A_1}}
    \ar[d]^{\tstr {A_2} {A_1}}
    \\
    {\funbara {A_1 \tensorc A_2}}
    \ar[r]^{\funbara {\cc {A_1} {A_2}}}
    &
    {\funbara {A_2 \tensorc A_1}}
    }
\end{equation}


\subsection{Commutativity $\cSna$.}
We lift the commutativity to the subscone, assuming $\catc$ and $\catd$ are
symmetric monoidal, as follows.  The back and front face are the definition of
the two tensor products of $\langle S_1, m_1, A_1\rangle$ and $\langle S_2,
m_2, A_2\rangle$, the top face is by naturality of commutativity, the right
face is coherence~(\ref{eq:theta:coh:c}).  Finally $\widehat {\cdna}$ is given
by a diagonal fill-in, and all expected diagrams commute by Fact~\ref{f_eq}.

\begin{equation}
  \label{d_cS}
  \xymatrix@-10pt{
    S_1 \tensord S_2
    \ar[rr]^{m_1 \tensord m_2}
    \arrepixy[dd]_{e_{12}}
    \ar[rd]^{\cd {S_1} {S_2}}
    &
    &
    {\funbara {A_1} \tensord \funbara {A_2}}
    \ar[dd]|\hole_(0.3){\tstr {A_1} {A_2}}
    \ar[rd]^{\cd {\funbara {A_1}} {\funbara {A_2}}}
    &
    \\
    &
    S_2 \tensord S_1
    \ar[rr]_(0.7){m_2 \tensord m_1}
    \arrepixy[dd]_(0.3){e_{21}}
    &
    &
    {\funbara {A_2} \tensord \funbara {A_1}}
    \ar[dd]^{\tstr {A_2} {A_1}}
    \\
    S_{12}
    \ar@{.>}[rd]_{\widehat {\cdna}}
    \arrmonoxy[rr]|(0.45)\hole_(0.7){m_{12}}
    &
    &
    {\funbara {A_1 \tensorc A_2}}
    \ar[rd]_{\funbara {\cc {A_1} {A_2}}}
    &
    \\
    &
    S_{21}
    \arrmonoxy[rr]_{m_{21}}
    &
    &
    {\funbara {A_2 \tensorc A_1}}
    }
\end{equation}

We recap what we need to lift {\em symmetric\/} monoidal structure to the
subscone:

\begin{tabular}{|l|}
  \hline
  {\bf (i.b)} symmetric monoidal categories $(\catc, \tensorc, \Ic, \alphacna, \lc{},
  \rc{}, \ccna)$ \\
  \qquad and $(\catd, \tensord, \Id, \alphadna, \ld{}, \rd{}, \cdna)$, \\
  \qquad and a symmetric monoidal functor $\funbar : \catc \to \catd$,\\
  {\bf (iii.a)} a monoidal mono factorization system on $\catd$.\\
  \hline
\end{tabular}


\subsection{Lifting Cartesian Products}
\label{sec:monoidal:cart}

An important special case of symmetric monoidal structure is that given by
finite products.  This is given by one {\em terminal object\/} $\termobjc$
such that, for every object $A$ in $\catc$, there is a unique morphism $A
{\buildrel !\over\longrightarrow} \termobjc$,
and by a {\em binary product\/} operation as explained in
Section~\ref{relations.s}.
For any two morphisms $f$ from $A$ to
$A'$, $g$ from $B$ to $B'$, we write $f \times g$ for the morphism $\pair {f
  \circ \pi_1} {g \circ \pi_2}$ from $A \times B$ to $A' \times B'$.

It is well-known that binary product can be turned into a functor from $\catc
\times \catc$ to $\catc$, which is symmetric monoidal with unit $\termobj$,
associativity $\pair {\pi_1 \circ \pi_1} {\pair {\pi_2 \circ \pi_1} {\pi_2}}$,
left unit $\pi_2$, right unit $\pi_1$, and commutativity $\pair {\pi_2}
{\pi_1}$.

When $\catc$ and $\catd$ are both equipped with finite products, and $\funbar$
is a functor from $\catc$ to $\catd$ that is monoidal with respect to these
products, then the construction of Sections~\ref{sec:monoidal:1}
and~\ref{sec:monoidal:sym} yields a symmetric monoidal structure on $\subscone
\catc \catd \funbar$ that we claim stems from a finite product structure on
the subscone.

\noindent
\begin{minipage}{6cm}
  To this end, we assume that $\funbar$ satisfies the coherence condition on
  the right, for $i \in \{1, 2\}$.  We shall say that such a functor is {\em
    cartesian monoidal}.  (Then $\funbar$ is automatically symmetric
  monoidal.)
\end{minipage}
\begin{minipage}{6cm}
  \begin{equation}
    \label{eq:theta:coh:proj}
    \xymatrix{
      {\funbara {A_1} \times \funbara {A_2}}
      \ar[rd]^{\pi_i}
      \ar[d]_{\tstr {A_1} {A_2}}
      &
      \\
      {\funbara {A_1 \times A_2}}
      \ar[r]_{\funbara {\pi_i}}
      &
      \funbara {A_i}
      }
  \end{equation}
\end{minipage}

\noindent
\begin{minipage}{6cm}
  \subsection{Terminal object $\lift\termobj$.}
  Let $\lift\termobj$ be the object $\langle \overline I, \overline \tstri,
  \termobjc\rangle$ given by diagram~(\ref{d_IS}). Specializing this diagram to
  the case at hand, this is given as the unique object up to iso making the
  following diagram commute:
\end{minipage}
\begin{minipage}{6cm}
  \begin{equation}
    \label{d_1S}
    \xymatrix@-5pt{
      {\termobjd}
      \ar[rd]^{\tstri}
      \arrepixy[d]_{e_I}
      & \\
      {\overline I}
      \arrmonoxy[r]_{\overline \tstri}    % {m_I}
      &
      {\funbara \termobjc}
      }
  \end{equation}
\end{minipage}

\noindent
\begin{minipage}{5cm}
  For any object $\langle S, m, A\rangle$ of the subscone, there is a unique
  arrow $\langle u, v\rangle$ from $\langle S, m, A\rangle$ to
  $\langle \overline I, \overline \tstri, \termobjc\rangle$.  
  Indeed, $v$ is the unique
  arrow $!$ from $A$ to $\termobjc$, and $u$ is given by $e_I \circ !$; $u$ is
  also unique, by Fact~\ref{f_eq}.
\end{minipage}
\begin{minipage}{7cm}
  \[
  \xymatrix@-5pt{
    &
    {\termobjd}
    \ar[rd]^{\tstri}
    \arrepixy[d]_{e_I}
    & \\
    &
    {\overline I}
    \arrmonoxy[r]_{\overline \tstri}    % {m_I}
    &
    {\funbara \termobjc}
    \\
    S
    \arrmonoxy[r]_{m}
    \ar@/^1pc/[ruu]^{!}
    \ar@{.>}[ru]|{u}
    &
    {\funbara {A}}
    \ar[ru]_{\funbara v}
    &
    }
  \]
\end{minipage}

\noindent
\begin{minipage}{6cm}
  \subsection{Binary product $\lift\times$.}
  Specializing the definition (\ref{d_tensorS}) of the lifted tensor product
  $\tensorS$ to the case at hand yields the object $\langle S_{12}, m_{12},
  A_1 \tensorc A_2\rangle = \langle S_1, m_1, A_1 \rangle \lift\times \langle
  S_2, m_2, A_2 \rangle$ defined by the diagram on the right.
\end{minipage}
\begin{minipage}{6cm}
  \begin{equation}
    \label{d_timesS}
    \xymatrix@C+10pt{
      S_1 \times S_2
      \ar[r]^{m_1 \times m_2}
      \arrepixy[d]_{e_{12}}
      &
      {\funbara {A_1} \times \funbara {A_2}}
      \ar[d]_{\tstr {A_1} {A_2}}
      \\
      S_{12}
      \arrmonoxy[r]_{m_{12}}
      &
      {\funbara {A_1 \times A_2}}
      }
  \end{equation}
\end{minipage}

\noindent
\begin{minipage}{4.5cm}
  The $i$th projection $\langle \lift\pi_i, \pi_i\rangle$ is then given by the
  diagram on the right.  The back square is a copy of (\ref{d_timesS}), the
  right triangle is an instance of the coherence condition
  (\ref{eq:theta:coh:proj}), while the top, slanted face is by standard
  properties of $\pi_i$.  From two routes from $S_1 \times S_2$ to $\funbara
  {A_i}$, we get $\lift\pi_i$ by a diagonal fill-in.
\end{minipage}
\begin{minipage}{7.5cm}
  \[
  \xymatrix@C+10pt{
    S_1 \times S_2
    \ar[r]^{m_1 \times m_2}
    \ar[rdd]^(0.4){\pi_i}
    \arrepixy[d]_{e_{12}}
    &
    {\funbara {A_1} \times \funbara {A_2}}
    \ar[d]_{\tstr {A_1} {A_2}}
    \ar[rdd]^(0.4){\pi_i}
    &
    \\
    S_{12}
    \arrmonoxy[r]|\hole_(0.3){m_{12}}
    \ar@{.>}[rd]_{\lift\pi_i}
    &
    {\funbara {A_1 \times A_2}}
    \ar[rd]|{\funbara {\pi_i}}
    &
    \\
    &
    S_i
    \arrmonoxy[r]_{m_i}
    &
    {\funbara {A_i}}
    }
  \]
\end{minipage}

\noindent
It remains to show that whenever we have two subscone morphisms $\langle \lift
f_1, f_1\rangle$ from $\langle S, m, A\rangle$ to $\langle S_1, m_1,
A_1\rangle$ and $\langle \lift f_2, f_2\rangle$ from $\langle S, m, A\rangle$
to $\langle S_2, m_2, A_2\rangle$, there is a unique morphism $\langle \lift
h, h \rangle$ from $\langle S, m, A\rangle$ to the product $\langle S_{12},
m_{12}, A_1 \times A_2 \rangle$ such that $\langle \lift \pi_i, \pi_i\rangle
\circ \langle \lift h, h\rangle = \langle \lift f_i, f_i\rangle$ ($i\in \{1,
2\}$).  Existence is assured: take $h = \pair {f_1} {f_2}$, $\lift h = e_{12}
\circ \pair {\lift f_1} {\lift f_2}$, which satisfies the claim: this is an
easy consequence of the diagram above. Uniqueness follows from the uniqueness
of $h$ given by the definition of binary product in $\catc$, and from
Fact~\ref{f_eq} guaranteeing the uniqueness of $\widetilde h$.

As is now usual, we recap what we need to lift products to the subscone:

\begin{tabular}{|l|}
  \hline
  {\bf (i.c)} categories $\catc$ and $\catd$ with finite products, \\
  \qquad and a cartesian monoidal functor $\funbar : \catc \to \catd$,\\
  {\bf (iii.a)} a monoidal mono factorization system on $\catd$.\\
  \hline
\end{tabular}



\section{Lifting Strong, Monoidal, and Commutative Monads to a Scone and a Subscone}
\label{strong.s}

Once we have got a monoidal structure on $\catc$ and $\catd$, we may consider
{\em strong\/} monads $\tc{}$ and $\td{}$ instead of just monads on each
category.  This is what we need to develop a theory of logical relations for
Moggi's monadic $\lambda$-calculus.  We shall also consider the more demanding cases
of {\em monoidal\/} monads, and of {\em commutative\/} monads.


\subsection{Lifting Strong Monads}
\label{strong.s:strong}


That $\td{}$ is a strong monad means that a {\em strength} natural
transformation $\strd{A}{B} : A \tensord \td B \to \td (A \tensord B)$ is
given such that the diagrams in Definition 3.2 in~\cite{Mog91} commute, that
is:

\noindent
\hfill
\begin{minipage}{5cm}
  \begin{equation}
    \label{eq:strong:l}
    \xymatrix{
      {\Id \tensord \td B}
      \ar[r]^{\strd \Id B}
      \ar[rd]_{\ld {\td B}}
      &
      {\td (\Id \tensord B)}
      \ar[d]^{\td {\ld B}}
      \\
      &
      {\td B}
      }
  \end{equation}
\end{minipage}
\qquad
\begin{minipage}{5cm}
  \begin{equation}
    \label{eq:strong:eta}
    \xymatrix{
      A \tensord B
      \ar[r]^{\identity A \tensord \unitd B}
      \ar[rd]_{\unitd {A \tensord B}}
      &
      A \tensord \td B
      \ar[d]^{\strd A B}
      \\
      &
      {\td (A \tensord B)}
      }
  \end{equation}
\end{minipage}

\noindent
\begin{equation}
  \label{eq:strong:double}
  \xymatrix{
    (A \tensord B) \tensord \td C
    \ar[d]^{\alphad A B {\td C}}
    \ar[rr]^{\strd {A \tensord B} C}
    &
    &
    {\td {((A \tensord B) \tensord C)}}
    \ar[d]^{\td {\alphad A B C}}
    \\
    A \tensord (B \tensord \td C)
    \ar[r]_{\identity A \tensord \strd B C}
    &
    A \tensord \td (B \tensord C)
    \ar[r]_{\strd A {B \tensord C}}
    &
    {\td (A \tensord (B \tensord C))}
    }
\end{equation}

\noindent
\begin{equation}
  \label{eq:strong:mu}
  \xymatrix{
    A \tensord \td^2 B
    \ar[r]^{\strd A {\td B}}
    \ar[d]_{\identity A \tensord \multd B}
    &
    {\td (A \tensord \td B)}
    \ar[r]^{\td {\strd A B}}
    &
    {\td^2 (A \tensord B)}
    \ar[d]^{\multd {A \tensord B}}
    \\
    A \tensord \td B
    \ar[rr]_{\strd A B}
    &
    &
    {\td (A \tensord B)}
    }
\end{equation}

Formally, a {\em strong monad\/} is a four-tuple $(\td, \unitd{}, \multd{},
\strdna)$ where $(\td, \unitd{}, \multd{})$ is a monad and $\strdna$ is a
strength making the above diagrams commute.

%Our definition of monad lifting $\tc$ to scones (or subscones) in
%diagram~(\ref{d_lifting1}) and equations~(\ref{e_lifting2}) will be extended
%to strong monads below.  First observe that we do have finite products and
%natural isomorphisms $\rS{}$ and $\alphaSna$ in scones and subscones,
%if we put $\rS{\langle S, f, A \rangle} = \langle \rd{S}, \rc{A} \rangle$
%and 
%$\alphaS{\langle S, f, A \rangle}{\langle R, g, B \rangle}{\langle Q, h, C \rangle}
%= \langle \alphad{S}{R}{Q}, \alphac{A}{B}{C}\rangle$.
%\begin{lemma}
%\label{prod.l}
%Both $\scone{\catc}{\catd}$ and $\subscone{\catc}{\catd}$ have 
%finite products, given explicitly.
%Functor $\forfun$ preserves strictly finite products as well as 
%$\rS{}$ and $\alphaSna$.
%\qed
%\end{lemma}
%\iflong%
%\begin{proof}
%  \input{appendix}
%\end{proof}
%\fi%

By lifting of $\tc$ to $\scone{\catc}{\catd}{\funbar}$ we now mean a strong
monad, i.e. a monad $(\tS, \unitS{}, \multS{})$ together with a strength
$\strS{X}{Y} : X {\tensorS} \tS Y \to \tS (X {\tensorS} Y)$, such that
diagram~(\ref{d_lifting1}) commutes, equations~(\ref{e_lifting2}) hold and
\iflong
\begin{equation*}
\forfun \strS{X}{Y} = \strc{\forfun X}{\forfun Y},
\end{equation*}
\else
$
\forfun \strS{X}{Y} = \strc{\forfun X}{\forfun Y},
$
\fi
i.e., $\forfun$ preserves strength.

To be able to give an appropriate lifting, we extend the monad morphism to a
{\em strong monad\/} morphism, i.e., a monad morphism making the following
additional diagram commute, which relates the strengths $\strc{A_1}{A_2}$ and
$\strd{\funbara{A_1}}{\funbara{A_2}}$:
\begin{equation}
  \label{d_diststr}
  \xymatrix@C+10pt@R-10pt{
    {\funbara{A_1} \tensord \td \funbara{A_2}}
    \ar[r]^{\strd{\funbara{A_1}}{\funbara{A_2}}}
    \ar[d]_{\identity {\funbara {A_1}} \tensord \dist {A_2}}
    &
    {\td (\funbara {A_1} \tensord \funbara {A_2})}
    \ar[d]^{\td (\tstr {A_1} {A_2})}
    \\
    {\funbara {A_1} \tensord \funbara {\tc {A_2}}}
    \ar[d]_{\tstr {A_1} {\tc {A_2}}}
    &
    {\td \funbara {A_1 \tensorc A_2}}
    \ar[d]^{\dist {A_1 \tensorc A_2}}
    \\
    {\funbara {A_1 \tensorc \tc {A_2}}}
    \ar[r]_{\funbara {\strc {A_1} {A_2}}}
    &
    {\funbara {\tc (A_1 \tensorc A_2)}}
    }
\end{equation}


Having lifted $\tc$ to scones and subscones in previous sections, we only need
to give a lifting of the strength $\strcna$. For scones this is
straightforward---define $\strSna$ pointwise by
\[
\strS{\langle S_1, m_1, A_1 \rangle}{\langle S_2, m_2, A_2 \rangle} =
\langle \strd{S_1}{S_2}, \strc{A_1}{A_2} \rangle.
\]

Verifying that this is well-defined amounts to pasting together a naturality
square for $\strdna$ and a diagram~(\ref{d_diststr}):
\[
\xymatrix@C+10pt{
  S_1 \tensord \td S_2
  \ar[rr]^{m_1 \tensord \td m_2}
  \ar[d]^{\strd{S_1}{S_2}}
  & &
  {\funbara{A_1} \tensord \td \funbara{A_2}}
  \ar[d]_{\strd{\funbara{A_1}}{\funbara{A_2}}} 
  \ar[rr]^{\tstr {A_1} {\tc A_2} \circ (\identity {\funbara {A_1}} \tensord \dist {A_2})}
  & & 
  {\funbara{A_1 \tensorc \tc A_2}}
  \ar[d]_{\funbara {\strc{A_1}{A_2}}}
  \\
  {\td (S_1 \tensord S_2)}
  \ar[rr]^{\td (m_1 \tensord m_2)}
  & & 
  {\td (\funbara{A_1} \tensord \funbara{A_2})}
  \ar[rr]^{\dist{A_1 \tensord A_2} \circ \td (\tstr {A_1} {A_2})}
  & &
  {\funbara{\tc (A_1 \tensorc A_2)}}
  }
\]

\noindent
The upper side of this diagram is precisely $\langle S_1, m_1, A_1 \rangle \tensorS \tS \langle
S_2, m_2, A_2 \rangle$ in the scone while the lower side is $\tS (\langle S_1, m_1, A_1 \rangle
\tensorS \langle S_2, m_2, A_2 \rangle)$. (We let the interested reader define for herself
the tensor product $\tensorS$ in the scone.)  Checking naturality of $\strSna$
and strength laws
% ~(\ref{d_strength})
is immediate since $\strSna$, $\alphaSna$, $\rS{}$, $\unitS{}$ and $\multS{}$
are all defined pointwise.

Now we move to subscones.  Call $\tS$ the lifted monad defined
in~(\ref{d_tsonobj}), (\ref{d_tsonmor}), (\ref{d_units}) and~(\ref{d_mults}) 
in Section~\ref{s_liftsubscone}.

As in previous sections, $\strSna$ in subscones will differ from the case of
scones only in its $\catd$-component $\hat \strdna$, and this component will
be induced as a unique diagonal guaranteed by diagram~(\ref{d_factordiag}) in
the diagram below.
\begin{equation}
  \label{t_cube}
  \xymatrix@-10pt@C-10pt{
    S_1 \tensord \td S_2
    \ar[rr]^{\identity {S_1} \tensord \td m_2}
    \arrepixy[dd]|{\identity {S_1} \tensord e'_2}
    \ar[rd]^{\strd {S_1} {S_2}}
    &
    &
    S_1 \tensord \td \funbara {A_2}
    \ar[rr]^{m_1 \tensord \identity {\td \funbara {A_2}}}
    \ar[dd]|\hole_(0.3){\identity {S_1} \tensord \dist {A_2}}
    &
    &
    {\funbara {A_1} \tensord \td \funbara {A_2}}
    \ar[dd]|\hole_(0.3){\identity {\funbara {A_1}} \tensord \dist {A_2}}
    \ar[rd]^{\strd {\funbara {A_1}} {\funbara {A_2}}}
    &
    \\
    &
    {\td (S_1 \tensord S_2)}
    \ar[rrrr]_{\td (m_1 \tensord m_2)}
    \ar[dd]^(0.3){\td e_{12}}
    &
    &
    &
    &
    {\td (\funbara {A_1} \tensord \funbara {A_2})}
    \ar[dd]|{\td (\tstr {A_1} {A_2})}
    \\
    S_1 \tensord \widetilde {S_2}
    \ar[rr]|\hole^(0.3){\identity {S_1} \tensord m'_2}
    \arrepixy[dd]_{e'_{12}}
    \ar@{-->}[rddd]
    &
    &
    S_1 \tensord \funbara {\tc A_2}
    \ar[rr]^{m_1 \tensord \identity {\funbara {\tc A_2}}}
    &
    &
    {\funbara {A_1} \tensord \funbara {\tc A_2}}
    \ar[dd]|\hole^(0.3){\tstr {A_1} {\tc A_2}}
    &
    \\
    &
    {\td S_{12}}
    \ar[rrrr]^{\td m_{12}}
    \arrepixy[dd]^(0.3){e'}
    &
    &
    &
    &
    {\td \funbara {A_1 \tensorc A_2}}
    \ar[dd]|{\dist {A_1 \tensorc A_2}}
    \\
    S'_{12}
    \arrmonoxy[rrrr]|(0.29)\hole^{m'_{12}}
    \ar@{.>}[rd]_{\hat \strdna}
    &
    &
    &
    &
    {\funbara {A_1 \tensorc \tc A_2}}
    \ar[rd]^{\funbara {\strc {A_1} {A_2}}}
    &
    \\
    &
    {\widetilde {S_{12}}}
    \arrmonoxy[rrrr]_{m'}
    &
    &
    &
    &
    {\funbara {\tc (A_1 \tensorc A_2)}}
    }
\end{equation}

As ingredients of this diagram we have used:
\begin{itemize}
\item An instance $
  \xymatrix@-5pt{
    {\td S_2}
    \ar[r]^{\td m_2}
    \arrepixy[d]_{e'_2}
    &
    {\td \funbara {A_2}}
    \ar[d]^{\dist {A_2}}
    \\
    {\widetilde {S_2}}
    \arrmonoxy[r]_{m'_2}
    &
    {\funbara {\tc A_2}}
    }
  $ of Diagram~(\ref{d_tsonobj}) defining $\tS \langle S_2,
  m_2, A_2\rangle$; this is tensored by $S_1$ on the left to get the upper
  left square of the back face.  Notice that $\identity {S_1} \tensord e'_2$
  is pseudoepi because our mono factorization system is monoidal.
\item An instance $
  \xymatrix@C+20pt{
    S_1 \tensord \widetilde {S_2}
    \ar[r]^{m_1 \tensord m'_2}
    \arrepixy[d]_{e'_{12}}
    &
    {\funbara {A_1} \tensord \funbara {\tc A_2}}
    \ar[d]^{\tstr {A_1} {\tc A_2}}
    \\
    S'_{12}
    \arrmonoxy[r]_{m'_{12}}
    &
    {\funbara {A_1 \tensorc \tc A_2}}
    }
  $ of Diagram~(\ref{d_tensorS}) defining the tensor product
  of $\langle S_1, m_1, A_1\rangle$ with $\tS \langle S_2, m_2, A_2\rangle =
  \langle \widetilde {S_2}, m'_2, \tc A_2\rangle$; this is the lower square of
  the back face.  (Note that the upper right square of the back face commutes
  trivially.)
\item Another instance $ \xymatrix@C+20pt{ S_1 \tensord S_2 \ar[r]^{m_1 \tensord
      m_2} \arrepixy[d]_{e_{12}} & {\funbara {A_1} \tensord \funbara {A_2}}
    \ar[d]^{\tstr {A_1} {A_2}}
    \\
    S_{12} \arrmonoxy[r]_{m_{12}} & {\funbara {A_1 \tensorc A_2}} } $ of
  Diagram~(\ref{d_tensorS}) defining the tensor product $\langle S_{12},
  m_{12}, A_1 \tensorc A_2\rangle$ of $\langle S_1, m_1, A_1\rangle$ with
  $\langle S_2, m_2, A_2\rangle$; we apply $\td$ to this square to get the
  upper half of the front face.
\item Another instance of Diagram~(\ref{d_tsonobj}) defining the application
  of $\tS$ to the just mentioned tensor product $\langle S_{12}, m_{12}, A_1
  \tensorc A_2\rangle$: this is the lower half of the front face.
\item A naturality square for $\strdna$ (top face), and
\item An instance of Diagram~(\ref{d_diststr}), which defines the right face.
\end{itemize}

As usual, the dashed and the dotted arrows are given by diagonal fill-ins,
therefore $\strSna = (\hat \strdna, \strcna)$ is well-defined.
Again, checking naturality of $\strSna$ and
strength laws
% ~(\ref{d_strength})
is immediate by Fact~\ref{f_eq}.

Here is the final set of ingredients for lifting a strong monad $( \tc,
\unitc{}, \multc{}, \strcna )$ on category $\catc$
to $\subscone{\catc}{\catd}{\funbar}$:\\

\noindent
\begin{tabular}{|l|}
  \hline
  {\bf (i.a)} monoidal categories $(\catc, \tensorc, \Ic, \alphacna, \lc{},
  \rc{})$ and $(\catd, \tensord, \Id, \alphadna, \ld{}, \rd{})$, \\
  \qquad and a monoidal functor $\funbar : \catc \to \catd$,\\
  {\bf (ii.a)} a strong monad $( \td, \unitd{}, \multd{}, \strdna)$ on $\catd$,
        related to $(\tc, \unitc{}, \multc{}, \strcna)$ 
        by \\
        \qquad 
        a strong monad morphism $(\funbar, \dist{})$ defined 
        in~(\ref{d_distlaw}) and~(\ref{d_diststr}),\\
  {\bf (iii.a)} a monoidal mono factorization system on $\catd$.\\
  {\bf (iv)}\ $\td$ maps relevant pseudoepis to pseudoepis.\\
  \hline
\end{tabular}


\subsection{Monoidal Monads}
\label{strong.s:monoidal}


Several strong monads are in fact monoidal---in fact all the monads of
Section~\ref{examples.s} are monoidal, except the continuation
and continuation-like monads.
\ifmscs
\else
While this notion is not needed in
Moggi's account of computation \cite{Mog91}, this occurs naturally, and will
be used in Section~\ref{distr.s.monoidal}%
\comment{DN 07/01/04
and in Section~\ref{ccc.s:simplicial}
}.
\fi
A {\em monoidal\/} monad is a four-tuple
$(\td, \unitd{}, \multd{}, \bistrdna)$, where $\bistrd A B : \td A \tensord
\td B \to \td (A \tensord B)$ is a {\em mediator\/} natural transformation,
making the following diagrams commute:

\noindent
\begin{minipage}{6cm}
  \begin{equation}
    \label{eq:monoidal:l}
    \xymatrix@R-12pt{
      {\Id \tensord \td B}
      \ar[rdd]^{\ld {\td B}}
      \ar[d]_{\unitd {\Id} \tensord \identity {\td B}}
      &
      \\
      {\td \Id \tensord \td B}
      \ar[d]_{\bistrd {\Id} B}
      &
      \\
      {\td (\Id \tensord B)}
      \ar[r]_(0.7){\td \ld B}
      &
      {\td B}
      }
  \end{equation}
\end{minipage}
\begin{minipage}{6cm}
  \begin{equation}
    \label{eq:monoidal:r}
    \xymatrix@R-12pt{
      {\td A \tensord \Id}
      \ar[rdd]^{\rd {\td A}}
      \ar[d]_{\identity {\td A} \tensord \unitd {\Id}}
      &
      \\
      {\td A \tensord \td \Id}
      \ar[d]_{\bistrd A \Id}
      &
      \\
      \td (A \tensord \Id)
      \ar[r]_(0.7){\td \rd A}
      &
      \td A
      }
  \end{equation}
\end{minipage}

\noindent
\begin{equation}
  \label{eq:monoidal:eta}
  \xymatrix@R-10pt{
    {A \tensord B}
    \ar[r]^{\unitd A \tensord \unitd B}
    \ar[rd]_{\unitd {A \tensord B}}
    &
    {\td A \tensord \td B}
    \ar[d]^{\bistrd A B}
    \\
    &
    {\td (A \tensord B)}
    }
\end{equation}

\noindent
\begin{equation}
  \label{eq:monoidal:double}
  \xymatrix@R-5pt{
    {(\td A \tensord \td B) \tensord \td C}
    \ar[d]^{\alphad {\td A} {\td B} {\td C}}
    \ar[r]^{\bistrd A B \tensord \identity {\td C}}
    &
    {\td (A \tensord B) \tensord \td C}
    \ar[r]^{\bistrd {A \tensord B} C}
    &
    {\td ((A \tensord B) \tensord C)}
    \ar[d]^{\td \alphad A B C}
    \\
    {\td A \tensord (\td B \tensord \td C)}
    \ar[r]_{\identity {\td A} \tensord \bistrd B C}
    &
    {\td A \tensord \td (B \tensord C)}
    \ar[r]_{\bistrd A {B \tensord C}}
    &
    {\td (A \tensord (B \tensord C))}
    }
\end{equation}

\noindent
\begin{equation}
  \label{eq:monoidal:mu}
  \xymatrix@R-5pt{
    {\td^2 A \tensord \td^2 B}
    \ar[r]^{\bistrd {\td A} {\td B}}
    \ar[d]_{\multd A \tensord \multd B}
    &
    {\td (\td A \tensord \td B)}
    \ar[r]^{\td \bistrd A B}
    &
    {\td^2 (A \tensord B)}
    \ar[d]^{\multd {A \tensord B}}
    \\
    {\td A \tensord \td B}
    \ar[rr]_{\bistrd A B}
    &
    &
    {\td (A \tensord B)}
    }
\end{equation}

Diagrams (\ref{eq:monoidal:l}), (\ref{eq:monoidal:r}),
(\ref{eq:monoidal:double}) state that $\td$ is a monoidal functor with
mediating pair $(\bistrdna, \unitd{\Id})$.  Diagram~(\ref{eq:monoidal:eta})
states that $\unitd{}$ is a so-called monoidal natural transformation, while
Diagram~(\ref{eq:monoidal:mu}) states that $\multd{}$ is another monoidal
natural transformation.
%  Alternatively,
%Diagrams~(\ref{eq:monoidal:eta}) and (\ref{eq:monoidal:mu}) state that
%$(\tensord, \bistrdna)$ is a monad morphism from the monad $(\td, \unitd{},
%\multd{})$ on $\catd$ to the monad $(

Given any monoidal monad $(\td, \unitd{}, \multd{}, \bistrdna)$ on $\catd$, it
is easy to check that $(\td, \unitd{}, \multd{}, \strdna)$ is a strong monad,
where $\strd A B = \bistrd A B \circ (\unitd A \tensord \identity {\td B})$.
Furthermore, $\strd A B'$ defined as $\bistrd A B \circ (\identity {\td A}
\tensord \unitd B)$ is a {\em dual strength}, that is, a natural
transformation $\strd A B' : \td A \tensord B \to \td (A \tensord B)$ obeying
the obvious duals of the strength laws (\ref{eq:strong:l}),
(\ref{eq:strong:eta}), (\ref{eq:strong:double}), (\ref{eq:strong:mu}).
(Formally, a dual strength is a strength on the dual monoidal category
$(\catd, \Id, \tensord^{op}, \alphadna^{-1}, \rdna, \ldna)$, where $A
\tensord^{op} B$ is defined as $B \tensord A$.)

Moreover, the strength $\strdna$ and the dual strength $\strdna'$ are
compatible with the associativity, in the sense that the diagram below
commutes.
\begin{equation}
  \label{eq:tt'_alpha}
  \xymatrix@C+10pt@R-10pt{
    {(A \tensord \td B) \tensord C}
    \ar[r]^{\strd A B \tensord \identity C}
    \ar[d]_{\alphad A {\td B} C}
    &
    {\td {(A \tensord B)} \tensord C}
    \ar[r]^{\strd {A \tensord B} C'}
    &
    {\td {((A \tensord B) \tensord C)}}
    \ar[d]^{\td \alphad A B C}
    \\
    {A \tensord (\td B \tensord C)}
    \ar[r]^{\identity A \tensord \strd B C'}
    &
    {A \tensord \td {(B \tensord C)}}
    \ar[r]^{\strd A {B \tensord C}}
    &
    {\td {(A \tensord (B \tensord C))}}
    }
\end{equation}

\noindent
\begin{minipage}{4.2cm}
  Finally, the strength and the dual strength commute, in the sense that the
  diagram on the right commutes.  In fact, the common diagonal from $\td A
  \tensord \td B$ to $\td (A \tensord B)$ is just $\bistrd A B$.
\end{minipage}
\begin{minipage}{7.8cm}
  \begin{equation}
    \label{eq:tt'}
    \xymatrix@-10pt{
      {\td A \tensord \td B}
      \ar[rr]^{\strd {\td A} B}
      \ar[dd]_{\strd A {\td B}'}
      &&
      {\td (\td A \tensord B)}
      \ar[d]^{\td \strd A B'}
      \\
      &&
      {\td^2 (A \tensord B)}
      \ar[d]^{\multd {A \tensord B}}
      \\
      {\td (A \tensord \td B)}
      \ar[r]_{\td \strd A B}
      &
      {\td^2 (A \tensord B)}
      \ar[r]_{\multd {A \tensord B}}
      &
      {\td (A \tensord B)}
      }
  \end{equation}
\end{minipage}

\noindent
In general, a monoidal monad can be defined equivalently as a monad with a
strength and a dual strength that make the diagrams (\ref{eq:tt'_alpha}) and
(\ref{eq:tt'}) commute.
\ifmscs
See Appendix~A, in particular
Appendix~A.1 and Appendix~A.2, in \cite{GLN02}, for a
proof.
\else
See Appendix~\ref{app:monoidal}, in particular
Appendix~\ref{app:monoidal:->} and Appendix~\ref{app:monoidal:<-}, for a
proof.
\fi

%equipped with both a strength and a dual strength such
%that the diagram above commutes may fail to be a monoidal monad by an inch: we
%have been unable to show that Diagram~(\ref{eq:monoidal:double}) commutes in
%this setting.

It is natural to define a {\em monoidal monad morphism\/} from $(\tc,
\unitc{}, \multc{}, \bistrcna)$ to $(\td, \unitd{}, \multd{}, \bistrdna)$ as a
monad morphism $\dist {}$ from $(\tc, \unitc{}, \multc{})$ to $(\td, \unitd{},
\multd{})$ making the following diagram commute:
\begin{equation}
  \label{d_distbistr}
  \xymatrix@C+10pt@R-10pt{
    {\td \funbara{A_1} \tensord \td \funbara{A_2}}
    \ar[r]^{\bistrd{\funbara{A_1}}{\funbara{A_2}}}
    \ar[d]_{\dist {A_1} \tensord \dist {A_2}}
    &
    {\td (\funbara {A_1} \tensord \funbara {A_2})}
    \ar[d]^{\td (\tstr {A_1} {A_2})}
    \\
    {\funbara {\tc {A_1}} \tensord \funbara {\tc {A_2}}}
    \ar[d]_{\tstr {\tc {A_1}} {\tc {A_2}}}
    &
    {\td \funbara {A_1 \tensorc A_2}}
    \ar[d]^{\dist {A_1 \tensorc A_2}}
    \\
    {\funbara {\tc {A_1} \tensorc \tc {A_2}}}
    \ar[r]_{\funbara {\bistrc {A_1} {A_2}}}
    &
    {\funbara {\tc (A_1 \tensorc A_2)}}
    }
\end{equation}

%It is easy to see, using a copy of (\ref{d_distbistr}), a copy of
%(\ref{d_distlaw}) (left), and a naturality square for $\tstrna$, that 
Every monoidal monad morphism $\dist{}$ is also a strong monad morphism from
$(\tc, \unitc{}, \multc{}, \strcna)$ to $(\td, \unitd{}, \multd{}, \strdna)$,
and also from $(\tc, \unitc{}, \multc{}, \strcna')$ to $(\td, \unitd{},
\multd{}, \strdna')$, where $\strc A B = \bistrc A B \circ (\unitc A \tensorc
\identity {\tc B})$, $\strd A B = \bistrd A B \circ (\unitd A \tensord
\identity {\td B})$, $\strc A B' = \bistrc A B \circ (\identity {\tc A}
\tensorc \unitc B)$, $\strd A B' = \bistrd A B \circ (\identity {\tc A}
\tensord \unitd B)$.
\ifmscs
In Appendix~A.3 of \cite{GLN02},
\else
In Appendix~\ref{app:monoidal:monmor},
\fi
 we show that the
monoidal monad morphisms are exactly the natural transformations $\dist{}$ that
are both a strong monad morphism and a dual strong monad morphism.

One may think that lifting monoidal monads to scones and subscones is
easy: get the strength and the dual strength from the mediator, and
lift them as in Section~\ref{strong.s:strong}.  However, it is not
immediately clear that what one would get would arise as strength and
dual strengths of a mediator, in particular that (\ref{eq:tt'}) would
commute.  Let us therefore state the construction explicitly.
%
%It is easy to lift monoidal monads to scones and subscones. One way is to
%realize that we just have to get the strength and dual strength from the
%mediator, lift them as in Section~\ref{strong.s:strong}, and reconstruct the
%lifted mediator from the lifted strength and dual strength by
%(\ref{eq:tt'}).  However it is not immediately clear what we get in the end.
%We therefore state the construction explicitly.
%
This mimicks the construction of the lifted strength from
Section~\ref{strong.s:strong}. For scones, the lifted mediator is
again defined pointwise by
\[
\bistrS {\langle S_1, m_1, A_1\rangle} {\langle S_2, m_2, A_2\rangle}
= \langle \bistrc {S_1} {S_2}, \bistrd {A_1} {A_2} \rangle
\]
For subscones, we mimick Diagram~(\ref{t_cube}) in Diagram~(\ref{d_cube})
below.  We let the reader check all commutations.
\begin{equation}
  \label{d_cube}
  \xymatrix@-10pt@C-10pt{
    {\td S_1 \tensord \td S_2}
    \ar[rrrr]^{\td m_1 \tensord \td m_2}
    \arrepixy[dd]|{e'_1 \tensord e'_2}
    \ar[rd]^{\bistrd {S_1} {S_2}}
    &
    &
    &
    &
    {\td \funbara {A_1} \tensord \td \funbara {A_2}}
    \ar[dd]|\hole_(0.3){\dist {A_1} \tensord \dist {A_2}}
    \ar[rd]^{\bistrd {\funbara {A_1}} {\funbara {A_2}}}
    &
    \\
    &
    {\td (S_1 \tensord S_2)}
    \ar[rrrr]_(0.3){\td (m_1 \tensord m_2)}
    \ar[dd]_(0.3){\td e_{12}}
    &
    &
    &
    &
    {\td (\funbara {A_1} \tensord \funbara {A_2})}
    \ar[dd]|{\td (\tstr {A_1} {A_2})}
    \\
    {\widetilde {S_1} \tensord \widetilde {S_2}}
    \ar[rrrr]|(0.4)\hole^(0.6){m'_1 \tensord m'_2}
    \arrepixy[dd]_{e'_{12}}
    \ar@{-->}[rddd]
    &
    &
    &
    &
    {\funbara {\tc A_1} \tensord \funbara {\tc A_2}}
    \ar[dd]|\hole^(0.3){\tstr {\tc A_1} {\tc A_2}}
    &
    \\
    &
    {\td S_{12}}
    \ar[rrrr]^(0.4){\td m_{12}}
    \arrepixy[dd]_(0.3){e'}
    &
    &
    &
    &
    {\td \funbara {A_1 \tensorc A_2}}
    \ar[dd]|{\dist {A_1 \tensorc A_2}}
    \\
    S'_{12}
    \arrmonoxy[rrrr]|(0.4)\hole^{m'_{12}}
    \ar@{.>}[rd]_{\hat \bistrdna}
    &
    &
    &
    &
    {\funbara {\tc A_1 \tensorc \tc A_2}}
    \ar[rd]^{\funbara {\bistrc {A_1} {A_2}}}
    &
    \\
    &
    {\widetilde {S_{12}}}
    \arrmonoxy[rrrr]_{m'}
    &
    &
    &
    &
    {\funbara {\tc (A_1 \tensorc A_2)}}
    }
\end{equation}

So, to lift a monoidal monad $(\tc, \unitc{}, \multc{}, \bistrcna)$ on
category $\catc$
to $\subscone{\catc}{\catd}{\funbar}$, we require:\\

\noindent
\begin{tabular}{|l|}
  \hline
  {\bf (i.a)} monoidal categories $(\catc, \tensorc, \Ic, \alphacna, \lc{},
  \rc{})$ and $(\catd, \tensord, \Id, \alphadna, \ld{}, \rd{})$, \\
  \qquad and a monoidal functor $\funbar : \catc \to \catd$,\\
  {\bf (ii.b)} a monoidal monad $( \td, \unitd{}, \multd{}, \bistrdna)$ on $\catd$,
        related to\\
        \qquad the monoidal monad $(\tc, \unitc{}, \multc{}, \bistrcna)$ on $\catc$
        by \\
        \qquad 
        a monoidal monad morphism $(\funbar, \dist{})$ defined 
        in~(\ref{d_distlaw}) and~(\ref{d_distbistr}),\\
  {\bf (iii.a)} a monoidal mono factorization system on $\catd$.\\
  {\bf (iv)}\ $\td$ maps relevant pseudoepis to pseudoepis.\\
  \hline
\end{tabular}

%Note that lifting a monoidal monad directly as we did here, or lifting both
%the associated strength and mediator as in Section~\ref{strong.s:strong},
%yield the same construction.  This is because of Fact~\ref{f_eq}.

\subsection{Commutative Monads}
\label{strong.s:comm}



In the case of {\em symmetric\/} monoidal categories $\catc$ and $\catd$,
recall that if we also want to make the subscone a symmetric monoidal
category, it suffices to replace {\bf (i.a)} by {\bf (i.b)}, which requires
$\funbar$ to be a {\em symmetric\/} monoidal functor.  This case occurs
notably if we want to lift a {\em commutative\/} monad to the subscone.

Recall that a strong monad $( \td, \unitd{}, \multd{}, \strdna)$ is
commutative if and only if, letting $\strd A B'$ be the dual strength $\td
{\cd B A} \circ \strd B A \circ \cd {\td A} B$, then Diagram~(\ref{eq:tt'})
commutes.

\noindent
\begin{minipage}{6.5cm}
  Let $\bistrd A B$ be the common diagonal $\multd {A \tensord B} \circ \td
  {\strd A B'} \circ \strd {\td A} B = \multd {A \tensord B} \circ \td {\strd
    A B} \circ \strd A {\td B}'$.  We can check that $\bistrdna$ is then a
  mediator
, whence every commutative monad is monoidal.  In fact, a monoidal
  monad is commutative if and only if the following additional diagram
  commutes
\ifmscs
(see Appendix~A.4 in \cite{GLN02}).
\else
(see Appendix~\ref{app:commmonoidal}).
\fi
\end{minipage}
\begin{minipage}{6.5cm}
  \begin{equation}
    \label{eq:monoidal:comm}
    \xymatrix{
      {\td A \tensord \td B}
      \ar[d]_{\cd {\td A} {\td B}}
      \ar[r]^{\bistrd A B}
      &
      {\td (A \tensord B)}
      \ar[d]^{\td \cd A B}
      \\
      {\td B \tensord \td A}
      \ar[r]_{\bistrd B A}
      &
      {\td (B \tensord A)}
      }
  \end{equation}
\end{minipage}

\noindent
For convenience, we shall now understand commutative monads as monoidal monads
satisfying (\ref{eq:monoidal:comm}). The lifting of monoidal monads of
Section~\ref{strong.s:monoidal} then yields a lifting of commutative monads,
by Fact~\ref{f_eq}.  Therefore, to lift a commutative monad $(\tc, \unitc{},
\multc{}, \strcna)$ on category $\catc$
to $\subscone{\catc}{\catd}{\funbar}$, we require:\\

\noindent
\begin{tabular}{|l|}
  \hline
  {\bf (i.b)} symmetric monoidal categories $(\catc, \tensorc, \Ic, \alphacna, \lc{},
  \rc{}, \ccna)$ and $(\catd, \tensord, \Id, \alphadna, \ld{}, \rd{}, \cdna)$, \\
  \qquad and a symmetric monoidal functor $\funbar : \catc \to \catd$,\\
  {\bf (ii.c)} a commutative monad $( \td, \unitd{}, \multd{}, \bistrdna)$ on $\catd$,
        related to \\
        \qquad the commutative monad $(\tc, \unitc{}, \multc{}, \bistrcna)$ on
        $\catc$ by \\
        \qquad 
        a monoidal monad morphism $(\funbar, \dist{})$ defined 
        in~(\ref{d_distlaw}) and~(\ref{d_distbistr}),\\
  {\bf (iii.a)} a monoidal mono factorization system on $\catd$.\\
  {\bf (iv)}\ $\td$ maps relevant pseudoepis to pseudoepis.\\
  \hline
\end{tabular}

%added JGL 06 may 2004.

When $\catd$ has all finite products and we consider the induced symmetric
monoidal structure, we might require that the monoidal monad $(\td, \unitd{},
\multd{}, \bistrdna)$ is not just commutative but even {\em cartesian\/}, by
which we mean that $\td$ is a cartesian monoidal functor with mediating pair
$(\bistrdna, \unitd{\Id})$.  (Recall that $\td$ is always a monoidal functor
with this very mediating pair.)  This means that $\td \pi_i \circ \bistrd A B =
\pi_i$, $i \in \{1, 2\}$.  We just do not need this in our constructions; but it is
often easier to prove that a monad is cartesian and infer that it is
commutative than to prove that it is commutative directly: we shall see
examples of cartesian monads in Section~\ref{examples.s}.




%Recall that to lift the CCC structure of $\catc$ to the subscone, we
%additionally require $\catd$ to be a CCC with pullbacks, and $\funbar$ to
%preserve finite products \cite{MS93}.

%\subsubsection*{Final summary of assumptions}

%\begin{itemize}
%\item
%We are given two categories
%$\catc$ and $\catd$ with explicitly given finite products
%and natural isomorphisms $\rc{}$ and $\alphacna$
%($\rd{}$ and $\alphadna$, respectively)
%together with a functor $\funbar : \catc \to \catd$
%preserving strictly finite products, $\rc{}$ and $\alphacna$.

%\item
%We are given two strong monads, $( \tc, \unitc{}, \multc{}, \strcna )$
%on $\catc$
%and $( \td, \unitd{}, \multd{}, \strdna )$ on $\catd$,
%related by a distributivity law $\dist{}$ defined 
%in~(\ref{d_distlaw}) and~(\ref{d_diststr}).

%\item
%Category $\catd$ has a mono factorization system.

%\item
%Functor $\td$ preserves pseudoepis.

%\item
%Products preserve pseudoepis.

%\end{itemize}


%\bibliographystyle{alpha} 
%\bibliography{lifting}







%\end{document}


==> lts.tex <==

\subsection{Labelled transition systems and bisimulations}
\label{sec:lts}

The case $\td A = {\pfin A}$ allows one to define labelled transition systems
as elements of $(\td A)^{A \times L}$, with labels in $L$ and states in $A$,
as functions mapping states $a$ and labels $\ell$ to the set of states $a'$
such that $a {\buildrel \ell \over\longrightarrow} a'$.  Our monad lifting
$\lift S$ in this case is parameterized by a binary relation on $R_L$ on
labels and is defined by: {\small
\begin{eqnarray*}
 (f_1, f_2) \in \lift S & \iff & \forall a_1, a_2, \ell_1, \ell_2 \cdot (a_1, a_2) \in
 S \land (\ell_1, \ell_2) \in R_L \Rightarrow \\
 && \left\{
   \begin{array}{l}
     \forall b_1 \in f_1 (a_1, \ell_1) . \exists b_2 \in f_2 (a_2, \ell_2) . (b_1,
     b_2) \in S \ \land \\
     \forall b_2 \in f_2 (a_2, \ell_2) . \exists b_1 \in f_1 (a_1, \ell_1) . (b_1,
     b_2) \in S
   \end{array}
 \right.%\bigg)
\end{eqnarray*}
} In case $R_L$ is the equality relation, the relation $\lift S$ relates $f_1$
and $f_2$ iff $S$ is a {\em strong bisimulation\/} between the labelled transition
systems $f_1$ and $f_2$. 
%When labels contain a special element $\pmb{\tau}$ and $R_L$ is defined by
%$(\ell_1, \ell_2) \in R_L$ if and only if $\ell_1=\ell_2$ or
%$\ell_1=\pmb{\tau}$ or $\ell_2=\pmb{\tau}$, then we get {\em weak
%  bisimulation}.

\comment{DN 07/01/04
It is also interesting to see what the constructions of
Section~\ref{ccc.s:simplicial} yields here.  We consider the non-empty finite
powerset monad $\pfsna$ instead of the finite powerset monad, because the
former is a cartesian monad and the latter is not. The functor $\BBna \pfsna$
maps every set $A$ to ${(\pfsna^{q+1} (A))}_{q\geq -1}$.  The elements of
$\pfsna^{q+1} (A)$ are non-empty finite sets of \ldots{} of non-empty finite
sets of elements of $A$, that is, finitely branching trees whose branches are
all of depth $q+1$, and whose leaves are elements of $A$.

\noindent
\begin{minipage}{5cm}
  For instance, the sets $\{\{1\}, \{1, 2\}\}$ and $\{\{1\}, \{3\}\}$ in
  $\pfsna^2 (\nat)$ can be represented as the trees on the right.
\end{minipage}
\begin{minipage}{7cm}
  \begin{center} % 75%
    \includegraphics{tree.eps}
  \end{center}
\end{minipage}

\noindent
Alternatively, these trees can be seen as sets of computation paths from their
roots to their leaves, making $q+1$ choices until a leaf is reached.

Cofaces $\partial^i_q$ add dummy nodes on each branch at level $i$, while
codegeneracies $s^i_q$ remove the nodes at level $i+1$, flattening the tree
partially.  For example, the cofaces $0$, $1$, $2$ and the codegeneracy $0$
(there are no others) of the left-hand tree $(a)$ above are:
\begin{center} % 75%
  \includegraphics{tree_face.eps}
\end{center}
Looking at trees as sets of paths, $\partial^i_q$ inserts a stuttering step at
choice point number $i$, while $s^i_q$ makes two consecutive choices into one
aggregate choice.

Since $\funbar$ is the cartesian product functor from $\catset \times \catset$
to $\catset$, the brutal functor maps $(A_1, A_2)$ to ${(\pfsna^{q+1} (A_1)
  \times \pfsna^{q+1} (A_2))}_{q\geq -1}$, while the considerate functor maps
it to ${(\pfsna^{q+1} (A_1 \times A_2))}_{q\geq -1}$.  The brutal monad
morphism is the identity, while the considerate monad morphism $\distBB{}$ is
for each $q\geq -1$ the function mapping $R \in \pfsna^{q+2} (A \times B)$,
i.e., a tree with leaves labeled by pairs $(x, y)$, to the pair of trees with
only the $x$ components (resp.\ $y$ components) at the leaves.  Call the
resulting pair of trees the {\em domain\/} and {\em codomain\/} of the input
tree, respectively.

\noindent
\begin{minipage}{4cm}
  This is illustrated on the right.  Notice that identical subtrees are merged
  in the process (see second component on the right).
\end{minipage}
\begin{minipage}{8cm}
  \begin{center} % 75%
    \includegraphics{tree_dist.eps}
  \end{center}
\end{minipage}

\noindent
An object of the subscone $\subscone {\catset \times \catset}
{\catset^\Delta}$ is a triple $\langle S, m, A \rangle$ where $R$ is a binary
relation (a set of pairs), and $S = {(S_q)}_{q\geq -1}$ is a cosimplicial set
with ${(m_q : S_q \to \pfsna^{q+1} (R))}_{q\geq -1}$ a pointwise injective
cosimplicial map.  Since isos in $\catset^\Delta$ are pointwise, $S$ is---up
to iso---a cosimplicial subset of ${(\pfsna^{q+1} (R))}_{q\geq -1}$.  In other
words, each $S_q$ is a set of trees of depth $q+1$ whose leaves are pairs $(x,
y) \in R$, and whose cofaces are codegeneracies are in the expected $S_{q \pm
  1}$.

\ForAuthors{I've stopped here for now.  I don't know whether this yields
  anything interesting yet.}

\paragraph{Brutal case.}
Since the brutal monad morphism is just the identity, $\tS \langle S, m,
A\rangle$ is just $\langle \decalaged S, \decalaged m, \decalaged A\rangle$.


\paragraph{Considerate case.}
}


==> monadj.tex <==
\section{Composition of Monoidal Adjunctions}
\label{app:monadj:comp}


We first show that $\funbara U$ is a monoidal functor, with mediating pair
$(\funbara {\theta^U} \circ \tstrna, \funbara {\iota^U} \circ \tstri)$.

We must check all three coherence conditions~(\ref{eq:theta:coh:alpha}),
(\ref{eq:theta:coh:l}), (\ref{eq:theta:coh:r}).

\paragraph{Diagram~(\ref{eq:theta:coh:alpha}).}

{\small
  \[
    \xymatrix@R-15pt@C-5pt{
      {\hbox{$
          \begin{array}{c}
            (\funbara {U(A)} \tensord \funbara {U(B)})\\ \tensord \funbara {U(C)}
          \end{array}
          $}}
      \ar[rrr]^{\alphadna}
      \ar[d]_{\tstrna \tensord \identity {\funbara {U(C)}}}
      \ar@{}[rrrdd]|{\txt{(coherence (\ref{eq:theta:coh:alpha}) for $\tstrna$)}}
      &&&
      {\hbox{$
          \begin{array}{c}
            \funbara {U (A)} \tensord\\ (\funbara {U (B)} \tensord \funbara {U (C)})
          \end{array}
          $}}
      \ar[d]^{\identity {\funbara {U (A)}} \tensord \tstrna}
      \\
      {\hbox{$
          \begin{array}{c}
            \funbara {U (A) \tensorc U (B)}\\ \tensord \funbara {U (C)}
          \end{array}
          $}}
      \ar[rd]^{\tstrna}
      \ar[d]_{\funbara {\theta^U} \tensord \identity {\funbara {U (C)}}}
      &&&
      {\hbox{$
          \begin{array}{c}
            \funbara {U (A)} \tensord\\ \funbara {U (B) \tensorc U (C)}
          \end{array}
          $}}
      \ar[ld]_{\tstrna}
      \ar[d]^{\identity {\funbara {U (A)}} \tensord \funbara {\theta^U}}
      \\
      {\hbox{$
          \begin{array}{c}
            \funbara {U (A \otimes^{\cal D} B)}\\ \tensord \funbara {U (C)}
          \end{array}
          $}}
      \ar[d]_{\tstrna}
      \ar@{}[r]|{\txt{(natur-\\ality of\\$\tstrna$)}}
      \ar@{}[rrrdd]|{\txt{($\funbar$ applied to coherence (\ref{eq:theta:coh:alpha}) for $\theta^U$)}}
      &
      {\hbox{$
          \funbara {
            \begin{array}{c}
              (U (A)\\ \tensorc U (B))\\ \tensorc U (C)
            \end{array}
            }
          $}}
      \ar[r]^{\funbara {\alphacna}}
      \ar[ld]^{\funbara {\theta^U \tensorc \identity {U (C)}}}
      &
      {\hbox{$
          \funbara {
            \begin{array}{c}
              U (A) \tensorc\\ (U (B) \tensorc\\ U (C))
            \end{array}
            }
          $}}
      \ar[rd]_{\funbara {\identity {U (A)} \tensorc \theta^U}}
      \ar@{}[r]|{\txt{(natur-\\ality of\\$\tstrna$)}}
      &
      {\hbox{$
          \begin{array}{c}
            \funbara {U (A)} \tensord\\ \funbara {U (B \otimes^{\cal D} C)}
          \end{array}
          $}}
      \ar[d]^{\tstrna}
      \\
      {\hbox{$
          \funbara {
            \begin{array}{c}
              U (A \otimes^{\cal D} B)\\ \tensorc U (C)
            \end{array}
            }
          $}}
      \ar[d]_{\funbara {\theta^U}}
      &&&
      {\hbox{$
          \funbara {
            \begin{array}{c}
              U (A) \tensorc\\ U (B \otimes^{\cal D} C)
            \end{array}
            }
          $}}
      \ar[d]^{\funbara {\theta^U}}
      \\
      {\hbox{$
          \funbara {
            \begin{array}{c}
              U ((A \otimes^{\cal D} B)\\ \otimes^{\cal D} C)
            \end{array}
            }
          $}}
      \ar[rrr]_{\funbara {U \alpha^{\cal D}}}
      &&&
      {\hbox{$
          \funbara {
            \begin{array}{c}
              U (A \otimes^{\cal D}\\ (B \otimes^{\cal D} C))
            \end{array}
            }
          $}}
      }
    \]
    }

\paragraph{Diagram~(\ref{eq:theta:coh:l}).}

{\small
  \[
  \xymatrix@C+30pt{
    {\Id \tensord \funbara {U A}}
    \ar[rrdd]^{\ld {\funbara {U A}}}
    \ar[d]|{\tstri \tensord \identity {\funbara {U A}}}
    &&
    \\
    {\funbara \Ic \tensord \funbara {U A}}
    \ar@{}[rrd]|{\txt{(coherence\\condition\\(\ref{eq:theta:coh:l}))}}
    \ar[d]|{\funbara {\iota^U} \tensord \identity {\funbara {U A}}}
    \ar[rd]^{\tstr \Ic {U A}}
    &&
    \\
    {\funbara {U I^{\cal D}} \tensord \funbara {U A}}
    \ar[d]|{\tstr {U I^{\cal D}} {U A}}
    \ar@{}[r]|{\txt{(natur-\\ality\\of $\tstrna$)}}
    &
    {\funbara {\Ic \tensorc U A}}
    \ar[ld]^{\funbara {\iota^U \tensorc \identity {U A}}}
    \ar[r]|{\funbara {\lc {U A}}}
    &
    {\funbara {U A}}
    \\
    {\funbara {U I^{\cal D} \tensorc U A}}
    \ar@{}[rru]|{\txt{(coherence\\condition\\(\ref{eq:theta:coh:l}))}}
    \ar[d]|{\funbara {\theta^U_{I^{\cal D}, A}}}
    &&
    \\
    {\funbara {U (I^{\cal D} \otimes^{\cal D} A)}}
    \ar[rruu]_{\funbara {U \ell^{\cal D}_A}}
    }
  \]
  }

\paragraph{Diagram~(\ref{eq:theta:coh:r}).}
This is checked by a diagram similar to the latter.

By the same reasoning, $F \discr$ is also a monoidal functor, with mediating
pair $(F \tstrcna \circ \theta^F, F \tstrci \circ \iota^F)$.

We now check the monoidal adjunction conditions (\ref{eq:moneta:I}),
(\ref{eq:moneta:tensor}), (\ref{eq:moneps:I}), (\ref{eq:moneps:tensor}). Let
$\counita$ the counit, and $\unita$ the unit of $\discr \dashv \funbar$, and
$\pmb{\epsilon}$ the counit, and $\unitc{}$ the unit of $F \dashv U$.

\paragraph{Diagram~(\ref{eq:moneta:I}).}

{\small
  \[
  \xymatrix@C+60pt{
    {\Id}
    \ar[r]^{\tstri}
    \ar[rd]_{\unita_{\tstri}}^{\txt{((\ref{eq:moneta:I}) for $\discr \dashv \funbar$)}}
    &
    {\funbara {\Ic}}
    \ar[r]^{\funbara {\iota^U}}
    \ar[d]|{\funbara {\tstrci}}
    \ar[rd]_{\funbara {\unitc \Ic}}^{\txt{((\ref{eq:moneta:I}) for $F \dashv U$)}}
    &
    {\funbara {U I^{\cal D}}}
    \ar[d]^{\funbara {U \iota^F}}
    \\
    &
    {\funbara {\discr \Id}}
    \ar[rd]_{\funbara {\unitc {\discr \Id}}}
    \ar@{}[r]|{\txt{(naturality\\of $\funbara {\unitc{}}$)}}
    &
    {\funbara {UF \Ic}}
    \ar[d]^{\funbara {UF I^{\cal D}}}
    \\
    &&
    {\funbara {UF \discr \Id}}
    }
  \]
  }

\paragraph{Diagram~(\ref{eq:moneta:tensor}).}

{\small
  \[
  \xymatrix@C-40pt{
    {A \tensord B}
    \ar[rr]^{\unita_A \tensord \unita_B}
    \ar[dd]|{\unita_{A \tensord B}}
    \ar@{}[rd]|{\txt{((\ref{eq:moneta:tensor}) for\\$\discr \dashv \funbar$)}}
    &&
    {\funbara {\discr A} \tensord \funbara {\discr B}}
    \ar[rr]^{\funbara {\unitc {\discr A}} \tensord \funbara {\unitc {\discr
          B}}}
    \ar[ld]|{\tstr {\discr A} {\discr B}}
    \ar@{}[rd]|{\txt{(natur-\\ality\\of $\tstrna$)}}
    &&
    {\funbara {UF \discr A} \tensord \funbara {UF \discr B}}
    \ar[ld]^{\tstr {UF \discr A} {UF\discr B}}
    \\
    &
    {\funbara {\discr A \tensorc \discr B}}
    \ar[ld]|{\funbara {\tstrc A B}}
    \ar[rr]^{\funbara {\unitc {\discr A} \tensorc \unitc {\discr B}}}
    \ar[dd]|{\funbara {\unitc {\discr A \tensorc \discr B}}}
    \ar@{}[rd]|{\txt{((\ref{eq:moneta:tensor}) for\\$F \dashv U$)}}
    &&
    {\funbara {UF \discr A \tensorc UF \discr B}}
    \ar[ld]^{\funbara {\theta^U_{F \discr A, F \discr B}}}
    &
    \\
    {\funbara {\discr (A \tensord B)}}
    \ar[dd]|{\funbara {\unitc {\discr (A \tensord B)}}}
    \ar@{}[rd]|{\txt{(natur-\\ality\\of $\funbara {\unitc {}}$)}}
    &&
    {\funbara {U (F \discr A \otimes^{\cal D} F \discr B)}}
    \ar[ld]^{\funbara {U \theta^F_{\discr A, \discr B}}}
    &&
    \\
    &
    {\funbara {UF (\discr A \tensorc \discr B)}}
    \ar[ld]^{\funbara {UF \tstrc A B}}
    &
    &&
    \\
    {\funbara {UF \discr (A \tensord B)}}
    &&
    &&
    }
  \]
  }

Diagrams~(\ref{eq:moneps:I}) and~(\ref{eq:moneps:tensor}) are dealt with
similar, and give rise to similar verifications.



==> names.tex <==

\subsection{Logical relations for dynamic name creation}
\label{sec:names}

Consider the categorical model of dynamic name creation defined in
\cite{Sta96}.
%\ForAuthors{
%  David, is this really Moggi's?  In your paper with Yu, you cite this as
%  Stark's model of dynamic name creation.
%  }
%
Let $\ordinalcat$ be the category of finite sets and injective functions, and
%
$\setcat^\ordinalcat$ be the category of functors from $\ordinalcat$ to
$\setcat$ and natural transformations (the category of {\em covariant
  presheaves\/} over $\ordinalcat$).
%
%Note that $\setcat^\ordinalcat$ has a mono factorization, where pseudoepis are
%{\em pointwise epis\/} (presheaf morphisms $f$ such that $fs$ is epi for every
%$s$), and relevant monos are pointwise monos.
For short, write $\monad A s$ for $\monad (A) (s)$ and similarly for other
notations.
%Let $+$ denote coproduct in $\ordinalcat$. 
Let $+$ denote disjoint union in $\ordinalcat$.%
\footnote{ Note that $+$ is not a coproduct in $\ordinalcat$.  In fact,
  $\ordinalcat$ does not have a coproduct.  However $+$ is functorial in both
  components, associative, and has a neutral element, and this is all we need.}

We define the strong monad 
\iflong $(\monad, \unit, \mult, \strength)$ \else $\monad$ \fi 
on $\setcat^\ordinalcat$ 
\iflong by: \else as follows. \fi
\iflong
\begin{itemize}
  
\item \fi
  $\monad A = \colim_{s'} A (\_ + s') : \ordinalcat \to
  \setcat$.
  
  On objects, this is given by $\monad A s = \colim_{s'} A (s+s')$, i.e.,
  $\monad A s$ is the set of all equivalence classes of pairs $(s', a)$ with
  $s' \in \ordinalcat$ and $a \in A (s+s')$ modulo the smallest equivalence
  relation $\equiv$ such that $(s', a) \equiv (s'', A (\identity s+j) a)$ for
  every morphism $s' {\buildrel j \over\longrightarrow} s''$ in $\ordinalcat$
  (intuitively, given a set of {\em names\/} $s$, elements of $\monad A s$ are
  formal expressions $(\nu s') a$ where all names in $s'$ are bound and every
  name free in $a$ is in $s+s'$---modulo the fact that $(\nu s', s'') a \equiv
  (\nu s') a$ for any additional set of new names $s''$ not free in $a$).  We
  shall write $[s', a]$ the equivalence class of $(s', a)$.
  
  On morphisms $s_1 {\buildrel i\over\longrightarrow} s_2$, $\monad A i$ maps
  $[s', a]$ to the equivalence class of $[s',
  A(i+\identity{s'}) a]$.
  
\item For any $f : A \to B$ in $\setcat^\ordinalcat$, $\monad f s :
  \monad A s \to \monad B s$ is defined by $\monad f s [s', a] = [s',
  f(s+s') a]$.  This is compatible with $\equiv$ because $f$ is natural.
  
\item $\unit_A s : A s \to \monad A s$ is defined by $ \unit_A s a =
  [\emptyset, a]$.
  
\item $\mult_A s : \monad^2 A s \to \monad A s$ is defined by $
  \mult_A s [s', [s'', a]] = [s'+s'', a]$.
  
\item $\strength_{A, B} s : A s \times \monad B s \to \monad (A \times
  B) s$ is defined by $\strength_{A, B} s (a, [s', b]) = [s', (A \inl{s}{s'}
  a, b)]$ where $\inl{s}{s'} : s \to s+s'$ is the canonical injection.
\end{itemize}
Furthermore, $\tc$ is a commutative monad, whose mediator $\bistrd A B s :
\tc A s \times \tc B s \to \tc (A \times B) s$ maps $([s', a], [s'', b])$ to
$[s'+s'', (A (\identity s + \inl {s'} {s''}) a, A (\identity s + \inr {s''}
{s'}) b)]$, where $\inr {s''} {s'} : s'' \to s' + s''$ is the other canonical
injection.  In fact, $\tc$ is a cartesian monad.  Indeed, $(\tc \pi_1 \circ
\bistrd A B) s$ maps $([s', a], [s'', b])$ to $[s'+s'', A (\identity s + \inl
{s'} {s''}) a] = [s', a]$, so $\tc \pi_1 \circ \bistrd A B = \pi_1$, and
similarly $\tc \pi_2 \circ \bistrd A B = \pi_2$.

It is important to note how $\equiv$ works.  The category $\ordinalcat$ has
pushouts: in particular, if $s_0 {\buildrel i_1 \over\longrightarrow} s_1$ and
$s_0 {\buildrel i_2 \over\longrightarrow} s_2$ are two morphisms in
$\ordinalcat$, then there is a finite set $s_1 +_{s_0} s_2$ and two morphisms
$s_1 {\buildrel j_1 \over\longrightarrow} s_1 +_{s_0} s_2$, $s_2 {\buildrel
  j_2 \over\longrightarrow} s_1 +_{s_0} s_2$ such that $j_1 \circ i_1 = j_2
\circ i_2$---take $s_1 +_{s_0} s_2$ to be the disjoint sum $s_1+s_2$ modulo
the equivalence relation relating $i_1 (a_0) = i_2 (a_0)$ for every $a_0 \in
s_0$.

It follows that $(*)$ for every $a_1 \in A (s+s_1)$, $a_2 \in A (s+s_2)$,
$(s_1, a_1) \equiv (s_2, a_2)$ if and only if there is a finite set $s_{12}$
and two arrows $s_1 {\buildrel j_1 \over\longrightarrow} s_{12}$ and $s_2
{\buildrel j_2 \over\longrightarrow} s_{12}$ such that $A (\identity{s_1}+j_1)
a_1 = A (\identity{s_2}+j_2) a_2$.

We take ${\pmb C}_1={\pmb C}_2=\mathbb{C}=\setcat^\ordinalcat$, hence objects
in the subscone give rise to $\ordinalcat$-indexed {\em Kripke logical
  relations}.
%
Furthermore, $|\_|_1=|\_|_2=|\_|$ is the identity functor and
%
$\monadrel$ is just $\monad$.
%
The category $\setcat^\ordinalcat$ has a mono factorization consisting of
pointwise surjections and pointwise injections.
\comment{DN 07/01/03
(see Lemma~\ref{lemma:presh:epimono}).
}

As in Section~\ref{relations.s}, the monad morphism $\distr_{\langle A_1, A_2
  \rangle} s : \monadrel ( A_1 \times A_2 ) s \to \monad A_1 s \times
\monad A_2 s$ is equal to $\langle \monadrel \pi_1 , \monadrel \pi_2 \rangle
s$. \iflong That is to say
\[
\distr_{\langle A_1, A_2 \rangle} s [s', (a_1, a_2)] =
([s', a_1], [s', a_2])
\]
where $s' \in \ordinalcat$, $a_1 \in A_1 (s+s')$, $a_2 \in A_2 (s+s')$.

Again as in $\setcat$, every functor $S$ from $\ordinalcat$ to $A_1 \times
A_2$ has a representation
\[
\langle \projrel_1, \projrel_2 \rangle : S \hookrightarrow A_1 \times A_2
\]
where each arrow $\langle \projrel_1, \projrel_2 \rangle s : S s \hookrightarrow A_1 s
\times A_2 s$ is an inclusion.

%Then, using the mono factorization above, which acts pointwise, $\monadrel S$
%is given by the existence of 

Hence, $S$ is a family of relations $S s$ between $A_1 s$ and $A_2 s$,
functorial in $s$ (for each $s' {\buildrel i \over\longrightarrow} s''$, $S i$
is the appropriate restriction of $A_1 i \times A_2 i$). Recall from
Section~\ref{relations.s} that $\lift S$ is defined as the direct image of
$\langle \td \projrel_1, \td \projrel_2 \rangle$. So, $(\dagger)$ $[s_1, a_1]
\; \lift S s\; [s_2, a_2]$ if and only if for some $s' \in \ordinalcat$, $a'_1
\in A_1 s'$, $a'_2 \in A_2 s'$, $(s_1, a_1) \equiv (s', a'_1)$, $(s_2, a_2)
\equiv (s', a'_2)$ and $a'_1\; S (s+s')\; a'_2$.

Using $(*)$ above, $(s_1, a_1) \equiv (s', a'_1)$ means that there is a finite
set $s'_1$ and two arrows $s_1 {\buildrel j_1 \over\longrightarrow} s'_1$, $s'
{\buildrel j'_1 \over\longrightarrow} s'_1$ in $\ordinalcat$ such that: (a)
$A_1 (\identity s + j_1) a_1 = A_1 (\identity s + j'_1) a'_1$.  Similarly,
$(s_2, a_2) \equiv (s', a'_2)$ means there is a finite set $s'_2$ and two
arrows $s_2 {\buildrel j_2 \over\longrightarrow} s'_2$, $s' {\buildrel j'_2
  \over\longrightarrow} s'_2$ in $\ordinalcat$ such that: (b) $A_2 (\identity
s + j_2) a_2 = A_2 (\identity s + j'_2) a'_2$.  Consider arrows $j'_1$ and
$j'_2$, which both have $s'$ as source, and build their pushout $s_0 = s'_1
+_{s'} s'_2$, with arrows $s'_1 {\buildrel j''_1 \over\longrightarrow} s_0$,
$s'_2 {\buildrel j''_2 \over\longrightarrow} s_0$.  Let $j$ be $j''_1 \circ
j'_1 = j''_2 \circ j'_2$.  By applying $A_1 (\identity s + j''_1)$ to both
sides of (a), $A_1 (\identity s + (j''_1 \circ j_1)) a_1 = A_1 (\identity s +
j) a'_1$.  By applying $A_2 (\identity s + j''_2)$ to both sides of (b), $A_2
(\identity s + (j''_2 \circ j_2)) a_2 = A_2 (\identity s + j) a'_2$.  Since
$a'_1\; S(s+s')\; a'_2$ and $S$ is functorial, $A_1 (\identity s + j) a'_1 \;
S(s+s_0)\; A_2 (\identity s + j) a'_2$, so $A_1 (\identity s + (j''_1 \circ
j_1)) a_1\; S(s+s_0)\; A_2 (\identity s + (j''_2 \circ j_2)) a_2$.
% Now observe that being
% in relation through $R(s+s_0)$ means being in relation through $S(s+s_0)$.

So if $(s_1, a_1) \; \widetilde{S} s \; (s_2, a_2)$ then there are arrows $s_1
{\buildrel i_1 \over\longrightarrow} s_0$ and $s_2 {\buildrel i_2
  \over\longrightarrow} s_0$, namely $i_1 = j''_1 \circ j_1$ and $i_2 = j''_2
\circ j_2$, such that $A_1 (\identity s + i_1) a_1 \; S (s+s_0) \; A_2
(\identity s + i_2) a_2$.

\comment{

  modified by SL, 20.06.2002

Conversely, if the latter holds for every $s$, define the binary relation $R
s'$ as the smallest such that for every $s_1$, for every $a_1 \in A_1 (s_1)$,
for every $s_2$, for every $a_2 \in A_2 (s_2)$, for every arrows $s_1
{\buildrel i_1 \over\longrightarrow} s'$ and $s_2 {\buildrel i_2
  \over\longrightarrow} s'$, $A_1 i_1 a_1\; Rs'\; A_2 i_2 s_2$ if $A_1 i_1
a_1\; Ss'\; A_2 i_2 s_2$.  $R$ is functorial since $S$, $A_1$ and $A_2$ are,
and $(\dagger)$ above clearly holds.
}

Conversely, if the latter holds, then $(\dagger)$ above clearly holds
for $s' = s_0$, $a'_1 = A_1 (\identity s + i_1) a_1$ and
$s'_2 = A_2 (\identity s + i_2) a_2$.


%$\monadrel \langle \pi_1, \pi_2 \rangle s :
%\monadrel S s \to \monadrel (A_1 \times A_2) s$
%is given by
%\[
%\monadrel \langle \pi_1, \pi_2 \rangle s (s', (a_1, a_2)) = (s', (a_1, a_2))
%\]
\else%
\fi%
$\widetilde{S} s \hookrightarrow \monad A_1 s \times \monad A_2 s$ is
thus given by
\begin{equation}
  \label{eq:name:logrel}
  \begin{array}{rcl}
    [s_1, a_1] \; \widetilde{S} s \; [s_2, a_2] & \iff &
    \exists s_0 \in \ordinalcat \cdot
    \exists i_1 : s_1 \to s_0 \in \ordinalcat \cdot
    \exists i_2 : s_2 \to s_0 \in \ordinalcat \cdot \\
    && %\qquad
    (A_1 (\identity{s}+i_1) a_1) \; S (s+s_0) \; (A_2 (\identity{s}+i_2) a_2)
  \end{array}
\end{equation}
where $a_1 \in A_1(s+s_1)$ and $a_2 \in A_2(s+s_2)$%
\iflong%
.
\else%
% \ (exercise)
.
\fi%

From (\ref{eq:name:logrel}) we define a logical relation for Moggi's
metalanguage, as suggested in Section~\ref{relations.s}, by induction on types
$\tau$.  Each relation $\Eval {\tau}$ is a functor from $\ordinalcat$ to
$\catset \times \catset$, so that $\Eval {\tau} s$ is a binary relation for
each type $\tau$ and each finite set $s$.  We have:
\begin{eqnarray*}
  (f_1, f_2) \in \Eval {\tau \to \tau'} s & \iff &
  \forall s', i : s \to s' \in \ordinalcat, (a_1, a_2) \in \Eval {\tau} s'
  \cdot
  \\
  && \qquad (f_1 s' (i, a_1), f_2 s' (i, a_2)) \in \Eval {\tau'} s'
  \\
  ((a_1, a'_1), (a_2, a'_2)) \in \Eval {\tau \times \tau'} s & \iff &
  (a_1, a_2) \in \Eval {\tau} s \land (a'_1, a'_2) \in \Eval {\tau'} s
  \\
  ([s_1, a_1], [s_2, a_2]) \in \Eval {\tc \tau} s & \iff &
  \exists s_0, i_1 : s_1 \to s_0, i_2 : s_2 \to s_0 \in \ordinalcat \cdot \\
    && %\qquad
    (A_1 (\identity{s}+i_1) a_1, A_2 (\identity{s}+i_2) a_2) \in \Eval {\tau} (s+s_0)
\end{eqnarray*}

This is similar to the logical relations of
\cite{pitts/stark:obsphown,stark:namerp-fi}.  While (\ref{eq:name:logrel}) is
roughly similar to the notion of logical relation of
\cite{pitts/stark:obsphown}, this paper does not rest on Moggi's computational
$\lambda$-calculus.  On the other hand \cite{stark:namerp-fi} does rest on the
computational $\lambda$-calculus but does not define a suitable notion of
logical relation.

Zhang and Nowak show in \cite{ZN:logrelnames} that the logical relation above
is in fact strictly weaker than Pitts and Stark's logical relation
\cite{pitts/stark:obsphown} when restricted to the latter's nu-calculus; Zhang
and Nowak also claim that by reinstantiating our construction of the subscone
with $\catc_1 = \catc_2 = \catset^\ordinalcat$ as above but $\catd =
\catset^{\ordinalcat^\to}$, where $\ordinalcat^\to$ is the comma category
whose objects are the morphisms of $\ordinalcat$, another Kripke
logical relation is obtained that coincides with Pitts and Stark's on
the nu-calculus up to first order.
%
This is in fact wrong, but Zhang \cite{Zha:05} shows that
this can be repaired by replacing $\mathcal I^\to$ by the category
$\mathcal{PI}^\to$ whose objects are, again, morphisms of $\mathcal
I$, but whose morphisms are pullback diagrams in $\mathcal I$.
%
It extends it to the full monadic meta-language, and rests purely on
semantic principles, while Pitts and Stark's definition of their
logical relation relies on normalization properties of the
nu-calculus.

\comment{DN 07/01/03
\ForAuthors{My main purpose in doing the cosimplicial construction of
  Section~\ref{ccc.s:simplicial} was to use it here.  Note that the monad is
  cartesian, which is the most suitable case for this construction to work.
  Why I do this is mainly because it allows me to do some cohomology on top
  of it, which I plan to develop in a later paper.  I had some hope that this
  could generalize Zhang and Nowak's construction, but it does not.  Maybe
  it would be better to leave the cosimplicial construction out of this paper,
  right?
  }
}


==> proba3.tex <==


\subsection{Monads of Measures and Probabilities}
\label{sec:proba}

Defining $\tc A$ to be space of all probability distributions over the space
$A$ allows us to define probabilistic transition systems as objects of ${(\tc
  A)}^A$.  In principle, this should work just like ordinary transition
systems (Section~\ref{sec:lts}).  In actual practice, defining what the right
spaces should be, and ensuring that the required monads exist and have the
required properties, is much subtler.

As regards the right category of spaces, the obvious choice is $\Mes$, the
category of measurable sets (sets equipped with a $\sigma$-algebra) and
measurable functions (such that the inverse image of any measurable subset is
measurable).  F. W. Lawvere, then M. Giry \cite{Lawvere:proba,Giry:proba}
showed that $\Mes$ indeed admits a monad $(\tc {}, \unitc{}, \multc{})$ : $\tc
A$ is the set of (probability) measures over $A$, together with the smallest
$\sigma$-algebra such that, for every measurable subset $X$ of $A$, the map
$p_X$ mapping $\nu \in \tc A$ to $\nu (X)$ is measurable.

$\Mes$ has bad properties.  It is very unlikely to be cartesian
closed\footnote{Although we have been unable to find a proof of this negative
  assertion.}, and the monad above is not strong.  In fact, the category
$\catc$ that is best suited for our purposes here is the category $\Dcpo$ of
dcpos and continuous maps, using the continuous valuation monad of Jones
\cite{Jones:proba}.  We examine this case in Section~\ref{sec:proba:dcpo:set},
taking $\catset$ as the observation category $\catd$.  We shall see that we
retrieve Larsen and Skou's notion of probabilistic bisimulation
\cite{LS:proba} in this case, at least when specialized to finite sets and
discrete probabilities.  In the case of continuous (non-discrete) state
spaces, this notion is too weak for most purposes, and we extend it: we
present in Section~\ref{sec:proba:dcpo} the most precise notion of logical
relation that our construction apparently affords us.  This is rather
technical, and the main obstacle is condition {\bf (iv)} stating that $\td$
should map relevant pseudoepis to pseudoepis. Another different route is taken
in Section~\ref{sec:proba:met}, where we examine the category $\catc = \Met$
of metric spaces and non-expansive maps, which has a monad of probability
measures; observed from $\catd = \Met$ again, our logical relations define a
notion of families of metric spaces indexed by types, extending
\cite{DGJP:approx:Markov,DGJP:metric:proba}, modulo some technicalities.
%  We observe that we can instead
%observe metric spaces, or even analytic spaces, from $\catd = \Dcpo$ instead,
%using dcpo embedding techniques, in Section~\ref{sec:proba:met:dcpo}.
% Finally,
%we examine the case of analytic spaces in Section~\ref{sec:proba:souslin},
%where we have a strong monad but no cartesian or even symmetric monoidal
%closed structure.


\subsection{Continuous Valuations on Dcpos, observed from $\catset$}
\label{sec:proba:dcpo:set}

Let us consider a natural CCC equipped with a notion of measure: $\Dcpo$, the
category of {\em directed complete partial orders}, a.k.a., {\em dcpos}. The
objects (dcpos) are partial orders such that every directed subset (every
non-empty set such that any two elements have an upper bound) has a least
upper bound; the morphisms are continuous functions.  This is
cartesian-closed, and has pullbacks.

\subsubsection{Dcpos and the Continuous Valuation Monad.}

For every dcpo $A$, Jones \cite{Jones:proba} observed that the set $\tc A$ of
all continuous valuations, to be defined next, was again a dcpo, and that this
construction could be used to define a probabilistic powerdomain monad.
(Jones calls dcpos {\em ipos}, i.e., {\em inductive\/} partial orders, and
calls continuous valuations {\em evaluations}.  We follow the majority of
authors in using ``dcpo'' and ``valuation''.)  Recall that a Scott open of a
dcpo $A$ is an upper closed subset $O$ such that every directed family whose
sup is in $O$ intersects $O$, that Scott opens form the {\em Scott topology\/}
on $A$, so that we can look at dcpos as particular topological spaces.

Let $(A, {\cal O})$ be a topological space.  A (bounded) {\em valuation\/} on
$A$ is a map $\pmb{\nu} : {\cal O} \to \real_+$ such that $\pmb{\nu}
(\emptyset) = 0$ ({\em strictness\/}); $U \subseteq V$ implies $\pmb{\nu}
(U)\leq \pmb{\nu} (V)$ for every opens $U, V \in {\cal O}$ ({\em
  monotonicity\/}); and $\pmb{\nu} (U \cup V) + \pmb{\nu} (U \cap V) =
\pmb{\nu} (U) + \pmb{\nu} (V)$ for every opens $U, V \in {\cal O}$ ({\em
  modularity\/}).  A {\em continuous\/} valuation in addition satisfies
$\pmb{\nu} (\bigcup_i U_i) = \sup_i \pmb{\nu} (U_i)$ for every directed family
${(U_i)}_{i \in I}$ of opens---such a family is {\em directed\/} if and only
if $I \neq \emptyset$ and for every $i, j \in I$, there is $k\in I$ such that
$U_i, U_j \subseteq U_k$.  All the valuations we shall consider are bounded,
i.e., $\pmb{\nu} (A) < +\infty$; we shall not mention this any longer.
Continuous valuations are a concept close to that of measure; while measures
are defined on $\sigma$-algebras, valuations are naturally defined on
topological spaces.

The set $\tc A$ of continuous valuations on the topological space $A$ is a
dcpo, with ordering $\pmb{\nu} \leq \pmb{\xi}$ if and only if $\pmb{\nu} (O)
\leq \pmb{\xi} (O)$ for every open $O$ in $A$.  When we restrict $A$ to be a
dcpo, $\tc {}$ is functorial: for every $A {\buildrel f \over\longrightarrow}
B$, $\tc f$ maps the continuous valuation $\pmb{\nu} \in \tc A$ to the
continuous valuation mapping every open $O$ in $B$ to $\pmb{\nu} (f^{-1}
(O))$.  This gives rise to a monad, whose unit $\unitc A$ maps $x \in A$ to
the {\em Dirac valuation\/} $\delta_x$ on $A$, such that $\delta_x (O) = 1$
for every open $O$ of $A$ containing $x$, $\delta_x (O) = 0$ otherwise.  Its
multiplication $\multc A$ maps continuous valuations $\pmb{\nu}$ on $\tc A$ to
the continuous valuation on $A$ mapping every open $O \subseteq A$ to
$\int_{\pmb{\xi} \in \tc A} \pmb{\xi} (O) d\pmb{\nu}$ (the average of all
possible evaluations $\pmb{\xi} (O)$ of $O$, weighted by the probability of
each valuation $\pmb{\xi}$), and the strength $\strc A B$ maps $a \in A$ and
$\pmb{\nu} \in \tc B$ to the continuous valuation on $A \times B$ mapping
every open $O \subseteq A \times B$ to $\pmb{\nu} (\{y \in B | (a, y) \in
O\})$.  Then $(\tc{}, \unitc{}, \multc{}, \strcna {})$ is a strong monad on
$\Dcpo$ \cite{Jones:proba}.

There is no real need to recall the definition of the Jones integral used
above.  There are several definitions, the original one by Jones
\cite{Jones:proba}, and extensions by Kirch \cite{Kirch:val}, by Tix
\cite{Tix:bewertung}, by Heckmann \cite{Heckmann:space:val}.  They are all
equivalent on dcpos, and define a function mapping every continuous function
$f : A \to (\real_+ \cup \{+\infty\})$, where $(\real_+ \cup \{+\infty\})$ is seen as a dcpo (such
Scott continuous functions are usually called {\em upper continuous\/}; note
that the Scott topology on $(\real_+ \cup \{+\infty\})$ is strictly coarser than its
metric topology) and every continuous valuation $\pmb{\nu}$ on $A$ to $\int_{x\in A}
f (x) d\pmb{\nu} \in (\real_+ \cup \{+\infty\})$. Its main properties on $\Dcpo$ are (see
\cite[Theorem~7.1]{Heckmann:space:val}):
\begin{enumerate}
\item the map $f \in \real_+^A, \pmb{\nu} \in \tc A \mapsto \int_{x \in A} f
  (x) d\pmb{\nu}$ is continuous in each argument separately (hence jointly,
  since joint continuity and separate continuity coincide in $\Dcpo$), and
  linear in $f$ and $\pmb{\nu}$;
\item $\int_{x \in A} f (x) d\delta_{x_0} = f (x_0)$;
\item ({\em Change of Variables formula.\/}) For every continuous function $g
  : A \to B$, $\int_{x \in A} (f \circ g) (x) d\pmb{\nu} = \int_{y\in B} f (y)
  d\tc g (\pmb{\nu})$;
\item for every open $O$ of $A$, letting $\chi_O$ be the characteristic
  function of $O$ in $A$, $\int_{x\in A} \chi_O (x) d\pmb{\nu} = \pmb{\nu}
  (O)$.
\end{enumerate}

For the sake of completeness, note that $\tc{}$ is in fact a monoidal monad on
$\Dcpo$, whose mediator $\bistrc A B$ maps $\pmb{\nu} \in \tc A$ and $\pmb{\xi} \in
\tc B$ to the continuous valuation that Jones (\cite{Jones:proba},
Section~3.10) writes $\pmb{\nu} \otimes \pmb{\xi}$, which maps every Scott open subset
$O$ of the dcpo $A \times B$ to $\int_{x\in A} \left(\int_{y\in B} \chi_O (x,y) d\pmb{\xi}\right)
d\pmb{\nu}$.  On the subcategory of continuous dcpos, this yields a commutative
monad by Fubini's Theorem on valuations \cite[Theorem~3.17]{Jones:proba}.  On
$\Dcpo$, it is unknown whether Fubini's Theorem holds, hence whether the monad
is commutative; in case it is not, $\tc$ would be an example of a monoidal
monad that is not commutative.

%It is useful to recall the definition of the Jones integral used above.  A
%function $f : A \to [0, +\infty]$ is {\em upper-continuous}, or {\em u.c.}, if
%and only if $f^{-1} (a, +\infty]$ is open for every $a \geq 0$.  A {\em simple
%  u.c.\ function\/} in addition only takes finitely many values.  Every simple
%u.c.\ function can be written as a finite sum $\sum_{i=1}^n a_i \chi_{U_i}$,
%where $a_i$ is real non-negative and $U_i$ are open; $\chi_U$ denotes the
%characteristic function of $U$.  Then
%\[
%\int_{x\in A} f (x) d\nu = \sup_{\sum_{i=1}^n a_i \chi_{U_i}\mathrm{\ simple\ 
%    }\leq f} \sum_{i=1}^n a_i \nu (U_i)
%\]

\subsubsection{Constructing a Logical Relation for the Continuous Valuation
  Monad.}

Contrarily to the previous examples, we do not take $\catc_1 = \catc_2 = \catd
= \Dcpo$; we have been unable to show that $\tc{}$ preserved pseudoepis for
any notion of pseudoepi in $\Dcpo$.  We take here a simple solution, which we
shall refine in Section~\ref{sec:proba:dcpo}.

Take $\catd = \catset$, and use Proposition~\ref{prop:adj:distr:2}.  Equip
$\catc = \Dcpo$ and $\catd = \catset$ with the standard (symmetric) monoidal
structure given by finite products.  There is a forgetful functor $\funbar$
from $\Dcpo$ to $\catset$ sending every dcpo $A$ to its set of elements
$\funbara A$, and every continuous function $f : A \to B$ to the underlying
set-theoretic function.  It has a left adjoint $\discr$ mapping every set $E$
to $E$ seen as an dcpo with equality as ordering.  This is called the {\em
  discretization\/} functor, and $\discr E$ is called a {\em discrete\/} dcpo.
Note that all subsets of $\discr E$ are open, so that as a topological space,
$\discr E$ has the discrete topology.

Proposition~\ref{prop:adj:distr:2} applies: $\funbar$ and $\discr$ preserve
products exactly, hence are monoidal (with trivial mediating pairs).  The unit
$\unita_E$ is the identity on $E$, while the counit $\counita_A$ is the
identity function from the dcpo $\discr \funbara A$ ($A$ with equality as
ordering) to $A$, and are clearly monoidal.  This yields a monoidal monad
$(\td, \unitd{}, \multd{}, \bistrdna)$ on $\catset$.  For every set $E$, $\td
E$ is the set of all continuous valuations on $E$ equipped with the discrete
topology; such a continuous valuation $\nu$ is entirely determined by the values
$\nu \{x\}$, $x\in E$, since then for every $X \subseteq E$, $\nu (X)$ must equal $\sum_{x\in X} \nu
\{x\}$.  This implies that $\nu$ has countable support, and is a countable linear
combination $\sum_{x \in E} a_x \delta_x$ of Dirac valuations; such valuations are
called {\em discrete\/} in \cite{JGL:val:ext}.  The unit $\unitd E$ maps $x \in
E$ to $\delta_x$, multiplication simplifies to $\multd E (\sum_{\xi \in \td X} a_{\xi}
\delta_{\xi}) = \sum_{\xi \in \td X} a_{\xi} \xi$.  The mediator $\bistrd E F$ maps $(\sum_{x \in X}
a_x \delta_x, \sum_{y \in Y} b_y \delta_y)$ to $\sum_{x \in X, y \in Y} a_x b_y \delta_{(x, y)}$; the
induced strength $\strd E F$ maps $(x, \sum_{y \in Y} b_y \delta_y)$ to $\sum_{y \in Y} b_y
\delta_{(x, y)}$.  Finally, the monad morphism maps the discrete valuation $\nu \in \td
\funbara A$ to $\nu$ seen as a continuous valuation in $\funbara {\tc A}$.

In the binary relation case, take $\catc = \catc_1 \times \catc_2$, where
$\catc_1 = \catc_2 = \Dcpo$.  $\catc$ is cartesian closed, with all products
and exponentials taken componentwise.  Also, there is a monoidal monad $(\tc
\times \tc, (\unitc{}, \unitc{}), (\multc{}, \multc{}), (\bistrcna,
\bistrcna))$, given componentwise, on $\catc$.  The product functor from
$\catc$ to $\catc_1$ has the diagonal functor as left adjoint.  Composing this
adjunction with the adjunction $\discr \dashv \funbar$ above yields a monoidal
adjunction again, so that Proposition~\ref{prop:adj:distr:2} applies. This
yields a slightly different monoidal monad $\td'$ on $\catset$, where $\td' A
= \td A \times \td A$; it is easily seen to be isomorphic to $\td$.


Whatever route we take, letting $\funbar$ be the product functor and $\dist
{A_1, A_2}$ map $\nu \in \td (\funbara {A_1} \times \funbara {A_2})$ to
$(\pmb{\nu}_1, \pmb{\nu}_2) \in \funbara {\tc {A_1}} \times \funbara {\tc {A_2}}$, 
where
$\pmb{\nu}_i = \td \pi_i \nu$ ($i=1, 2$) yields a monad morphism from $\tc \times \tc$
to $\td$.

As before, we take injections as pseudoepis and surjections as relevant monos;
$\td{}$ preserves pseudoepis, because every functor does so in $\catset$.

Let us spell out the resulting construction: for any relation $S \subseteq
\funbara {A_1} \times \funbara {A_2}$, let $\pair{\projrel_1}{\projrel_2}$ 
be the inclusion $\xymatrix@-5pt{S \arrmonoxy[r] & \funbara {A_1}
  \times \funbara {A_2}}$, then the diagram defining the lifting of the monad
is:
\[
\xymatrix{
  {\td S}
%  \ar[rrrd]^{\pair \funbara {\tc {\discr (\projrel_1)}}, \funbara
%    {\tc {\discr (\projrel_2)}} \pair}
  \ar[rrr]^{\td \pair{\projrel_1}{\projrel_2}}
  \ar@{=}[d]
  &&&
  {\td (\funbara  {A_1} \times \funbara {A_2})}
  \ar@{=}[d] 
  &
  \\
  {\funbara {\tc {\discr S}}} 
  \ar[rrr]^{\funbara {\tc {\discr \pair{\projrel_1}{\projrel_2}}}}
  \arrepixy[d]
  \ar[rrrd]_(.4){f}
  &&&
  {\funbara {\tc {\discr (\funbara {A_1} \times \funbara {A_2})}}}
  \ar[d]|{\pair{\funbara{\tc \discr \pi_1}}{\funbara{\tc \discr \pi_2}}}
  \ar[rd]^{\dist {A_1, A_2}}
  &
  \\
  {\lift S}
  \arrmonoxy[rrr]^(.3)m
  &&&
  {\funbara {\tc {\discr \funbara{A_1}}}} \times {\funbara {\tc {\discr \funbara{A_2}}}} 
  \arrmonoxy[r]
  &
  {\funbara {\tc A_1} \times \funbara {\tc A_2}}
  }
\]
The inclusion arrow that ends in the bottom-right corner, corresponds to the
fact that any discrete valuation $\nu_i \in \funbara{ \tc \discr \funbara{A_i}}$
can be seen as a continuous valuation in $A_i$, i.e., an element of $\funbara
{\tc A_i}$, for $i = 1,2$.

So $\lift S$ is the range of the function $f = \pair{\funbara{\tc \discr
    \pi_1}}{\funbara{\tc \discr \pi_2}} \circ {\funbara {\tc {\discr
      \pair{\projrel_1}{\projrel_2}}}}$. Now $\funbara{\tc {\discr
    \pair{\projrel_1}{\projrel_2}}}$ maps every discrete valuation $\nu$ on
$\discr S$ to a discrete valuation $\nu'$ on $\discr (\funbara {A_1} \times \funbara
{A_2})$ mapping any subset $X$ of $\funbara {A_1} \times \funbara {A_2}$ to $\nu(X \cap
S)$.  Further, $\funbara{\tc \discr \pi_1}$ maps a discrete valuation $\nu'$ on
$\discr (\funbara {A_1} \times \funbara {A_2})$ to a discrete valuation $\pmb{\nu}_1$
on $\discr \funbara{A_1}$ that maps the subset $O_1$ of $A_1$ to $\nu'(O_1 \times
A_2)$. Similarly, $\funbara{\tc \discr \pi_2}$ maps a discrete valuation $\nu'$ on
$\discr (\funbara {A_1} \times \funbara {A_2})$ to a discrete valuation $\pmb{\nu}_2$
on $\discr \funbara{A_2}$ that maps the subset $O_2$ of $A_2$ to $\nu'(A_1 \times
O_2)$. Therefore $f$ maps $\nu \in \td S$ to $(\pmb{\nu}_1, \pmb{\nu}_2)$ such that
for every subset $O_1$ of $A_1$, $\pmb{\nu}_1 (O_1) = \nu ((O_1 \times \funbara{A_2}) \cap
S)$, and for every subset $O_2$ of $A_2$, $\pmb{\nu}_2 (O_2) = \nu ((\funbara{A_1}
\times O_2) \cap S)$.

As $\lift S$ is the range of this function $f$, the lifted relation $\lift S$
between continuous valuations $\pmb{\nu}_1 \in \funbara {\tc {A_1}}$ and
$\pmb{\nu}_2 \in \funbara {\tc {A_2}}$ is given by: {\small
  \begin{eqnarray*}
    (\pmb{\nu}_1, \pmb{\nu}_2) \in \lift S & \iff & \bigg(\exists \nu \in \td S .
    \left\{
      \begin{array}{l}
        \forall O_1 \subseteq A_1 %\mbox{ open}
        . \pmb{\nu}_1 (O_1) = \nu ((O_1 \times
        A_2) \cap S)\ \land \\
        \forall O_2 \subseteq A_2 %\mbox{ open}
        . \pmb{\nu}_2 (O_2) = \nu ((A_1 \times
        O_2) \cap S)
      \end{array}
    \right.\bigg)
  \end{eqnarray*}
  }



\comment{

left as a copy, before substantial modifications were introduced
SL, 29.11.2003


Whatever route we take, letting $\funbar$ be the product functor and $\dist
{A_1, A_2}$ map $\nu \in \td (\funbara {A_1} \times \funbara {A_2})$ to
$(\nu_1, \nu_2) \in \funbara {\tc {A_1}} \times \funbara {\tc {A_2}}$, where
$\nu_i = \td \pi_i$ ($i=1, 2$) yields a monad morphism from $\tc \times \tc$
to $\td$.

As before, we take injections as pseudoepis and surjections as relevant monos;
$\td{}$ preserves pseudoepis, because every functor does so in $\catset$.

Let us spell out the resulting construction: for any relation $S \subseteq
\funbara {A_1} \times \funbara {A_2}$, let $\langle \projrel_1, \projrel_2
\rangle$ be the inclusion $\xymatrix@-5pt{S \arrmonoxy[r] & \funbara {A_1}
  \times \funbara {A_2}}$, then the diagram defining the lifting of the monad
is:
\[
\xymatrix{
  {\td S}
  \ar[rrr]^{\left\langle \funbara {\tc {\discr (\projrel_1)}}, \funbara
    {\tc {\discr (\projrel_2)}} \right\rangle}
  \arrepixy[d]
  &&&
  {\td {\funbara  {A_1} \times \funbara {A_2}}}
  \ar@{=}[r]
  &
  {\funbara {\tc {\discr \funbara {A_1}}}
    \times \funbara {\tc {\discr \funbara {A_2}}}}
  \ar[d]^{\dist {A_1, A_2}}
                                %^{\funbara {\tc {\counita_{A_1}}} \times \funbara {\tc {\counita_{A_2}}}}
  \\
  {\lift S}
  \arrmonoxy[rrrr]^m
  &&&
%  \funbara {\tc {(A_1, A_2)}}
%  \ar@{=}[r]
  &
  {\funbara {\tc A_1} \times \funbara {\tc A_2}}
  }
\]
So $\lift S$ is the range of the function $f = \dist {A_1, A_2} \circ \langle
\funbara {\tc {\discr (\projrel_1)}}, \funbara {\tc {\discr (\projrel_2)}}
\rangle$.  Now $\funbara {\tc {\discr (\projrel_1)}}$ maps every $\nu \in \td
S$ to the continuous valuation $\nu_1$ on $\discr \funbara {A_1}$ mapping any
subset $X_1$ of $A_1$ to $\nu_1 (X_1) = \nu (\projrel_1^{-1} (X_1)) = \nu
((X_1 \times A_2) \cap S)$.  Similarly, $\funbara {\tc {\discr (\projrel_2)}}$
maps $\nu$ to $\nu_2$ defined by $\nu_2 (X_2) = \nu ((A_1 \times X_2) \cap
S)$.  On the other hand, $\dist {A_1, A_2}$ maps $(\nu_1, \nu_2)$ to the pair
$(\pmb{\nu}_1, \pmb{\nu}_2)$ of continuous valuations on $A_1$, resp.\ $A_2$,
that map the open $O_1$ of $A_1$, resp.\ $O_2$ of $A_2$, to $\nu_1 (O_1)$,
resp.\ $\nu_2 (O_2)$.  Therefore $f$ maps $\nu \in \td S$ to $(\pmb{\nu}_1,
\pmb{\nu}_2)$ such that for every open $O_1$ of $A_1$, $\pmb{\nu}_1 (O_1) =
\nu ((O_1 \times A_2) \cap S)$, and for every open $O_2$ of $A_2$,
$\pmb{\nu}_2 (O_2) = \nu ((A_1 \times O_2) \cap S)$.

As $\lift S$ is the range of this function $f$, the lifted relation $\lift S$
between continuous valuations $\pmb{\nu}_1 \in \funbara {\tc {A_1}}$ and
$\pmb{\nu}_2 \in \funbara {\tc {A_2}}$ is given by: {\small
  \begin{eqnarray*}
    (\pmb{\nu}_1, \pmb{\nu}_2) \in \lift S & \iff & \bigg(\exists \nu \in \td S .
    \left\{
      \begin{array}{l}
        \forall O_1 \subseteq A_1\mbox{ open} . \pmb{\nu}_1 (O_1) = \nu ((O_1 \times
        A_2) \cap S)\ \land \\
        \forall O_2 \subseteq A_2\mbox{ open} . \pmb{\nu}_2 (O_2) = \nu ((A_1 \times
        O_2) \cap S)
      \end{array}
    \right.\bigg)
  \end{eqnarray*}
  }


end of a copy

}


\subsubsection{Probabilistic Transition Systems.}
Interestingly, and analogously with Section~\ref{sec:lts}, we may define a
{\em probabilistic\/} labelled transition system as an element of ${(\tc
  A)}^{A \times L}$.  Then two such transition systems $f_1$ and $f_2$ are in
relation if and only if: {\small
  \begin{eqnarray}
    \label{eq:proba:bisim}
    \forall a_1 \in \funbara {A_1}, a_2 \in \funbara {A_2}
    & , & \ell_1, \ell_2 \in L . (a_1, a_2) \in S
    \land (\ell_1, \ell_2) \in R_L \Rightarrow \\
    \nonumber
    \bigg(\exists \nu \in \td S & . & \left\{
      \begin{array}{l}
        \forall O_1 \subseteq A_1 %\mbox{ open}
        . f_1 (a_1, \ell) (O_1) = \nu ((O_1 \times
        A_2) \cap S)\ \land \\
        \forall O_2 \subseteq A_2 %\mbox{ open}
        . f_2 (a_2, \ell) (O_2) = \nu ((A_1 \times
        O_2) \cap S)
      \end{array}
    \right.\bigg)
  \end{eqnarray}
  }

Note that this all works with the monad of probability valuations (where the
measure of whole spaces must be $1$), or of subprobability evaluations (where
the measure of whole spaces must be at most $1$), for example.

Look at the special case of finite sets $A_1$, $A_2$ seen as discrete dcpos,
and with discrete probability distributions,
% (in particular, every set is measurable),
and the relation on labels $R_L$ is equality.  View the disjoint union
$A_1+A_2$ as the state space of a unique combined probabilistic transition
system.  Write $p_\ell (a, a')$ the probability of the transition $a
{\buildrel \ell \over\longrightarrow} a'$: this is $f_1 (a, \ell) (\{a'\})$ if
$a, a' \in A_1$, $f_2 (a, \ell) (\{a'\})$ if $a, a' \in A_2$, zero otherwise.
Let $\equiv$ be the smallest equivalence relation on $A_1+A_2$ containing $S$.
For every $C \in (A_1+A_2)/\equiv$: {\small
  \begin{equation}
    \label{eq:A1A2}
    ((C \cap A_1) \times A_2) \cap S = (A_1 \times (C \cap A_2)) \cap S
  \end{equation}
  }
Indeed, the inclusion of the left-hand side in the right-hand side means that
for every $a_1 \in C \cap A_1$ and for every $a_2 \in A_2$ such that $(a_1,
a_2) \in S$, then $a_2$ is in $C$. The converse inclusion means that for every
$a_2 \in C \cap a_2$ and every $a_1 \in A_1$ such that $(a_1, a_2) \in S$ then
$a_1 \in C$.  Both inclusions hold because in each case $a_1\equiv a_2$ and
$C$ is an equivalence class for $\equiv$.  So, if (\ref{eq:proba:bisim})
holds, letting $\pmb{\nu}_i$ be $f_i (a_i, \ell)$, $O_1 = C \cap A_1$, $O_2 =
C \cap A_2$, then $\pmb{\nu}_1 (C \cap A_1) = \pmb{\nu}_2 (C \cap A_2)$. Since
$\pmb{\nu}_i (C \cap A_i) = \sum_{a \in C} p_\ell (a_i, a)$,
(\ref{eq:proba:bisim}) implies:
 {\small
  \begin{eqnarray}
    \label{eq:LS:1}
    \forall a_1, a_2 \in A_1 + A_2 . (a_1, a_2) \in S & \Rightarrow &
    \forall \ell \in L . \forall C \in (A_1+A_2)/\equiv . \\
    \nonumber
    && \sum_{a \in C} p_\ell (a_1, a) = \sum_{a \in C} p_\ell (a_2, a)
  \end{eqnarray}
  }
Since $\equiv$ is the reflexive symmetric transitive closure of $S$,
iterating (\ref{eq:LS:1}) entails:
 {\small
  \begin{eqnarray}
    \label{eq:LS}
    \forall a_1 \in A_1, a_2 \in A_2 . a_1 \equiv a_2 & \Rightarrow &
    \forall \ell \in L . \forall C \in (A_1+A_2)/\equiv . \\
    \nonumber
    && \sum_{a \in C} p_\ell (a_1, a) = \sum_{a \in C} p_\ell (a_2, a)
  \end{eqnarray}
  } This is exactly Larsen and Skou's condition that $\equiv$ be a {\em
  probabilistic bisimulation\/} \cite{LS:proba}.

Conversely, (\ref{eq:LS}), i.e., that $\pmb{\nu}_1 (C \cap A_1) = \pmb{\nu}_2
(C \cap A_2)$ for every equivalence class $C$ of $\equiv$ where $\pmb{\nu}_1$
and $\pmb{\nu}_2$ are defined as above, implies (\ref{eq:proba:bisim}) in case
$S$ is an equivalence relation already ($S = {\equiv}$): take $\nu (\{(a'_1,
a'_2)\}) = \pmb{\nu}_1 (\{a'_1\}) \times \pmb{\nu}_2 (\{a'_2\}) / \pmb{\nu}_1
(C \cap A_1) = \pmb{\nu}_1 (\{a'_1\}) \times \pmb{\nu}_2 (\{a'_2\}) /
\pmb{\nu}_2 (C \cap A_2)$ if $a'_1 \equiv a'_2$, where $C$ is the equivalence
class of $a'_1$ and $a'_2$, and provided $\pmb{\nu}_1 (C \cap A_1) =
\pmb{\nu}_2 (C \cap A_2) \neq 0$; zero otherwise. Indeed, first observe that
this is a probability distribution: $\sum_{a'_1 \in A_1, a'_2 \in A_2} \nu
(\{(a'_1, a'_2)\}) = \sum_C \sum_{a'_1 \in C \cap A_1} \sum_{a'_2 \in C \cap
  A_2} \pmb{\nu}_1 (\{a'_1\}) \times \pmb{\nu}_2 (\{a'_2\}) / \pmb{\nu}_2 (C
\cap A_2)) = \sum_C \sum_{a'_1 \in C \cap A_1} \pmb{\nu}_1 (\{a'_1\}) = \sum_C
\pmb{\nu}_1 (C \cap A_1) = 1$.

Second, $\nu ((\{a'_1\} \times A_2) \cap S) = \sum_{a'_2 / a'_1 \equiv a'_2}
\nu (\{a'_1, a'_2\}) = \sum_{a'_2 \in C \cap A_2} \nu (\{a'_1, a'_2\})$ (where
$C$ is the equivalence class of $a'_1$) $= \sum_{a'_2 \in C \cap A_2}
\pmb{\nu}_1 (\{a'_1\}) \times \pmb{\nu}_2 (\{a'_2\}) / \pmb{\nu}_2 (C \cap
A_2) = \pmb{\nu}_1 (\{a'_1\})$. Summing over all $a'_1 \in O_1$, where $O_1
\subseteq A_1$, we obtain $\nu ((O_1 \times A_2) \cap S) = \pmb{\nu}_1 (O_1)$.
Symmetrically, $\nu ((A_1 \times O_2) \cap S) = \pmb{\nu}_2 (O_2)$, and this
is exactly condition~(\ref{eq:proba:bisim}). Recall that $\pmb{\nu}_i = f_i
(a_i, \ell)$.

So the two notions are equivalent, in the discrete case: relations $S$ as
described by our subscone construction have probabilistic bisimulations as
reflexive symmetric transitive closures, and probabilistic bisimulations are
equivalence relations $S$ as described by our construction---in the discrete
probability case.




\subsection{Continuous Valuations on Dcpos, observed from $\Dcpo$}
\label{sec:proba:dcpo}

The construction of the previous section is somewhat limited, since the only
valuations in $\td S$ are discrete.  In particular, and this can be seen on
condition~(\ref{eq:proba:bisim}), the only transition systems that can be
related by the construction of the previous section are themselves discrete
transition systems.

In the case of continuous transition systems, a more expressive construction
must be sought.  Here we take $\catd = \Dcpo$.  Our first concern is to define
a relevant mono factorization system on $\Dcpo$.
%There are several mono factorization systems on $\pmb{Cpo}$.  As in any
%category, there is the trivial one, where all morphisms are pseudoepis and the
%relevant monos are exactly the isos; this is rather uninteresting.
%
%List others!
%
One that works here is as follows.  First, for every dcpo $A$ and every $X
\subseteq A$, the {\em sup-closure\/} $\overline X$ of $X$ in $A$ is the
smallest sup-closed subset of $A$ containing $X$ (i.e., the smallest sub-dcpo
of $A$ containing $X$).  Note two pitfalls here: first, $\overline X$ is in
general not just the set of sups in $A$ of directed subsets of $X$, and the
process of taking sups may have to be iterated transfinitely; second, the
sup-closure is in general much smaller than the Scott-topological closure of
$X$ in $A$, which is $\downarrow \overline X$. Now $e : \xymatrix@-5pt{A
  \arrepixy[r] & C}$ is a pseudoepi if and only if $\overline {e (A)} = C$,
i.e., every element in $C$ is in the sup-closure of the range of $e$.  And $m
: \xymatrix@-5pt{C \arrmonoxy[r] & B}$ is a relevant mono if and only if $m$
is a {\em dcpo embedding}, meaning a Scott-continuous function such that $m
(x) \leq m (y)$ if and only if $x \leq y$.  If this is the case, then the
range $m (C)$ of $m$ is a dcpo, $m$ is injective, and the inverse $m^{-1} : m
(C) \to C$ is continuous.  This yields a mono factorization, even an epi-mono
factorization on $\Dcpo$, as can be checked easily.  In fact what we called
pseudoepis are just the epis in $\Dcpo$, and the relevant monos are exactly
the {\em extremal monos}; the latter correspond exactly to sub-dcpos up to
iso.

It is tempting to define the monad $\td{}$ just as $\tc{}$, since the
categories $\catc$ and $\catd$ are the same.  However, condition~{\bf (iv)}
would be problematic.  Indeed, we have not been able to show that $\tc$
preserved pseudoepis in $\Dcpo$; we conjecture that it does not, although we
have been unable to find any counterexample.  Moreover, the structure of
relevant pseudoepis seems intricate, and showing that $\tc$ maps relevant
pseudoepis to pseudoepis seems arduous, too.

Let us discuss this a bit more. Following Jones \cite{Jones:proba}, call a
valuation {\em simple\/} if and only if it is a finite linear combination
$\sum_{i=1}^n a_i \delta_{x_i}$ of Dirac valuations.  Call a valuation {\em
  quasi-simple\/} if and only if it is a sup of a directed family of simple
valuations, and {\em accessible\/} if and only if it is in the sup-closure of
the set of all simple valuations.  Every discrete valuation is quasi-simple,
and every quasi-simple valuation is accessible, but converses do not hold in
general \cite{JGL:val:ext}.  Now it seems likely that there should be a dcpo
$A$ on which some continuous valuation $\pmb{\nu}$ is not in the sup-closure of
the set of simple valuations, i.e., containing a continuous, but not
accessible valuation.  We have no example of this, but Alvarez-Manilla
\cite[Section~2.7, p.73]{AM:PhD} shows an example of a dcpo and a continuous
valuation on it that is not quasi-simple, which comes close; also, all
accessible valuations are point-continuous valuations since the space of
point-continuous valuations forms a dcpo containing all simple valuations
\cite{Heckmann:space:val}.  So any dcpo on which there is a continuous, but
not point-continuous valuation $\pmb{\nu}$ would yield an example of a
continuous valuation $\pmb{\nu}$ that is not accessible.  In any case, if $A$
and $\pmb{\nu}$ exist so that $\pmb{\nu}$ is continuous but not accessible, then
let $B$ be the dcpo have the same underlying set as $A$ but with equality as
ordering, and let $i : B \to A$ the continuous function mapping $x \in B$ to $x\in
A$. Clearly $i$ is surjective, hence pseudoepi.  On the other hand, every
continuous valuation on the discrete space $B$ is discrete
\cite[Proposition~3]{JGL:val:ext}, and the image $\sum_{x \in B} a_x \delta_{i (x)}$ of
any discrete valuation $\sum_{x \in B} a_x \delta_x$ by $\td i$ is again discrete, so
$\pmb{\nu}$ cannot be in the sup-closure of the range of $\td i$, showing that
$\td i$ is not pseudoepi.


Instead of defining $\td A$ as the dcpo of all continuous valuations on $A$,
we let $\td A$ be the dcpo of all accessible valuations on $A$.  Note that by
Theorem~5.2 of \cite{Jones:proba}, if $A$ is a {\em continuous\/} dcpo, every
continuous valuation on $A$ is quasi-simple, in particular accessible.  So
there would be no difference between $\td A$ and $\tc A$ if we restricted
ourselves to a category of continuous dcpos.  Moreover, if $A$ is a continuous
dcpo, so is $\tc A$ \cite[Corollary~5.4]{Jones:proba}.  Unfortunately, no
cartesian-closed subcategory of $\Dcpo$ is known that consists only of
continuous dcpos and to which the monad $\tc$ has a restriction
\cite{Jung:prob}.

All this forces us to be content with accessible valuations.  We start with a
few required technical lemmas.  Recall that $\overline X$ denotes the
sup-closure of $X$.
\begin{lemma}
  \label{lemma:supclos}
  Let $X$ be any subset of the dcpo $A$.  Every sup of a directed family of
  elements of the sup-closure $\overline X$ is in $\overline X$.
\end{lemma}
\begin{proof}
  Obvious.
\end{proof}
\begin{corollary}
  \label{corl:supclos}
  Every sup of a directed family of accessible valuations is accessible.
\end{corollary}

\begin{lemma}
  \label{lemma:supclos:val}
  Let $X$ be any subset of $\tc A$ that is closed under linear combinations,
  i.e., such that whenever $\nu_1, \ldots, \nu_n \in X$, and $a_1, \ldots, a_n
  \in \real_+$, then $\sum_{i=1}^n a_i \nu_i \in X$.  Then $\overline X$ is
  closed under linear combinations.
\end{lemma}
\begin{proof}
  Define $\overline X_\alpha$ for each ordinal $\alpha$ by $\overline X_0 =
  X$, and if $\alpha\neq 0$ then $\overline X_\alpha$ is the set of all sups
  of directed families ${(\nu_i)}_{i\in I}$ of continuous valuations $\nu_i
  \in \overline X_{\alpha_i}$, $\alpha_i < \alpha$.  Clearly $\overline X =
  \bigcup_\alpha \overline X_\alpha$.
  
  We first claim that if $\nu$ is in $\overline X_\alpha$ then $a\nu$ is in
  $\overline X_\alpha$, by induction on $\alpha$.  If $\alpha=0$, then by
  assumption $a\nu \in X = \overline X_0$.  Otherwise, $\nu = \sup_{i\in I}
  \nu_i$ for some directed family ${(\nu_i)}_{i\in I}$ of valuations in
  $\overline X_{\alpha_i}$.  Then the family ${(a\nu_i)}_{i \in I}$ is also
  directed, $a\nu_i$ is in $\overline X_{\alpha_i}$ by induction hypothesis,
  and $a\nu = \sup_{i\in I} a\nu_i$.
  
  We then claim that if $\nu$ is in $\overline X_\alpha$ and $\nu'$ is in
  $\overline X_{\alpha'}$, then $\nu+\nu'$ is in $\overline X$.  This is by
  induction on $\alpha, \alpha'$ ordered lexicographically.  If
  $\alpha=\alpha' = 0$, then both $\nu$ and $\nu'$ are in $X$, hence
  $\nu+\nu'$ is in $X$ by assumption, therefore in $\overline X$.  If
  $\alpha'\neq 0$, then $\nu'$ is the sup of some directed family
  ${(\nu'_j)}_{j\in J}$ of valuations in $\overline X_{\alpha'_j}$, $\alpha'_j
  < \alpha'$.  By induction hypothesis $\nu+\nu'_j$ is in $\overline X$; the
  family ${(\nu+\nu'_j)}_{j\in J}$ is clearly directed, and $\sup_{j\in J}
  \nu+\nu'_j = \nu+\nu'$, so $\nu+\nu'$ is in $\overline X$.  If $\alpha\neq
  0$, then $\nu$ is the sup of some directed family ${(\nu_i)}_{i\in I}$ of
  valuations in $\overline X_{\alpha_i}$, $\alpha_i < \alpha$.  By induction
  hypothesis, $\nu_i + \nu'$ is in $\overline X$, so similarly $\nu+\nu'$ is
  in $\overline X$.
\end{proof}

\begin{corollary}
  \label{corl:acc:val}
  Every finite linear combination of accessible valuations is accessible.
\end{corollary}
\begin{proof}
  Take $X$ the set of simple valuations on $A$.
\end{proof}
In the sequel, call a valuation {\em $\alpha$-accessible\/} if and only if it
is in $\overline X_\alpha$ where $X$ is the set of simple valuations.  In
other words, the $0$-accessible valuations are the simple valuations; if
${(\nu_i)}_{i\in I}$ is a directed family of valuations, where $\nu_i$ is
$\alpha_i$-accessible for some $\alpha_i < \alpha$, then $\sup_{i\in I} \nu_i$
is $\alpha$-accessible.  The accessible valuations are those that are
$\alpha$-accessible for some ordinal $\alpha$.

Define $\unitd A$ as mapping $x \in A$ to $\delta_x$ in $\td A$.  This is
clearly natural in $A$.  Define $\multd A$ as mapping every accessible
valuation $\nu$ on $A$ to the continuous valuation $\int_{\xi \in \td A} \xi
(O) d\nu$.
\begin{lemma}
  \label{lemma:multd:acc}
  For every accessible valuation $\nu$, $\multd A (\nu)$ is an accessible
  valuation.
\end{lemma}
\begin{proof}
  We show that $\multd A (\nu)$ is accessible whenever $\nu$ is
  $\alpha$-accessible, by induction on $\alpha$.  If $\alpha = 0$, then $\nu$
  is simple, that is, $\nu$ is of the form $\sum_{i=1}^n a_i \delta_{\xi_i}$.
  Then $\multd A (\nu) = \sum_{i=1}^n a_i \xi_i$, which is accessible by
  Corollary~\ref{corl:acc:val}.  If $\alpha\neq 0$, then $\nu$ is the directed
  sup of a family of $\alpha_i$-accessible valuations $\nu_i$, $\alpha_i <
  \alpha$.  Since integration is continuous in its valuation argument, $\multd
  A (\nu) = \sup_{i\in I} \multd A (\nu_i)$, hence is accessible again by
  Corollary~\ref{corl:supclos}.
\end{proof}
So $\multd A$ is a map from $\td^2 A$ to $\td A$.  It is also continuous,
since integration is continuous in its function argument, and the map $\xi \mapsto \xi
(O)$ is Scott-continuous for every open $O$.  Moreover, $\multd A$ is natural
in $A$: if $f$ is continuous from $A$ to $B$, then $\multd B (\td^2 f (\nu)) (O)
= \int_{\eta \in \td B} \eta (O) d \td^2 f (\nu) = \int_{\xi \in \td A} \td f (\xi) (O) d\nu$ (using
the Change of Variables formula) \allowbreak $= \int_{\xi \in \td A} \xi (f^{-1} (O))
d\nu$ (by definition of $\td f$) $= \multd A (\nu) (f^{-1} (O)) = \td f (\multd A
(\nu)) (O)$ (by definition of $\td f$).

We define $\bistrd A B$ as mapping $\nu \in \td A$ and $\xi \in \td B$ to the
continuous valuation $\nu \otimes \xi$ that takes the open subset of the dcpo
$A \times B$ to $\int_{x\in A} \left(\int_{y\in B} \chi_O (x,y) d\xi\right)
d\nu$.
\begin{lemma}
  \label{lemma:bistrd:acc}
  For every accessible valuations $\nu$ and $\xi$, $\nu \otimes \xi$ is an
  accessible valuation.
\end{lemma}
\begin{proof}
  We show the claim under the assumption that $\nu$ is $\alpha$-accessible and
  $\xi$ is $\alpha'$-accessible, by induction on $\alpha, \alpha'$ ordered
  lexicographically.  If $\alpha = \alpha' = 0$, then $\nu$ and $\xi$ are
  simple, say $\nu = \sum_{i=1}^m a_i \delta_{x_i}$ and $\xi = \sum_{j=1}^n
  b_j \delta_{y_j}$, so $\nu \otimes \xi = \sum_{i=1}^m \sum_{j=1}^n a_i b_j
  \delta_{(x_i, y_j)}$ is simple, hence accessible.  If $\alpha'\neq 0$, then
  $\xi$ is the sup of some directed family ${(\xi_j)}_{j\in J}$ of
  $\alpha'_j$-accessible valuations, $\alpha'_j < \alpha'$.  Since integration
  is continuous, $\bistrd A B (\nu, \xi) (O) = \sup_{j \in J} \bistrd A B
  (\nu, \xi_j) (O)$, where $\bistrd A B (\nu, \xi_j)$ is accessible by
  induction hypothesis; so $\bistrd A B (\nu, \xi)$ is accessible.  By a
  similar argument, $\bistrd A B (\nu, \xi)$ is accessible when $\alpha\neq
  0$.
\end{proof}
Clearly $\bistrd A B$ is continuous, since $\bistrc A B$ is, and the two
coincide on accessible valuations.  Also, $\bistrd A B$ is natural in $A$ and
$B$: if $f$ is a continuous map from $A$ to $A'$ and $g$ is a continuous map
from $B$ to $B'$, $\bistrd {A'} {B'} (\td f (\nu), \td g (\xi)) (O) = \int_{x'\in A'}
\int_{y'\in B'} \chi_O (x', y') d\td g (\xi) d\td f (\nu) = \int_{x\in A} \int_{y\in B} \chi_O (f (x),
g (y)) d\xi d\nu$ (using the Change of Variables formula).  This is equal to
$\int_{x\in A} \int_{y\in B} \chi_{{(f \times g)}^{-1} (O)} (x, y) d\xi d\nu = \bistrd A B (\nu, \xi)
((f \times g)^{-1} (O)) = \td (f \times g) (\bistrd A B (\nu, \xi))$.

All this leads to:
\begin{lemma}
  \label{lemma:td:proba}
  $(\td, \unitd {}, \multd{}, \bistrdna)$ is a monoidal monad on $\Dcpo$, the
  {\em accessible valuation monad}.  Letting $\funbar$ be the identity
  endofunctor on $\Dcpo$, and $\dist A : \td \funbara A \to \funbara {\tc A}$
  map every accessible valuation $\nu$ on $A$ to itself, seen as a continuous
  valuation on $A$, $(\funbar, \dist{})$ is a monoidal monad morphism from
  $\tc$ to $\td$.
\end{lemma}
\begin{proof}
  It remains to show that $(\funbar, \dist{})$ is a monoidal monad morphism.
  But since both $\funbar$ and $\dist{}$ are identities,
  Diagrams~(\ref{d_distlaw}) and~(\ref{d_distbistr}) are obvious.  (Note that
  the mediating pair $(\tstrna, \tstri)$ of $\funbar$ consists of identities
  exclusively.)
\end{proof}


%equipped with its Scott topology, we use the following construction.  Let
%$\leq$ be the ordering of the dcpo $A$, and build the {\em Alexandroff
%  topology\/} on $\leq$: the Alexandroff opens are all upward-closed subsets
%of $A$.  This is finer than the Scott topology on $A$.  Now let $\td A$ be the
%set of all continuous valuations on $A$ equipped with its Alexandroff
%topology.  With the ordering given by $\nu \leq \xi$ if and only if $\nu (O)
%\leq \xi (O)$ for every Alexandroff open $O$ of $A$, $\td A$ is again a dcpo.
%Let again $\unitd A$ map $x_0 \in A$ to the Dirac valuation $\delta_{x_0}$.  This is
%Scott continuous: if ${(x_i)}_{i \in I}$ is any directed family in $A$, then
%$\sup_{i \in I} \delta_{x_i} (O)$ equals one if and only if $x_i \in O$ for
%some $i \in I$.

So conditions~{\bf (i.c)}, {\bf (ii.a)} hold.  (In fact even condition {\bf
  (ii.b)}.) Condition {\bf (iii.a)} holds, too: our mono factorization system
on $\Dcpo$ is monoidal, since for every two pseudoepis $f$ and $g$, $f \times
g$ is pseudoepi, for sups are taken componentwise. As we said earlier, the
main difficulty with probabilistic powerdomains is in showing that
condition~{\bf (iv)} holds:
\begin{lemma}
  \label{lemma:proba:iv}
  If $f : A \to B$ is pseudoepi in $\Dcpo$, then so is $\td f$.
\end{lemma}
\begin{proof}
  Let $X$ be the set of valuations of the form $\sum_{i=1}^m a_i \delta_{f
    (x_i)}$, where $m\in \nat$, $a_i \in \real_+$, $x_i \in A$.  Observe that
  $\sum_{i=1}^m a_i \delta_{f (x_i)} = \td f (\sum_{i=1}^m a_i \delta_{x_i})$,
  so $X$ is included in the range of $f$.  We show that every accessible
  valuation $\xi$ on $B$ is in $\overline X$, which will imply that it is in
  the sup-closure of the range of $f$, hence that $\td f$ is pseudoepi.
  
  It suffices to show that every $\alpha$-accessible valuation $\xi$ in $\td
  B$ is in $\overline X$, by induction on $\alpha$.  If $\alpha = 0$, then
  $\xi$ is simple, hence can be written under the form $\sum_{j=1}^n b_j
  \delta_{y_j}$, for some finite family of elements $y_j$ in $B$.  Since $f$
  is pseudoepi, $y_j$ is in the sup-closure of the range of $f$.  Since the
  map $x \mapsto \delta_x$ (i.e., $\unitd A$) is Scott continuous,
  $\delta_{y_j}$ is in the sup-closure of the set of all Dirac maps of the
  form $\delta_{f (x)}$, $x\in A$.  (Note indeed that, for every Scott
  continuous map $g$, $g$ maps the sup-closure of any subset to the
  sup-closure of its direct image.)  So $\delta_{y_j}$ is in $\overline X$,
  therefore $\xi = \sum_{j=1}^n b_j \delta_{y_j}$ is in $\overline X$, too, by
  Lemma~\ref{lemma:supclos:val}.  If $\alpha\neq 0$, then $\nu$ is the sup of
  some directed family ${(\nu_i)}_{i \in I}$ of $\alpha_i$-accessible
  valuations $\nu_i$, $\alpha_i < \alpha$.  By induction hypothesis, $\nu_i$
  is in $\overline X$, so $\nu$ is, too.
\end{proof}

Next, condition~{\bf (v)}, that $\Dcpo$ has pullbacks, holds: if $f$ is a
continuous map from $A$ to $C$, and $g$ is continuous from $B$ to $C$, their
pullback is the set $\{(x, y) \in A \times B | f (x) = g (y)\}$ with the
product ordering.  Finally, we show condition~{\bf (vi)}:
\begin{lemma}
  \label{lemma:cpo:vi}
  For every dcpo $A$, $\ihom A \_$ preserves relevant monos in $\Dcpo$.
\end{lemma}
\begin{proof}
  For every dcpo embedding (relevant mono) $m$ from $B$ to $C$, $\ihom A m$ is
  the continuous map sending every continuous map $f \in \ihom A B$ to $m
  \circ f \in \ihom A C$.  Then $\ihom A m (f) \leq \ihom A m (g)$ if and only
  if $m \circ f \leq m \circ g$, if and only if $m (f (x)) \leq m (g (x))$ for
  every $x \in A$, if and only if $f (x) \leq g (x)$ for every $x\in A$ (since
  $m$ is a dcpo embedding), if and only if $f \leq g$.  Since $\ihom A m$ is
  continuous, it is a a dcpo embedding.
\end{proof}
So all conditions {\bf (i.c)}, {\bf (ii.a)}, {\bf (iii.a)}, {\bf (iv)}, {\bf
  (v)}, {\bf (vi)} necessary to define a notion of subscone in $\Dcpo$ for
Moggi's meta-language are met.  It is fair to call such a subscone a {\em cpo
  logical relation}, extending Plotkin's cpo logical relations for the
(non-monadic) lambda-calculus \cite{Mit96}.

All this yields the following notion of binary logical relation $\Eval \tau$
between dcpos $\Eval \tau_1$ and $\Eval \tau_2$ indexed by types of Moggi's
meta-language, where the interpretations $\Eval \__i$ are defined so that
$\Eval {\tau \to \tau'}_i$ is the dcpo of all continuous functions from $\Eval
\tau_i$ to $\Eval {\tau'}_i$ and $\Eval {\tc \tau}_i = \tc \Eval {\tau}_i$.
Call a binary relation $R$ between partial orders a {\em dcpo relation\/} if
and only if $R$, as a set of pairs, is a dcpo.  The family of dcpo relations
$\Eval \tau$ indexed by types $\tau$ is a {\em dcpo logical relation\/} if and
only if:
\begin{eqnarray*}
  (f_1, f_2) \in \Eval {\tau \to \tau'} & \iff &
  \forall a_1 \in \Eval \tau_1, a_2 \in \Eval \tau_2 \cdot
  \\
  && \quad (a_1, a_2) \in \Eval \tau \Rightarrow (f_1 (a_1), f_2 (a_2)) \in \Eval {\tau'}
  \\
  ((a_1, a'_1), (a_2, a'_2)) \in \Eval {\tau \times \tau'} & \iff &
  (a_1, a_2) \in \Eval {\tau} \land (a'_1, a'_2) \in \Eval {\tau'}
\end{eqnarray*}
and finally $(\pmb{\nu}_1, \pmb{\nu}_2) \in \Eval {\tc \tau}$ if and only if
$(\pmb{\nu}_1, \pmb{\nu}_2)$ is in the sup-closure inside $\tc \Eval \tau_1
\times \tc \Eval \tau_2$ of the set of all pairs of continuous valuations
$(\pmb{\nu}'_1, \pmb{\nu}'_2)$ such that there is an accessible valuation
$\nu$ on the dcpo $\Eval \tau$ with
\[
\left\{
  \begin{array}{l}
    \forall O_1 \mbox{ open of }\Eval \tau_1 \cdot \pmb{\nu}'_1 (O_1) = \nu ((O_1 \times \Eval \tau_2) \cap \Eval \tau) \land \\
    \forall O_2 \mbox{ open of }\Eval \tau_2 \cdot \pmb{\nu}'_2 (O_2) = \nu ((\Eval \tau_1 \times O_2) \cap \Eval \tau)
  \end{array}
\right.
\]
In other words, $\pmb{\nu}_1$ and $\pmb{\nu}_2$ are related provided they are
transfinitely iterated directed sups of valuations $\pmb{\nu}'_1$ and
$\pmb{\nu}'_2$ related by some accessible valuation $\nu$ on $\Eval \tau$ as
in the formula above. (We do not need to mention any sup-closure in the
clauses for $\Eval {\tau \to \tau'}$ and $\Eval {\tau \times \tau'}$ because
the definitions above are already sup-closed.)

This definition is not quite perfect.  First, it is complex.  Second, as shown
above, $\Eval {\tc \tau}$ is only able to relate accessible valuations.  If
there are any dcpos on which not all continuous valuations are accessible,
then $\Eval {\tc \tau}$ will not be reflexive, which is a bit surprising.  We
have not been able to generalize the construction further.  On the other hand,
most dcpos of interest are continuous, and on continuous dcpos every
continuous valuation is quasi-simple, hence accessible.



\subsection{Probability Measures on Metric Spaces}
\label{sec:proba:met}


The standard approach to probability theory is not through valuations, as used
until now, but through measures.  As we said in Section~\ref{sec:proba}, the
category of measurable spaces is ill-suited to this task.  A much
better-behaved category is the category $\Pol$ of Polish spaces and continuous
maps.  A {\em Polish space\/} is the topological space underlying a complete
separable metric space.  (Separable means that the space has a countable dense
subset.)  It was shown by Giry \cite{Giry:proba} that there is a probability
monad $\tc$ on $\Pol$, where $\tc A$ is the set of all probability measures on
the Borel $\sigma$-algebra of $A$, topologized with the {\em weak topology},
that is, the smallest topology making the function $\lambda \pmb{\nu} \in \tc
A \cdot \int_{x\in A} f (x) d\pmb{\nu}$ continuous, for every bounded
continuous function $f$ from $A$ to $\real_+$.

The closest category to $\Pol$ that we know of, and which is symmetric
monoidal closed, is the category $\CMet$ of complete metric spaces, with
non-expansive maps as morphisms.  The separability condition has to be
dropped, which is not preserved by exponentials.  We shall also drop the
completeness requirement, which we simply do not need---the interested reader
may check that the whole construction works directly on complete spaces, too.

So consider the category $\Met$ of metric spaces and non-expansive maps. We
write $d_A$ for the distance on $A$, and allow distances to take the value
$+\infty$.  (This is as in \cite{Lawvere:metric}, who considers additional
relaxations on the notion of distance.)
%
%We take most of the basic material from
%Worrell \cite{Worrell:PhD}.  While Worrell considers Lawvere's asymmetric
%generalization of metric spaces \cite{Lawvere:metric}, we use here a more
%usual, symmetric definition not to disturb the reader.  We write $d_A$ for the
%distance on $A$; we assume that distances may take the value $+\infty$.
%%, and we do not require that $d_A (x, y) = 0$ imply $x=y$, just like Lawvere.
In other words, a distance $d_A$ on $A$ is any function from $A$ to $\real_+
\cup \{+\infty\}$, such that $d_A (x,y) = 0$ if and only if $x=y$, for every
$x,y \in A$; $d_A (x,y) = d_A (y,x)$ for every $x,y\in A$; and $d_A (x,z) \leq
d_A (x,y) + d_A (y,z)$ for every $x,y,z \in A$.  A map $f$ is {\em
  non-expansive\/} from $A$ to $B$ if and only if $d_B (f (x), f (x')) \leq
d_A (x, x')$ for every $x, x' \in A$.
% An {\em isometry\/} is any map that preserves distance.

Every metric space $A$ has a topology, generated by its open balls $\OBall x
\epsilon = \{y | d_A (x, y) < \epsilon\}$, for which it is Hausdorff.  There
is a cartesian product on $\Met$: $A \times B$ is the set of pairs $(x, y)$,
$x \in A$, $y \in B$, with distance $d_{A \times B}$ defined by $d_{A \times
  B} ((x, y), (x', y')) = \max (d_A (x, x'), d_B (y, y'))$.  But $\Met$ is not
cartesian closed, as there is no corresponding notion of exponential.

On the other hand, $\Met$ is symmetric monoidal closed.  The tensor product $A
\tensorc B$ is the set of pairs $(x, y)$, $x \in A$, $y \in B$, with distance
$d_{A \tensorc B}$ defined by $d_{A \tensorc B} ((x, y), (x', y')) = d_A (x,
x') + d_B (y, y')$.  The exponential $\ihom B C$ is the set of non-expansive
maps $f$ from $B$ to $C$, with distance $d_{\ihom B C} (f, f') = \sup_{x \in
  B} d_C (f (x), f' (x))$. (This is well-defined because we allow distances to
take the value $+\infty$.) The underlying topology of $A \tensorc B$, as well
as of $A \times B$, is the product topology of $A$ and $B$.

A {\em measure\/} on $A$ is by convention a measure on the Borel
$\sigma$-algebra of its topology.  A {\em probability\/} measure maps $A$ to
$1$.  A natural choice for the probability monad $\tc$ on $\Met$ is to let
%  An important
%property is that on any complete separable metric space $A$, every measure
%$\pmb{\nu}$ is {\em tight\/} or {\em inner regular\/}, i.e., for every
%measurable subset $X$ of $A$, $\pmb{\nu} (X) = \sup_{K\mathrm{\ compact\ 
%    }\subseteq X} \pmb{\nu} (K)$; alternatively, for every $\epsilon > 0$,
%there is a compact subset $K_\epsilon$ of $A$ such that $\pmb{\nu} (A
%\setminus K_\epsilon) < \epsilon$.
$\tc A$ be the set of all probability measures on $A$, equipped with the {\em
  Hutchinson metric\/}:
\[
d_{\tc A} (\pmb{\nu}, \pmb{\xi}) = \sup_{g \in \homset \Met A {[0, 1]}}
\left|
  \int_{x \in A} g (x) d\pmb{\nu} - \int_{x\in A} g (x) d\pmb{\xi}
\right|
\]
making $\tc A$ a metric space.
%  (The only delicate point is to check that
%$d_{\tc A} (\pmb{\nu}, \pmb{\xi}) = 0$ implies $\pmb{\nu} = \pmb{\xi}$; for
%each closed subset $C$ of $A$, and each $n \in \nat \setminus \{0\}$, consider
%$g (x) = \max (0, 1/n-d_A (x, C))$; by making $n$ tend to $+\infty$,
%$\pmb{\nu} (C) = \pmb{\xi} (C)$; as this holds for each $C$, $\pmb{\nu} =
%\pmb{\xi}$.)
It can be checked that $\tc$ gives rise to a monoidal monad.

%Moreover, if $A$ is complete, then so is $\tc A$; this is Theorem~2.5.25 of
%\cite{Edgar:fractal}.  The topology induced by the Hutchinson metric is
%exactly the weak topology.  (There are other distances inducing the weak
%topology, among which the L\'evy-Prohorov metric.)  It is easy to check that
%for every non-expansive map $f : A \to B$, $\tc f : \tc A \to \tc B$ defined
%by $\tc f (\pmb{\nu}) (X) = \pmb{\nu} (f^{-1} (X))$ is again non-expansive.
%This follows from the Change of Variables formula, which holds for the
%Lebesgue integral just as for the Jones integral.  Therefore $\tc$ is an
%endofunctor on $\Met$, the category of metric spaces and non-expansive maps,
%as well as on $\CMet$.

%The map $x \in A \mapsto \delta_x \in \tc A$, which we call $\unitc A$, is
%also non-expansive, and natural in $A$.  It is less obvious that $\multc A$
%defined as mapping $\pmb{\nu} \in \tc A$ to the probability measure mapping
%every measurable subset $X$ of $A$ to $\int_{\pmb{\xi} \in \tc A} \pmb{\xi}
%(X) d\pmb{\nu}$, is non-expansive.  For every non-expansive map $g$ from $A$
%to $[0, 1]$,
%\begin{eqnarray*}
%  &&
%  \left|
%    \int_{x\in A} g (x) d\multc A (\pmb{\nu}) - \int_{\times\in A} g (x) d\multc A (\pmb{\nu}')
%  \right|
%  \\
%  & = &
%  \left|
%    \int_{\pmb{\xi} \in \tc A} \int_{x\in A}  g (x) d\pmb{\xi} d\pmb{\nu} -
%    \int_{\pmb{\xi} \in \tc A} \int_{x\in A}  g (x) d\pmb{\xi} d\pmb{\nu}'
%  \right|
%\end{eqnarray*}
%by an easy application of the Monotone Convergence Theorem.  Now this is less
%than or equal to $d_{\tc A} (\pmb{\nu}, \pmb{\nu}')$, showing that $\multc A$
%is non-expansive, provided we can show that the map $\pmb{\xi} \mapsto
%\int_{x\in A} g (x) d\pmb{\xi}$ is non-expansive.  And indeed this is so, by
%the very definition of the Hutchinson metric.

%The function $\bistrc A B$ mapping $(\pmb{\nu}, \pmb{\xi})$ to the product
%probability measure $\pmb{\nu} \otimes \pmb{\xi}$
%%probability measure mapping every measurable subset $X$ of $A \tensorc B$ to $\int_{x\in
%%  A} \left(\int_{y\in B} \chi_X (x,y) d\pmb{\xi}\right) d\pmb{\nu}$
%is non-expansive, too.  Indeed, for every non-expansive map $g : \tc (A
%\tensorc B) \to [0, 1]$, we use Fubini's Theorem to derive:
%\begin{eqnarray*}
%  &&
%  \left|
%    \int_{(x, y) \in A \tensorc B} g (x, y) d\bistrc A B (\pmb{\nu}, \pmb{\xi}) -
%    \int_{(x, y) \in A \tensorc B} g (x, y) d\bistrc A B (\pmb{\nu}', \pmb{\xi}')
%  \right|
%  \\
%  & = &
%  \left|
%    \int_{x\in A} \int_{y\in B} g (x, y) d\pmb{\xi} d\pmb{\nu} -
%    \int_{x\in A} \int_{y\in B} g (x, y) d\pmb{\xi}' d\pmb{\nu}'
%  \right|
%  \\
%  & = &
%  \Bigg|
%  \int_{x\in A} \int_{y\in B} g (x, y) d\pmb{\xi} d\pmb{\nu} -
%  \int_{x\in A} \int_{y\in B} g (x, y) d\pmb{\xi} d\pmb{\nu}' +
%  \\
%  &&\qquad 
%  \int_{x\in A} \int_{y\in B} g (x, y) d\pmb{\xi} d\pmb{\nu}' -
%  \int_{x\in A} \int_{y\in B} g (x, y) d\pmb{\xi}' d\pmb{\nu}'
%  \Bigg|
%  \\
%  & = &
%  \Bigg|
%  \int_{x\in A} \int_{y\in B} g (x, y) d\pmb{\xi} d\pmb{\nu} -
%  \int_{x\in A} \int_{y\in B} g (x, y) d\pmb{\xi} d\pmb{\nu}' +
%  \\
%  && \qquad
%  \int_{x\in A} \left(\int_{y\in B} g (x, y) d\pmb{\xi} -
%    \int_{y\in B} g (x, y) d\pmb{\xi}'\right) d\pmb{\nu}'
%  \Bigg|
%  \\
%  & \leq &
%  \left|
%    \int_{x\in A} \int_{y\in B} g (x, y) d\pmb{\xi} d\pmb{\nu} -
%    \int_{x\in A} \int_{y\in B} g (x, y) d\pmb{\xi} d\pmb{\nu}'
%  \right|
%  +
%  \\
%  &&\qquad
%  \left|
%    \int_{x\in A} \left|\int_{y\in B} g (x, y) d\pmb{\xi} -
%      \int_{y\in B} g (x, y) d\pmb{\xi}'\right| d\pmb{\nu}'
%  \right|
%  \\
%  & \leq & d_{\tc A} (\pmb{\nu}, \pmb{\nu'}) + d_{\tc B} (\pmb{\nu}',
%  \pmb{\xi}')
%  = d_{\tc A \tensorc \tc B} ((\pmb{\nu}, \pmb{\xi}), (\pmb{\nu}', \pmb{\xi}'))
%\end{eqnarray*}
%The last line is because $x \mapsto \int_{y\in B} g (x, y) d\pmb{\xi}$ is
%non-expansive, and $\pmb{\nu'} (A) \leq 1$.  (So this only works for
%probabilities, not general measures.  The case of bounded measures can be
%dealt with by replacing $\Met$ or $\CMet$ with the category of (complete)
%metric spaces with pairs $(f, c)$ of a constant $c$ and a $c$-Lipschitz
%function $f$, as in \cite{EH:metric:comp}.)  Easy calculations show that
%$\bistrcna$ is a mediator, and in fact a commutative one, by Fubini's
%Theorem again.
%%  (In the case of general measures, we let the reader show
%%that there is still a strength.)

%%Since we have already taken the pain of exploring the case of monads in
%%$\Dcpo$, it is interesting to see whether we can observe complete separable
%%metric spaces through the looking-glass of dcpos.  This means defining a
%%monoidal functor $\funbar$ from $\CMet$ to $\Dcpo$ and a monoidal monad
%%morphism from the monad $\tc$ of probability measures on complete separable
%%metric spaces to the monad $\td$ of accessible probability valuations on
%%dcpos.

%%There are many ways to define such a functor $\funbar$, see \cite{AM:PhD},
%%Chapter~5, for a survey.  We shall take one of the simplest, originally due to
%%Weihrauch and Schreiber \cite{WS:metric->cpo}.  We take the presentation of
%%\cite{EH:metric:comp}, only replacing the notation $\mathbf B (A)$ by
%%$\funbara A$.  Given any metric space $A$, the set $\funbara A$ of {\em formal
%%  balls\/} is the set of pairs $(x, r)$, $x\in A$, $r \in \real_+$, ordered by
%%$(x, r) \leq (y, s)$ if and only if $d_A (x, y) \leq r-s$.  When $A$ is
%%complete, $\funbara A$ is a continuous dcpo.  (The way-below relation $\ll$ is
%%given by $(x, r) \ll (y, s)$ if and only if $d_A (x, y) < r-s$.)  The map $i_A
%%: A \to \funbara A$ sending $x$ to $(x, 0)$ is a continuous embedding.  That
%%is, it is continuous as a function from $A$ with its metric topology to
%%$\funbara A$ with its Scott topology, is injective, and its inverse is
%%continuous on its range.  Moreover, the set $\max \funbara A$ of maximal
%%elements of $\funbara A$ is a $G_\delta$ subset of $\funbara A$ (a countable
%%intersection of Scott opens) that is homeomorphic to $A$. Finally, if $A$ is
%%separable, then $\funbara A$ is even $\omega$-continuous. By adapting
%%Theorem~17 of \cite{EH:metric:comp} to the category $\CMet$, $\funbar$ is a
%%functor from $\CMet$ to $\Dcpo$, where $\funbara f$ maps $(x, r)$ to $(f (x),
%%r)$.  It is such that, for every non-expansive map $f : A \to B$, $\funbara f
%%\circ i_A = i_B \circ f$.

%%This is a monoidal functor: $\tstri : 1 \to \funbara I$ (where $1$ is the
%%one-element dcpo, and $I$ is the one-element metric space) maps the unique
%%element $*$ of $1$ to $(*, 0)$, and $\tstr A B : $\funbara A \times \funbara B
%%\to \funbara {A \tensorc B}$ maps $((x, r), (y, s))$ to $((x, y), r+s)$.

%%Building the monad morphism is slightly more intricate.  We need $\dist A$ to
%%be a continuous map from $\td \funbara A$ to $\funbara {\tc A}$, that is,
%%mapping an accessible probability valuation on the space of formal balls
%%$\funbara A$ to some formal ball on the space of probability measures of $A$.
%%Fortunately, 


It is then tempting to observe $\tc$ from $\Met$ again.  That is, we are
tempted to let $\catd = \Met$ again, and $\td$ to be the same monad as $\tc$.
However, we do not know whether this preserves pseudoepis.  Let us make this
clear.

There is a natural epi-mono factorization on $\Met$: relevant monos are {\em
  isometric embeddings}, that is, maps $m : C \to B$ such that $d_B (m (x), m
(y)) = d_C (x, y)$ for all $x, y\in C$.  Pseudoepis from $A$ to $C$ are {\em
  surjective\/} non-expansive maps from $A$ to $C$. It is fairly easy to see
that this yields a monoidal mono factorization system on $\Met$.  (By the way,
we {\em cannot\/} take $\catd$ to be $\CMet$, even if we had chosen $\catc$ to
be $\CMet$.  In that case, we could not insist that pseudoepis be surjective.
Then it would be natural to take pseudoepis as non-expansive maps with dense
range, but this would not be enough for the construction to come in
Lemma~\ref{lemma:td:met} below, which requires surjectivity.)

Does $\tc$ defined above preserve surjective non-expansive maps?  A standard
result \cite[2.4, Lemma~1]{Bourbaki:int:IX} states that if $f$ is continuous
surjective from $A$ to $B$, and both $A$ and $B$ are compact Hausdorff, then
$\tc f$ is surjective.  (Since $\tc$ is a functor on $\Met$, $\tc f$ is always
non-expansive as soon as $f$ is.)  Similarly if the underlying topological
space of $A$ is an analytic space \cite[2.4, Proposition~9]{Bourbaki:int:IX}.
However, we cannot restrict to compact metric spaces, or to metric analytic
spaces---there is no reason why the monoidal closed structure on $\Met$ would
survive this restriction.

Instead, we use another monad $\td$ on $\Met$.  Let $\cbf A$ be the vector
space of all bounded non-expansive functions from the metric space $A$ to
$\real$, with the sup norm: for all $g \in \cbf A$, $||g|| = \sup_{x\in A} |g
(x)|$.  Let ${\cal L}_A$ be the vector space of all continuous linear forms on
$\cbf A$, that is, of all continuous linear functions $F : \cbf A \to \real$.
Recall that a linear function $F$ from $\cbf A$ to $\real$ is continuous if
and only if it is Lipschitz, i.e., if and only if $||F|| = \sup_{||g|| = 1} |F
(g)|$ is a well-defined real (i.e., not $+\infty$).  Then $||F||$ is called
the {\em norm\/} of $F$.  Let ${\cal L}^1_A$ be the subset of those $F$ in
${\cal L}_A$ of norm $1$.  Finally, let $\td A$ be the subset of those $F$ in
${\cal L}^1_A$ which are positive, i.e., such that $g \geq 0$ implies $F (g)
\geq 0$.  Both ${\cal L}^1_A$ and $\td A$ inherit the distance on ${\cal L}_A$
that is induced by norm.  Equivalently, $\td A$ is a metric space whose
distance is defined by $d_{\td A} (F, G) = \sup_{g \in \homset \Met A {[-1,
    1]}} |F (g) - G (g)|$.  $\td$ then defines an endofunctor on $\Met$ by
letting $\td f$ map $F \in \td A$ to $\lambda g \in \cbf B \cdot F (g \circ
f)$, for every non-expansive map $f$ from $A$ to $B$.

The space of all probability measures on $A$ embeds in $\td A$ by $\pmb{\nu}
\mapsto \lambda g \in \cbf A \cdot \int_{x\in A} g (x) d\pmb{\nu}$.  In fact,
the distance on probability measures on $A$ inherited from the metric
structure on $\td A$ is a slight variant of the Hutchinson metric introduced
above.  Moreover, if $A$ is compact, then every element of $\td A$ arises from
a probability measure in this way, by the Riesz Representation Theorem.  This
makes $\td A$ a metric space that is arguably close enough to a space of
probability measures.

The point of this definition of $\td$ is that $\td$ preserves pseudoepis in
$\Met$.  The proof is similar to that of \cite[2.4, Lemma~1]{Bourbaki:int:IX}.
\begin{lemma}
  \label{lemma:td:met}
  If $f$ is any surjective non-expansive map from $A$ to $B$, then $\td f$ is
  surjective from $\td A$ to $\td B$.
\end{lemma}
\begin{proof}
  Let $\lambda_f$ be the function mapping $g \in \cbf B$ to $g \circ f$.  Note
  that $\lambda_f (g)$ is bounded and non-expansive, hence in $\cbf A$.  Also,
  $||\lambda_f (g)|| = \sup_{x \in A} |g (f (x))| = \sup_{y \in B} |g (y)|$
  (since $f$ is surjective) $= ||g||$, so that $\lambda_f$ is an isometric
  embedding of $\cbf B$ into $\cbf A$.
  
  Let $H$ be the range of $\lambda_f$ in $\cbf A$.  $H$ is a linear subspace
  of $\cbf A$, which is by construction isometrically isomorphic to $\cbf B$.
  In particular, $\lambda_f^{-1}$ is a continuous linear map from $H$ to $\cbf
  B$.
  
  Given $G \in \td B$, $G \circ \lambda_f^{-1}$ is therefore a continuous
  linear form on $H$.  By the Hahn-Banach Theorem, $G \circ \lambda_f^{-1}$
  can be extended to a continuous linear form $F$ on $\cbf A$, with the same
  norm, i.e., $||F|| = ||G \circ \lambda_f^{-1}||$.  The latter means that
  $||F|| = \sup_{h \in \cbf A, ||h||=1} |F (h)| = \sup_{h \in H, ||h||=1} |G
  (\lambda_f^{-1} (h))| = \sup_{g \in \cbf B, ||g \circ f|| = 1} |G (g)| =
  ||G|| = 1$.
  
  As far as positivity is concerned, we first note that $||G|| = G (\lambda y
  \in B \cdot 1)$.  Indeed, first, $||\lambda y \in B \cdot 1|| = 1$, so
  $||G|| \geq G (\lambda y \in B \cdot 1)$.  To show the converse inequality,
  note first that for every $g \in \cbf B$, we may write $g$ as the difference
  $g_+ - g_-$ of two positive functions, so $|G (g)| = |G (g_+) - G (g_-)|
  \leq \max (G (g_+), G (g_-))$ (since $G (g_+), G (g_-) \geq 0$); if
  $||g||=1$, then $g_+ (y) \leq 1$ and $g_- (y) \leq 1$ for all $y\in B$, so
  $|G (g)| \leq G (\lambda y \in B \cdot 1)$; taking the sup over all $g$,
  $||G|| \leq G (\lambda y \in B \cdot 1)$.
  
  Then $F (\lambda x \in A \cdot 1) = F (\lambda_f (\lambda y \in B \cdot 1))
  = G (\lambda y \in B \cdot 1)$.  So $F (\lambda x \in A \cdot 1) = ||G|| =
  ||F||$.  If $F$ was not positive, there would be some $g \in \cbf A$, $g
  \geq 0$, with $F (g) < 0$.  We may assume without loss of generality that $g
  \leq 1$, so $\lambda x \in A \cdot 1-g(x)$ is of norm at most $1$.  But then
  $||F|| \geq F (\lambda x \in A \cdot 1-g(x)) = F (\lambda x \in A \cdot 1) -
  F (g) > F (\lambda x \in A \cdot 1)$, a contradiction.  So $F$ is positive.

  Finally, $\td f (F) = \lambda g \in \cbf B \cdot F (g \circ f) = \lambda g
  \in \cbf B \cdot G (\eta (g \circ f)) = \lambda g \in \cbf B \cdot G (g) =
  G$.  Since $G$ is arbitrary, $\td f$ is surjective.
\end{proof}

$\td$ can be used to form a monoidal monad on $\Met$.  Define $\unitd A$ as
the function mapping $x \in A$ to $\lambda g \in \cbf A \cdot g (x)$.  This is
natural in $A$, and non-expansive in $x$.  Define $\multd A$ as mapping $F \in
\td^2 A$ to $\lambda g \in \cbf {\td A} \cdot F (\lambda G \in \td A \cdot G
(g))$.  It requires a bit more work to show that $\multd A$ is well-defined
and non-expansive in $F$; it is however clear that this is natural in $A$.
Furthermore, the monad laws are satisfied, so that $(\td, \unitd{}, \multd{})$
is a monad on $\Met$.  (One might remark that the formulae for $\unitd A$ and
$\multd A$ are formally analogous to those of the continuation monad.)
Finally, define $\bistrd A B$ as mapping $(F, G) \in \td A \tensord \td B$ to
$\lambda h \in \cbf {A \tensord B} \cdot F (\lambda x \in A \cdot G (\lambda y
\in B \cdot h (x, y)))$.  This is a mediator, which is not in general
commutative. The underlying strength $\strd A B$ maps $(x, G) \in A \tensord
\td B$ to $\lambda h \in \cbf {A \tensord B} \cdot G (\lambda y \in B \cdot h
(x, y))$.




%\paragraph{Unary case.}
%We observe the category $\CMet$ through itself.  That is, we take $\funbar$
%as the identity functor, $(\td, \unitd{}, \multd{}, \bistrdna)$ to be the same
%as $(\tc, \unitc{}, \multc{}, \bistrcna)$, and $\dist A$ as the identity from
%$\td \funbara A$ to $\funbara {\tc A}$.  As relevant monos from $C$ to $B$, we
%take all {\em isometric embeddings}, that is, all maps $m : C \to B$ such that
%$d_B (m (x), m (y)) = d_C (x, y)$ for all $x, y\in C$.  As pseudoepis from $A$
%to $C$, we take all non-expansive maps $e$ whose range is dense in $C$.  It is
%equivalent to require that $C$ be isometric to the Cauchy-completion of the
%range of $e$.  It is fairly easy to see that this yields a monoidal mono
%factorization system on $\CMet$.

%\noindent
%\begin{minipage}{8cm}
%  A standard result states that the functor $\td$ preserves isometric
%  embeddings.  (This can be proved similarly to Proposition~4.8.3 of
%  \cite{Worrell:PhD}, for example.)  Now consider any diagram defining a
%  relevant pseudoepi $e$:
%\end{minipage}
%\begin{minipage}{4cm}
%  \[
%  \xymatrix@-5pt{
%    \td S \ar[r]^{\td f} \arrepixy[d]_{e} & 
%    \td \funbara{A} \ar[d]^{\dist{A}} \\
%    \lift{S} \arrmonoxy[r]_{m} & \funbara{\tc A}
%    }
%  \]
%\end{minipage}

%\noindent
%By the result above, $\td f$ is an isometric embedding, that is, a relevant
%mono, and $\dist A$ is the identity, so the composite morphism $\dist A \circ
%\td f$ is a relevant mono.  By the diagonal fill-in property, $e$ is therefore
%iso.  Indeed, since $\dist A \circ \td f$ is a relevant mono, $e$ followed by
%$m$ and $\identity {\td S}$ followed by $\dist A \circ \td f$ are two
%factorizations of the same map.  It follows that $\lift S$ and $\td S$ are
%isomorphic, with $e$ being one component of the iso.  We have just proved that
%relevant epis are iso: then Condition~{\bf (iv)}, stating that $\td$ maps
%relevant pseudoepis to pseudoepis, is obvious.

%\paragraph{Binary case.}
%The above paragraph deals with subscones with $\catc = \CMet$, which account
%for unary, not binary logical relations.  We argue that the binary case, where
%$\catc = \CMet \times \CMet$, is more difficult.  The main problem is that
%$\dist {}$ cannot just be the identity any more, so that $\dist A \circ \td f$
%will not be a relevant mono.  (We invite the reader to check it on $\dist{}$
%as defined below.)  So we take a more classical route and try to show that
%$\td$ preserves pseudoepis.  If pseudoepis were just surjective non-expansive
%maps, then we could hope to use standard theorems stating that $\td$ sends
%surjective continuous maps to surjective maps, as in the categories of compact
%Hausdorff spaces, or of analytic spaces.

%This justifies changing $\catd$ to be $\Met$, not $\CMet$: on $\Met$, we may
%take relevant monos to be isometric embeddings as above, but also pseudoepis
%to be the surjective non-expansive maps.  This solves half the problem, since
%the probability monad may fail to send surjective maps to surjective maps,
%except in compact Hausdorff or analytic spaces.  To solve the other half, use
%another monad on $\Met$, which behaves better.  This will be the monad of
%positive continuous linear forms of norm one on the spaces $\cbf A$ of bounded
%non-expansive functions from $A$ to $\real$.  The reason of this choice is
%that every probability measure $\nu$ on $A$ defines such a positive continuous
%linear form, namely $g \mapsto \int_{x\in A} g(x) d\nu$.

%To sum up, let $\catd$ be $\Met$.  


To define a notion of binary metric logical relations, we take $\catc = \Met
\times \Met$, define a monad $\tc$ on $\catc$ pointwise (i.e., $\tc (A_1, A_2)
= (\td A_1, \td A_2)$).  It remains to define a monad morphism from $\tc$ to
$\td$.

Define $\funbara {A_1, A_2}$ as the cartesian product $A_1 \times A_2$, much
as in $\catset$.  Note that the only difference between cartesian product and
tensor product is that their distances differ: $d_{A_1 \times A_2} ((x, y),
(x', y'))$ is the max of the distances $d_{A_1} (x, x')$ and $d_{A_2} (y,
y')$, while $d_{A_1 \tensord A_2} ((x, y), (x', y'))$ is the sum of the same
distances.

Similarly as in $\catset$, define the monad morphism $\dist {A_1, A_2}$ as $\langle
\td \pi_1, \td \pi_2 \rangle$.  That is, for every $F \in \td (A_1 \times A_2)$, $\dist {A_1,
  A_2} (F) = (\lambda g_1 \in \cbf {A_1} \cdot F (\lambda (x, y) \cdot g_1 (x)), \lambda g_2 \in \cbf {A_2}
\cdot F (\lambda (x, y) \cdot g_2 (y)))$. The functor $\funbar$ is symmetric monoidal.  Its
mediating pair $(\tstrna, \tstri)$ consists of $\tstri : \Id \to \funbara \Ic$
(where $\Id$ is the one-element complete separable metric space $\{*\}$, and
$\Ic$ is the pair $\Id, \Id$) mapping $*$ to $(*, *)$; and of the natural
transformation $\tstr {(A_1, A_2)} {(B_1, B_2)} : \funbara {A_1, A_2} \tensord
\funbara {B_1, B_2} \to \funbara {A_1 \tensorc B_1, A_2 \tensorc B_2}$ which
maps $((x_1, x_2), (y_1, y_2))$ to $((x_1,\allowbreak y_1),\allowbreak
(x_2,\allowbreak y_2))$.  The latter is non-expansive, because we have chosen
$\dist {A_1, A_2}$ to be $A_1 \times A_2$ and not $A_1 \tensord A_2$ for example.
Indeed,
\begin{eqnarray*}
  &&
  d_{\funbara {A_1 \tensorc B_1, A_2 \tensorc B_2}} (((x_1, y_1), (x_2, y_2)),
  ((x'_1, y'_1), (x'_2, y'_2))
  \\
  & = & \max (d_{A_1 \tensorc B_1} ((x_1, y_1), (x'_1, y'_1)),
  d_{A_2 \tensorc B_2} ((x_2, y_2), (x'_2, y'_2))) \\
  & = & \max (d_{A_1} (x_1, x'_1) + d_{B_1} (y_1, y'_1), d_{A_2} (x_2, x'_2) +
  d_{B_2} (y_2, y'_2))
  \\
  & \leq & \max (d_{A_1} (x_1, x'_1), d_{A_2} (x_2, x'_2)) +
  \max (d_{B_1} (x_1, x'_1), d_{B_2} (x_2, x'_2)) \\
  & = & d_{\funbara {A_1, A_2}} ((x_1, x_2), (x'_1, x'_2)) +
  d_{\funbara {B_1, B_2}} ((y_1, y_2), (y'_1, y'_2)) \\
  & = & d_{\funbara {A_1, A_2} \tensord \funbara {B_1, B_2}} (((x_1, x_2), (y_1,
  y_2)), ((x'_1, x'_2), (y'_1, y'_2)))
\end{eqnarray*}
It is clear that $\tstrna$ is natural, and that the coherence conditions
(\ref{eq:theta:coh:alpha})--(\ref{eq:theta:coh:r}) as well as
(\ref{eq:theta:coh:c}) are satisfied.

%Define $\dist {A_1, A_2} (\nu)$ as the pair $(\td \pi_1 (\nu), \td \pi_2
%(\nu))$, that is, as the pair of measures $(\nu_1, \nu_2)$ such that, for
%every measurable subset $X$ of $A_i$, $\nu_i (X) = \nu (\pi_i^{-1} (X))$.
%This is non-expansive.  Indeed,
%\begin{eqnarray*}
%  &&
%  d_{\funbara {\tc A_1, \tc A_2}} (\dist {A_1, A_2} (\nu), \dist {A_1, A_2}
%  (\nu'))
%  \\
%  & = & \max \Bigg(
%  \sup_{g \in \homset \CMet {A_1} {[0,1]}}
%  \left|
%    \int_{x\in A_1} g (x) d \td \pi_1 (\nu) - \int_{x\in A_1} g (x) d \td
%    \pi_1 (\nu')
%  \right|,
%  \\
%  && \phantom{\max \Bigg(}
%  \sup_{h \in \homset \CMet {A_2} {[0,1]}}
%  \left|
%    \int_{y\in A_2} h (y) d \td \pi_2 (\nu) - \int_{y\in A_2} h (y) d \td
%    \pi_2 (\nu')
%  \right|
%  \Bigg)
%  \\
%  & = & \max \Bigg (
%  \sup_{g \in \homset \CMet {A_1} {[0,1]}}
%  \left|
%    \int_{(x, y)\in \funbara {A_1, A_2}} g (x) d\nu - \int_{(x, y)\in \funbara {A_1, A_2}} g (x) d\nu'
%  \right|,
%  \\
%  && \phantom{\max \Bigg (}
%  \sup_{h \in \homset \CMet {A_2} {[0,1]}}
%  \left|
%    \int_{(x, y)\in \funbara {A_1, A_2}} h (y) d\nu - \int_{(x, y)\in \funbara {A_1, A_2}} h (y) d\nu'
%  \right|
%  \Bigg)
%  \\
%  & \leq & \max (d_{\td \funbara {A_1, A_2}} (\nu, \nu'),
%  d_{\td \funbara {A_1, A_2}} (\nu, \nu'))
%  =  d_{\td \funbara {A_1, A_2}} (\nu, \nu')
%\end{eqnarray*}
%where the last line follows by the fact that the maps $(x, y) \mapsto g (x)$
%and $(x, y) \mapsto h (y)$ from $\funbara {A_1, A_2}$ to $[0, 1]$ are
%non-expansive as soon as $g$ and $h$ are.

%It is easy to see that $\dist {A_1, A_2}$ is natural in $A_1$ and $A_2$, and
%that the monad morphism law (\ref{d_distlaw}) is satisfied.

Then $(\funbar, \dist{})$ is a monoidal monad morphism, as
Diagram~(\ref{d_distbistr}) commutes.  It is also easy to check that $\Met$
has pullbacks: the pullback of $f : A \to C$ and $g : B \to C$ is the subspace
of $A \times B$ consisting of all $(x, y)$ such that $f (x) = g (y)$; and
$\ihom A \_$ preserves relevant monos: $\ihom A \_$ maps $f : B \to C$ to
$\lambda g \in \ihom A B \cdot f \circ g$, which is an isometric embedding as
soon as $f$ is.

%This means that, for every pair of
%measures $\nu$ on $\funbara {A_1, B_1}$ and $\xi$ on $\funbara {A_2, B_2}$,
%$\dist {A_1 \tensorc A_2, B_1 \tensorc B_2} \circ \td (\tstr {(A_1, B_1)}
%{(A_2, B_2)}) \circ \bistrd {\funbara {A_1, B_1}} {\funbara {A_2, B_2}} (\nu,
%\xi) = \funbara {\bistrc {A_1} {A_2}, \bistrc {B_1} {B_2}} \allowbreak \circ
%\tstr {(\tc A_1, \tc B_1)} {(\tc A_2, \tc B_2)} \circ (\dist {A_1, B_1}
%\tensord \dist {A_2, B_2}) (\nu, \xi)$.  The left-hand side is the measure
%mapping $X$ to $((\nu \otimes \xi) ((\pi_1 \circ \tstr{(A_1, B_1)}
%{(A_2, B_2)})^{-1} (X)), (\nu \otimes \xi) ((\pi_2 \circ \tstr{(A_1, B_1)}
%{(A_2, B_2)})^{-1} (X)))$.  The right-hand side is the measure mapping $X$ to 

%We come to the harder part, namely showing that Condition~{\bf (iv)} is met.
%We first notice that, as a map of topological spaces, $\dist {A_1, A_2}$ is
%not only continuous but maps closed sets to closed sets.  That is, given any
%closed subset $C$ of $\td \funbara {A_1, A_2}$, every sequence $(\nu_n,
%\nu'_n)$ of pairs of probability measures in $\dist {A_1, A_2} (C)$, i.e.,
%$(\nu_n, \nu'_n) = \dist {A_1, A_2} (\xi_n)$ with $\xi_n \in C$, $n\in \nat$,
%that converges to some pair $(\nu, \nu')$ in $\funbara {\tc A_1, \tc A_2}$ is
%such that $(\nu, \nu') \in \dist {A_1, A_2} (C)$.  Since $(\nu_n, \nu'_n)$
%converge, it is a Cauchy sequence, hence both sequences

This yields the following notion of binary metric logical relation $\Eval
\tau$ between metric spaces $\Eval \tau_1$ and $\Eval \tau_2$ indexed by types
in the linear version of Moggi's meta-language adumbrated in
Section~\ref{ccc.s:linear}:
\[
\tau ::= b | \tau \otimes \tau | \tau \llimp \tau | ? \tau
\]
Note that $\Eval {\tau \otimes \tau'}_i = \Eval \tau_i \tensord \Eval
{\tau'}_i$, $\Eval {\tau \llimp \tau'}_i = \ihom {\Eval \tau_i} {\Eval
  {\tau'}_i}$, $\Eval {? \tau}_i = \td \Eval \tau_i$.  Then the definition
of the subscone specializes to:
\begin{eqnarray*}
  (f_1, f_2) \in \Eval {\tau \llimp \tau'} & \iff &
  \forall a_1 \in \Eval \tau_1, a_2 \in \Eval \tau_2 \cdot
  \\
  && \quad (a_1, a_2) \in \Eval \tau \Rightarrow (f_1 (a_1), f_2 (a_2)) \in \Eval {\tau'}
  \\
  ((a_1, a'_1), (a_2, a'_2)) \in \Eval {\tau \otimes \tau'} & \iff &
  (a_1, a_2) \in \Eval {\tau} \land (a'_1, a'_2) \in \Eval {\tau'}
\end{eqnarray*}
Finally, $(F_1, F_2) \in \Eval {? \tau}$ if and only if there is $F \in \td
\Eval \tau$ such that
\begin{eqnarray*}
  F_1 (g_1) & = & F (\lambda (x, y) \in \Eval \tau \cdot g_1 (x))
  \mbox{ for every }g_1 \in \cbf {\Eval \tau_1} \\
  F_2 (g_2) & = & F (\lambda (x, y) \in \Eval \tau \cdot g_2 (y))
  \mbox{ for every }g_2 \in \cbf {\Eval \tau_2}
\end{eqnarray*}
(Up to isomorphism, relevant monos are inclusions, so we may consider that
$\Eval \tau \subseteq \Eval \tau_1 \times \Eval \tau_2$.)  This condition
implies that, if $(F_1, F_2) \in \Eval {? \tau}$, then for every $g_1 \in \cbf
{\Eval \tau_1}$ and $g_2 \in \cbf {\Eval \tau_2}$ such that $g_1 (a_1) = g_2
(a_2)$ for every $(a_1, a_2) \in \Eval \tau$, then $F_1 (g_1) = F_2 (g_2)$.
It turns out that this is equivalent to it, just as in the case of the
continuation monad:
\begin{lemma}
  \label{lemma:proba:met:cont}
  $(F_1, F_2) \in \Eval {? \tau}$ if and only if, for every $g_1 \in \cbf
  {\Eval \tau_1}$ and $g_2 \in \cbf {\Eval \tau_2}$ such that $g_1 (a_1) = g_2
  (a_2)$ for every $(a_1, a_2) \in \Eval \tau$, then $F_1 (g_1) = F_2 (g_2)$.
\end{lemma}
\begin{proof}
  The only if direction is clear.  Conversely, assume that $F_1 (g_1) = F_2
  (g_2)$ for every $g_1 \in \cbf {\Eval \tau_1}$ and $g_2 \in \cbf {\Eval
    \tau_2}$ such that $g_1 (a_1) = g_2 (a_2)$ for every $(a_1, a_2) \in \Eval
  \tau$.  Let $S$ be $\Eval \tau$, and $H$ be the subspace of $\cbf S$ of
  those functions of the form $\lambda (x, y) \in S \cdot g_1 (x)+g_2 (y)$,
  where $g_1$ ranges over $\cbf {\Eval \tau_1}$, $g_2$ ranges over $\cbf
  {\Eval \tau_2}$.  Let $F_0 (g)$ be defined as $F_1 (g_1) + F_2 (g_2)$ for
  every $g = \lambda (x, y) \in S \cdot g_1 (x)+g_2 (y)$ in $H$.  This is
  independent of the choice of $g_1$ and $g_2$, since if $g$ can also be
  written as $\lambda (x, y) \in S \cdot g'_1 (x)+g'_2 (y)$, then by
  construction $g_1 (a_1) - g'_1 (a_1) = g'_2 (a_2) - g_2 (a_2)$ for every
  $(a_1, a_2) \in S = \Eval \tau$, so $F_1 (g_1-g'_1) = F_2 (g'_2-g_2)$, which
  implies $F_1 (g_1) + F_2 (g_2) = F_1 (g'_1) + F_2 (g'_2)$.  It is easy to
  see that $F_0$ is a continuous linear form, so it extends to a continuous
  linear form $F$ with the same norm on the whole of $\cbf S$, by the
  Hahn-Banach Theorem.  By the same argument as in Lemma~\ref{lemma:td:met},
  $F$ is a positive linear form.  Clearly $F_1 (g_1) = F (\lambda (x, y) \in
  \Eval \tau \cdot g_1 (x))$ for every $g_1 \in \cbf {\Eval \tau_1}$, and $F_2
  (g_2) = F (\lambda (x, y) \in \Eval \tau \cdot g_2 (y))$ for every $g_2 \in
  \cbf {\Eval \tau_2}$, whence the claim.
\end{proof}

It is reasonable to represent the set of probabilistic transition systems on a
metric space $A$ as the metric space $\ihom A {\td A}$ of all non-expansive
maps from the set of states $A$ to the set of probability measures on $A$. The
subscone construction provides a condition when two such probabilistic
transition systems are related.  Given any relation $S$ on $A$ (defining a
metric subspace of $A \times A$), define the relation $\lift S$ on $\ihom A
{\td A}$ by: for any non-expansive maps $f_1, f_2$ from $A$ to $\td A$, $(f_1,
f_2) \in \lift S$ if and only if, for every $(a_1, a_2) \in S$, there is $F
\in \td S$ such that
\begin{eqnarray*}
  f_1 (a_1) (g_1) & = & F (\lambda (x, y) \in S \cdot g_1 (x))
  \mbox{ for every }g_1 \in \cbf A \\
  f_2 (a_2) (g_2) & = & F (\lambda (x, y) \in S \cdot g_2 (y))
  \mbox{ for every }g_2 \in \cbf A
\end{eqnarray*}
or, equivalently, for every $g_1, g_2 \in \cbf A$ such that $g_1 (x) = g_2
(y)$ for every $(x, y) \in S$, then $f_1 (a_1) (g_1) = f_2 (a_2) (g_2)$.  (Use
Lemma~\ref{lemma:proba:met:cont}.) In case $A$ is compact, by the Riesz
Representation Theorem, we may replace positive continuous linear functionals
on $\cbf A$ by probability measures.  Rephrasing the above, we get: for any
non-expansive maps $f_1, f_2$ from $A$ to the space of probability measures on
$A$, $(f_1, f_2) \in \lift S$ if and only if, for every $(a_1, a_2) \in S$,
there is a probability measure $\nu$ on $S$ such that
\begin{eqnarray*}
  f_1 (a_1) (X_1) & = & \nu ((X_1 \times A) \cap S)
  \mbox{ for every measurable subset }X_1\mbox{ of }A
  \\
  f_2 (a_2) (X_2) & = & \nu ((A \times X_2) \cap S)
  \mbox{ for every measurable subset }X_2\mbox{ of }A
\end{eqnarray*}
We retrieve a notion of probabilistic bisimulation similar to that of
Section~\ref{sec:proba:dcpo}, yet simpler: $S$ is a {\em bisimulation\/} on
the space $A$ of states between the transition systems $f_1$ and $f_2$ if and
only if $\lift S$ relates $f_1$ and $f_2$.

This notion is formally analogous to the notion of probabilistic bisimulation
of \cite{DEP:markov:bisim}; i.e., the formulas we use and theirs for defining
bisimulations is the same.  A difference is that the latter define
bisimulations on the category of analytic spaces; this is awkward in our
setting, since we do not know any monoidal closed structure on the category of
analytic spaces.  (But there is a monoidal monad of probability measures on
completely regular analytic spaces, where the space of probability measures is
equipped with the weak topology.)  This is also formally analogous to metric
bisimulations as introduced by de Vink and Rutten \cite{dVR:proba:bisim} for
ultrametric spaces, and extended by Worrell \cite{Worrell:PhD} to generalized
metric spaces.  A difference is that the latter authors use a coalgebraic
approach; in particular, their construction requires a $\td$ functor that
preserves isometric embeddings (our relevant monos), while we require it to
preserve pseudoepis (surjective non-expansive maps).  There seems to be no
connection between the approach of this section and the metric defined in
\cite{DGJP:metric:proba}, where the goal is to define a distance between
processes that vanishes exactly on bisimilar processes; our construction only
yields relations as sets of pairs equipped with a distance.

We won't pursue this comparison.  After all, our purpose in this paper was not
to define any new approach to the theory of probabilistic bisimulations per
se, but to adapt logical relations to the case of monads.  It can be
considered a nice byproduct that our approach is able to define extensions of
some bisimulations to all higher orders.


%\subsection{Probability Measures on Analytic Spaces}
%\label{sec:proba:souslin}



==> proba_disc.tex <==

\subsection{Discrete Probabilities and Subprobabilities}
\label{sec:proba}


Defining $\tc A$ to be space of all probability distributions over the space
$A$ allows us to define probabilistic transition systems as objects of ${(\tc
  A)}^A$.  In principle, this should work just like ordinary transition
systems (Section~\ref{sec:lts}).

In fact, defining what the right spaces should be, and ensuring that
the required monads exist and have the required properties, is much
subtler.  For one, as far as we know, the category of measurable
spaces and measurable functions is not known to be cartesian closed.
As we don't want to delve into measure theoretic considerations at
this point, let us deal with a simpler case: the monad of {\em
  discrete\/} (sub-)probability distributions over $\catset$.

A discrete sub-probability distribution $\nu$ over some set $A$ is
simply a function mapping each element $x \in A$ to some non-negative
number $a_x \in \real^+$, so that $\sum_{x\in A} a_x \leq 1$.  This sum, which
is in general infinite, denotes the supremum of all partial sums $\sum_{x
  \in B} a_x$, when $B$ ranges over the finite subsets of $A$.  It is an
easy exercise to show that only countably many coefficients $a_x$ can
be non-zero, then.  A discrete probability distribution additionally
satisfies $\sum_{x\in A} a_x = 1$.  The Dirac distribution $\delta_{x_0}$ at
$x_0$ maps $x_0$ to $1$ and every $x \neq x_0$ to $0$.  Accordingly, we
write $\sum_{x\in A} a_x \delta_x$ for the discrete distribution mapping $x$ to
$a_x$.  The measure of a subset $B$ of $A$ under $\nu = \sum_{x\in A} a_x
\delta_x$ is $\nu (B) = \sum_{x\in B} a_x$.

Let $\tc A$ be the set of all discrete (sub-)probability distributions
over $A$, $\unitc A$ map $x \in A$ to $\delta_x \in \tc A$, and $\multc A$ be
defined as mapping $\nu_2 = \sum_{\nu \in \tc A} a_{\nu} \delta_\nu \in \tc^2 A$ to the
discrete distribution $\multc A (\nu_2)$ such that $\multc A (\nu_2) (B) =
\sum_{\nu \in \tc A} a_\nu \nu (B)$ for every $B \subseteq A$; in other words, $\multc A
(\nu_2) = \sum_{x \in A} \left(\sum_{\nu \in \tc A} a_\nu \nu (\{x\})\right) \delta_x$.  It is
easy to check that $(\tc {}, \unitc{}, \multc{})$ is a monad on
$\catset$.  Moreover, it is strong: the strength $\strc A B$ maps $x \in
A$ and $\nu = \sum_{y \in B} b_y \delta_y \in \tc B$ to $\sum_{y \in B} b_y \delta_{(x,y)}$.

Our construction in the case of the (sub-)probability distribution
monad on $\catset$ yields the following.  Again, $\tc{} = \td{}$, and
recall that $\tS$ maps relations $S$ on $A_1 \times A_2$ to the direct
image $\lift S$ of $\langle \td \proj_1, \td \proj_2 \rangle : \td S \to \td A_1 {\times}
\td A_2$.  In other words, given $\nu_1 \in \tc A_1$, $\nu_2 \in \tc A_2$,
$(\nu_1, \nu_2) \in \lift S$ if and only if there is a discrete
(sub-)probability distribution $\nu$ on $S$ such that $\nu_1 (B_1) = \nu
((B_1 \times A_2) \cap S)$ for every $B_1 \subseteq A_1$ and $\nu_2 (B_2) = \nu ((A_1 \times
B_2) \cap S)$ for every $B_2 \subseteq A_2$.

Write $\nu_1$ as $\sum_{x_1 \in A_1} a_{x_1} \delta_{x_1}$, $\nu_2$ as $\sum_{x_2 \in
  A_2} b_{x_2} \delta_{x_2}$.  Then $(\nu_1, \nu_2) \in \lift S$ if and only if
there is a discrete (sub-)probability distribution $\nu =
\sum_{\substack{x_1 \in A_1, x_2 \in A_2\\(x_1,x_2) \in S}} c_{x_1, x_2}
\delta_{(x_1, x_2)}$ on $S$ such that $a_{x_1} = \sum_{x_2 \in A_2 / (x_1, x_2)
  \in S} c_{x_1, x_2}$ for all $x_1 \in A_1$ and $b_{x_2} = \sum_{x_1 \in A_1 /
  (x_1, x_2) \in S} c_{x_1, x_2}$ for all $x_2 \in A_2$.  This may be
pictured by requiring that we have a matrix of non-negative reals
$c_{x_1, x_2}$ such that: the only non-zero entries $(x_1, x_2)$ of
this matrix are such that $(x_1, x_2) \in S$; the sum of the $x_1$ row
is $a_{x_1}$; the sum of the $x_2$ column is $b_{x_2}$.  This is a
well-known problem in probability theory: find $\nu$ on the product $A_1
\times A_2$ having given {\em marginals\/} $\nu_1$ and $\nu_2$ and whose {\em
  support\/} $\{(x_1, x_2) \in A_1 \times A_2 | \nu (\{(x_1, x_2)\}) \neq 0\}$ is
included in $S$.

Let us play with the definition of $\lift S$ for a moment.  Consider
the disjoint sum $A_1 \oplus A_2$, and the smallest equivalence $\equiv_S$
relation containing $S$.
%Define $\nu_1 \oplus \nu_2$ as the discrete distribution mapping $x_1 \in A_1$ to $\nu_1 (x_1)$, $x_2 \in A_2$ to $\nu_2 (x_2)$.
It is easy to see that, for every $\equiv_S$-equivalence class $C$,
\begin{equation}
  \label{eq:A1A2}
  ((C \cap A_1) \times A_2) \cap S = (A_1 \times (C \cap A_2)) \cap S
\end{equation}
% Indeed, the inclusion of the left-hand side in the right-hand side
% means that for every $a_1 \in C \cap A_1$ and for every $a_2 \in A_2$ such
% that $(a_1, a_2) \in S$, then $a_2$ is in $C$. The converse inclusion
% means that for every $a_2 \in C \cap a_2$ and every $a_1 \in A_1$ such that
% $(a_1, a_2) \in S$ then $a_1 \in C$.  Both inclusions hold because in each
% case $a_1\equiv_S a_2$ and $C$ is an equivalence class for $\equiv_S$.

It follows that if there is a discrete distribution $\nu$ with support
contained in $S$ and whose marginals are $\nu_1$ and $\nu_2$, then for any
$\equiv_S$-equivalence class $C$, $\nu_1 (C \cap A_1) = \nu_2 (C \cap A_2)$.  Indeed,
$\nu_1 (C \cap A_1) = \nu (((C \cap A_1) \times A_2) \cap S)$, $\nu_2 (C \cap A_2) = \nu ((A_1
\times (C \cap A_2)) \cap S)$; then use (\ref{eq:A1A2}).

Conversely, if $\nu_1 (C \cap A_1) = \nu_2 (C \cap A_2)$ for every
$\equiv_S$-equivalence class $C$, then whenever $x_1 \equiv_S x_2$, let $d_{x_1,
  x_2} = \nu_1 (C \cap A_1) = \nu_2 (C \cap A_2)$, where $C$ is the equivalence
class of $x_1$ (equivalently, of $x_2$).  Now define $\nu$ as
$\sum_{\substack{(x_1, x_2) \in A_1 \times A_2\\x_1 \equiv_S x_2\\d_{x_1, x_2} \neq 0}}
\frac {a_{x_1} b_{x_2}} {d_{x_1, x_2}} \delta_{(x_1, x_2)}$.  Clearly the
support of $\nu$ is contained in the relation $\equiv_S$, and $\nu_1$ and $\nu_2$
are the marginals of $\nu$.  So $(\nu_1, \nu_2) \in \lift {\equiv_S}$.

Let $S$ be {\em saturated\/} if and only if, for any $x_1 \in A_1$, $x_2
\in A_2$, $x_1 \equiv_S x_2$ implies $(x_1, x_2) \in S$.  We have just shown
the following: for any saturated relation $S \subseteq A_1 \times A_2$, $(\nu_1, \nu_2)
\in \lift S$ if and only if $\nu_1 (C \cap A_1) = \nu_2 (C \cap A_2)$ for every
$\equiv_S$-equivalence class $C$.  The restriction to saturated relations
is not too demanding; indeed, we can always saturate any binary
relation $S$ by considering the restriction of $\equiv_S$ to $A_1 \times A_2$
instead.

Analogously with Section~\ref{sec:lts}, we may define a {\em
  probabilistic\/} labelled transition system as an element of ${(\tc
  A)}^{A \times L}$.  Then two such transition systems $f_1$ and $f_2$ are
in relation if and only if: {\small
  \begin{eqnarray}
    \label{eq:proba:bisim}
    \forall x_1 \in A_1, x_2 \in A_2, \ell_1, \ell_2 \in L . (x_1, x_2) \in S
    & \land & (\ell_1, \ell_2) \in R_L \Rightarrow \\
    && \nonumber
    (f_1 (x_1, \ell_1), f_2 (x_2, \ell_2)) \in \lift S
  \end{eqnarray}
} When $S$ is saturated, this condition is equivalent to: for every
$x_1 \in A_1$, $x_2 \in A_2$, $\ell_1, \ell_2 \in L$, if $x_1 \equiv_S x_2$ and $(\ell_1,
\ell_2) \in R_L$ then for every $\equiv_S$-equivalence class $C$, $f_1 (x_1,
\ell_1) (C \cap A_1) = f_2 (x_2, \ell_2) (C \cap A_2)$.  This is exactly Larsen
and Skou's \cite{LS:proba} notion of probabilistic bisimulation, when
$L_1=L_2$, $R_L$ is the equality relation, and $A_1$ and $A_2$ are
finite.  To see this, write $p_\ell (x) = f_1 (x, \ell)$ if $x \in A_1$, $p_\ell
(x) = f_2 (x, \ell)$ if $x \in A_2$, and rewrite the condition above as: if
$x_1 \equiv_S x_2$ then for every $\equiv_S$-equivalence class $C$, $p_\ell (x_1)
(C) = p_\ell (x_2) (C)$.

It is therefore fair to say that any saturated relation $S$ (and by
extension, any relation at all) such that $f_1$ and $f_2$ are in
relation at type $A \times L \to \tc A$, as defined in
(\ref{eq:proba:bisim}), is again a probabilistic bisimulation.

A note on discreteness: the monad of discrete (sub-)probability
distributions is enough to model coin flips $\sum_{x \in \{0, 1\}} 1/2 \delta_x$.
One may argue that, in any finite computation of a $\lambda$-term augmented
with coin flips, only finite linear combinations of Dirac measures
({\em simple\/} valuations) will ever crop up, so that discrete
distributions are general enough to accomodate all practical forms of
probabilistic choice.  This would not be true in the case of infinite
computations, where at least all least upper bounds of directed chains
of simple distributions ({\em quasi-simple\/} valuations
\cite{JGL:val:ext}) would be needed.  Notwithstanding the fact that we
should incorporate fixpoints in the language and replace $\catset$
with some other category such as $\Dcpo$, this would exceed the realm
of discrete distributions anyway: for example, the Lebesgue measure on
$[0,1]$ is a quasi-simple valuation but is definitely not discrete.



==> related.tex <==
\section{Related work.}
\label{related.s}

One succesful approach to categorical generalization of logical
relations is the setting of \cite{Her93} based on fibrations. We do
not assume in this paper the forgetful functor to be a fibration,
similarly to other authors (e.g. \cite{PPST00}).  Even if we lose
thereby the equivalence to logic, this is justified, since we do not
focus on logical rules corresponding to logical relations in this
paper.

We have already said that there is no
unique notion of monad lifting. One of the simplest is the lifting, proposed
in \cite{Pitts92}, $\tS$ of $\tc$, which maps the object $\langle S, f, A \rangle$ of the
scone to $\langle S, \funbara{\unitc{A}} \circ f, \tc A \rangle$.  This is a special case of
our notion of lifting on the scone $\scone \catc \catd \funbar$
(Section~\ref{scone.s}), taking $\td$ the identity monad and $\dist A =
\funbara {\unitc A}$.
%(see Section~\ref{prelim.s} for notations).
%
%Our lifting is obviously not the unique one satisfying (\ref{d_lifting1}) and
%(\ref{e_lifting2}). For instance, Pitts in~\cite{Pitts92} defines another
%lifting, namely
%\iflong
%\[
%\xymatrix@-5pt{
%& S \ar[r]^{f} &\funbara{A} &  \ar@{|.>}[r] & &
%S \ar[r]^{f} & {\funbara{A}} \ar[r]^{\funbara{\unitc{A}}} &
%\funbara{\tc A} 
%}
%\]
%\else
%$
%\xymatrix@-5pt{
%S \ar[r]^{f} &\funbara{A} \ar@{|.>}[r]
%S \ar[r]^{f} & {\funbara{A}} \ar[r]^{\funbara{\unitc{A}}} &
%\funbara{\tc A} 
%}
%$.
%\fi
%
Turi \cite{Turi96} considers lifting monads to the category of coalgebras of a
given endofunctor.  This is a special case of our framework, when $\catc =
\catd$ (and $\tc = \td$) and moreover only objects of the form
\smash{$\xymatrix@-5pt{S \ar[r]^{f} & \funbara{S}}$} are taken into
consideration, and only morphisms of the form $\langle g, g \rangle$. This
defines the category of $\funbar$-coalgebras as a proper subcategory of
scones. Turi uses a simpler version of our monad morphisms%
%(we recall monad morphisms %in~(\ref{d_distlaw}) in Section~\ref{scone.s})
, namely distributivity law of a monad over an endofunctor; monad
morphisms involve two monads and a functor between distinct
categories.  Turi's distributivity laws are similar enough to monad
morphisms that we had called the latter {\em distributivity laws\/}
for monads in the conference version of this paper.  This also
influenced \cite{GG01}, where comonad morphisms are used, but are
called distributivity laws for comonads.  (This relies on pullbacks,
whereas we use mono factorization systems.)  Calling these monad
morphisms distributivities turned out to be a bad choice, as
distributivity laws denote a close but different concept, due to Jon
Beck \cite{Beck:distr}; also, while distributivity laws tend to be
rare, monad morphisms abound.

In~\cite{PW02} different possible ways to combine a monad and a comonad were
studied in a systematic way. In particular, the authors used a notion of a
distributivity of a monad over a comonad (and dual distributivity of the
comonad over the monad). This is a stronger notion than monad morphisms, as it
requires commutativity of two copies of diagrams~(\ref{d_distlaw}), one
for the monad and another one for the comonad. On the other hand, both the
monad and the comonad live in a single category, unlike in our case.

We also note that neither Pitts nor Turi deal with subscones.

\cite{KP99} consider lifting a monad on $\catset$ to the category of
relations in $\catset$.  This is a particular case of our setting.
However, the main topic of this paper is a more complex situation of
lax logical relations and data-refinement for the computational lambda
calculus. A subsequent paper \cite{PT00} develops further the ideas of
\cite{KP99}. It addresses in particular lax logical relations for the
computational lambda calculus and for the linear lambda calculus.

%Lifting of a monad to relations is briefly mentioned in \cite{KP99}.
%Lax logical relations for the computational lambda-calculus are addressed in \cite{PT00}.

In the same way that we lift a monad to relations, Rutten \cite{Rut98} defines
an extension of an endofunctor in $\catset$ to a category of relations. The
latter has relations as {\em morphisms} between sets.  An endofunctor extends
to relations iff it preserves weak pullbacks\iflong (which in particular
implies preserving monos)\else \fi, and if so, the extension is unique.
\iflong (This is actually a special case of a more general fact, proved
in~\cite{CKW90} for regular categories.) \else \fi The approach taken by
Rutten is different from ours, where relations are {\em objects} rather than
morphisms. Hence, Rutten imposes a different functoriality condition: the
action of a lifted endofunctor on a composition of two relations must coincide
with a composition of actions of the lifted endofunctor on these two
relations. This amounts to closedness under composition of relations yielded
by the lifted endofunctor.

\cite{Pit91} proposes the Evaluation Logic for reasoning about
programs with computational effects. It is based on the computational
lambda-calculus \cite{Mog91}. Semantics of Pitts' Evaluation Logic is
studied further in \cite{Mog95}.

\cite{Pit96} considers litfing of certain constructions on
domains to relations on these domains. He focuses on categories on
domains and does not consider (strong) monads. Instead of category
of relations he assumes a relational structure, relaxing a notion
of mapping (morphism) of relations.

% An approach related to ours is \cite{GG01}, where a {\em comonad\/} lifting is
% defined.  This relies on pullbacks, whereas we use mono factorization systems.
% Nonetheless, the so-called distributivity laws of \cite{GG01} {\em are\/}
% comonad morphisms, dual to the monad morphisms we use.

%\ForAuthors{
%  Should also discuss Power and Watanabe (they call their [op-]monad morphism
%  a distributivity law; see Slawek's mail).
%  }
%
% done - few lines above (SL, 29.11.2003)
%



